Dynamical mean-field analysis of adaptive Langevin diffusions: Replica-symmetric fixed point and empirical Bayes

In many applications of statistical estimation via sampling, one may wish to sample from a high-dimensional target distribution that is adaptively evolving to the samples already seen. We study an example of such dynamics, given by a Langevin diffusion for posterior sampling in a Bayesian linear regression model with i.i.d. regression design, whose prior continuously adapts to the Langevin trajectory via a maximum marginal-likelihood scheme. Results of dynamical mean-field theory (DMFT) developed in our companion paper establish a precise high-dimensional asymptotic limit for the joint evolution of the prior parameter and law of the Langevin sample. In this work, we carry out an analysis of the equations that describe this DMFT limit, under conditions of approximate time-translation-invariance which include, in particular, settings where the posterior law satisfies a log-Sobolev inequality. In such settings, we show that this adaptive Langevin trajectory converges on a dimension-independent time horizon to an equilibrium state that is characterized by a system of scalar fixed-point equations, and the associated prior parameter converges to a critical point of a replica-symmetric limit for the model free energy. As a by-product of our analyses, we obtain a new dynamical proof that this replica-symmetric limit for the free energy is exact, in models having a possibly misspecified prior and where a log-Sobolev inequality holds for the posterior law.

==> dmftapprox.tex <==
\section{Proof of Theorem \ref{thm:dmft_approx}}
%\subsection{Proof of Parts (a)-(b)}

The proof consists of three steps:
\begin{itemize}
\item (\textbf{Step 1}) We discretize the adaptive Langevin (\ref{eq:langevin_sde})-(\ref{eq:gflow}) and characterize explicitly the discretization error
\item (\textbf{Step 2}) We prove the dynamic mean field limit of this discretized dynamic
\item (\textbf{Step 3}) We show that, as the discretization step size goes to zero, the discrete dynamic mean field equations obtained in the previous step will converge in an appropriate sense to (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}) and (\ref{def:response_theta})-(\ref{def:response_g}).
\end{itemize}

\subsection{Step 1: Discretization of the Langevin dynamic} Recall from (\ref{eq:langevin_sde})-(\ref{eq:gflow}) that with initialization $(\btheta^0, \hat{\alpha}^0)$, the dynamic $\{\btheta^t, \hat{\alpha}^t\}$ follows the update
\begin{align}\label{eq:langevin}
\d\btheta^t &= \Big(- \frac{1}{\sigma^2}\X^\top (\X\btheta^t - \y) + (\log g)'(\btheta^t;\hat{\alpha}^t)\Big)\d t + \sqrt{2}\,\d \b^t,\\
\frac{\d }{\d t}\hat{\alpha}^t &= \cG\Big(\hat{\alpha}^t, d^{-1}\sum_{j=1}^d \delta_{\theta^t_j}\Big),
\end{align}
where $(\log g)'(\btheta^t;\hat{\alpha}^t) = ((\log g)'(\theta^t_1;\hat{\alpha}^t), \ldots, (\log g)'(\theta^t_d;\hat{\alpha}^t)) \in \R^d$. Fix a step size $\gamma > 0$. To define the discretized version $\{\btheta_\gamma^t\}$ and $\{\hat{\alpha}^t_\gamma\}$, let $t_i = i\gamma$ for $i\in \Z_+$, and at these time points, define
\begin{align}
\btheta^{t_{i+1}}_\gamma &= \btheta^{t_i}_\gamma + \gamma\bigg(-\frac{1}{\sigma^2}\X^\top (\X\btheta^{t_i}_\gamma - \y) + \partial_\theta \log g(\btheta^{t_i}_\gamma; \hat{\alpha}^{t_i}_\gamma)\bigg) + \sqrt{2}(\b^{t_{i+1}} - \b^{t_i}), \label{eq:langevin_discrete_1}\\
\hat{\alpha}^{t_{i+1}}_\gamma &= \hat{\alpha}^{t_i}_\gamma + \gamma \cdot \cG\Big(\hat{\alpha}^{t_i}_\gamma, d^{-1}\sum_{j=1}^d \delta_{\theta^{t_i}_{\gamma,j}}\Big)\label{eq:langevin_discrete_2},
\end{align}
with initialization $\btheta^{t_0}_\gamma = \btheta^0$ and $\hat{\alpha}^{t_0}_\gamma = \hat{\alpha}^0$. We now extend the definition to $t\in \R_+$ via linear interpolation. For any $t \geq 0$, let
\begin{align}\label{eq:t_floor_ceil}
\floor{t} = \max\{i\gamma: i\gamma\leq t, i\in \Z_+\},\quad \ceil{t} = \floor{t} + \gamma. 
\end{align}
For any $t\in [i\gamma, (i+1)\gamma)$, let
\begin{align}\label{eq:discrete_langevin}
\btheta_\gamma^{t} &= \frac{t-i\gamma}{\gamma}\btheta_\gamma^{(i+1)\gamma} + \frac{(i+1)\gamma - t}{\eta}\btheta_\gamma^{i\gamma},\\
\hat{\alpha}^t_\gamma &= \frac{t-i\gamma}{\gamma}\hat{\alpha}_\gamma^{(i+1)\gamma} + \frac{(i+1)\gamma - t}{\gamma}\hat{\alpha}_\gamma^{i\gamma}.
\end{align}
Same as before, let $(\bbeta^t)_{t\geq 0} = (\X\btheta^t_\gamma)_{t\geq 0}$.
%For any $m\in \Z_+$ and $t_1,\ldots, t_m \in \R_+$, define the two empirical distributions over $\R^m$:
%\begin{align*}
%\hat{\mu}^{(t_1,\ldots,t_m)} \equiv \frac{1}{d}\sum_{j=1}^d \delta_{(\theta^{t_1}_j, \ldots, \theta^{t_m}_j)}, \quad \hat{\mu}^{(t_1,\ldots,t_m)}_\gamma \equiv \frac{1}{d}\sum_{j=1}^d \delta_{(\theta^{t_1}_{\gamma,j}, \ldots, \theta_{\gamma,j}^{t_m})}.
%\end{align*}

%\begin{assumption}\label{ass:prior}
%We assume the negative log prior $f(\cdot)$ is twice differentiable with $\pnorm{f''}{\infty}\leq L$ for some $L > 0$. 
%\end{assumption}


%\begin{lemma}
%For some universal $K > 0$, it holds almost surely that
%\begin{align*}
%\limsup_{n,d}\limsup_{t\in[0,T]} \frac{1}{\sqrt{d}}\pnorm{\B^t}{} \vee \limsup_{n,d}\limsup_{t\in[0,T]} \frac{1}{\sqrt{d\gamma}}\pnorm{\B^t - \B^{\floor{t}}}{} &\leq K.
%\end{align*}
%\end{lemma}
%\begin{proof}
%For the first claim, since $t\mapsto \pnorm{\B^t}{}$ is a sub-martingale, Doob's maximal inequality yields that 
%\begin{align*}
%\Prob(\limsup_{t\in[0,T]} \frac{1}{\sqrt{d}}\pnorm{\B^t}{} \geq K) \leq 
%\end{align*}
%\end{proof}

\begin{lemma}\label{lem:alpha_boundedness}
Suppose Assumptions \ref{assump:model}, \ref{assump:prior}, \ref{assump:gradient} hold. For any fixed $T > 0$, there exists some $(n,d)$-independent constant $C$ (but depending on $T$ and other problem parameters) such that almost surely as $n,d\rightarrow\infty$, $\sup_{t\in[0,T]} (\pnorm{\btheta^t}{}/\sqrt{d} + \pnorm{\hat{\alpha}^t}{}) \leq C$. Moreover, it holds that $\sup_{t\in[0,T]} \E(\pnorm{\btheta^t}{}^2/d + \pnorm{\hat{\alpha}^t}{}^2) \leq C$.
\end{lemma}
\begin{proof}
Since
\begin{align*}
\btheta^t = \btheta^0 - \int_0^t \Big(\frac{1}{\sigma^2}\X^\top(\X\btheta^s - \y) - \partial_\theta \log g(\btheta^s;\hat{\alpha}^s)\Big)\d s + \sqrt{2}\b^t, 
\end{align*}
by Assumption \ref{assump:prior} we have for every $t\in[0,T]$ that
\begin{align*}
\pnorm{\btheta^t }{} \leq \pnorm{\btheta^0}{} + C(\pnorm{\X}{\op}^2+1)\int_0^t \Big(\pnorm{\btheta^s}{} + \sqrt{d}\pnorm{\hat\alpha^s}{}\Big)\d s + C(\pnorm{\X^\top\y}{} + \sqrt{d} + \sup_{t\in[0,T]} \pnorm{\b^t}{}).
\end{align*}
Next by Assumption \ref{assump:gradient}, we have
\begin{align*}
\pnorm{\hat\alpha^t}{} \leq \pnorm{\hat\alpha^0}{} + C\int_0^t \Big(1+d^{-1}\sum_{j=1}^d |\theta^s_j| + \pnorm{\hat\alpha^s}{}\Big) \d s \leq \pnorm{\hat\alpha^0}{} + C\int_0^t \big(1 + \pnorm{\btheta^s}{}/\sqrt{d} + \pnorm{\hat\alpha^s}{}\big)\d s.
\end{align*}
Combining the above two bounds yields
\begin{align*}
\frac{\pnorm{\btheta^t }{}}{\sqrt{d}} + \pnorm{\hat\alpha^t}{} \leq C(\pnorm{\X}{\op}^2+1)\int_0^t \Big(\frac{\pnorm{\btheta^s}{}}{\sqrt{d}} + \pnorm{\hat\alpha^s}{}\Big)\d s + C\Big(\frac{\pnorm{\btheta^0}{}}{\sqrt{d}} + \pnorm{\hat\alpha^0}{} + \frac{\pnorm{\X^\top\y}{}}{\sqrt{d}} + \sup_{t\in[0,T]} \frac{\pnorm{\b^t}{}}{\sqrt{d}} + 1\Big).
\end{align*}
Hence by Lemma \ref{lem:gronwall}, we have for any $t\in[0,T]$ that
\begin{align*}
\frac{\pnorm{\btheta^t }{}}{\sqrt{d}} + \pnorm{\hat\alpha^t}{} \leq C\exp(C(\pnorm{\X}{\op}^2+1)t)\Big(\frac{\pnorm{\btheta^0}{}}{\sqrt{d}} + \pnorm{\hat\alpha^0}{} + \frac{\pnorm{\X^\top\y}{}}{\sqrt{d}} + \sup_{t\in[0,T]} \frac{\pnorm{\b^t}{}}{\sqrt{d}} + 1\Big).
\end{align*}
%and $\sup_{t\in [0,T]} \pnorm{\hat{\alpha}^t}{} \leq C(T,\pnorm{\hat{\alpha}^0}{})$ which can be readily deduced from Assumption \ref{assump:gradient},
%\begin{align*}
%\pnorm{\partial_\theta \log g(\btheta^s;\hat{\alpha}^s)}{} \leq C(\pnorm{\btheta^s}{} + \pnorm{\partial_\theta \log g(\mathbf{0}_d;\hat{\alpha}^s)}{}) \leq C(\pnorm{\btheta^s}{} + \sqrt{d}),
%\end{align*}
%where here and below $C$ is some constant depending on $T$ and other problem parameters but not on $\gamma$. Hence we have for any $t\in [0,T]$
%\begin{align*}
%\sup_{u\in[0,t]}\pnorm{\btheta^u}{} &\leq \pnorm{\btheta^0}{} + \int_0^t \Big(\frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + C\Big)\pnorm{\btheta^s}{} + C\Big(\pnorm{\X^\top \y}{} + \sqrt{d}\Big)\d s + \sqrt{2}\pnorm{\b^t}{}\\
%&\leq \underbrace{\bigg(\pnorm{\btheta^0}{} + CT\Big(\pnorm{\X^\top \y}{} + \sqrt{d}\Big) + \sqrt{2} \max_{t\in [0,T]} \pnorm{\b^t}{}\bigg)}_{A_1(T)} + \underbrace{\Big(\frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + C\Big)}_{M} \int_0^t \sup_{u\in[0,s]} \pnorm{\btheta^u}{}\d s.
%\end{align*}
%Hence by applying Lemma \ref{lem:gronwall} to the function $t\mapsto \sup_{u\in[0,t]} \pnorm{\btheta^u}{}$, we obtain the bound
%\begin{align}\label{eq:cont_langevin_l2_bound}
%\sup_{u\in[0,t]} \pnorm{\btheta^u}{} \leq A_1(T)\exp(Mt), \quad t\in[0,T]. 
%\end{align}
It is easy to see that under Assumption \ref{assump:model} we have almost surely that
\begin{align*}
\limsup_{n,d} \pnorm{\hat\alpha^0}{} \vee \limsup_{n,d} \frac{1}{\sqrt{d}}\pnorm{\btheta^0}{} \vee \limsup_{n,d}\frac{1}{\sqrt{d}}\pnorm{\X^\top \y}{} \vee \limsup_{n,d}\pnorm{\X}{\op} \leq C,
\end{align*}
so the conclusion follows from the first claim of Lemma \ref{lem:BM_maximal}. The in-expectation claim follows from a simple truncation argument on $\pnorm{\X}{\op}$ and is omitted.
\end{proof}
%\begin{proof}
%Fix $T > 0$. By Assumption \ref{assump:prior}, we have
%\begin{align*}
%\pnorm{\btheta^t}{} &\leq \pnorm{\btheta^0}{} + \int_0^t \Big(\frac{\pnorm{\X}{\op}^2}{\sigma^2}\pnorm{\btheta^s}{} + \frac{1}{\sigma^2}\pnorm{\X^\top \y}{} + \pnorm{\partial_\theta \log g(\btheta^s;\hat{\alpha}^s)}{}\Big) \d s + \pnorm{\b^t}{}\\
%&\leq \pnorm{\btheta^0}{} + \int_0^t \Big(\frac{\pnorm{\X}{\op}^2}{\sigma^2}\pnorm{\btheta^s}{} + \frac{1}{\sigma^2}\pnorm{\X^\top \y}{} + M(\pnorm{\btheta^s}{} + \pnorm{\hat{\alpha}^s}{})\Big) \d s + \pnorm{\b^t}{}, 
%\end{align*}
%and by Assumption \ref{assump:gradient}, 
%\begin{align*}
%\pnorm{\hat{\alpha}}{} \leq \pnorm{\hat{\alpha}^0}{} + \int_0^t M\Big(\pnorm{\hat{\alpha}^s}{} + d^{-1}\sum_{j=1}^d |\theta^t_j| \Big)\d s \leq \pnorm{\hat{\alpha}^0}{} + \int_0^t M\Big(\pnorm{\hat{\alpha}^s}{} + d^{-1/2}\pnorm{\btheta^s}{} \Big)\d s,
%\end{align*}
%where $M > 0$ only depends on the constants in Assumption \ref{assump:prior} and \ref{assump:gradient}. Consider the event $\mathcal{E}_n := \{\pnorm{\X}{\op} \leq C_0, \pnorm{\X^\top \y}{}/\sqrt{d} \leq C_0, \max_{t\in[0,T]} \pnorm{\b^t}{}/\sqrt{d} \leq C_0, \pnorm{\btheta^0}{}/\sqrt{d} \vee \pnorm{\hat{\alpha}^0}{}\leq C_0\}$ for some large enough $C_0 > 0$ (depending on $T$ but independent of $n,d$). By Assumption \ref{assump:model} and standard concentration, event $\mathcal{E}_n$ holds almost surely as $n,d\rightarrow\infty$. On this event, we have for some $C > 0$ (depending on $T$ but independent of $n,d$) that
%\begin{align*}
%\pnorm{\btheta^t}{} \leq C\int_0^t (\pnorm{\btheta^s}{} + \pnorm{\hat{\alpha}^s}{}) \d s + C\sqrt{d}, \qquad \pnorm{\hat{\alpha}^t}{} \leq C + \int_0^t C(\pnorm{\hat{\alpha}^s}{} + \pnorm{\btheta^s}{}/\sqrt{d})\d s,
%\end{align*}
%which further implies that
%\begin{align*}
%\pnorm{\btheta^t}{}/\sqrt{d} + \pnorm{\hat{\alpha}^t}{} \leq C + \int_0^t (\pnorm{\btheta^s}{}/\sqrt{d} + \pnorm{\hat{\alpha}^s}{}) \d s. 
%\end{align*}
%Hence by Lemma \ref{lem:gronwall}, it holds that $\sup_{t\in[0,T]} (\pnorm{\btheta^t}{}/\sqrt{d} +  \pnorm{\hat{\alpha}^t}{}) \leq C'$, as desired. 
%\end{proof}

\begin{lemma}\label{lem:langevin_discretize_error}
Assume the conditions of Theorem \ref{thm:dmft_approx}. Fix $T > 0$. For any fixed $m\in \Z_+$ and $t_1,\ldots, t_m \in [0,T]$, it holds almost surely (with respect to the randomness of $(\X,\y,\b,\btheta^0)$) that as $\gamma \rightarrow 0$,
\begin{align*}
\limsup_{n,d\rightarrow\infty}W_2\Big( \frac{1}{d}\sum_{j=1}^d \delta_{(\theta^{t_1}_j, \ldots, \theta^{t_m}_j)}, \frac{1}{d}\sum_{j=1}^d \delta_{(\theta^{t_1}_{\gamma,j}, \ldots, \theta_{\gamma,j}^{t_m})}\Big) \rightarrow 0,\\
\limsup_{n,d\rightarrow\infty}W_2\Big( \frac{1}{d}\sum_{j=1}^d \delta_{(\eta^{t_1}_j, \ldots, \eta^{t_m}_j)}, \frac{1}{d}\sum_{j=1}^d \delta_{(\eta^{t_1}_{\gamma,j}, \ldots, \eta_{\gamma,j}^{t_m})}\Big) \rightarrow 0,\\
\limsup_{n,d\rightarrow\infty} \bigpnorm{(\hat{\alpha}^{\tau_1}, \ldots, \hat{\alpha}^{\tau_m}) - (\hat{\alpha}_\gamma^{\tau_1}, \ldots, \hat{\alpha}^{\tau_m}_\gamma)}{} \rightarrow 0.
\end{align*}
Moreover, as $\gamma\rightarrow 0$, it holds that
\begin{align*}
\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]} \frac{1}{d}\E \pnorm{\btheta^t - \btheta^t_\gamma}{}^2 \vee \frac{1}{d}\E \pnorm{\bbeta^t - \bbeta^t_\gamma}{}^2 \vee \E \pnorm{\hat\alpha^t - \hat\alpha^t_\gamma}{}^2 \rightarrow 0.
\end{align*}
\end{lemma}
\begin{proof}
We only prove the first set of claims. Note that
\begin{align*}
W_2\Big( \frac{1}{d}\sum_{j=1}^d \delta_{(\theta^{t_1}_j, \ldots, \theta^{t_m}_j)}, \frac{1}{d}\sum_{j=1}^d \delta_{(\theta^{t_1}_{\gamma,j}, \ldots, \theta_{\gamma,j}^{t_m})}\Big) \leq \sqrt{\frac{1}{d}\sum_{\ell=1}^m\sum_{j=1}^d \big(\theta^{t_\ell}_j - (\theta^{t_\ell}_\gamma)_j\big)^2} \leq \sqrt{m} \cdot \frac{1}{\sqrt{d}}\sup_{t\in[0,T]}\pnorm{\btheta^t - \btheta^t_\gamma}{},
\end{align*}
so it suffices to bound $\frac{1}{\sqrt{d}}\max_{t\in[0,T]}\pnorm{\btheta^t - \btheta^t_\gamma}{}$. 


%A similar argument yields that
%\begin{align}\label{eq:bound_theta_norm}
%\sup_{u\in[0,t]} \pnorm{\btheta^u_\gamma}{} \leq A_1(T)\exp(Mt), \quad t\in[0,T],
%\end{align}
%upon noting that $\sup_{t\in[0,T]} \pnorm{\B^t}{} = \sup_{t\in[0,T]} \pnorm{\B^t_\gamma}{}$ (assuming for simplicity that $T = i_0\eta$ for some $i_0\in\Z_+$). 
Now note that the process defined in (\ref{eq:discrete_langevin}) can be equivalently written as
\begin{align*}
\btheta_\gamma^t &= \btheta^0_\gamma - \int_0^t \bigg(\frac{1}{\sigma^2}\X^\top (\X\btheta^{\floor{s}}_\gamma - \y) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma; \hat{\alpha}^{\floor{s}}_\gamma)\bigg)\d s + \sqrt{2}\b^t_\gamma,\\
\hat{\alpha}^t_\gamma &= \hat{\alpha}^0 + \int_0^t \cG\Big(\hat{\alpha}^{\floor{s}}_\gamma, d^{-1}\sum_{j=1}^d \delta_{(\btheta^{\floor{s}}_{\gamma})_j}\Big)\d s,
\end{align*}
where $\{\b^t_\gamma\}_{t\geq 0}$ is a piecewise linear interpolation of $\{\B^t\}$ defined as
\begin{align}\label{eq:hd_BM_linear}
\b^t_\gamma = \frac{t-i\gamma}{\gamma}\b^{(i+1)\gamma} + \frac{(i+1)\gamma - t}{\gamma}\b^{i\gamma}, \quad t\in[i\gamma, (i+1)\gamma).
\end{align} 
Then for any $0 \leq t \leq T$, 
\begin{align*}
\pnorm{\btheta^{t} - \btheta^{t}_\gamma}{} &\leq \int_0^t \pnorm{\Big(\frac{1}{\sigma^2}\X^\top(\X\btheta^s - \y) - \partial_\theta \log g(\btheta^s; \hat{\alpha}^s)\Big) - \Big(\frac{1}{\sigma^2}\X^\top(\X\btheta^{\floor{s}}_\gamma - \y) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma;\hat{\alpha}^{\floor{s}}_\gamma)\Big)}{}\d s + \sqrt{2}\pnorm{\b^t - \b^t_\gamma}{}\\
&\leq  \frac{\pnorm{\X}{\op}^2}{\sigma^2}\int_0^t\pnorm{\btheta^s - \btheta^{\floor{s}}_\gamma}{}\d s + \int_0^t \pnorm{\partial_\theta \log g(\btheta^{s};\hat{\alpha}^{s}) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma;\hat{\alpha}^{\floor{s}}_\gamma)}{}\d s + \sqrt{2}\pnorm{\b^t - \b^t_\gamma}{},
%&\leq  M\int_0^t \big(\pnorm{\btheta^s - \btheta^s_\eta}{} + \pnorm{\btheta^{\floor{s}}_\eta - \btheta^s_\eta}{}\big)\d s  + \sqrt{2}\pnorm{\B^t - \B^t_\eta}{}. 
\end{align*}
where, using Assumption \ref{assump:prior}, bound of $\sup_{t\in[0,T]}\pnorm{\hat{\alpha}^t}{}$ in Proposition \ref{prop:langevinsolution}, and an analogous bound for $\sup_{t\in[0, T]}\pnorm{\hat{\alpha}^t_\gamma}{}$,
\begin{align*}
&\pnorm{\partial_\theta \log g(\btheta^{s};\hat{\alpha}^{s}) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma;\hat{\alpha}^{\floor{s}}_\gamma)}{}\\
&\leq \pnorm{\partial_\theta \log g(\btheta^{s};\hat{\alpha}^{s}) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma;\hat{\alpha}^{s})}{} + \pnorm{\partial_\theta \log g(\btheta^{\floor{s}}_\gamma;\hat{\alpha}^{s}) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma;\hat{\alpha}^{\floor{s}}_\gamma)}{}\\
&\leq C(\pnorm{\btheta^{s} - \btheta^{\floor{s}}_\gamma}{} + \pnorm{\hat{\alpha}^{s} - \hat{\alpha}^{\floor{s}}_\gamma}{}),
\end{align*}
so we have, with $M = \pnorm{\X}{\op}^2/\sigma^2 + C$,
\begin{align*}
\pnorm{\btheta^{t} - \btheta^{t}_\gamma}{} &\leq M\int_0^t\pnorm{\btheta^s - \btheta^{\floor{s}}_\gamma}{}\d s + C\int_0^t \pnorm{\hat{\alpha}^{s} - \hat{\alpha}^{\floor{s}}_\gamma}{}\d s + \sqrt{2}\pnorm{\b^t - \b^t_\gamma}{}\\
&\leq M\int_0^t\big(\pnorm{\btheta^s - \btheta^{s}_\gamma}{} + \pnorm{\btheta^{s}_\gamma - \btheta^{\floor{s}}_\gamma}{}\big)\d s + C\int_0^t \big(\pnorm{\hat{\alpha}^{s} - \hat{\alpha}^{s}_\gamma}{} + \pnorm{\hat{\alpha}^{s}_\gamma - \hat{\alpha}^{\floor{s}}_\gamma}{}\big)\d s + \sqrt{2}\pnorm{\b^t - \b^t_\gamma}{}.
\end{align*}
To bound the middle term, we have by the bound (\ref{eq:cont_langevin_l2_bound}) that for every $s\leq t$,
\begin{align}\label{eq:theta_discrete_error}
\notag\pnorm{\btheta^s_\gamma - \btheta^{\floor{s}}_\gamma}{} &= \biggpnorm{-(s-\floor{s})\Big(\frac{1}{\sigma^2}\X^\top(\X\btheta^{\floor{s}}_\gamma - \y) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma;\hat{\alpha}^{\floor{s}}_\gamma)\Big) + \sqrt{2}(\b^s_\gamma - \b^{\floor{s}}_\gamma)}{}\\
\notag&\leq \gamma \big(M \pnorm{\btheta_\gamma^{\floor{s}}}{} + C\sqrt{d}\big) + \sqrt{2}\pnorm{\b^s_\gamma - \b^{\floor{s}}_\gamma}{}\\
\notag&\leq \gamma \big(M \pnorm{\btheta_\gamma^{\floor{s}} - \btheta^{\floor{s}}}{} + \pnorm{\btheta^{\floor{s}}}{} + C\sqrt{d}\big) + \sqrt{2}\pnorm{\b^s_\gamma - \b^{\floor{s}}_\gamma}{}\\
&\leq \gamma M \sup_{u\in[0,s]}\pnorm{\btheta_\gamma^u - \btheta^u}{} + C\gamma A_1(T)\exp(MT) + \sqrt{2}\sup_{t\in[0,T]}\pnorm{\b^t_\gamma - \b^{\floor{t}}_\gamma}{}, 
\end{align}
and, using the growth condition of $\cG$ in Assumption \ref{assump:gradient}, 
\begin{align}\label{eq:alpha_discrete_error}
\pnorm{\hat{\alpha}^{s}_\gamma - \hat{\alpha}^{\floor{s}}_\gamma}{} = (s - \floor{s})\biggpnorm{\cG\Big(\hat{\alpha}^{\floor{s}}_\gamma, d^{-1}\sum_{j=1}^d \delta_{(\btheta^{\floor{s}}_{\gamma})_j}\Big)}{} \leq C\gamma (\pnorm{\hat{\alpha}^{\floor{s}}_\gamma}{} + 1)\leq C\gamma,
\end{align}
so we have
\begin{align}\label{eq:gronwall_theta}
\notag\pnorm{\btheta^t - \btheta^{t}_\gamma}{} &\leq M^2\int_0^t\sup_{u\in[0,s]}\big(\pnorm{\btheta^u - \btheta^u_\gamma}{} + \pnorm{\hat{\alpha}^{s} - \hat{\alpha}^{s}_\gamma}{}\big)\d s\\
&\quad + C\gamma MA_1(T)\exp(MT) + CM\sup_{t\in[0,T]}\big(\pnorm{\b^t - \b^{\floor{t}}}{} + \pnorm{\b^t - \b^{\ceil{t}}}{}\big).
\end{align}
%We note that the bound on the right side actually applies to $\pnorm{\btheta^u - \btheta^u_\gamma}{}$ for any $u\in[0,t]$, hence
%\begin{align}\label{eq:gronwall_theta_2}
%\notag\sup_{u\in[0,t]}\pnorm{\btheta^u - \btheta^u_\gamma}{} &\leq \gamma M^2\int_0^t\sup_{u\in[0,s]}\big(\pnorm{\btheta^u - \btheta^u_\gamma}{} + \pnorm{\hat{\alpha}^{s} - \hat{\alpha}^{s}_\gamma}{}\big)\d s\\
%&\quad + C\gamma MA_1(T)\exp(MT) + CM\sup_{t\in[0,T]}\big(\pnorm{\b^t - \b^{\floor{t}}}{} + \pnorm{\b^t - \b^{\ceil{t}}}{}\big)
%\end{align}
On the other hand, using Assumption \ref{assump:gradient} and $W_2^2(d^{-1}\sum_{j=1}^d \delta_{u_j}, d^{-1}\sum_{j=1}^d \delta_{v_j}) \leq d^{-1}\pnorm{u-v}{}^2$ for $u,v\in\R^d$, we have
\begin{align*}
\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_\gamma}{} &\leq \int_0^t \biggpnorm{\cG\Big(\hat{\alpha}^s, \frac{1}{d}\sum_{j=1}^d \delta_{(\btheta^s)_j}\Big) - \cG\Big(\hat{\alpha}^{\floor{s}}_\gamma, \frac{1}{d}\sum_{j=1}^d \delta_{(\btheta^{\floor{s}}_\gamma)_j}\Big)}{}\d s\\
&\leq C\int_0^t \Big(\pnorm{\hat{\alpha}^s - \hat{\alpha}^{\floor{s}}_\gamma}{} + \pnorm{\btheta^s - \btheta^{\floor{s}}_\gamma}{}/\sqrt{d}\Big) \d s\\
&\leq CM\int_0^t \sup_{u\in[0,s]}(\pnorm{\hat{\alpha}^u - \hat{\alpha}_\gamma^u}{} + \frac{1}{\sqrt{d}}\pnorm{\btheta^s - \btheta_\gamma^s}{}) \d s\\
&\quad + \frac{C}{\sqrt{d}}\Big(\gamma A_1(T)\exp(MT) + \sqrt{2}\sup_{t\in[0,T]}\big(\pnorm{\b^t - \b^{\floor{t}}}{} + \pnorm{\b^t - \b^{\ceil{t}}}{}\big)\Big).
\end{align*}
Combining the above display with (\ref{eq:gronwall_theta}), we have, with $m(t) = \sup_{u\in[0,t]} (\pnorm{\hat{\alpha}^u - \hat{\alpha}^u_\gamma}{} + \frac{1}{\sqrt{d}}\pnorm{\btheta^u - \btheta^u_\gamma}{})$,
\begin{align*}
\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_\gamma}{} + \frac{1}{\sqrt{d}}\pnorm{\btheta^t - \btheta^t_\gamma}{} \leq M^2\int_0^t m(u)\d s + \underbrace{\frac{CM}{\sqrt{d}}\Big(\gamma A_1(T)\exp(MT)  + \sup_{t\in[0,T]}\big(\pnorm{\b^t - \b^{\floor{t}}}{} + \pnorm{\b^t - \b^{\ceil{t}}}{}\big)\Big)}_{A_2(T)}.
\end{align*}
We note that the right side bound holds actually for $\pnorm{\hat{\alpha}^u - \hat{\alpha}^u_\gamma}{} + \frac{1}{\sqrt{d}}\pnorm{\btheta^u - \btheta^u_\gamma}{}$ for any $u\in[0,t]$, so we conclude that for any $t\in[0,T]$,
\begin{align*}
m(t) \leq M^2\int_0^t m(u)\d s + A_2(T).
\end{align*}
Hence by Lemma \ref{lem:gronwall}, for any $t\in[0,T]$,
\begin{align}\label{eq:joint_alpha_theta}
\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_\gamma}{} + \frac{1}{\sqrt{d}}\pnorm{\btheta^t - \btheta^{t}_\gamma}{} \leq A_2(T)\exp(M^2t).
\end{align}
By Lemma \ref{lem:BM_maximal}, there exists some $K = K(T) > 0$ such that almost surely
\begin{align*}
\limsup_{d}\limsup_{t\in[0,T]} \frac{1}{\sqrt{d}}\pnorm{\b^t}{} \leq K,\quad \limsup_{d}\limsup_{t\in[0,T]} \frac{1}{\sqrt{d\gamma}}\big(\pnorm{\b^t - \b^{\floor{t}}}{} + \pnorm{\b^t - \b^{\ceil{t}}}{}\big) \leq K\sqrt{\log_+(1/\gamma)}.
\end{align*}
On the other hand, it is easy to see that under Assumption \ref{assump:model} we have almost surely that
\begin{align*}
\limsup_{n,d} \frac{1}{\sqrt{d}}\pnorm{\btheta^0}{} \vee \limsup_{n,d}\frac{1}{\sqrt{d}}\pnorm{\X^\top \y}{} \vee \limsup_{n,d}\pnorm{\X}{\op} \leq C,
\end{align*}
proving the claim on $\theta$. The claim on $\eta$ follows from similar arguments and the claim on $\alpha$ follows analogously from (\ref{eq:joint_alpha_theta}).
\end{proof}

\begin{lemma}\label{lem:BM_maximal}
Let $\{\B^t\}_{t\geq 0}$ be a standard Brownian motion on $\R^d$. Then almost surely
\begin{align*}
\limsup_{d}\sup_{t\in[0,T]} \frac{1}{\sqrt{d}}\pnorm{\b^t}{} \leq K, \quad \limsup_{d}\sup_{t\in[0,T]} \frac{1}{\sqrt{d\gamma}}\big(\pnorm{\b^t - \b^{\floor{t}}}{} + \pnorm{\b^t - \b^{\ceil{t}}}{}\big) \leq K\sqrt{\log_+(1/\gamma)}.
\end{align*}
for some $K = K(T) > 0$.
\end{lemma}
\begin{proof}
We first show that for any $a, b \in \R_+$ with $a\leq b$,  $\Prob(\sup_{t\in[a,b]} d^{-1/2}\pnorm{\B^t - \B^a}{} \geq u) \leq \exp\big(-\frac{cdu^2}{2(b-a)}\big)$ for any $u \geq \sqrt{2}(b-a)$. To see this, for any small enough $\lambda > 0$, we have
\begin{align*}
\Prob(\sup_{t\in[a,b]} d^{-1/2}\pnorm{\B^t - \B^a}{} \geq u) &= \Prob(\sup_{t\in[a,b]} \exp(\lambda \pnorm{\B^t - \B^a}{}^2/d) \geq \exp(\lambda u^2))\\
&\leq e^{-\lambda u^2} \E[\sup_{t\in[a,b]}  \exp(\lambda \pnorm{\B^t - \B^a}{}^2/d)]\\
&\stackrel{(*)}{\leq} e^{-\lambda u^2} \E[\exp(\lambda \pnorm{\B^b - \B^a}{}^2/d)] \stackrel{(*)}{=} e^{-\lambda u^2} (1 - \lambda(b-a)/d)^{-d/2},
\end{align*}
where $(*)$ applies Doob's maximal inequality for submartingales since $\x \mapsto \exp(\lambda \pnorm{\x}{}^2)$ is convex, and $(**)$ applies the moment generating function of $\chi^2$ distribution. Choosing $\lambda = cd/(b-a)$ for some small enough $c > 0$ and applying $(1-x) \geq e^{-2x}$ for small $x > 0$, we have 
\begin{align*}
\Prob(\sup_{t\in[a,b]} d^{-1/2}\pnorm{\B^t - \B^a}{} \geq u) \leq \exp\Big(-\frac{cdu^2}{b-a} + cd\Big) \leq \exp\Big(-\frac{cdu^2}{2(b-a)}\Big)
\end{align*}
for $u \geq \sqrt{2(b-a)}$, proving the inequality. For the first claim, we apply this fact with $a = 0, b = T, u = \sqrt{2T}$ to yield that $\Prob(\sup_{t\in[0,T]} d^{-1/2}\pnorm{\B^t}{} \geq \sqrt{2T}) \leq \exp(-cd)$, so the claim follows by summing up the probability over $d$ and applying Borel Cantelli lemma. For the second claim, let $N = T/\gamma$ (assumed for simplicity to be an integer), and $I_i = [(i-1)\gamma, i\gamma)$ for $i\in [N]$, then applying the inequality over these intervals yields
\begin{align*}
\Prob(\sup_{t\in [0,T]} (d\gamma)^{-1/2}\pnorm{\b^t - \b^{\floor{t}}}{} \geq u) \leq N \max_{i\leq N}\Prob\Big(\sup_{t\in I_i} (d\gamma)^{-1/2}\pnorm{\b^t - \b^{i\gamma}}{} \geq u\Big) \leq Ne^{-cdu^2}
\end{align*} 
for any $u\geq \sqrt{2}$. Hence by choosing $u = C\sqrt{\log N}$ for some large enough $C > 0$, we have $\Prob(\sup_{t\in [0,T]} (d\gamma)^{-1/2}\pnorm{\b^t - \b^{\floor{t}}}{} \geq C\sqrt{\log N}) \leq \exp(-cd)$. A similar argument applies to $\sup_{t\in [0,T]} (d\gamma)^{-1/2}\pnorm{\b^t - \b^{\ceil{t}}}{}$, proving the second claim. 
\end{proof}

\subsection{Step 2: Convergence of discrete Langevin dynamic to discrete DMFT equation} 
%\ys{Switch the notation in this section to bar} 
We first define a discretized version of the dynamic mean field equations (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}) and (\ref{def:response_theta})-(\ref{def:response_g}). Recall that $t_i = i \gamma$ for $i\in \Z$, and at these time points, define
\begin{align}
\bar{\theta}^{t_{i+1}}_\gamma &=  \bar{\theta}^{t_i}_\gamma - \frac{\gamma\delta}{\sigma^2}(\bar{\theta}^{t_i}_\gamma - \theta^\ast) + \gamma \partial_\theta \log g(\bar{\theta}^{t_i}_\gamma;\bar{\alpha}^{t_i}_\gamma) + \gamma\sum_{\ell=0}^{i-1} \bar{R}_\eta^\gamma(i,\ell)(\bar{\theta}^{t_\ell}_\gamma - \theta^\ast) +\gamma \bar{u}^{t_i}_\gamma + \sqrt{2}(b^{t_{i+1}} - b^{t_i}),\label{eq:dmft_theta_discrete1}\\
\bar{\eta}^{t_i}_\gamma &= -\frac{1}{\sigma^2}\sum_{\ell=0}^{i-1} \bar{R}^\gamma_\theta(i,\ell)(\bar{\eta}^{t_\ell}_\gamma + \bar{w}^\ast_\gamma - \eps) - \bar{w}^{t_i}_\gamma,\label{eq:dmft_eta_discrete1}\\
\bar{\alpha}_\gamma^{t_{i+1}} &= \bar{\alpha}_\gamma^{t_i} + \gamma \cdot \cG(\bar{\alpha}_\gamma^{t_i}, \cL(\bar{\theta}^{t_i}_\gamma)), \label{eq:dmft_alpha_discrete1}
\end{align}
with initialization $\bar{\theta}^{t_0}_\gamma = \theta^0$, $\bar{\alpha}^{t_0}_\gamma = \alpha^0$ given the same as the system (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}). Here $\theta^\ast, \eps$ and $\delta = \lim n/d$ are given by (\ref{eq:DMFTscalars}), $\{b^t\}_{t\geq 0}$ is an independent univariate standard Brownian motion, and $\{\bar{u}_\gamma^t\}_{t\geq 0}$ and $(\bar{w}_\gamma^\ast, \{\bar{w}_\gamma^t\}_{t\geq 0})$ are independent univariate centered Gaussian processes with covariance kernels 
\begin{align*}
\E[\bar{u}^{t_i}_\gamma \bar{u}^{t_j}_\gamma] = \bar{C}^\gamma_\eta(i,j), \qquad \E[\bar{w}^{t_i}_\gamma \bar{w}^{t_j}_\gamma] = \bar{C}^\gamma_\theta(i,j),\qquad \E[\bar{w}^{t_i}_\gamma \bar{w}^{\ast}_\gamma] = \bar{C}^\gamma_\theta(i,\ast).
\end{align*}
The above covariance and response functions $\bar{C}^\gamma_\theta, \bar{C}^\gamma_\eta, \bar{R}^\gamma_\theta, \bar{R}^\gamma_\eta$ are recursively defined for all $i\geq j \geq 0$ by
\begin{align}
\bar{C}^\gamma_\theta(i,j) &= \E[\bar{\theta}^{t_i}_\gamma\bar{\theta}^{t_j}_\gamma], \quad \bar{C}_\theta^\gamma(i,\ast) = \E[\bar{\theta}^{t_i}_\gamma\theta^\ast],\quad \bar{C}^\gamma_\eta(i,j) = \frac{\delta}{\sigma^4}\E[(\bar{\eta}^{t_i}_\gamma + \bar{w}^\ast_\gamma - \eps)(\bar{\eta}_\gamma^{t_j} + \bar{w}^\ast_\gamma - \eps)] \label{eq:dmft_covariance},\\
\bar{R}^\gamma_\theta(i,j) &= \E\Big[\overline{\frac{\partial \theta^{t_i}_\gamma}{\partial u^{t_j}_\gamma}}\Big], \quad \bar{R}^\gamma_\eta(i,j) = \frac{\delta}{\sigma^2}\E\Big[\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^{t_j}_\gamma}}\Big], \label{eq:dmft_response}%\quad \bar{R}^\gamma_\eta(i,\ast) = \frac{\delta}{\sigma^2}\E\Big[\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^\ast_\gamma}}\Big], 
\end{align}
where the stochastic processes $\{\overline{\frac{\partial \theta^{t_i}_\gamma}{\partial u^{t_j}_\gamma}}\}_{i>j}$, $\{\overline{\frac{\partial \eta_\gamma^{t_i}}{\partial w_\gamma^{t_j}}}\}_{i > j}$ are understood in the standard sense of derivatives and therefore satisfy by direct calculation
\begin{align}
\overline{\frac{\partial \theta^{t_i}_\gamma}{\partial u^{t_j}_\gamma}}  &= 
\begin{cases}
\Big[1-\frac{\gamma\delta}{\sigma^2} + \gamma \partial^2_\theta \log g(\bar{\theta}^{t_{i-1}}_\gamma;\bar{\alpha}^{t_{i-1}}_\gamma)\Big]\overline{\frac{\partial \theta_\gamma^{t_{i-1}}}{\partial u_\gamma^{t_j}}} + \gamma\sum_{\ell=j+1}^{i-2} \bar{R}^\gamma_\eta(i-1,\ell)\overline{\frac{\partial \theta_\gamma^{t_\ell}}{\partial u_\gamma^{t_j}}} & j < i-1,\\
\gamma & j = i-1,
\end{cases}\label{eq:response_1}\\
\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^{t_j}_\gamma}} &= -\frac{1}{\sigma^2}\sum_{\ell=j}^{i-1} \bar{R}^\gamma_\theta(i,\ell) \overline{\frac{\partial \eta_\gamma^{t_\ell}}{\partial w_\gamma^{t_j}}} = \frac{1}{\sigma^2}\Big[-\sum_{\ell=j+1}^{i-1}\bar{R}^\gamma_\theta(i,\ell) \overline{\frac{\partial \eta^{t_\ell}_\gamma}{\partial w^{t_j}_\gamma}} + \bar{R}^\gamma_\theta(i,j)\Big], \quad j < i \label{eq:response_2}.
%\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w_\gamma^\ast}} &= -\frac{1}{\sigma^2}\sum_{\ell=0}^{i-1} \bar{R}_\theta^\gamma(i,\ell)\Big(\overline{\frac{\partial \eta^{t_\ell}_\gamma}{\partial w^\ast_\gamma}} - 1\Big)\label{eq:response_3}.
\end{align}
Similar to (\ref{eq:discrete_langevin}), we may extend (\ref{eq:dmft_theta_discrete1})-(\ref{eq:dmft_alpha_discrete1}) to continuous-time processes: for any $t\in \R_+$, let
\begin{align}\label{eq:discrete_dmft}
\bar{\theta}_\gamma^{t} = \frac{t-\floor{t}}{\gamma}\bar{\theta}_\gamma^{\ceil{t}} + \frac{\ceil{t} - t}{\gamma}\bar{\theta}_\gamma^{\floor{t}}, \qquad \bar{\eta}_\gamma^{t} = \bar{\eta}_\gamma^{\floor{t}}, \qquad \bar{\alpha}^t_\gamma = \frac{t-\floor{t}}{\gamma}\bar{\alpha}_\gamma^{\ceil{t}} + \frac{\ceil{t} - t}{\gamma}\bar{\alpha}_\gamma^{\floor{t}}.
%\eta_\gamma^{t} = \frac{t-i\gamma}{\gamma}\eta_\gamma^{(i+1)\gamma} + \frac{(i+1)\gamma - t}{\eta}\eta_\gamma^{i\gamma}.
%\hat{\alpha}^t_\gamma &= \frac{t-i\gamma}{\gamma}\hat{\alpha}_\gamma^{(i+1)\gamma} + \frac{(i+1)\gamma - t}{\gamma}\hat{\alpha}_\gamma^{i\gamma}.
\end{align}
The reason that we use piecewise linear interpolation for $\{\bar{\theta}^t_\gamma\}_{t\in\R_+}$ and piecewise constant interpolation for $\{\bar{\eta}_\gamma^t\}_{t\in\R_+}$ will become clear in Lemma \ref{lem:discrete_dmft_rewrite} below.

In addition to the two responses in (\ref{eq:response_1})-(\ref{eq:response_2}), consider the following auxiliary response function
\begin{align}
\bar{R}^\gamma_\eta(i,\ast) = \frac{\delta}{\sigma^2}\E\Big[\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^\ast_\gamma}}\Big] \quad \text{ where }\quad \overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w_\gamma^\ast}} &= -\frac{1}{\sigma^2}\sum_{\ell=0}^{i-1} \bar{R}_\theta^\gamma(i,\ell)\Big(\overline{\frac{\partial \eta^{t_\ell}_\gamma}{\partial w^\ast_\gamma}} + 1\Big)\label{eq:response_3},
\end{align}
initialized from $\overline{\frac{\partial \eta^{t_0}_\gamma}{\partial w_\gamma^\ast}} = 0$. This is the standard derivative of $\bar{\eta}^{t_i}_\gamma$ with respect to $\bar{w}_\gamma^\ast$. We have the following basic fact relating the response functions (\ref{eq:response_2}) and (\ref{eq:response_3}).
\begin{lemma}\label{lem:eta_response_id}
The sequences $\{\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^{t_j}_\gamma}}\}_{i > j}$ and $\{\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^\ast_\gamma}}\}$ are deterministic and satisfy $\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^\ast_\gamma}} = -\sum_{j=0}^{i-1} \overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^{t_j}_\gamma}}$. Consequently, for any $i\geq 1$, $\bar{R}_\eta^\gamma(i,\ast) = -\sum_{j=0}^{i-1} \bar{R}_\eta^\gamma(i,j)$.
\end{lemma}
\begin{proof}
Let us use shorthand $r_\eta(i,j) = \overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^{t_j}_\gamma}}$ for $j<i$ and $r_\eta(i,\ast) = \overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^\ast_\gamma}}$.
Since the initializations $r_\eta(1,0) = \gamma/\sigma^2$ and $r_\eta(1,\ast) = -\gamma/\sigma^2$ are deterministic, both sequences are deterministic. We prove the identity by induction, with the baseline case just verified. Suppose the claim holds for some $i$, then
\begin{align*}
r_\eta(i+1,\ast) &= -\frac{1}{\sigma^2}\sum_{\ell=0}^i \bar{R}_\theta^\gamma(i+1,\ell)(r_\eta(\ell, \ast) + 1)\\
&= -\frac{1}{\sigma^2}\sum_{\ell=0}^i \bar{R}_\theta^\gamma(i+1,\ell)\Big(-\sum_{s=0}^{\ell-1} r_\eta(\ell,s) + 1\Big)\\
&= \frac{1}{\sigma^2}\Big[\sum_{s=0}^{i-1} \sum_{\ell=s+1}^i \bar{R}_\theta^\gamma(i+1,\ell)r_\eta(\ell,s) - \sum_{s=0}^i \bar{R}_\theta^\gamma(i+1,s)\Big]\\
&= \frac{1}{\sigma^2}\sum_{s=0}^{i-1}\Big(\sum_{\ell=s+1}^i \bar{R}_\theta^\gamma(i+1,\ell)r_\eta(\ell,s) - \bar{R}_\theta^\gamma(i+1,s)\Big) - \frac{1}{\sigma^2}\bar{R}_\theta^\gamma(i+1,i)\\
&= -\sum_{s=0}^{i-1} r_\eta(i+1,s) - r_\eta(i+1,i) =  -\sum_{s=0}^{i} r_\eta(i+1,s),
\end{align*}
as desired.
\end{proof}

Recall $\btheta^t_{\gamma}, \hat{\alpha}^t_\gamma$ defined in (\ref{eq:discrete_langevin}) and $\bbeta^t_\gamma = \X\btheta^t_\gamma$.
\begin{lemma}\label{lem:finite_dim_converge}
Assume the conditions of Theorem \ref{thm:dmft_approx}. For any $m\in\Z_+$ and $\tau_1,\ldots,\tau_m \in \R_+$, it holds almost surely as $n,d\rightarrow\infty$ that
\begin{gather}
\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_{\gamma,j}, \ldots, \btheta^{\tau_m}_{\gamma,j},\btheta^\ast_j\big)}  \overset{W_2}{\to}  \sP\big(\bar{\theta}^{\tau_0}_\gamma,\ldots, \bar{\theta}^{\tau_m}_\gamma,\theta^\ast\big),\label{eq:finite_dim_converge_knot_theta}\\
\qquad \frac{1}{n}\sum_{i=1}^n \delta_{\big(\bbeta^{\tau_1}_{\gamma,i}, \ldots, \bbeta^{\tau_m}_{\gamma,i}, (\X\btheta^\ast)_i, \beps_i\big)} \overset{W_2}{\to} \sP\big(\bar{\eta}^{\tau_1}_\gamma,\ldots, \bar{\eta}^{\tau_m}_\gamma, w^\ast,\eps\big),\label{eq:finite_dim_converge_knot_eta}\\
(\hat{\alpha}^{\tau_1}_\gamma,\ldots,\hat{\alpha}^{\tau_m}_\gamma) \rightarrow (\bar{\alpha}^{\tau_1}_\gamma, \ldots, \bar{\alpha}^{\tau_m}_\gamma)\label{eq:finite_dim_converge_knot_alpha}.
%\frac{1}{d}\sum_{j=1}^d \psi\Big((\btheta^{t_{i_1}}_{\gamma})_j,\ldots, (\btheta^{t_{i_m}}_{\gamma})_j, (\btheta^\ast)_j\Big) &\rightarrow_P \E\Big[\psi(\theta^{t_{i_1}}_\gamma, \ldots, \theta^{t_{i_m}}_\gamma, \theta^\ast)\Big],\\
%\frac{1}{n}\sum_{i=1}^n \phi\Big((\boldeta^{t_{i_1}}_{\gamma})_i,\ldots, (\boldeta^{t_{i_m}}_{\gamma})_i; (\X\btheta^\ast)_i, (\beps)_i\Big) &\rightarrow_P \E\Big[\phi(\eta^{t_{i_1}}_\gamma, \ldots, \eta^{t_{i_m}}_\gamma; \omega^\ast,\eps)\Big].
\end{gather}
%and bounded Lipschitz functions $\psi: \R^m \times \R\rightarrow \R$ and $\phi: \R^{m}\times \R^2\rightarrow \R$,
%\begin{align}\label{eq:finite_dim_converge}
%\frac{1}{d}\sum_{j=1}^d \psi\Big((\btheta^{\tau_1}_{\gamma})_j,\ldots, (\btheta^{\tau_m}_{\gamma})_j; (\btheta^\ast)_j\Big) \rightarrow_P \E\Big[\psi(\theta^{\tau_1}_\gamma, \ldots, \theta^{\tau_m}_\gamma; \theta^\ast)\Big],\\
%\frac{1}{n}\sum_{i=1}^n \phi\Big((\boldeta^{\tau_1}_{\gamma})_i,\ldots, (\boldeta^{\tau_m}_{\gamma})_i; (\X\btheta^\ast)_i, (\beps)_i\Big) \rightarrow_P \E\Big[\phi(\eta^{\tau_1}_\gamma, \ldots, \eta^{\tau_m}_\gamma; \omega^\ast,\eps)\Big].
%\end{align}
%Consequently,
%\begin{align*}
%\dbl\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1}_{\gamma})_j,\ldots, (\btheta^{\tau_m}_{\gamma})_j, (\btheta^\ast)_j\big)}, \cL\big(\theta^{\tau_1}_\gamma, \ldots, \theta^{\tau_m}_\gamma,\theta^\ast\big)\Big) &\rightarrow_P 0,\\
%\dbl\Big(\frac{1}{n}\sum_{i=1}^n \delta_{\big((\boldeta^{\tau_1}_{\gamma})_i,\ldots, (\boldeta^{\tau_m}_{\gamma})_i, (\X\btheta^\ast)_i, (\beps)_i\big)}, \cL\big(\eta^{\tau_1}_\gamma, \ldots, \eta^{\tau_m}_\gamma,\omega^\ast,\eps\big)\Big) &\rightarrow_P 0.
%\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:finite_dim_converge}]
\textbf{Step 1: Reduction to knots} Fix some $T > 0$ such that $\tau_1,\ldots,\tau_m \in [0,T]$. Let $N = T/\gamma$, and it suffices to prove the desired conclusion for the knots $\{t_i\}_{i=0}^{N}$, i.e, almost surely as $n,d\rightarrow\infty$,
\begin{gather}
\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{t_0}_{\gamma,j}, \ldots, \btheta^{t_N}_{\gamma,j},\btheta^\ast_j\big)}  \overset{W_2}{\to}  \sP\big(\bar{\theta}^{t_0}_\gamma,\ldots, \bar{\theta}^{t_N}_\gamma, \theta^\ast\big),\label{eq:finite_dim_converge_knot_theta}\\
\frac{1}{n}\sum_{i=1}^n \delta_{\big(\bbeta^{t_0}_{\gamma,i}, \ldots, \bbeta^{t_N}_{\gamma,i}, (\X\btheta^\ast)_i, \beps_i\big)} \overset{W_2}{\to} \sP\big(\bar{\eta}^{t_0}_\gamma,\ldots, \bar{\eta}^{t_N}_\gamma, w^\ast,\eps\big),\label{eq:finite_dim_converge_knot_eta}\\
(\hat{\alpha}^{t_0}_\gamma,\ldots,\hat{\alpha}_\gamma^{t_N}) \rightarrow (\bar{\alpha}^{t_0}_\gamma, \ldots, \bar{\alpha}_\gamma^{t_N})\label{eq:finite_dim_converge_knot_alpha}.
%\frac{1}{d}\sum_{j=1}^d \psi\Big((\btheta^{t_{i_1}}_{\gamma})_j,\ldots, (\btheta^{t_{i_m}}_{\gamma})_j, (\btheta^\ast)_j\Big) &\rightarrow_P \E\Big[\psi(\theta^{t_{i_1}}_\gamma, \ldots, \theta^{t_{i_m}}_\gamma, \theta^\ast)\Big],\\
%\frac{1}{n}\sum_{i=1}^n \phi\Big((\boldeta^{t_{i_1}}_{\gamma})_i,\ldots, (\boldeta^{t_{i_m}}_{\gamma})_i; (\X\btheta^\ast)_i, (\beps)_i\Big) &\rightarrow_P \E\Big[\phi(\eta^{t_{i_1}}_\gamma, \ldots, \eta^{t_{i_m}}_\gamma; \omega^\ast,\eps)\Big].
\end{gather}

Indeed, if (\ref{eq:finite_dim_converge_knot_theta}) holds for any $\{t_{i_\ell}\}$, then for any $\{\tau_i\}_{i=1}^m$, we can write $\tau_\ell = \lambda_\ell t_{i_\ell} + (1-\lambda_\ell) t_{i_\ell+1}$. Let $U = (U_0,\ldots, U_N)$ and $V = (V_0,\ldots,V_N)$ be an optimal $W_2$-coupling of $\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{t_0}_{\gamma,j}, \ldots, \btheta^{t_N}_{\gamma,j}\big)}$ and $ \sP\big(\bar{\theta}^{t_0}_\gamma,\ldots, \bar{\theta}^{t_N}_\gamma\big)$. Now define $\tilde{U} = (\tilde{U}_1,\ldots, \tilde{U}_m)$ and $\tilde{V} = (\tilde{V}_1,\ldots,\tilde{V}_m)$, where $\tilde{U}_\ell = \lambda_\ell X_{i_\ell} + (1-\lambda_\ell)X_{i_\ell+1}$ and $\tilde{V}_\ell = \lambda_\ell V_{i_\ell} + (1-\lambda_\ell) V_{i_\ell+1}$. Then it is easy to check that $(\tilde{U}, \tilde{V})$ is a coupling of $\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_{\gamma,j}, \ldots, \btheta^{\tau_m}_{\gamma,j}\big)}$ and $\sP\big(\bar{\theta}^{\tau_1}_\gamma,\ldots, \bar{\theta}^{\tau_m}_\gamma\big)$ (for $\tilde{U}$ this follows by viewing $U$ as a realization of the pair $(U,J)$ where $J$ is uniform on $[d]$ and $U|J=j$ takes value $(\btheta^{t_0}_{\gamma,j},\ldots, \btheta^{t_N}_{\gamma,j})$), and by convexity of the square function
\begin{align*}
W_2\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_{\gamma,j}, \ldots, \btheta^{\tau_m}_{\gamma,j}\big)}, \sP\big(\bar{\theta}^{\tau_1}_\gamma,\ldots, \bar{\theta}^{\tau_m}_\gamma\big)\Big) &\leq \E \pnorm{\tilde{U}-\tilde{V}}{}^2 \leq m \cdot\E\pnorm{U-V}{}^2\\
&= m\cdot W_2\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{t_0}_{\gamma,j}, \ldots, \btheta^{t_N}_{\gamma,j}\big)}, \sP\big(\bar{\theta}^{t_0}_\gamma,\ldots, \bar{\theta}^{t_N}_\gamma\big)\Big) \rightarrow_{a.s.} 0.
\end{align*}
A similar argument holds for the $\eta$ side, proving the claim. We will now prove (\ref{eq:finite_dim_converge_knot_theta})-(\ref{eq:finite_dim_converge_knot_alpha}).

\textbf{Step 2: Construction of auxiliary dynamic}
Consider the following sequence (here and for the rest of the proof we denote temporarily the Brownian motion $\b^{t_i}$ in (\ref{eq:langevin_discrete_1}) as $\B^{t_i}$ to avoid notation clash)
\begin{align}\label{def:langevin_auxiliary}
\tilde{\btheta}_\gamma^{t_{i+1}} = \tilde{\btheta}_\gamma^{t_i} - \gamma\bigg(\frac{1}{\sigma^2}\X^\top (\X\tilde{\btheta}^{t_i}_\gamma - \X\btheta^\ast - \beps) - \partial_\theta \log g(\tilde{\btheta}^{t_i}_\gamma;\bar{\alpha}^{t_i}_\gamma)\bigg) + \sqrt{2}(\B^{t_{i+1}} - \B^{t_i}),
\end{align}
where $\{\B^t\}$ is the same as in (\ref{eq:langevin_discrete_1}), and the initialization is $\tilde{\btheta}^{t_0}_\gamma = \btheta^{t_0}_\gamma$. Note that we replace $\{\hat{\alpha}^{t_i}_\gamma\}$ in $\{\btheta^{t_i}_\gamma\}$ by $\{\bar{\alpha}^{t_i}_\gamma\}$. Let $\tilde{\bbeta}^{t_i}_{\gamma} := \X\tilde{\btheta}^{t_i}_{\gamma}$. We will show
\begin{align}\label{eq:emp_converge_aux}
\frac{1}{d}\sum_{j=1}^d \delta_{\big(\tilde{\btheta}^{t_0}_{\gamma,j}, \ldots, \tilde{\btheta}^{t_N}_{\gamma,j}, \btheta^\ast_j\big)}  \overset{W_2}{\to}  \sP\big(\bar{\theta}^{t_0}_\gamma,\ldots, \bar{\theta}^{t_N}_\gamma,\theta^\ast\big), \qquad \frac{1}{n}\sum_{i=1}^n \delta_{\big(\tilde{\bbeta}^{t_0}_{\gamma,i}, \ldots, \tilde{\bbeta}^{t_N}_{\gamma,i}, (\X\btheta^\ast)_i, \beps_i\big)} \overset{W_2}{\to} \sP\big(\bar{\eta}^{t_0}_\gamma,\ldots, \bar{\eta}^{t_N}_\gamma, w^\ast, \eps\big).
\end{align}




%For simplicity, we assume $i_1,i_1+1,i_2,i_2+1,\ldots, i_m, i_m+1$ are mutually distinct (the other cases with duplicated indices follow from similar arguments). Then for each $j\in [d]$
%\begin{align*}
%\psi\Big((\btheta^{\tau_1}_{\gamma})_j,\ldots, (\btheta^{\tau_m}_{\gamma})_j; (\btheta^\ast)_j\Big) = \tilde{\psi}\Big((\btheta^{t_{i_1}}_{\gamma})_j,(\btheta^{t_{i_1+1}}_{\gamma})_j\ldots, (\btheta^{t_{i_m}}_{\gamma})_j, (\btheta^{t_{i_m+1}}_{\gamma})_j; (\btheta^\ast)_j\Big),
%\end{align*}
%where the function $\tilde{\psi}: \R^{2m+1}\rightarrow\R$ is defined by
%\begin{align*}
%\tilde{\psi}(u_1,v_1,\ldots, u_m,v_m; w) = \psi(\lambda_1u_1 + (1-\lambda_1) v_1, \ldots, \lambda_m u_m + (1-\lambda_m) v_m; w). 
%\end{align*}
%It is easy to verify that if $\psi$ is bounded and $L$-Lipschitz, then $\tilde{\psi}$ is also bounded and $CL$-Lipschitz for some $C$ that only depends on $m$, hence the desired conclusion will follow. 


The proof is based on reduction to an AMP algorithm. Given external randomness $\z\in\R^{n\times m_1}$ and $\v \in \R^{d\times m_2}$ such that, with $z_i$ (resp. $v_j$) denoting the (transpose of) the $i$th (resp. $j$th) row of $\z$ (resp. $\v$),
\begin{align}\label{eq:amp_empirical}
\frac{1}{n}\sum_{i=1}^n \delta_{z_i} \overset{W_2}{\to} Z \in \R^{m_1}, \quad \frac{1}{d}\sum_{j=1}^d \delta_{v_j} \overset{W_2}{\to} V\in\R^{m_2},
\end{align}
consider the AMP algorithm: with initialization $\b^0 = \X g_0(\v)$,
\begin{equation}\label{eq:amp}
\begin{aligned}
\a^{i+1} &= -\frac{1}{\delta}\X^\top f_i(\b^0,\ldots,\b^i;\z) + \sum_{j=0}^i g_j(\a^1,\ldots, \a^j;\v)\xi_{ij} \in \R^{d\times k},\\
\b^i &= \X g_i(\a^1,\ldots,\a^i;\v) + \frac{1}{\delta}\sum_{j=0}^{i-1} f_j(\b^0,\ldots,\b^j;\z) \zeta_{ij} \in \R^{n\times k}, 
\end{aligned}
\end{equation}
where the non-linearities 
\begin{align*}
f_i &=  \big(f_{i,1},\ldots, f_{i,k}\big): \R^{k(i+1)} \times \R^{m_1} \rightarrow \R^k,\qquad g_i = \big(g_{i,1},\ldots, g_{i,k}\big): \R^{ki} \times \R^{m_2} \rightarrow \R^k
\end{align*}
are applied row-wise . Once the non-linearities are fixed, the Onsager coefficients can be recursively defined as
\begin{align*}
\xi_{ij} &= \bigg(\E\Big[\frac{\partial}{\partial w^j}f_i(w^0,\ldots, w^i;Z)\Big]\bigg)^\top \in \R^{k\times k}, \quad 0\leq j\leq i,\\
\zeta_{ij} &= \bigg(\E\Big[\frac{\partial }{\partial u^{j+1}} g_i(u^1,\ldots,u^i;V)\Big]\bigg)^\top \in \R^{k\times k},\quad 0\leq j\leq i-1,
\end{align*}
where $\{w^j\}_{0\leq j\leq i}$ and $\{u^j\}_{0\leq j\leq i-1}$ are Gaussian vectors in $\R^k$ with covariance structure
\begin{align}\label{eq:amp_gp_cov}
\notag\E[w^i(w^j)^\top] &= \E\Big[g_i(u^1,\ldots,u^i;V)  \Big(g_j(u^1,\ldots,u^j;V)\Big)^\top\Big] \in \R^{k\times k}, \quad 0\leq j\leq i < \infty,\\
\E[u^{i+1}(u^{j+1})^\top] &=  \frac{1}{\delta}\E\Big[f_i(w^0,\ldots, w^{i};U) \Big(f_j(w^0,\ldots, w^j;U)\Big)^\top\Big] \in \R^{k\times k},\quad 0\leq j\leq i < \infty. 
\end{align}
State evolution predicts that almost surely as $n,d\rightarrow\infty$, with $V$ (resp. $Z$) independent of $(u^1,\ldots,u^m)$ (resp. $w^0,\ldots,w^m$) in the joint laws below, %for any bounded Lipschitz functions $\psi_j:\R^{mk} \times \R^k \rightarrow \R$ and $\phi_i:\R^{(m+1)k} \times \R \rightarrow \R$, as $n,d\rightarrow\infty$, 
\begin{equation}\label{eq:state_evolution}
\begin{gathered}
\frac{1}{d}\sum_{j=1}^d \delta_{(\a^1)_j,\ldots, (\a^m)_j, (\v)_j} \overset{W_2}{\to} \sP(u^1,\ldots,u^m;V),\\
\frac{1}{n}\sum_{i=1}^n \delta_{(\b^0)_i,\ldots, (\b^m)_i, (\z)_i} \overset{W_2}{\to} \sP(w^0,\ldots,w^m;Z).
\end{gathered}
\end{equation}

We will now use the above state evolution to prove the desired conclusion (\ref{eq:emp_converge_aux}). We start by lifting the $\R^d$-dynamic $\{\tilde{\btheta}^{t_i}_\gamma\}_{i\in\Z}$ in (\ref{def:langevin_auxiliary}) to the following $\R^{d\times 2}$ dynamic $\bar{\btheta}^{t_{i+1}}_\gamma = (\tilde{\btheta}_\gamma^{t_{i+1}},\btheta^\ast)$, where $\{\tilde{\btheta}_\gamma^{t_{i}}\}$
%\begin{align*}
%\btheta_\gamma^{t_{i+1}} = \btheta_\gamma^{t_i} - \gamma\bigg(\frac{1}{\sigma^2}\X^\top (\X\btheta^{t_i}_\gamma - \X\btheta^\ast - \beps) - \partial_\theta \log g(\btheta^{t_i}_\gamma;\hat{\alpha}^{t_i}_\gamma)\bigg) + \sqrt{2}(\B^{t_{i+1}} - \B^{t_i})
%\end{align*}
is the same as in (\ref{def:langevin_auxiliary}), and the initialization is $\bar{\btheta}^{t_0}_\gamma = (\tilde{\btheta}^{t_0}_\gamma, \btheta^\ast)$. In the AMP algorithm (\ref{eq:amp}), let $k = 2$, $\z = \beps \in \R^n$ and $\v = (\btheta^0, \btheta^\ast, \B^{t_1}-\B^{t_0}, \ldots, \B^{t_{N+1}} - \B^{t_N}) \in \R^{d\times (2 + (N+1))}$, such that (\ref{eq:amp_empirical}) holds with
\begin{align}\label{eq:side_empirical}
Z = \sP(\eps), \quad V = g_0 \otimes g_\ast \otimes \N(0, \gamma I_{N+1})
\end{align}
by Assumption \ref{assump:model}. We will now show the existence of nonlinearities $g_j = (g_{j,1}, g_{j,2}): \R^{2j} \times \R^{2+(N+1)} \rightarrow \R^2$ and $f_j = (f_{j,1}, f_{j,2}): \R^{2(j+1)} \times \R \rightarrow \R^2$ such that %\ys{change the brownian motion notation to $\w^t$ or $\W^t$?}
\begin{align}%\label{eq:nonlinearity_planted}
\bar{\btheta}^{t_j}_\gamma = (\tilde{\btheta}^{t_j}_\gamma, \btheta^\ast) &= g_j(\a^1,\ldots,\a^j;\v),\label{eq:nonlinearity_1}\\ %+ (\sqrt{2}(\w^{t_j} - \w^{t_{j-1}}), 0_d),\\
\Big(\frac{1}{\sigma^2}(\X\tilde{\btheta}^{t_j}_\gamma - \X\btheta^\ast - \beps), 0\Big) &= f_j(\b^0,\ldots, \b^j; \beps),\label{eq:nonlinearity_2}
\end{align}
which represent $\bar{\btheta}^{t_j}_\gamma$ and $\X\bar{\btheta}_\gamma^{t_j}$ as nonlinear transforms of aymptotically Gaussian covariates $\{\a^i\}, \{\b^i\}$. The baseline case is $g_0(\v) = \bar{\btheta}^0_\gamma$ and with  $\b^0 = \X\bar{\btheta}^0_\gamma = (\X\tilde{\btheta}^0_\gamma, \X\btheta^\ast) := (\b^0_1,\b^0_2) \in \R^{n\times 2}$, we choose $f_{0,1}(\b^0;\beps) = \frac{1}{\sigma^2}(\b^0_1 - \b^0_2 - \beps)$, $f_{0,2}(\b^0;\beps) = 0$. For induction, suppose the nonlinearities have been chosen up until $g_j$ and $f_j$ so that up to $\a^{j+1}$ and $\b^j$ in the AMP are defined, and it holds that $g_{\ell,2}(\a^1,\ldots,\a^\ell;\v) = \btheta^\ast$ and $f_{\ell,2}(\b^0,\ldots,\b^\ell;\beps) = 0$ for $\ell\leq j$, which further implies that $(\xi_{\ell \ell'})_{12} = (\xi_{\ell \ell'})_{22} = (\zeta_{\ell \ell'})_{12} = (\zeta_{\ell \ell'})_{22} = 0$. Note that with $\a^{j} = (\a^j_1, \a^j_2) \in \R^{d\times 2}$,
\begin{align*}
\a^{j+1}_1 &= -\frac{1}{\delta}\X^\top f_{j,1}(\b^0,\ldots,\b^j;\beps) + \sum_{\ell=0}^j \Big(g_{\ell,1}(\a^1,\ldots, \a^\ell;\v)(\xi_{j\ell})_{11} + g_{\ell,2}(\a^1,\ldots, \a^\ell;\v)(\xi_{j\ell})_{21}\Big)\\
&= -\frac{1}{\delta\sigma^2}\X^\top(\X\tilde{\btheta}^{t_{j}}_\gamma - \X\btheta^\ast - \beps) + \sum_{\ell=0}^j g_{\ell,1}(\a^1,\ldots, \a^\ell;\v)(\xi_{j\ell})_{11} + \sum_{\ell=0}^j (\xi_{j\ell})_{21} \cdot \btheta^\ast, 
\end{align*}
we have 
\begin{align*}
\tilde{\btheta}^{t_{j+1}}_\gamma &= \tilde{\btheta}^{t_j}_\gamma - \gamma\bigg(\frac{1}{\sigma^2}\X^\top (\X\tilde{\btheta}^{t_j}_\gamma - \X\btheta^\ast - \beps) - \partial_\theta \log g(\tilde{\btheta}^{t_j}_\gamma;\bar{\alpha}^{t_j}_\gamma)\bigg) + \sqrt{2} (\B^{t_{j+1}} - \B^{t_j})\\
&= \tilde{\btheta}^{t_j}_\gamma + \gamma \delta \cdot \Big(\a^{j+1}_1 - \sum_{\ell=0}^j g_{\ell,1}(\a^1,\ldots, \a^\ell;\v)(\xi_{j\ell})_{11} -  \sum_{\ell=0}^j (\xi_{j\ell})_{21} \cdot \btheta^\ast\Big) + \gamma\partial_\theta \log g(\tilde{\btheta}^{t_j}_\gamma;\bar{\alpha}^{t_j}_\gamma) + \sqrt{2} (\B^{t_{j+1}} - \B^{t_j}),
\end{align*}
so to satisfy (\ref{eq:nonlinearity_1}) we may define $g_{j+1}(\cdot)$ as: $g_{j+1,2}(a^1,\ldots, a^{j+1};v) = \theta^\ast$, and
\begin{align}\label{eq:g_planted}
\notag g_{j+1,1}(a^1,\ldots, a^{j+1};v) &= g_{j,1}(a^1,\ldots, a^{j};v) + \gamma \delta \cdot \Big(a^{j+1}_1- \sum_{\ell=0}^j g_{\ell,1}(a^1,\ldots, a^\ell;v)(\xi_{j\ell})_{11} -  \sum_{\ell=0}^j (\xi_{j\ell})_{21} \cdot \theta^\ast\Big)\\
&\quad + \gamma \partial_\theta \log g\big(g_{j,1}(a^1,\ldots, a^{j};v);\bar{\alpha}^{t_j}_\gamma\big) + \sqrt{2} \rho_j,
\end{align}
where we write $v = (\theta^0,\theta^\ast,\rho_1,\ldots,\rho_{N+1})$. This implies $(\zeta_{j+1,\ell})_{12} = (\zeta_{j+1,\ell})_{22} = 0$ for $\ell\leq j$, and allows us to compute $\b^{j+1} = (\b^{j+1}_1, \b^{j+1}_2)$ as $\b^{j+1}_2 = \X\btheta^\ast$, and 
\begin{align*}
\b^{j+1}_1 &= \X g_{j+1,1}(\a^1,\ldots,\a^{j+1};\v) + \frac{1}{\delta}\sum_{\ell=0}^{j} \Big(f_{\ell,1}(\b^0,\ldots,\b^\ell;\beps) (\zeta_{j+1,\ell})_{11} + f_{\ell,2}(\b^0,\ldots,\b^\ell;\beps) (\zeta_{j+1,\ell})_{21}\Big)\\
&= \X\tilde{\btheta}^{t_{j+1}}_\gamma + \frac{1}{\delta}\sum_{\ell=0}^{j} f_{\ell,1}(\b^0,\ldots,\b^\ell;\beps) (\zeta_{j+1,\ell})_{11}.
\end{align*}
Hence with 
\begin{align*}
\frac{1}{\sigma^2}(\X\tilde{\btheta}^{t_{j+1}}_\gamma - \X\btheta^\ast - \beps) = \frac{1}{\sigma^2}\Big(\b^{j+1}_1 - \b^{j+1}_2 - \frac{1}{\delta}\sum_{\ell=0}^{j} f_{\ell,1}(\b^0,\ldots,\b^\ell;\beps) (\zeta_{j+1,\ell})_{11} - \beps\Big),
\end{align*}
to satisfy (\ref{eq:nonlinearity_2}) we can define: $f_{j+1,2} = 0$, and
\begin{align}\label{eq:f_planted}
f_{j+1,1}(b^0,\ldots, b^{j+1};\eps) = \frac{1}{\sigma^2}\Big(b^{j+1}_1 - b^{j+1}_2 - \frac{1}{\delta}\sum_{\ell=0}^{j} f_{\ell,1}(b^0,\ldots,b^\ell;\eps) (\zeta_{j+1,\ell})_{11} - \eps\Big).
\end{align}
Using an induction argument, it is easy to show that $f_j$ and $g_j$ are both Lipschitz functions. So using (\ref{eq:nonlinearity_1})-(\ref{eq:nonlinearity_2}), state evolution (\ref{eq:state_evolution}), and the fact that $f(X_n) \overset{W_2}{\to} f(X)$ for Lipschitz $f$ provided $X_n \overset{W_2}{\to} X$, we conclude that
\begin{align*}
\frac{1}{d}\sum_{j=1}^d \delta_{\big(\tilde{\btheta}^{t_0}_{\gamma,j}, \ldots, \tilde{\btheta}^{t_N}_{\gamma,j},\btheta^\ast_j\big)}  \overset{W_2}{\to}  \sP\big(\theta^{0},\ldots, \theta^{N},\theta^\ast\big),\qquad\frac{1}{n}\sum_{i=1}^n \delta_{\big(\tilde{\bbeta}^{t_0}_{\gamma,i}, \ldots, \tilde{\bbeta}^{t_N}_{\gamma,i}, (\X\btheta^\ast)_i, \beps_i\big)} \overset{W_2}{\to} \sP\big(\eta^0,\ldots, \eta^N, w^\ast, \eps\big)
\end{align*}
%With $f_j, g_j$ chosen according to (\ref{eq:g_planted}) and (\ref{eq:f_planted}) so that (\ref{eq:nonlinearity_1})-(\ref{eq:nonlinearity_2}) hold, for any bounded Lipschitz $\psi:\R^{m+1}\rightarrow\R$, 
%\begin{align*}
%\frac{1}{d}\sum_{j=1}^d \psi\Big((\btheta^0)_j,\ldots, (\btheta^m)_j; \btheta^\ast_j\Big) = \frac{1}{d}\sum_{j=1}^d \tilde{\psi}_j\Big((\a^1)_j, \ldots, (\a^m)_j; (\bar{\btheta}^0)_j\Big), 
%\end{align*}
%where
%\begin{align*}
%\tilde{\psi}_j(a_1,\ldots, a_m;\bar{\theta}^0) = \psi\Big(g_{1,1}^{(j)}(a_1;\bar{\theta}^0),\ldots, g_{m,1}^{(j)}(a_1,\ldots, a_m; \bar{\theta}^0); \theta^\ast\Big).
%\end{align*}
%Consequently, the state evolution (\ref{eq:state_evolution}) predicts that
%\begin{align*}
%\frac{1}{d}\sum_{j=1}^d \psi\Big((\btheta^{t_0})_j, \ldots, (\btheta^{t_m})_j;\btheta^\ast\Big) &\rightarrow_P \E\Big[\psi(\theta^0,\ldots, \theta^m;\theta^\ast)\Big],\\
%\frac{1}{n}\sum_{i=1}^n \phi\Big((\X\btheta^{t_0})_i, \ldots, (\X\btheta^{t_m})_i; \X\btheta^\ast,\beps\Big) &\rightarrow_P \E\Big[\phi(\eta^0,\ldots, \eta^m;\omega^\ast,\eps)\Big].
%\end{align*}
Here for $i\geq 1$, 
\begin{align*}
\theta^i = g_i(u^1,\ldots, u^i;v), \quad \eta^i = \sigma^2f_{i}(w^0,\ldots,w^i;\eps) + w^\ast + \eps,
\end{align*}
where $\{u^i\} = \{(u^i_1, u^i_2)\}$ and $\{w^i\} = \{(w^i_{1}, w^i_2)\} \equiv \{(w^i_1, w^\ast)\}$ are Gaussian processes with covariance kernel given by (\ref{eq:amp_gp_cov}), and $v = (\theta^0,\theta^\ast,\rho_1,\ldots,\rho_{N+1})$ (resp. $\eps$) is distributed as $V$ (resp. $Z$) in (\ref{eq:side_empirical}) independent of $\{u^i\}$ (resp. $\{w^i\}$).
% and in view of (\ref{eq:g_planted}) and (\ref{eq:f_planted}), $g_i: \R^{2i}\times \R^2 \rightarrow\R$ and $f_i: \R^{2(i+1)}\times \R \rightarrow\R$ are recursively defined by
%\begin{align}\label{eq:g_scalar}
% \notag g_{i+1}(a^1,\ldots, a^{i+1};v) &= g_i(a^1,\ldots, a^i;\bar{\theta}^0) + \gamma \delta \cdot \Big(a^{i+1}_1 - \sum_{\ell=0}^i g_{\ell}(a^1,\ldots, a^\ell;\bar{\theta}^0)(\xi_{i\ell})_{11} -  \sum_{\ell=0}^i (\xi_{i\ell})_{21} \cdot \theta^\ast\Big)\\
%&\quad - \gamma f'\big(g_i(a^1,\ldots, a^i;\bar{\theta}^0)\big) + \sqrt{2\gamma}\rho^i
%\end{align}
%and
%\begin{align}\label{eq:f_scalar}
%f_{i+1}(b^0,\ldots, b^{i+1};\eps) = \frac{1}{\sigma^2}\Big(b^{i+1}_1 - b^{i+1}_2 - \frac{1}{\delta}\sum_{\ell=0}^{i} f_{\ell}(b^0,\ldots,b^\ell;\eps) (\zeta_{i+1,\ell})_{11} - \eps\Big),
%\end{align}
%with $\{\rho^i\}$ denoting i.i.d. standard normal variables independent of $\{u^i\}, \{w^i\}, \bar{\theta}^0, \eps$.
Let us now show that
\begin{align}\label{eq:discrete_equald}
\sP(\theta^0,\ldots,\theta^N,\theta^\ast) = \sP\big(\bar{\theta}^{t_0}_\gamma,\ldots, \bar{\theta}^{t_N}_\gamma,\theta^\ast\big), \qquad \sP(\eta^0,\ldots,\eta^N,w^\ast,\eps) = \sP\big(\bar{\eta}^{t_0}_\gamma,\ldots, \bar{\eta}^{t_N}_\gamma, w^\ast, \eps\big),
\end{align}
which will conclude the proof of (\ref{eq:emp_converge_aux}). By definition of $g_{j+1,1}(\cdot)$ in (\ref{eq:g_planted}), we have
\begin{align}\label{eq:theta^t}
\notag\theta^{j+1} &= g_{j+1,1}(u^1,\ldots, u^{j+1};v)\\
\notag&= \theta^j + \gamma\delta\Big(u^{j+1}_1 - \sum_{\ell=0}^j \theta^\ell (\xi_{j,\ell})_{11} - \sum_{\ell=0}^j (\xi_{j,\ell})_{21} \cdot \theta^\ast\Big) + \gamma\partial_\theta \log g\big(\theta^j;\bar{\alpha}^{t_j}_\gamma\big) + \sqrt{2}\rho_j\\
&= \theta^j - \gamma\delta \Big((\xi_{j,j})_{11}\theta^j + (\xi_{j,j})_{21}\theta^\ast\Big) + \gamma\partial_\theta \log g\big(\theta^j;\bar{\alpha}^{t_j}_\gamma\big) - \gamma\delta \cdot \sum_{\ell=0}^{j-1} \theta^\ell (\xi_{j,\ell})_{11} - \gamma\delta \cdot \sum_{\ell=0}^{j-1} (\xi_{j,\ell})_{21} \cdot \theta^\ast+ \gamma\delta u^{j+1}_1 + \sqrt{2}\rho_j,
\end{align} 
and by definition of $f_{j,1}(\cdot)$ in (\ref{eq:f_planted}),
\begin{align}\label{eq:eta^t}
\eta^j &= \sigma^2 f_{j,1}(w^0,\ldots,w^t;\eps) + w^\ast + \eps = -\frac{1}{\delta\sigma^2}\sum_{\ell=0}^{j-1} (\zeta_{j,\ell})_{11}(\eta^\ell - w^\ast -  \eps) + w^j_1,
\end{align}
using the fact that $w^t_2 \equiv w^\ast$. Let us now derive the recursions of the following quantities:
%To specify $\{\xi_{t,s}\} = \{\E[\frac{\partial f_t}{\partial w^s}]\} \in \R^{2\times 2}$ and $\{\zeta_{t,s}\} = \{\E[\frac{\partial g_t}{\partial u^{s+1}}]\}\in\R^{2\times 2}$, recall that $(\frac{\partial f_t}{\partial w^s})_{12} = (\frac{\partial f_t}{\partial w^s})_{22} = (\frac{\partial g_t}{\partial u^{s+1}})_{12} = (\frac{\partial g_t}{\partial u^{s+1}})_{22} = 0$, so it remains to build a recursion for
\begin{equation}\label{eq:xi_zeta_simplify}
\begin{aligned}
(\zeta_{j,s})_{11} = \E\Big[\frac{\partial g_{j,1}}{\partial u^{s+1}_1}(u^1,\ldots,u^j;\bar{\theta}^0)\Big],\quad(\xi_{j,s})_{11} = \Big[\frac{\partial f_{j,1}}{\partial w^{s}_1}(w^1,\ldots,w^j;\eps)\Big],\quad(\xi_{j,s})_{21} = \E\Big[\frac{\partial f_{j,1}}{\partial w^{s}_2}(w^1,\ldots,w^j;\eps)\Big].
\end{aligned}
\end{equation}
%we will first build a recursion for $\{\frac{\partial f_t}{\partial w^s}\} = \{\frac{\partial f_t(w^0,\ldots,w^t;\eps)}{\partial w^s}\}$ and $\{\frac{\partial g_t}{\partial u^{s+1}}\} = \{\frac{\partial g_t(u^1,\ldots,u^t;\bar{\theta}^0)}{\partial u^{s+1}}\}$. 
By definition of $g_{j,1}$ in (\ref{eq:g_planted}), we have $\{\frac{\partial g_{j,1}}{\partial u^{s+1}_1}\} = 0$ for $s \geq j$, $\{\frac{\partial g_{j,1}}{\partial u_1^{s+1}}\} = \gamma\delta$ if $s = j-1$, and if $s \leq j-2$, 
\begin{align}\label{eq:g_recursion}
\notag\frac{\partial g_{j,1}}{\partial u^{s+1}_1} &= \frac{\partial g_{j-1,1}}{\partial u^{s+1}_1} - \gamma \delta \sum_{\ell=s+1}^{j-1} \frac{\partial g_{\ell,1}}{\partial u^{s+1}_1}(\xi_{j-1,\ell})_{11} + \gamma \partial_\theta^2 \log g(g_{j-1,1}; \bar{\alpha}^{t_{j-1}}_\gamma) \frac{\partial g_{j-1,1}}{\partial u_1^{s+1}}\\
&= \Big(1-\gamma\delta(\xi_{j-1,j-1})_{11} + \gamma \partial_\theta^2 \log g(g_{j-1,1}; \bar{\alpha}^{t_{j-1}}_\gamma)\Big)\frac{\partial g_{j-1,1}}{\partial u_1^{s+1}} - \gamma \delta \sum_{\ell=s+1}^{j-2} (\xi_{j-1,\ell})_{11}\frac{\partial g_{\ell,1}}{\partial u_1^{s+1}}.
\end{align}
Similarly, by definition of $f_{j,1}(\cdot)$ in (\ref{eq:f_planted}), we have $\{\frac{\partial f_{j,1}}{\partial w_1^s}\} = 0$ if $s > j$, $\{\frac{\partial f_{j,1}}{\partial w_1^s}\} = 1/\sigma^2$ if $s = j$, and if $s < j$,
\begin{align}\label{eq:f_recursion}
\frac{\partial f_{j,1}}{\partial w^s_1} = -\frac{1}{\delta\sigma^2}\sum_{\ell=s}^{j-1} \frac{\partial f_{\ell,1}}{\partial w^s_1} (\zeta_{j,\ell})_{11} = -\frac{1}{\delta\sigma^2}\Big(\sum_{\ell=s+1}^{j-1} \frac{\partial f_{\ell,1}}{\partial w^s_1} (\zeta_{j,\ell})_{11} + \frac{1}{\sigma^2}(\zeta_{j,s})_{11}\Big).
\end{align}
%Let $\bar{u}^j = \delta u^{j+1}_1$ with $\frac{\partial g_{j,1}}{\partial \bar{u}^s} = \frac{1}{\delta}\frac{\partial g_{j,1}}{\partial u^{s+1}_1}$, and
Define
\begin{align}\label{eq:amp_response}
\notag R_\theta(j,s) &:= \frac{1}{\delta}\E\Big[\frac{\partial g_{j,1}}{\partial u^{s+1}_1}(u^1,\ldots,u^j;\bar{\theta}^0)\Big] = \frac{1}{\delta}(\zeta_{j,s})_{11},\\
R_\eta(j,s) &:= -\delta\E\Big[\frac{\partial f_{j,1}}{\partial w^s_1}(w^1,\ldots,w^j;\eps)\Big] = -\delta (\xi_{j,s})_{11}.
\end{align}
Then by (\ref{eq:g_recursion}) and (\ref{eq:f_recursion}), $\{\frac{\partial g_{j,1}}{\partial u^{s+1}_1}\}$ and $\{\frac{\partial f_{j,1}}{\partial w^s_1}\}$ satisfy the recursion 
\begin{align*}
\frac{\partial g_{j,1}}{\partial u^{s+1}_1} &= \Big(1 - \frac{\gamma\delta}{\sigma^2} + \gamma \partial^2_\theta \log g(g_{j-1,1};\bar{\alpha}^{t_{j-1}}_\gamma)\Big)\frac{\partial g_{j-1,1}}{\partial u^{s+1}_1} + \gamma \sum_{\ell=s+1}^{j-2} R_\eta(j-1,\ell) \frac{\partial g_{\ell,1}}{\partial u^{s+1}_1},\\
\frac{\partial f_{j,1}}{\partial w^s_1} &= -\frac{1}{\sigma^2}\Big(\sum_{\ell=s+1}^{j-1} R_\theta(j,\ell)\frac{\partial f_{\ell,1}}{\partial w^s_1} + \frac{1}{\sigma^2}R_\theta(j,s)\Big).
\end{align*}
This identity hold for any arguments of $\frac{\partial g_{j,1}}{\partial u^{s+1}}$ and $\frac{\partial f_{j,1}}{\partial w^s_1}$, so plugging in $\{u^t\}$ and $\{w^t\}$, we arrive at the random processes
\begin{align*}
\frac{\partial g_{j,1}}{\partial u^{s+1}}(u^1,\ldots,u^j;v) &= \Big(1 - \frac{\gamma\delta}{\sigma^2} + \gamma \partial^2_\theta \log g(\theta^{j-1};\bar{\alpha}^{t_{j-1}}_\gamma)\Big)\frac{\partial g_{j-1,1}}{\partial u^{s+1}}(u^1,\ldots,u^{t-1};v) + \gamma \sum_{\ell=s+1}^{j-2} R_\eta(j-1,\ell) \frac{\partial g_{\ell,1}}{\partial u^{s+1}}(u^1,\ldots,u^\ell;v),\\
\frac{\partial f_{j,1}}{\partial w^s_1}(w^0,\ldots,w^j;\eps) &= -\frac{1}{\sigma^2}\Big(\sum_{\ell=s+1}^{j-1} R_\theta(j,\ell)\frac{\partial f_{\ell,1}}{\partial w^s_1}(w^0,\ldots,w^\ell;\eps) + \frac{1}{\sigma^2}R_\theta(j,s)\Big).
\end{align*}
In view of the boundary conditions established above, comparing with (\ref{eq:response_1})-(\ref{eq:response_2}) yields that
\begin{align*}
\delta\overline{\frac{\partial \theta^{t_{i}}_\gamma}{\partial u^{t_j}_\gamma}} \stackrel{d}{=} \frac{\partial g_{i,1}}{\partial u^{j+1}}(u^1,\ldots,u^i;v), \quad -\frac{1}{\sigma^2}\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial w^{t_j}_\gamma}} \stackrel{d}{=}\frac{\partial f_{i,1}}{\partial w^j_1}(w^0,\ldots,w^i;\eps), \quad  \bar{R}^\gamma_\theta(i,j) =  R_\theta(i,j), \quad  \bar{R}^\gamma_\eta(i,j) =  R_\eta(i,j).
\end{align*}
It remains to specify $A_j := \sum_{\ell=0}^{j-1} (\xi_{j,\ell})_{21} = \sum_{\ell=0}^{j-1}\frac{\partial f_{s,1}}{\partial w^{\ell}_2}$ in (\ref{eq:theta^t}). In view of (\ref{eq:xi_zeta_simplify}), we will build a recursion for $\frac{\partial f_{j,1}}{\partial w^{\ell}_2} (w^0,\ldots,w^j;\eps)$. By definition, we have (note that $\frac{\partial f_{j,1}}{\partial w^{\ell}_2}$ is a deterministic sequence)
\begin{align*}
(\xi_{j,\ell})_{21} = \frac{\partial f_{j,1}}{\partial w^{\ell}_2}  = 
\begin{cases}
-\frac{1}{\delta\sigma^2}\sum_{s=0}^{j-1}\frac{\partial f_{s,1}}{\partial w^{\ell}_2}  (\zeta_{js})_{11} & \ell < j,\\
-\frac{1}{\sigma^2} & \ell = j
\end{cases}.
\end{align*}
So using $\delta^{-1}(\zeta_{ts})_{11} = R_\theta(t,s)$, we have
\begin{align*}
A_j = -\frac{1}{\sigma^2}\sum_{\ell=0}^{j-1}\sum_{s=\ell}^{j-1} \frac{\partial f_{s,1}}{\partial w^\ell_2} R_\theta(j,s) = -\frac{1}{\sigma^2} \sum_{s=0}^{j-1} R_\theta(j,s) \sum_{\ell=0}^{s} \frac{\partial f_{s,1}}{\partial w^\ell_2} =  -\frac{1}{\sigma^2} \sum_{s=0}^{j-1} R_\theta(j,s) (A_s - \frac{1}{\sigma^2}),
\end{align*}
which coincides with the recursion for $-\{\frac{1}{\sigma^2} \overline{\frac{\partial \eta_\gamma^{t_i}}{\partial \omega^\ast}}\}$ in (\ref{eq:response_3}). So we conclude $A_i = -\frac{1}{\sigma^2}\overline{\frac{\partial \eta^{t_i}_\gamma}{\partial \omega^\ast}} = -\frac{1}{\delta} \bar{R}^\gamma_\eta(i,\ast) = \frac{1}{\delta}\sum_{j=0}^{i-1} \bar{R}^\gamma_\eta(i,j)$, where the last step follows from Lemma \ref{lem:eta_response_id}.



In view of Lemma \ref{lem:eta_response_id}, we may now rewrite the equations (\ref{eq:theta^t}) and (\ref{eq:eta^t}) as
\begin{align*}
\theta^{j+1} &= \theta^j - \frac{\gamma\delta}{\sigma^2}(\theta^j - \theta^\ast) + \gamma\partial_\theta \log g\big(\theta^j;\bar{\alpha}^{t_j}_\gamma\big) + \gamma \sum_{\ell=0}^{j-1} \bar{R}^\gamma_\eta(j,\ell)(\theta^\ell  - \theta^\ast) + \gamma \delta u^{j+1}_1 + \sqrt{2}\rho_j,\\
\eta^j &= -\frac{1}{\sigma^2}\sum_{\ell=0}^{j-1} \bar{R}^\gamma_\theta(j,\ell)(\eta^\ell - w^\ast - \eps) + w^j_1, 
\end{align*}
where $\{u^t_1\}$ and $\{w_1^t\}$ are centered Gaussian variables in $\R$ with covariance structure
\begin{align*}
 \E[u_1^{t+1}u_1^{s+1}] &= \frac{1}{\delta}\E[f_t(w^0,\ldots, w^t;\eps) f_s(w^0,\ldots, w^s;\eps)] = \frac{1}{\delta\sigma^4}\E[(\eta^t-w^\ast-\eps)(\eta^s - w^\ast - \eps)], \\
\E[w_1^tw_1^s] &= \E[g_t(u^1,\ldots,u^t;v)g_s(u^1,\ldots,u^s;v)] = \E[\theta^t\theta^s].
\end{align*}
This implies that $\delta u^{j+1} \stackrel{d}{=} \bar{u}^{t_j}_\gamma$ and $-(w^j,w^\ast) \stackrel{d}{=}( \bar{w}^{t_j}_\gamma,w^\ast)$, and concludes (\ref{eq:discrete_equald}) and therefore the proof of (\ref{eq:emp_converge_aux}).


\textbf{Step 3: Completing the proof} Let us finally prove (\ref{eq:finite_dim_converge_knot_theta})-(\ref{eq:finite_dim_converge_knot_alpha}), which concludes the whole proof. We will prove via induction the claim that, almost surely as $n,d\rightarrow\infty$
\begin{align}\label{eq:aux_diff}
\frac{1}{d}\sum_{j=0}^{N} \pnorm{\btheta^{t_j}_\gamma - \tilde{\btheta}^{t_j}_\gamma}{}^2 \rightarrow 0, \qquad (\hat{\alpha}^{t_0}_\gamma, \ldots, \hat{\alpha}^{t_N}_\gamma) \rightarrow (\bar{\alpha}^{t_0}_\gamma, \ldots, \bar{\alpha}^{t_N}_\gamma). 
\end{align}
By a standard coupling argument, we have
\begin{align*}
W_2\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{t_0}_{\gamma,j}, \ldots, \btheta^{t_N}_{\gamma,j},\btheta^\ast_j\big)}, \frac{1}{d}\sum_{j=1}^d \delta_{\big(\tilde{\btheta}^{t_0}_{\gamma,j}, \ldots, \btheta^{t_N}_{\gamma,j},\btheta^\ast_j\big)}\Big) \leq \frac{1}{d}\sum_{\ell=0}^N \pnorm{\btheta^{t_j}_\gamma - \tilde{\btheta}^{t_j}_\gamma}{}^2, 
\end{align*}
so together with (\ref{eq:emp_converge_aux}) the above claim will imply (\ref{eq:finite_dim_converge_knot_theta})-(\ref{eq:finite_dim_converge_knot_alpha}). We will prove by induction on the discrete time index. The base case of (\ref{eq:aux_diff}) holds exactly. Suppose (\ref{eq:aux_diff}) holds up to time $t_j$, so that $\frac{1}{d}\sum_{\ell=1}^d \delta_{\big(\btheta^{t_0}_{\gamma,\ell}, \ldots, \btheta^{t_j}_{\gamma,\ell}\big)}  \overset{W_2}{\to}  \sP\big(\bar{\theta}^{t_0}_\gamma,\ldots, \bar{\theta}^{t_j}_\gamma\big)$. For $t_{j+1}$, we see that
\begin{align*}
\frac{1}{d}\pnorm{\btheta^{t_{j+1}}_\gamma - \tilde{\btheta}^{t_{j+1}}_\gamma}{}^2 &\leq C\Big((1+\pnorm{\X}{\op}^4)\frac{1}{d}\pnorm{\btheta^{t_j}_\gamma - \tilde{\btheta}^{t_j}_\gamma}{}^2 + \frac{1}{d}\pnorm{\partial_\theta \log g(\btheta^{t_j}_\gamma; \hat{\alpha}^{t_j}_\gamma) - \partial_\theta \log g(\tilde{\btheta}^{t_j}_\gamma; \bar{\alpha}^{t_j}_\gamma)}{}^2\Big).
%&\leq C\Big((1+\pnorm{\X}{\op}^4)\frac{1}{d}\pnorm{\btheta^{t_j}_\gamma - \tilde{\btheta}^{t_j}_\gamma}{}^2 + \frac{1}{d}\pnorm{\partial_\theta \log g(\btheta^{t_j}_\gamma; \hat{\alpha}^{t_j}_\gamma) - \partial_\theta \log g(\tilde{\btheta}^{t_j}_\gamma; \bar{\alpha}^{t_j}_\gamma)}{}^2
\end{align*} 
Since $\pnorm{\X}{\op}$ is almost surely bounded, we have by the induction hypothesis that $(1+\pnorm{\X}{\op}^4)\frac{1}{d}\pnorm{\btheta^{t_j}_\gamma - \tilde{\btheta}^{t_j}_\gamma}{}^2 \rightarrow 0$ almost surely. Next using Assumption \ref{assump:prior}, we have
\begin{align*}
\frac{1}{d}\pnorm{\partial_\theta \log g(\btheta^{t_j}_\gamma; \hat{\alpha}^{t_j}_\gamma) - \partial_\theta \log g(\tilde{\btheta}^{t_j}_\gamma; \bar{\alpha}^{t_j}_\gamma)}{}^2 &\leq \frac{2}{d}\pnorm{\partial_\theta \log g(\btheta^{t_j}_\gamma; \hat{\alpha}^{t_j}_\gamma) - \partial_\theta \log g(\btheta^{t_j}_\gamma; \bar{\alpha}^{t_j}_\gamma)}{}^2\\
&\quad + \frac{2}{d}\pnorm{\partial_\theta \log g(\btheta^{t_j}_\gamma; \bar{\alpha}^{t_j}_\gamma) - \partial_\theta \log g(\tilde{\btheta}^{t_j}_\gamma; \bar{\alpha}^{t_j}_\gamma)}{}^2
\end{align*} 
and both terms converge almost surely to 0. We hence conclude $\frac{1}{d}\pnorm{\btheta^{t_{j+1}}_\gamma - \tilde{\btheta}^{t_{j+1}}_\gamma}{}^2 \rightarrow 0$ almost surely. Next we have by Assumption \ref{assump:gradient} that 
\begin{align*}
\pnorm{\hat{\alpha}^{t_{j+1}}_\gamma - \bar{\alpha}_\gamma^{t_{j+1}}}{} &\leq \pnorm{\hat{\alpha}^{t_{j}}_\gamma - \bar{\alpha}_\gamma^{t_{j}}}{} + \gamma \pnorm{\cG(\hat{\alpha}^{t_j}_\gamma, \frac{1}{d}\sum_{\ell=1}^d \delta_{(\btheta^{t_j}_{\gamma})_\ell}) - \cG(\bar{\alpha}^{t_{j}}_\gamma, \sP(\bar{\theta}^{t_j}_\gamma))}{}\\
&\leq C\pnorm{\hat{\alpha}^{t_{j}}_\gamma - \bar{\alpha}_\gamma^{t_{j}}}{} + CW_2\Big(\frac{1}{d}\sum_{\ell=1}^d  \delta_{(\btheta^{t_j}_{\gamma})_\ell}, \sP(\bar{\theta}^{t_j}_\gamma)\Big) \rightarrow 0
\end{align*}
almost surely by the induction hypothesis. This establishes the induction for (\ref{eq:aux_diff}) and hence completes the proof.
\end{proof}

\subsection{Step 3: Discretization error of DMFT equation} 
%\ys{change notation to without bar} 
We first show that the continuous-time processes (\ref{eq:discrete_dmft}) can be rewritten in a way that is closer to the DMFT equations (\ref{def:dmft_langevin_cont_theta})-(\ref{def:response_g}). Recall $\floor{t}$ and $\ceil{t}$ defined in (\ref{eq:t_floor_ceil}). Consider the following continuous-time system
\begin{align}
\theta^t_\gamma &= \theta^0 + \int_0^t\Big[-\frac{\delta}{\sigma^2}(\theta^{\floor{s}}_{\gamma} - \theta^\ast) + \partial_\theta \log g(\theta^{\floor{s}}_\gamma) + \int_0^{\floor{s}} R^\gamma_\eta(\floor{s}, \floor{s'})(\theta_\gamma^{\floor{s'}} - \theta^\ast)\d s'  + \bar{u}^s_\gamma\Big]\d s + \sqrt{2}b^{t}_\gamma,\label{def:dmft_piecelinear_theta}\\
\eta^t_\gamma &= -\frac{1}{\sigma^2}\int_0^{\floor{t}} R^\gamma_\theta(\floor{t},\ceil{s})(\eta^s_\gamma + w^\ast_\gamma - \eps)\d s - w^t_\gamma \label{def:dmft_piecelinear_eta},\\
\alpha^t_\gamma &= \alpha^0 + \int_0^t \cG(\alpha_\gamma^{\floor{s}}, \sP(\theta^{\floor{s}}_\gamma))\d s \label{def:dmft_piecelinear_alpha}. 
\end{align}
Here $(\theta^0, \alpha^0)$ are the same initialization as in (\ref{eq:discrete_dmft}), $(\theta^\ast, \eps)$ are auxiliary variables to the system also the same as in (\ref{eq:discrete_dmft}), $\{b^t_\gamma\}$ is defined as the linear interpolation of a standard Brownian motion similar to (\ref{eq:hd_BM_linear}), i.e., 
 \begin{align}\label{eq:bm_piece_linear}
 b^t_\gamma = 
% \begin{cases}
 %B^t & t = i\gamma,\\
 \frac{t-i\gamma}{\gamma}b^{(i+1)\gamma} + \frac{(i+1)\gamma - t}{\gamma}b^{i\gamma}, \quad t \in [i\eta, (i+1)\eta),
% \end{cases}
 \end{align}
$\{u^t_\gamma \}_{t\geq 0}$ and $(w^\ast_\gamma, \{w^t_\gamma\}_{t\geq 0})$ are independent univariate centered Gaussian processes with covariance kernels
\begin{align*}
\E[u^t_\gamma u^s_\gamma] = C^\gamma_\eta(t,s), \quad \E[w^t_\gamma w^s_\gamma] = C^\gamma_\theta(t,s), \quad \E[w^t_\gamma w^\ast_\gamma] = C^\gamma_\theta(t,\ast).
\end{align*}
The above covariance and response functions $C_\theta^\gamma, C_\eta^\gamma, R_\theta^\gamma, R_\eta^\gamma$ are self-consistently defined for all $t \geq s \geq 0$ by
%\frac{\d}{\d t}g^\gamma_t(u) &= F(g_{\floor{t}}^\gamma, \cL(\theta^{\floor{t}}_\gamma)),\\
\begin{align}
R^\gamma_\theta(t,s) &= \E\Big[\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}\Big], \quad R^\gamma_\eta(t,s) = \frac{\delta}{\sigma^2}\E\Big[\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma}\Big], \label{def:dmft_piecelinear_Rg}\\%\quad R^\gamma_\eta(t,\ast) = \frac{\delta}{\sigma^2}\E\Big[\frac{\partial \eta^t_\gamma}{\partial w^\ast_\gamma}\Big],
C_\theta^\gamma(t,s) &= \E\Big[\theta^{\floor{t}}_\gamma \theta^{\floor{s}}_\gamma\Big], \quad C_\theta^\gamma(t,\ast) = \E\Big[\theta^{\floor{t}}_\gamma \theta^\ast\Big], \quad C^\gamma_\eta(t,s) = \frac{\delta}{\sigma^4} \E\Big[(\eta^{\floor{t}}_\gamma + w^\ast_\gamma - \eps)(\eta^{\floor{s}}_\gamma + w^\ast_\gamma - \eps)\Big]\label{def:dmft_piecelinear_Cg},
\end{align}
where
%Here $\theta^0_\gamma$ is the initializing variable for $\{\theta^t_\gamma\}$, $g_0^\gamma(\cdot)$ is the initializing variable for $\{g_t^\gamma\}$, $\theta^\ast_\gamma$ and $e_\gamma$ are auxiliary variables such that $\theta^\ast_\gamma \sim g_\ast$ for some distribution $g_\ast$ and $e_\gamma \sim \N(0,\sigma^2)$, $\{B^t_\gamma\}$ is a standard Brownian motion, $\{u^t_\gamma\}$ and $\{\omega^t_\gamma,\omega^\ast_\gamma\}$ are two Gaussian processes
%\[\{u^t_\gamma\}_{t\geq 0} \sim \mathrm{GP}(0,\{C^\gamma_\eta(t,s)\}_{t,s \geq 0}),
%\qquad \begin{pmatrix} \omega_\gamma^\ast \\ \{\omega_\gamma^t\}_{t\geq 0}\end{pmatrix}
%\sim \mathrm{GP}\left(0,\begin{pmatrix} \E[{\theta^*_\gamma}^2] &
%\{C^\gamma_\theta(t,\ast)\}_{t \geq 0} \\ 
%\{C^\gamma_\theta(t,\ast)\}_{t \geq 0} & \{C^\gamma_\theta(t,s)\}_{t,s \geq 0}
%\end{pmatrix}\right)\]
%with covariance kernels as defined in \eqref{def:dmft_piecelinear_Cg}, and the quantities $(\theta^0_\gamma,\theta_\gamma^*),\{u_\gamma^t\}_{t \geq 0},\{B_\gamma^t\}_{t \geq 0}$ in \eqref{def:dmft_piecelinear_theta} and similarly $e$ and $(\omega_\gamma^*,\{\omega^t_\gamma\}_{t \geq 0})$ in \eqref{def:dmft_piecelinear_eta} are mutually independent. Moreover, 
$\{\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}\}_{t\geq s}, \{\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma}\}_{t\geq s}$ are stochastic proceses defined by
\begin{align}
\frac{\d }{\d t}\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma} &= \Big[-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log g(\theta_\gamma^{\floor{t}};\alpha^{\floor{t}}_\gamma)\Big]\frac{\partial \theta^{\floor{t}}_\gamma}{\partial u^s_\gamma} + \int_{s}^{\floor{t}} R_\eta^\gamma(\floor{t},\floor{s'})\frac{\partial \theta^{\floor{s'}}_\gamma}{\partial u^s_\gamma}\d s',\label{def:derivative_process_piecelinear_1}\\
\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma} &= 
\begin{cases}
\frac{1}{\sigma^2}\Big[-\int_{\ceil{s}}^{\floor{t}} R^\gamma_\theta(\floor{t},\ceil{s'})\frac{\partial \eta^{\floor{s'}}_\gamma}{\partial w^s_\gamma}\d s' + R^\gamma_\theta(\floor{t},\ceil{s})\Big] & \ceil{s}\leq \floor{t}\\
\frac{1}{\sigma^2} & \ceil{s} > \floor{t}
\end{cases},\label{def:derivative_process_piecelinear_3}
%&= -\gamma\ell''(\eta^t, \omega^\ast;z)\Big[\sum_{k=s+1}^{t-1} R_\theta(t,k)\frac{\partial \ell'(\eta^k, \omega^\ast;z)}{\partial \omega^s} + R_\theta(t,s) \ell''(\eta^s,\omega^\ast;z)\Big],\\
%\frac{\partial \eta^t_\gamma}{\partial w^\ast_\gamma} &= -\frac{1}{\sigma^2}\int_{0}^{\floor{t}} R_\theta^\gamma(\floor{t},\ceil{s'})\Big(\frac{\partial \eta^{\floor{s'}}_\gamma}{\partial w^\ast_\gamma}-1\Big)\d s'\label{def:derivative_process_piecelinear_3},
\end{align}
with boundary conditions $\frac{\partial \theta^t_\gamma}{\partial u^t_\gamma} = 1$. Note that
%: (1) in the definition (\ref{def:derivative_process_piecelinear_1}), we set as default $\overline{\frac{\partial \theta^t_\gamma}{\partial u^s_\gamma}} = 0$ if $t < s$, which implies that $\overline{\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}} = 0$ for any $s\neq i\gamma$ via a simple induction argument; (2) 
the definition of $\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma}$ in the case $ \ceil{s} > \floor{t}$ is never used in (\ref{def:dmft_piecelinear_theta}), we set it as $1/\sigma^2$ so that it is close to $\frac{\partial \eta^t}{\partial w^s}$ for such $t,s$, which is used in Lemma \ref{lem:gamma_mod_map2}.

%\ys{we note that (1) the definition of $\overline{\frac{\partial \eta^t_\gamma}{\partial \omega^s_\gamma}}$ in the case $ \ceil{s} > \floor{t}$ is not relevant in the sense that it is not used anywhere else%, but we set it as $-1/\sigma^2$ such that $\overline{\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}} = \overline{\frac{\partial\theta^{\floor{t}}_\gamma}{\partial u^{\floor{s}}_\gamma}}$ (to see this, note that the first case yields the value is $-1/\sigma^2$ when $t = (i+1)\gamma$ and $s = i\gamma$, and $t = (i+0.5)\gamma, s = i\gamma$ belongs to the second case).
 %(2) For any $s \neq i\gamma$, $\overline{\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}} = 0$.}

The following lemma shows that $\{\theta^t_\gamma, \eta^t_\gamma,\alpha^t_\gamma\}$ are equal in distribution to $\{\bar{\theta}^t_\gamma, \bar{\eta}^t_\gamma, \bar{\alpha}^t_\gamma\}$ defined in (\ref{eq:discrete_dmft}). %Consequently, to simplify notation in the following, we will use the notation 
%\begin{align}\label{eq:discrete_dmft_notation}
%\theta^t_\gamma, \eta^t_\gamma, u^t_\gamma, w^t_\gamma, w^\ast_\gamma, \{B^{t}_\gamma\}, R_\theta^\gamma(t,s), R_\eta^\gamma(t,s), R_\eta^\gamma(t,\ast), C_\theta^\gamma(t,s), C_\theta^\gamma(t,\ast), C_\eta^{\gamma}(t,s), \Big\{\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}\Big\}_{t\geq s}, \Big\{\frac{\partial \eta^t_\gamma}{\partial \omega^s_\gamma}\Big\}_{t\geq s}, \Big\{\frac{\partial \eta^t_\gamma}{\partial \omega^\ast_\gamma}\Big\}_{t\geq 0}
%\end{align}
%to denote the corresponding quantities in (\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}).

%(\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}) are essentially equivalent to (\ref{eq:dmft_theta})-(\ref{eq:dmft_response}) and (\ref{eq:response_1})-(\ref{eq:response_3}).

\begin{lemma}\label{lem:discrete_dmft_rewrite}
(\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}) admits a unique solution such that, for any $m\in \Z_+$ and $\tau_1,\ldots, \tau_m \in \R_+$, 
%and (\ref{eq:dmft_theta})-(\ref{eq:dmft_response}) and (\ref{eq:response_1})-(\ref{eq:response_3}) are initialized from some variable $\theta^0$, function $g_0(\cdot)$, and auxiliary variables $(\theta^\ast, e)$ such that $(\theta^0_\gamma,\theta^\ast_\gamma) \equald (\theta^0, \theta^\ast)$ and $g_0^\gamma = g_0$. Then for any fixed $t\geq 0$, the solutions of the two systems satisfy
\begin{equation}\label{eq:discrete_dmft_rewrite}
\begin{aligned}
(\bar{\theta}^{\tau_1}_\gamma,\ldots, \bar{\theta}^{\tau_m}_\gamma, \theta^\ast) &\equald (\theta^{\tau_1}_\gamma,\ldots, \theta^{\tau_m}_\gamma, \theta^\ast),\\
(\bar{\eta}^{\tau_1}_\gamma,\ldots, \bar{\eta}^{\tau_m}_\gamma, \bar{w}^\ast_\gamma, \eps) &\equald (\eta^{\tau_1}_\gamma,\ldots, \eta^{\tau_m}_\gamma, w^\ast_\gamma, \eps),\\
(\bar{\alpha}^{\tau_1}_\gamma,\ldots, \bar{\alpha}^{\tau_m}_\gamma) &= (\alpha^{\tau_1}_\gamma,\ldots, \alpha^{\tau_m}_\gamma).
\end{aligned}
\end{equation}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:discrete_dmft_rewrite}]%-Part (1): Existence and uniqueness of solution] 
%Since the proof is largely the same as that of Proposition \ref{prop:dmftsolexists}, we will only sketch an outline and introduce some notation for future reference. 

%For notational simplicity, we will adopt (\ref{eq:discrete_dmft_notation}) for (\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}).

First we claim that the solution of (\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}) is determined by the values at the knots $t_i = i\gamma, i\in \Z_+$. To see this, it suffices to note that if (\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}) do have a solution, then with knots $t_i = i\gamma$, the maps
\begin{align*}
t \mapsto u_\gamma^t, w_\gamma^t, \eta^t_\gamma, C^\gamma_\theta(t,\ast), \quad (t,s) \mapsto \frac{\partial\eta^t_\gamma}{\partial w^s_\gamma}, R_\eta^\gamma(t,s), C_\theta^\gamma(t,s), C_\eta^\gamma(t,s)
\end{align*}
are piecewise constant, i.e., $u^t_\gamma = u^{\floor{t}}_\gamma$ (and similarly for $w_\gamma^t, \eta^t_\gamma, C^\gamma_\theta(t,\ast)$) and $\frac{\partial\eta^t_\gamma}{\partial w^s_\gamma} = \frac{\partial\eta^{\floor{t}}_\gamma}{\partial w^{\floor{s}}_\gamma}$ (and similarly for $R_\eta^\gamma(t,s), C_\theta^\gamma(t,s), C_\eta^\gamma(t,s)$), and the maps 
\begin{align*}
t \mapsto \theta^t_\gamma, \quad t \mapsto \frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}, R_\theta^\gamma(t,s),\quad \forall s \geq 0
\end{align*}
are piecewise linear. Consequently, the knot values determine the solution except for $\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}$ and $R_\theta^\gamma(t,s)$. To specify their values from the knots, note that for any fixed $s\in\R_+$, the values of $\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}, R_\theta^\gamma(t,s)$ can be readily specified when $t = i\gamma$, $i\in \Z_+$, using the linearity of $t \mapsto \frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}, R_\theta^\gamma(t,s)$ for fixed $s$. From these values, since
\begin{align*}
\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma} = 1 + \int_s^t \Big[-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log g(\theta^{\floor{s'}};\alpha^{\floor{s'}})\Big]\frac{\partial \theta^{\floor{s'}}_\gamma}{\partial u^s_\gamma}\d s' - \int_s^t \d s'\int_s^{\floor{s'}} R_\eta^\gamma(\floor{s'},\floor{s''})\frac{\partial \theta^{\floor{s''}}_\gamma}{\partial u^s_\gamma}\d s'',
\end{align*}
the value of $\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}$ and $R_\theta^\gamma(t,s)$ can be specified for any $t\geq s\geq 0$.

%Recall the space $\cS_\theta$ and $\cS_\eta$ introduced in Section \ref{subsec:space_S_eta_theta}. Following the same arguments of Lemmas \ref{lem:sub_theta_solution} and \ref{lem:sub_eta_solution}, we may show the following. 
%\begin{itemize}
%\item Given any $X_\eta^\gamma = (\{R_\eta^\gamma(t,s)\}, \{R_\eta^\gamma(t,\ast)\}, \{C_\eta^\gamma(t,s)\})$, there exists a pathwise unique solution $\{\theta^t_\gamma\}, \Big\{\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}\Big\}_{s\leq t}$ of the system
%\begin{align*}
%\theta^t_\gamma &= \theta^0_\gamma + \int_0^t\Big[-\frac{\delta}{\sigma^2}(\theta^{\floor{s}}_{\gamma} - \theta^\ast) -f'(\theta^{\floor{s}}_\gamma) - \int_0^{\floor{s}} R^\gamma_\eta(\floor{s}, \floor{s'})\theta_\gamma^{\floor{s'}}\d s' - R^\gamma_\eta(\floor{s}, \ast)\theta^\ast + u^s_\gamma\Big]\d s\\
%&\quad + \sqrt{2}B^{\floor{t}}_\gamma, \\
%\frac{\d }{\d t}\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma} &= \Big[-\frac{\delta}{\sigma^2} -f''(\theta^{\floor{t}})\Big]\frac{\partial \theta^{\floor{t}}_\gamma}{\partial u^s_\gamma} -\int_s^{\floor{t}} R_\eta^\gamma(\floor{t},\floor{s'})\frac{\partial \theta^{\floor{s'}}_\gamma}{\partial u^s_\gamma}\d s'.
%\end{align*}
%Moreover, it is easy to see that with knots
%
%the maps $t\mapsto \theta^t_\gamma$ and $t\mapsto \frac{\d }{\d t}\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma}$ for each fixed $s$ are piecewise linear with knots $t_i = i\eta$, $i\in \Z$. 
%\item Given any $X_\theta^\gamma = (\{R_\theta^\gamma(t,s)\}, \{C_\theta^\gamma(t,s)\}, \{C_\theta(t,\ast)\})$
%\end{itemize}
%\end{proof}


%\begin{proof}[Proof of Lemma \ref{lem:discrete_dmft_rewrite}-Part (2): Claim (\ref{eq:discrete_dmft_rewrite})]
To specify the knot values, we will prove by induction the following set of claims: For any fixed $k \geq 0$, 
\begin{align}
\gamma \cdot \Big\{\frac{\partial \eta^{\beta\gamma}_\gamma}{\partial w^{\ell \gamma}_\gamma}\Big\}_{\beta \leq k-1, 0\leq\ell\leq \beta-1} &\equald \Big\{\overline{\frac{\partial \eta^{\beta\gamma}_\gamma}{\partial w^{\ell\gamma}_\gamma}}\Big\}_{\beta \leq k-1, 0\leq\ell\leq \beta-1}, \label{eq:induction_piecelinear_eta1}\\
%\Big\{\frac{\partial \eta^{\beta\gamma}_\gamma}{\partial w^\ast_\gamma}\Big\}_{\beta \leq k-1} &\equald \Big\{\overline{\frac{\partial \eta^{\beta\gamma}_\gamma}{\partial w_\gamma^\ast}}\Big\}_{\beta \leq k-1},\label{eq:induction_piecelinear_eta2}\\
\Big(\gamma\cdot\Big\{\frac{\partial \theta^{\beta\gamma}_\gamma}{\partial u^{j\gamma}_\gamma}\Big\}_{\beta\leq k, 1\leq j\leq \beta}, \{\theta^{\beta\gamma}_\gamma\}_{\beta\leq k}\Big) &\equald \Big(\Big\{\overline{\frac{\partial \theta_\gamma^{\beta\gamma}}{\partial u^{(j-1)\gamma}_\gamma}}\Big\}_{\beta\leq k, 1\leq j\leq \beta}, \{\bar{\theta}^{\beta\gamma}_\gamma\}_{\beta\leq k}\Big), \label{eq:induction_piecelinear_theta}\\
 \Big(w^\ast_\gamma, \{w^{\beta \gamma}_\gamma\}_{\beta\leq k}, \{\eta^{\beta\gamma}_\gamma\}_{\beta\leq k}\Big) &\equald  \Big(\bar{w}_\gamma^\ast, \{\bar{w}^{\beta\gamma}_\gamma\}_{\beta\leq k}, \{\bar{\eta}^{\beta\gamma}_\gamma\}_{\beta\leq k}\Big),\label{eq:induction_piecelinear_eta}\\
  \{u^{\beta \gamma}_\gamma\}_{\beta\leq k} &\equald  \{\bar{u}^{\beta\gamma}_\gamma\}_{\beta\leq k},\label{eq:induction_piecelinear_u},\\
\alpha_\gamma^{\beta\gamma} &= \bar{\alpha}_\gamma^{\beta\gamma}, \quad \beta \leq k \label{eq:induction_piecelinear_alpha}.
%u^{\alpha\gamma}_\gamma &= u^\alpha, \quad \alpha\leq k-1,\label{eq:induction_piecelinear_u}\\
%\omega^{\beta\gamma}_\gamma &= \omega^\beta,\quad \beta \leq k\label{eq:induction_piecelinear_omega}.
\end{align}
where the right side quantities are defined in (\ref{eq:dmft_theta_discrete1})-(\ref{eq:dmft_response}) and (\ref{eq:response_1})-(\ref{eq:response_3}).

For the baseline case $k = 0$, (\ref{eq:induction_piecelinear_eta1}) is void. (\ref{eq:induction_piecelinear_theta}) and (\ref{eq:induction_piecelinear_alpha}) hold since $\bar{\theta}_\gamma^0 = \theta^0_\gamma = \theta^0$ and $\alpha^0_\gamma = \bar{\alpha}^0_\gamma = \alpha^0$ (and the claim $\gamma \cdot \{\frac{\partial \theta^{\beta\gamma}_\gamma}{\partial u_\gamma^{j\gamma}}\}_{\beta\leq k, 1\leq j\leq \beta} \stackrel{d}{=} \{\overline{\frac{\partial \theta^\beta_\gamma}{\partial u^{(j-1)\gamma}_\gamma}}\}_{\beta\leq k, 1\leq j\leq \beta}$ is void). Next (\ref{eq:induction_piecelinear_eta}) holds since $(w^\ast_\gamma,w^0_\gamma)$ and $(\bar{w}^\ast_\gamma, \bar{w}_\gamma^0)$ have the same covariance structure, and $\eta^0_\gamma = w^0_\gamma$, $\bar{\eta}_\gamma^0 = \bar{w}_\gamma^0$, which further implies (\ref{eq:induction_piecelinear_u}). Suppose the above claims have been established up to some $k \geq 0$. To show (\ref{eq:induction_piecelinear_eta1}) for $\beta = k$ and $0 \leq \ell \leq k-1$, note that for any fixed $s$, the map $t \mapsto \frac{\partial \eta^t_\gamma}{\partial \omega^s_\gamma}$ is right-continuous, so using the induction hypothesis, 
\begin{align*}
\frac{\partial \eta^{k\gamma}_\gamma}{\partial w^{\ell \gamma}_\gamma} &= \frac{1}{\sigma^2}\Big[-\int_{(\ell+1)\gamma}^{k\gamma} R_\theta^\gamma(k\gamma, \ceil{s'})\frac{\partial \eta_\gamma^{\floor{s'}}}{\partial w^{\ell \gamma}_\gamma}\d s' + R_\theta^\gamma(k\gamma, (\ell+1)\gamma)\Big]\\
&= \frac{1}{\sigma^2}\Big[-\sum_{\alpha=\ell+1}^{k-1} R_\theta^\gamma(k\gamma, (\alpha+1)\gamma)\frac{\partial \eta_\gamma^{\alpha\gamma}}{\partial w^{\ell \gamma}_\gamma}\gamma + R_\theta^\gamma(k\gamma, (\ell+1)\gamma)\Big]\\
&\equald \frac{1}{\sigma^2\gamma}\Big[-\sum_{\alpha=\ell+1}^{k-1} \bar{R}_\theta^\gamma(k, \alpha)\overline{\frac{\partial \eta_\gamma^{t_\alpha}}{\partial w^{t_\ell}_\gamma}} + \bar{R}_\theta^\gamma(k, \ell)\Big] = \frac{1}{\gamma}\overline{\frac{\partial \eta^{t_k}_\gamma}{\partial w^{t_\ell}_\gamma}}.
\end{align*}
%To show (\ref{eq:induction_piecelinear_eta2}) for $\beta = k$, we have
%\begin{align*}
%\frac{\partial \eta^{k\gamma}_\gamma}{\partial w^\ast_\gamma} &= -\frac{1}{\sigma^2}\int_0^{k\gamma} R^\gamma_\theta(k\gamma, \ceil{s'})\Big(\frac{\partial \eta_\gamma^{\floor{s'}}}{\partial w^\ast_\gamma} - 1\Big)\d s'\\
%&= -\frac{1}{\sigma^2}\sum_{\ell=0}^{k-1} R_\theta^\gamma(k\gamma, (\ell+1)\gamma)\Big(\frac{\partial \eta^{\ell\gamma}_\gamma}{\partial w^\ast_\gamma} - 1\Big)\cdot \gamma\\
%&\equald -\frac{1}{\sigma^2}\sum_{\ell=0}^{k-1} \bar{R}^\gamma_\theta(k, \ell)\Big(\overline{\frac{\partial \eta^{t_\ell}_\gamma}{\partial w^\ast_\gamma}} - 1\Big) = \overline{\frac{\partial \eta^{t_k}_\gamma}{\partial w^\ast_\gamma}}.
%\end{align*}
To prove (\ref{eq:induction_piecelinear_theta}) for $\beta = k+1$, we note that the case $j = k+1$ holds trivially since $\frac{\partial \theta^{(k+1)\gamma}_\gamma}{\partial u^{(k+1)\gamma}_\gamma} = 1$ and $\overline{\frac{\partial \theta^{t_{k+1}}_\gamma}{\partial u^{t_k}_\gamma}} = \gamma$ by the boundary condition, and for any $j\leq k$, 
\begin{align*}
\frac{\partial \theta^{(k+1)\gamma}_\gamma}{\partial u^{j\gamma}_\gamma} &= \frac{\partial \theta^{k\gamma}_\gamma}{\partial u^{j\gamma}_\gamma} + \gamma\Big(-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log g(\theta^{k\gamma}_\gamma; \alpha^{k\gamma}_\gamma)\Big)\frac{\partial \theta^{k\gamma}_\gamma}{\partial u^{j\gamma}_\gamma} + \gamma\int_{j\gamma}^{k\gamma} R_\eta^\gamma(k\gamma, \floor{s'})\frac{\partial \theta^{\floor{s'}}_\gamma}{\partial u^{j\gamma}_\gamma}\d s'\\
&= \Big(1-\frac{\gamma\delta}{\sigma^2} + \gamma \partial_\theta^2 \log g(\theta^{k\gamma}_\gamma;\alpha^{k\gamma}_\gamma)\Big)\frac{\partial \theta^{k\gamma}_\gamma}{\partial u^{j\gamma}_\gamma}  + \gamma^2\sum_{\ell=j}^{k-1} R_\eta^\gamma(k\gamma, \ell\gamma)\frac{\partial \theta^{\ell\gamma}_\gamma}{\partial u^{j\gamma}_\gamma}\\
&\equald \Big(1-\frac{\gamma\delta}{\sigma^2} + \gamma \partial_\theta^2 \log g(\bar{\theta}^{t_k}_\gamma; \bar{\alpha}^{t_k}_\gamma)\Big)\frac{1}{\gamma}\overline{\frac{\partial \theta^{t_k}_\gamma}{\partial u^{t_{j-1}}_\gamma}} + \sum_{\ell=j}^{k-1} \bar{R}_\eta^\gamma(k, \ell)\overline{\frac{\partial \theta^{t_\ell}_\gamma}{\partial u^{t_{j-1}}_\gamma}} = \frac{1}{\gamma}\overline{\frac{\partial \theta^{t_{k+1}}_\gamma}{\partial u^{t_{j-1}}_\gamma}},
\end{align*}
and
\begin{align*}
\theta^{(k+1)\gamma}_\gamma &= \theta^{k\gamma}_\gamma + \int_{k\gamma}^{(k+1)\gamma} \Big[-\frac{\delta}{\sigma^2}(\theta^{k\gamma}_{\gamma} - \theta^\ast)  + \partial_\theta^2 \log g(\theta^{k\gamma}_\gamma;\alpha^{k\gamma}_\gamma) + \int_0^{k\gamma} R^\gamma_\eta(k\gamma, \floor{s'})(\theta_\gamma^{\floor{s'}} - \theta^\ast)\d s'  + u^s_\gamma\Big]\d s\\
&\quad + \sqrt{2}(b^{(k+1)\gamma} - b^{k\gamma})\\
&\equald \bar{\theta}_\gamma^{t_k} + \gamma\Big[-\frac{\delta}{\sigma^2}(\bar{\theta}^{t_k}_\gamma - \bar{\theta}_\gamma^\ast) + \partial_\theta^2(\bar{\theta}^{t_k}_\gamma;\bar{\alpha}^{t_k}_\gamma) + \sum_{\ell=0}^{k-1}\bar{R}^\gamma_\eta(k,\ell)(\bar{\theta}^{t_\ell}_\gamma - \theta^\ast) + \bar{u}^{t_k}_\gamma\Big] + \sqrt{2}(b^{(k+1)\gamma} - b^{k\gamma}) = \bar{\theta}^{t_{k+1}}_\gamma.
\end{align*}
To show (\ref{eq:induction_piecelinear_eta}) with $\beta = k+1$, we first note that for any $j\leq k+1$, $\E[\bar{w}^{(k+1)\gamma}_\gamma\bar{w}^{j\gamma}_\gamma] = \E[w^{t_{k+1}}_\gamma w^{t_j}_\gamma]$ and $\E[\bar{w}^{(k+1)\gamma}_\gamma\bar{w}^\ast_\gamma] = \E[w^{t_{k+1}}_\gamma w^\ast_\gamma]$ since $(\theta^\ast,\{\bar{\theta}^{\beta\gamma}_\gamma\}_{\beta\leq k+1}) \equald (\theta^\ast,\{\theta^{t_\beta}_\gamma\}_{\beta\leq k+1})$, which implies $(\bar{w}^\ast_\gamma, \{\bar{w}^{\beta\gamma}_\gamma\}_{\beta\leq k+1}) \equald (w^\ast_\gamma,\{w^{t_\beta}_\gamma\}_{\beta\leq k+1})$. Moreover,
\begin{align*}
\eta^{(k+1)\gamma}_\gamma &= -\frac{1}{\sigma^2}\sum_{\ell=0}^k R_\theta^\gamma((k+1)\gamma, (\ell+1)\gamma)(\eta^{\ell\gamma}_\gamma + w^\ast_\gamma - \eps)\gamma - w^{(k+1)\gamma}_\gamma\\
&\equald -\frac{1}{\sigma^2}\sum_{\ell=0}^k \bar{R}^\gamma_\theta(k+1, \ell)(\bar{\eta}^{t_\ell}_\gamma + \bar{w}^\ast_\gamma - \eps) - \bar{w}^{t_{k+1}}_\gamma = \bar{\eta}^{t_{k+1}}_\gamma.
\end{align*}
For (\ref{eq:induction_piecelinear_u}), we have $\E[\bar{u}^{(k+1)\gamma}_\gamma \bar{u}^{j\gamma}_\gamma] = \E[u^{t_{k+1}}_\gamma u^{t_j}_\gamma]$ for all $j\leq k+1$ by (\ref{eq:induction_piecelinear_eta}) with $\beta = k+1$. For (\ref{eq:induction_piecelinear_alpha}), we have
\begin{align*}
\alpha^{(k+1)\gamma}_\gamma = \alpha^{k\gamma}_\gamma + \gamma \cG(\alpha^{k\gamma}_\gamma, \cP(\theta^{k\gamma}_\gamma)) = \bar{\alpha}^{k\gamma}_\gamma + \gamma \cG(\bar{\alpha}^{k\gamma}_\gamma, \cP(\bar{\theta}^{k\gamma}_\gamma)) = \bar{\alpha}^{(k+1)\gamma}_\gamma,
\end{align*}
completing the proof.
%Lastly, (\ref{eq:induction_piecelinear_g}) holds for $\beta = k+1$ as
%\begin{align*}
%g^\gamma_{(k+1)\gamma}(u) &= g^\gamma_{k\gamma}(u) + \gamma g^\gamma_{k\gamma}\Big[\E \frac{\N_\tau(u-\theta^{(k+1)\gamma}_\gamma)}{\N_\tau \ast g^\gamma_{k\gamma}}(\theta^{(k+1)\gamma}_\gamma)-1\Big]\\
%&= (1-\gamma)g_k(u) + \gamma g_k(u)\E \frac{\N_\tau(u - \theta^{k+1})}{\N_\tau \ast g_k(\theta^{k+1})} = g_{k+1}(u),
%\end{align*}
%as desired.
%Next we prove (\ref{eq:induction_piecelinear_theta}) in the following few steps:
%\begin{enumerate}
%\item With $\mathcal{G}_\gamma$ denoting the $\sigma$-field generated by $\Big(\Big\{\frac{\partial \theta^{\beta\gamma}_\gamma}{\partial u^{\ell \gamma}_\gamma}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \Big\{\frac{\partial \eta^{\beta\gamma}_\gamma}{\partial \omega^{\ell \gamma}_\gamma}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \{\theta^{\beta\gamma}_\gamma\}_{\beta\leq k}\Big)$ and $\mathcal{G}$ the one generated by $\Big(\Big\{\frac{\partial \theta^{\beta}}{\partial u^{\ell-1}}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \Big\{\frac{\partial \eta^{\beta}}{\partial \omega^{\ell}}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \{\theta^{\beta}\}_{\beta\leq k}\Big)$,
%\begin{align*}
%\frac{\partial \theta^{(k+1)\gamma}_\gamma}{\partial u^{j\gamma}_\gamma}|_{\mathcal{G}_\gamma} \equald \frac{\partial \theta^{(k+1)}}{\partial u^{j-1}}|_{\mathcal{G}}.
%\end{align*}
%\item With $\mathcal{G}_\gamma$ denoting the $\sigma$-field generated by $\Big(\Big\{\frac{\partial \theta^{\beta\gamma}_\gamma}{\partial u^{\ell \gamma}_\gamma}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \Big\{\frac{\partial \eta^{\beta\gamma}_\gamma}{\partial \omega^{\ell \gamma}_\gamma}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \{\theta^{\beta\gamma}_\gamma\}_{\beta\leq k}\Big)$ and $\mathcal{G}$ the one generated by $\Big(\Big\{\frac{\partial \theta^{\beta}}{\partial u^{\ell-1}}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \Big\{\frac{\partial \eta^{\beta}}{\partial \omega^{\ell}}\Big\}_{\beta \leq k, 0\leq\ell\leq \beta-1}, \{\theta^{\beta}\}_{\beta\leq k}\Big)$,
%\begin{align*}
%\frac{\partial \theta^{(k+1)\gamma}_\gamma}{\partial u^{j\gamma}_\gamma}|_{\mathcal{G}_\gamma} \equald \frac{\partial \theta^{(k+1)}}{\partial u^{j-1}}|_{\mathcal{G}}
%\end{enumerate}
% In step 1, we show for $\beta = k+1$ and any $j\leq \beta - 1 = k$, $\frac{\partial \theta^{(k+1)\gamma}_\gamma}{\partial u^{j\gamma}_\gamma}| $
\end{proof}

\begin{lemma}\label{lem:dmft_discretization_error}
Assume the conditions of Theorem \ref{thm:dmft_approx}. For any $m \in \Z_+$ and $\tau_1,\ldots, \tau_m \in \R_+$, as $\gamma \rightarrow 0$, 
\begin{align*}
\sP(\theta^{\tau_1}_\gamma, \ldots, \theta^{\tau_m}_\gamma,\theta^\ast) &\overset{W_2}{\to} \sP(\theta^{\tau_1}, \ldots, \theta^{\tau_m},\theta^\ast),\\
\sP(\eta^{\tau_1}_\gamma, \ldots, \eta^{\tau_m}_\gamma, w^\ast, \eps) &\overset{W_2}{\to} \sP(\eta^{\tau_1}, \ldots, \eta^{\tau_m}, w^\ast, \eps),\\
(\alpha^{\tau_1}_\gamma,\ldots, \alpha^{\tau_m}_\gamma) &\rightarrow (\alpha^{\tau_1},\ldots, \alpha^{\tau_m}).
\end{align*}
%Consequently, 
%\begin{align*}
%\lim_{\gamma\rightarrow 0} \dbl\Big(\cL(\theta^{\tau_1}, \ldots, \theta^{\tau_m};\theta^\ast), \cL(\theta^{\tau_1}_\gamma, \ldots, \theta^{\tau_m}_\gamma;\theta^\ast)\Big) = 0,\\
%\lim_{\gamma\rightarrow 0} \dbl\Big(\cL(\eta^{\tau_1}, \ldots, \eta^{\tau_m};\eps), \cL(\theta^{\tau_1}_\gamma, \ldots, \theta^{\tau_m}_\gamma;\eps)\Big) = 0.
%\end{align*}
\end{lemma}
\begin{proof}
We only prove the $\theta$-claim, and the $\eta$-claim follows from analogous arguments. We first introduce some notation. Recall the spaces $\cS_\theta$ and $\cS_\eta$ introduced in Section \ref{subsec:space_S_eta_theta}. Given $X_\eta^\gamma = (\{R^\gamma_\eta(t,s)\}_{0\leq s\leq t\leq T}, \{C^\gamma_\eta(t,s)\}_{s,t\in[0,T]}) \in \cS_\eta$ and auxiliary variable $\theta^\ast$, consider the following system of equations on $\big(\{\theta^t_\gamma\}_{t\in[0,T]}, \{\frac{\partial \theta^t_\gamma}{\partial u^s_\gamma}\}_{0\leq s\leq t\leq T},\{\alpha^t_\gamma\}_{t\in[0,T]}\big)$:
\begin{align}\label{eq:discrete_dmft_sub_1}
\notag\theta^t_\gamma &= \theta^0_\gamma + \int_0^t\Big[-\frac{\delta}{\sigma^2}(\theta^{\floor{s}}_{\gamma} - \theta^\ast) + \partial_\theta \log g(\theta^{\floor{s}}_\gamma; \alpha^{\floor{s}}_\gamma) + \int_0^{\floor{s}} R^\gamma_\eta(\floor{s}, \floor{s'})(\theta_\gamma^{\floor{s'}} - \theta^\ast)\d s' + u^s_\gamma\Big]\d s + \sqrt{2}b^{t}_\gamma,\\
\notag\frac{\d }{\d t}\frac{\partial\theta^t_\gamma}{\partial u^s_\gamma} &= \Big[-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log g(\theta_\gamma^{\floor{t}};\alpha_\gamma^{\floor{t}})\Big]\frac{\partial \theta^{\floor{t}}_\gamma}{\partial u^s_\gamma} + \int_s^{\floor{t}} R_\eta^\gamma(\floor{t},\floor{s'})\frac{\partial \theta^{\floor{s'}}_\gamma}{\partial u^s_\gamma}\d s',\\
\alpha^t_\gamma &= \alpha^0 + \int_0^t \cG(\alpha_\gamma^{\floor{s}}, \sP(\theta^{\floor{s}}_\gamma))\d s,
\end{align}
where $\{u_\gamma^s\}_{s\geq 0}$ is a Gaussian process with covariance $\E[u^\gamma_tu^\gamma_s] = C^\gamma_\eta(t,s)$, and $\{b^{t}_\gamma\}_{t\geq 0}$ is given by (\ref{eq:bm_piece_linear}). Similarly, for any $X_\theta^\gamma = (\{R^\gamma_\theta(t,s)\}, \{C^\gamma_\theta(t,\ast)\}, \{C^\gamma_\theta(t,s)\}) \in \cS_\theta$ and auxiliary variable $\eps$, consider the following system of equations on $\big(\{\eta^t_\gamma\}_{t\geq 0}, \{\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma}\}_{0\leq s\leq t},\big)$:
\begin{align}\label{eq:discrete_dmft_sub_2}
\notag\eta^t_\gamma &= -\frac{1}{\sigma^2}\int_0^{\floor{t}} R^\gamma_\theta(\floor{t},\ceil{s})(\eta^s_\gamma + w^\ast_\gamma - \eps)\d s - w^t_\gamma ,\\
\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma} &= 
\begin{cases}
\frac{1}{\sigma^2}\Big[-\int_{\ceil{s}}^{\floor{t}} R^\gamma_\theta(\floor{t},\ceil{s'})\frac{\partial \eta^{s'}_\gamma}{\partial w^s_\gamma}\d s' + R^\gamma_\theta(\floor{t},\ceil{s})\Big] & \ceil{s}\leq \floor{t}\\
\frac{1}{\sigma^2} & \ceil{s} > \floor{t}
\end{cases},
%&= -\gamma\ell''(\eta^t, \omega^\ast;z)\Big[\sum_{k=s+1}^{t-1} R_\theta(t,k)\frac{\partial \ell'(\eta^k, \omega^\ast;z)}{\partial \omega^s} + R_\theta(t,s) \ell''(\eta^s,\omega^\ast;z)\Big],\\
%\frac{\partial \eta^t_\gamma}{\partial w^\ast_\gamma} &= -\frac{1}{\sigma^2}\int_{0}^{\floor{t}} R_\theta^\gamma(\floor{t},\ceil{s'})\Big(\frac{\partial \eta^{s'}_\gamma}{\partial w^\ast}-1\Big)\d s',
\end{align}
where $(\{w^t_\gamma\}_{t\geq 0}, w^\ast_\gamma)$ is a Gaussian process with covariance $\E[w^t_\gamma w^s_\gamma] = C_\theta^\gamma(t,s)$ and $\E[w^t_\gamma w^\ast_\gamma] = C_\theta^\gamma(t,\ast)$.

Now using similar arguments as in the proof of Lemma \ref{lem:discrete_dmft_rewrite}, both systems (\ref{eq:discrete_dmft_sub_1}) and (\ref{eq:discrete_dmft_sub_2}) admit a unique solution, which is determined by the values at the knots $t_i = i\gamma$, $i\in \Z$. Let $\cT_{\eta\rightarrow\theta}^\gamma: X_\eta^\gamma \rightarrow X_\theta^\gamma = (R_\theta^\gamma, \{C_\theta^\gamma(t,s)\}, \{C_\theta^\gamma(t,\ast)\})$, where, with $\{\theta^t_\gamma\}, \{\frac{\partial \theta^t_\gamma}{\partial u^s_\gamma}\}$ denoting the unique solution to (\ref{eq:discrete_dmft_sub_1}), 
\begin{align*}
R_\theta^\gamma(t,s) = \E\Big[\frac{\partial \theta^t_\gamma}{\partial u^s_\gamma}\Big], \quad C_\theta^\gamma(t,s) = \E[\theta^t_\gamma \theta^s_\gamma], \quad C_\theta^\gamma(t,\ast) = \E[\theta^t_\gamma \theta^\ast]. 
\end{align*}
Denote $\{C_\theta^{\gamma}(t,\ast)\} = C_\theta^{\ast\gamma}$. By arguments similar to the proof of Lemma \ref{lem:Trange_eta_2_theta}, $X_\theta^\gamma = (C_\theta^\gamma, C_\theta^{\ast\gamma}, R_\theta^\gamma) \in \cS_\theta$. Similarly, let $\cT_{\theta\rightarrow\eta}^\gamma: X_\theta^\gamma \rightarrow X_\eta^\gamma = (\{R_\eta^\gamma(t,s)\}, \{C_\eta^\gamma(t,s)\})$, where, with $\{\eta^t_\gamma\}, \{\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma}\}$ denoting the unique solution to (\ref{eq:discrete_dmft_sub_2}), 
\begin{align*}
R_\eta^\gamma(t,s) = \frac{\delta}{\sigma^2}\E\Big[\frac{\partial \eta^t_\gamma}{\partial w^s_\gamma}\Big], \quad C_\eta^\gamma(t,s) = \frac{\delta}{\sigma^4}\E[(\eta^t_\gamma + w^\ast_\gamma - \eps)(\eta^s_\gamma + w^\ast_\gamma - \eps)].
\end{align*}
%Denote $\{R_\eta^\gamma(t,\ast)\}$ by $R_\eta^{\ast\gamma}$. 
By arguments similar to the proof of Lemma \ref{lem:Trange_theta_2_eta}, $X_\eta^\gamma = (C_\eta^\gamma, R_\eta^{\gamma}) \in \cS_\eta$.

Define the composite map
\begin{align*}
\cT_{\eta\rightarrow\eta}^\gamma := \cT^\gamma_{\theta\rightarrow\eta} \circ \cT^\gamma_{\eta\rightarrow\theta}, 
\end{align*}
and recall $\cT_{\eta\rightarrow\eta} = \cT_{\theta\rightarrow\eta} \circ \cT_{\eta\rightarrow\theta}$ from (\ref{eq:composite_map}). Clearly the solution $X_\eta^\gamma = (\{R_\eta^\gamma(t,s)\}, \{C_\eta^\gamma(t,s)\})$ of Lemma \ref{lem:discrete_dmft_rewrite} is a fixed point of $\cT^\gamma_{\eta\rightarrow \eta}$, and $X_\eta = (\{R_\eta(t,s)\}, \{C_\eta(t,s)\})$ is a fixed point of $\cT_{\eta\rightarrow \eta}$, hence with the distances $d$ introduced in (\ref{eq:dist_Seta}) and (\ref{eq:dist_Stheta}), 
\begin{align*}
d(X_\eta, X_\eta^\gamma) = d\big(\cT_{\eta\rightarrow\eta}(X_\eta), \cT_{\eta\rightarrow\eta}^\gamma(X_\eta^\gamma)\big) \leq d\big(\cT_{\eta\rightarrow\eta}(X_\eta), \cT_{\eta\rightarrow\eta}(X_\eta^\gamma)\big) + d\big(\cT_{\eta\rightarrow\eta}(X_\eta^\gamma), \cT_{\eta\rightarrow\eta}^\gamma(X_\eta^\gamma)\big).
\end{align*}
By Lemma \ref{lem:T_contract}, the first term satisfies $d\big(\cT_{\eta\rightarrow\eta}(X_\eta), \cT_{\eta\rightarrow\eta}(X_\eta^\gamma)\big) \leq \frac{1}{2}d(X_\eta, X_\eta^\gamma)$. The second term satisfies
\begin{align*}
d\big(\cT_{\eta\rightarrow\eta}(X_\eta^\gamma), \cT_{\eta\rightarrow\eta}^\gamma(X_\eta^\gamma)\big) &= d\big(\cT_{\theta\rightarrow\eta}(\cT_{\eta\rightarrow\theta}(X_\eta^\gamma)), \cT_{\theta\rightarrow\eta}^\gamma(\cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma))\big)\\
&\leq d\big(\cT_{\theta\rightarrow\eta}(\cT_{\eta\rightarrow\theta}(X_\eta^\gamma)), \cT_{\theta\rightarrow\eta}(\cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma))\big) + d\big(\cT_{\theta\rightarrow\eta}(\cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma)), \cT_{\theta\rightarrow\eta}^\gamma(\cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma))\big)\\
&\leq C\sqrt{\gamma},
\end{align*}
applying Lemmas \ref{lem:gamma_mod_map1} and \ref{lem:gamma_mod_map2} and the modulus bound of $\cT_{\theta\rightarrow\eta}$ in Lemma \ref{lem:modulus_theta_2_eta}. The above two bounds yields
\begin{align}\label{eq:eta_response_discre_error}
d(X_\eta, X_\eta^\gamma) \leq C\sqrt{\gamma},
\end{align}
Consequently, by Lemma \ref{lem:theta_coupling}, there exists a coupling $\{\theta^t\}_{t\in[0,T]}, \{\theta^t_\gamma\}_{t\in[0,T]}$ of the law $\sP(\{\theta^t\}_{t\in[0,T]}), \sP(\{\theta^t_\gamma\}_{t\in[0,T]})$ such that $\sup_{t\in [0,T]} \E(\theta^t - \theta^t_\gamma)^2 \leq C\gamma$, which implies 
\begin{align*}
W_2^2\Big(\sP(\theta^{\tau_1}, \ldots, \theta^{\tau_m},\theta^\ast), \sP(\theta^{\tau_1}_\gamma, \ldots, \theta^{\tau_m}_\gamma,\theta^\ast)\Big) \leq m \cdot \sup_{t\in [0,T]} \E(\theta^t - \theta^t_\gamma)^2 \leq Cm\gamma,
\end{align*} 
proving the claim on $\theta$. The claim on $\eta$ follows from similar arguments, and the claim on $\alpha$ follows by combining (\ref{eq:alpha_discretization_bound}) and (\ref{eq:theta_L2_bound}) below.
\end{proof}


\begin{lemma}\label{lem:gamma_mod_map1}
Let $X_\eta^\gamma = (\{R_\eta^\gamma(t,s)\}_{0\leq s\leq t\leq T},  \{C_\eta^\gamma(t,s)\}_{s,t\in[0,T]})$ be part of the unique solution guaranteed by Lemma \ref{lem:discrete_dmft_rewrite}. There exists some $C > 0$ depending on parameters of the spaces $\cS_\theta$ and $\cS_\eta$ such that $d\big(\cT_{\eta\rightarrow\theta}(X_\eta^\gamma), \cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma)\big) \leq C\sqrt{\gamma}$.
\end{lemma}
\begin{proof}
Let $X_\theta = \cT_{\eta\rightarrow\theta}(X_\eta^\gamma) = (C_\theta, C_\theta^\ast, R_\theta)$ and $X_\theta^\gamma = \cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma) = (C_\theta^\gamma, C_\theta^{\ast\gamma}, R_\theta^\gamma)$.

\noindent \textbf{Part 1: Bound of $d\big((C_\theta, C_\theta^\ast), (C_\theta^\gamma, C_\theta^{\ast\gamma})\big)$}
By definition, we have
\begin{align*}
\theta^t &= \theta^0 + \int_0^t \Big[-\frac{\delta}{\sigma^2}(\theta^s-\theta^*) + \partial_\theta \log g(\theta^s;\alpha^s) + \int_0^s R_\eta^\gamma(s, s')(\theta^{s'} - \theta^\ast)\d s'  + u^s\Big] \d s + \sqrt{2}b^t,\\
\theta^t_\gamma &= \theta^0_\gamma + \int_0^t\Big[-\frac{\delta}{\sigma^2}(\theta^{\floor{s}}_{\gamma} - \theta^\ast) + \partial_\theta \log g(\theta^{\floor{s}}_\gamma; \alpha^{\floor{s}}_\gamma) +\int_0^{\floor{s}} R^\gamma_\eta(s, s')(\theta_\gamma^{\floor{s'}} - \theta^\ast)\d s' + u^s\Big]\d s + \sqrt{2}b^{t}_\gamma,
\end{align*}
where we use the fact that $t\mapsto R^\gamma_\eta(t,\ast)$ and $(t,s) \mapsto R^\gamma_\eta(t,s)$ are piecewise constant, i.e., $R^\gamma_\eta(t,\ast) = R^\gamma_\eta(\floor{t},\ast)$ and $R^\gamma_\eta(t,s) = R^\gamma_\eta(\floor{t},\floor{s})$. Note that we have coupled $\theta^t$ and $\theta^t_\gamma$ with the same Gaussian process $\{u^t\}$ and Brownian motion $b^t$, i.e., $b^{t}_\gamma = \frac{t-i\gamma}{\gamma}b^{(i+1)\gamma} + \frac{(i+1)\gamma - t}{\gamma}b^{i\gamma}$. Since $\theta^0 = \theta^0_\gamma$, we have
\begin{align*}
\theta^t - \theta^t_\gamma &= \int_0^t \Big[-\frac{\delta}{\sigma^2}(\theta^s-\theta^{\floor{s}}_\gamma) + \big(\partial_\theta \log g(\theta^s;\alpha^s) - \partial_\theta \log g(\theta^{\floor{s}}_\gamma;\alpha^{\floor{s}}_\gamma)\big)\\
&\quad + \Big(\int_0^s R_\eta^\gamma(s,s') (\theta^{s'} - \theta^\ast)\d s' - \int_0^{\floor{s}} R_\eta^\gamma(s,s')(\theta^{\floor{s'}}_\gamma - \theta^\ast)\d s'\Big)\Big]\d s  + \sqrt{2}(b^t - b^{t}_\gamma),
\end{align*}
so
\begin{align*}
\E(\theta^t - \theta^t_\gamma)^2 &\leq C \int_0^t \E(\theta^s-\theta^{\floor{s}}_\gamma)^2\d s + C\int_0^t \E\big(\partial_\theta \log g(\theta^s;\alpha^s) - \partial_\theta \log g(\theta^{\floor{s}}_\gamma;\alpha^{\floor{s}}_\gamma)\big)^2 \d s\\
&\quad + C\int_0^t \E\Big(\int_0^s R_\eta^\gamma(s,s') (\theta^{s'} - \theta^\ast)\d s' - \int_0^{\floor{s}} R_\eta^\gamma(s,s') (\theta^{\floor{s'}}_\gamma - \theta^\ast)\d s'\Big)^2\d s  + C\E(B^t - B^t_\gamma)^2 \equiv \sum_{i=1}^4 \zeta_i. 
\end{align*}
To bound $\zeta_1$, we have
\begin{align*}
\int_0^t \E(\theta^s-\theta^{\floor{s}}_\gamma)^2\d s &\leq 2\int_0^t \E(\theta^s-\theta^{s}_\gamma)^2\d s + 2\int_0^t \E(\theta^s_\gamma -\theta^{\floor{s}}_\gamma)^2\d s\\
&\leq \frac{1}{\lambda}e^{2\lambda t}\cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E(\theta^t-\theta^{t}_\gamma)^2 + 2\int_0^t \E(\theta^s_\gamma -\theta^{\floor{s}}_\gamma)^2\d s. 
\end{align*}
Since $t\mapsto \theta^t_\gamma$ is piecewise linear, we have
\begin{align*}
\theta^s_\gamma -\theta^{\floor{s}}_\gamma = (s-\floor{s})\Big[-\frac{\delta}{\sigma^2}(\theta^{\floor{s}}_\gamma-\theta^*) + \partial_\theta \log g(\theta^{\floor{s}}_\gamma;\alpha^{\floor{s}}_\gamma) + \int_0^{\floor{s}} R_\eta^\gamma(s, s')(\theta^{\floor{s'}}_\gamma - \theta^\ast)\d s' + u^s + \frac{b^{\ceil{s}} - b^{\floor{s}}}{\gamma}\Big]. 
\end{align*}
Since $C_\theta^\gamma(t,s) = \E[\theta^t_\gamma \theta^s_\gamma] \in \cS_\theta$ and $X_\eta = (C_\eta^\gamma, R^\gamma_\eta, R_\eta^{\ast\gamma}) \in \cS_\eta$, we have $\int_0^t \E(\theta^s_\gamma -\theta^{\floor{s}}_\gamma)^2\d s \leq C\gamma$, and thus
\begin{align*}
\zeta_1 \leq \frac{1}{\lambda}e^{2\lambda t}\cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E(\theta^t-\theta^{t}_\gamma)^2 + C\gamma.
\end{align*}
To bound $\zeta_2$, using Assumption \ref{assump:prior} and $\sup_{t\in[0,T]} \pnorm{\alpha^t}{} \vee \pnorm{\alpha^t_\gamma}{} \leq C(T,\pnorm{\alpha^0}{})$, we have
\begin{align*}
\E\big(\partial_\theta \log g(\theta^s;\alpha^s) - \partial_\theta \log g(\theta^{\floor{s}}_\gamma;\alpha^{\floor{s}}_\gamma)\big)^2 \leq C\E\pnorm{\theta^s - \theta^{\floor{s}}_\gamma}{}^2 + C\pnorm{\alpha^s - \alpha^{\floor{s}}_\gamma}{}^2.
\end{align*}
The term $\int_0^t \pnorm{\theta^s - \theta^{\floor{s}}_\gamma}{}^2 \d s$ can be bounded similar to $\zeta_1$. For the other term, it suffices to bound $\pnorm{\alpha^s - \alpha^s_\gamma}{}^2$ and $\pnorm{\alpha^s_\gamma - \alpha^{\floor{s}}_\gamma}{}^2$. It is easy to see that $\sup_{t\in[0,T]} \pnorm{\alpha^s_\gamma - \alpha^{\floor{s}}_\gamma}{} \leq C\gamma$, and using Assumption \ref{assump:gradient}, 
\begin{align*}
\pnorm{\alpha^t - \alpha^t_\gamma}{}^2 \leq C\int_0^t \pnorm{\alpha^s - \alpha^s_\gamma}{}^2\d s + C\gamma + C\int_0^t \pnorm{\theta^s - \theta^{\floor{s}}_\gamma}{}^2 \d s.
\end{align*}
Applying Lemma \ref{lem:gronwall} yields 
\begin{align}\label{eq:alpha_discretization_bound}
\pnorm{\alpha^t - \alpha^t_\gamma}{}^2 \leq C\big(\gamma + C\int_0^t \E\pnorm{\theta^s - \theta^{\floor{s}}_\gamma}{}^2 \d s\big),
\end{align}
hence we conclude
\begin{align*}
\zeta_2 \leq \frac{C}{\lambda}e^{2\lambda t}\cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E(\theta^t-\theta^{t}_\gamma)^2 + C\gamma.
\end{align*}
To bound $\zeta_3$, we have
\begin{align*}
&\E\Big(\int_0^s R_\eta^\gamma(s,s') (\theta^{s'} - \theta^\ast)\d s' - \int_0^{\floor{s}} R_\eta^\gamma(s,s')(\theta^{s'}_\gamma - \theta^\ast)\d s'\Big)^2\\
&\leq 2\E\Big(\int_{\floor{s}}^s R_\eta^\gamma(s,s') (\theta^{s'} - \theta^\ast)\d s' \Big)^2 + 2\E\Big(\int_0^{\floor{s}} R_\eta^\gamma(s,s') (\theta^{s'} - \theta^{\floor{s'}}_\gamma)\d s' \Big)^2\\
&\leq \frac{1}{\lambda}e^{2\lambda t}\cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E(\theta^t-\theta^{t}_\gamma)^2 + C\gamma, 
\end{align*}
using the same argument as above that controls $\E (\theta^s - \theta^{\floor{s}}_\gamma)^2$. This implies
\begin{align*}
\zeta_3 \leq \frac{C}{\lambda}e^{2\lambda t}\cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E(\theta^t-\theta^{t}_\gamma)^2 + C\gamma.
\end{align*}
Lastly, $\zeta_4$ satisfies $\E(B^t_\gamma - B^t)^2 \leq C\gamma$, so we conclude that
\begin{align*}
\E(\theta^t - \theta^t_\gamma)^2 \leq \frac{C}{\lambda}e^{2\lambda t}\cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E(\theta^t-\theta^{t}_\gamma)^2 + C\gamma. 
\end{align*}
Choosing a large enough $\lambda$ yields
\begin{align}\label{eq:theta_L2_bound}
\sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E(\theta^t-\theta^{t}_\gamma)^2} \leq C\sqrt{\gamma}.
\end{align}
Let $(\{g^t_1, g^t_2\}_{t\geq 0}, g^\ast)$ be a Gaussian process with covariance $\E[g^t_1 g^s_2] = \E[\theta^t \theta^s_\gamma], \E[g^t_1 g^\ast] = \E[\theta^t\theta^\ast], \E[g^t_2g^\ast] = \E[\theta^t_\gamma\theta^\ast]$, then
\begin{align*}
d\big((C_\theta, C_\theta^\ast), (C_\theta^\gamma, C_\theta^{\ast\gamma})\big) \leq \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E(g^t_1 - g^t_2)^2} = \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E(\theta^t - \theta^t_\gamma)^2} \leq C\sqrt{\gamma}, 
\end{align*}
as desired. 

\noindent \textbf{Part 2: Bound of $d\big(R_\theta, R_\theta^\gamma\big)$} Denote $r_\theta(t,s) = \frac{\partial \theta^t}{\partial u^s}$ and $r_\theta^\gamma(t,s) = \frac{\partial \theta^t_\gamma}{\partial u^s_\gamma}$. By definition, we have
\begin{align*}
r_{\theta}(t,s) &= 1 + \int_s^t \Big(-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log g(\theta^{s'}; \alpha^{s'})\Big)r_\theta(s',s)\d s' + \int_s^t \d s'\int_s^{s'} R_\eta^\gamma(s',s'')r_\theta(s'',s)\d s'',\\
r^\gamma_{\theta}(t,s) &= 1 + \int_s^t \Big(-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log g(\theta^{\floor{s'}}_\gamma;\alpha^{\floor{s'}}_\gamma)\Big)r_\theta^\gamma(s',s)\d s' + \int_s^t \d s'\int_s^{\floor{s'}} R_\eta^\gamma(s',s'')r^\gamma_\theta(s'',s)\d s''.
\end{align*}
Hence
\begin{align*}
|r_{\theta}(t,s) - r^\gamma_{\theta}(t,s)| &\leq \int_s^t \Big|\partial_\theta^2 \log g(\theta^{s'}; \alpha^{s'})r_\theta(s',s) - \partial_\theta^2 \log g(\theta^{\floor{s'}}_\gamma;\alpha^{\floor{s'}}_\gamma)r_\theta^\gamma(s',s)\Big|\d s'\\
&\quad + \int_s^t \d s' \Big|\int_s^{s'} R_\eta^\gamma(s',s'')r_\theta(s'',s)\d s'' - \int_s^{\floor{s'}} R_\eta^\gamma(s',s'')r^\gamma_\theta(s'',s)\d s''\Big|.
\end{align*}
For the first term, using $|\partial_\theta^2 \log g(\theta;\alpha)| \vee \pnorm{\partial_\theta^2\partial_\alpha \log g(\theta;\alpha)}{}  \vee |\partial_\theta^3 \log g(\theta;\alpha)|\leq C(S)$ uniformly over $(\theta,\alpha) \in \R \times S$ for compact set $S$, we have
\begin{align*}
&\int_s^t \Big|\partial_\theta^2 \log g(\theta^{s'}; \alpha^{s'})r_\theta(s',s) - \partial_\theta^2 \log g(\theta^{\floor{s'}}_\gamma;\alpha^{\floor{s'}}_\gamma)r_\theta^\gamma(s',s)\Big|\d s'\\
&\leq \int_s^t \Big|\partial_\theta^2 \log g(\theta^{s'}; \alpha^{s'}) - \partial_\theta^2 \log g(\theta^{\floor{s'}}_\gamma;\alpha^{\floor{s'}}_\gamma)\Big|r_\theta(s',s) \d s' + \int_s^t |\partial_\theta^2 \log g(\theta^{\floor{s'}}_\gamma;\alpha^{\floor{s'}}_\gamma)|\big|r_\theta(s',s) - r_\theta^\gamma(s',s)\big|\d s'\\
&\leq M \int_s^t (|\theta^{s'} - \theta^{\floor{s'}}_\gamma| + |\alpha^{s'} - \alpha^{\floor{s'}}_\gamma|)|r_\theta(s',s)| \d s' + M\int_s^t \big|r_\theta(s',s) - r_\theta^\gamma(s',s)\big|\d s'.
\end{align*}
So using $\E(\theta^{s'} - \theta^{\floor{s'}}_\gamma)^2 \leq C\gamma$ established in (\ref{eq:theta_L2_bound}), a similar bound for $|\alpha^{s'} - \alpha^{\floor{s'}}_\gamma|$,  and $r_\theta(s',s) \leq \Phi_{R_\theta}(s'-s)$ a.e., we have
\begin{align*}
\int_s^t \Big|\partial_\theta^2 \log g(\theta^{s'}; \alpha^{s'})r_\theta(s',s) - \partial_\theta^2 \log g(\theta^{\floor{s'}}_\gamma;\alpha^{\floor{s'}}_\gamma)r_\theta^\gamma(s',s)\Big|\d s' \leq \frac{C}{\lambda}e^{\lambda t}\cdot \sup_{0\leq s\leq t \leq T} e^{-\lambda t}\E\Big|r_\theta(t,s) - r_\theta^\gamma(t,s)\Big| + C\sqrt{\gamma}.
\end{align*}
For the second term, we have for any $s'\in[s,t]$
\begin{align*}
&\Big|\int_s^{s'} R_\eta^\gamma(s',s'')r_\theta(s'',s)\d s'' - \int_s^{\floor{s'}} R_\eta^\gamma(s',s'')r^\gamma_\theta(s'',s)\d s''\Big|\\
&\leq \Big|\int_{\floor{s'}}^{s'} R_\eta^\gamma(s',s'')r_\theta(s'',s)\d s''\Big|
 + \Big|\int_s^{\floor{s'}} R_\eta^\gamma(s',s'') \big|r_\theta(s'',s) - r^\gamma_\theta(s'',s)\big|\d s'',
\end{align*}
hence
\begin{align*}
\E\Big|\int_s^{s'} R_\eta^\gamma(s',s'')r_\theta(s'',s)\d s'' - \int_s^{\floor{s'}} R_\eta^\gamma(s',s'')r^\gamma_\theta(s'',s)\d s''\Big| \leq C\gamma + \frac{C}{\lambda}e^{\lambda t}\cdot \sup_{0\leq s\leq t \leq T}e^{-\lambda t}\E|r_{\theta}(t,s) - r^\gamma_{\theta}(t,s)|.
\end{align*}
Combining the above two estimates yields
\begin{align*}
\E|r_{\theta}(t,s) - r^\gamma_{\theta}(t,s)| \leq C\sqrt{\gamma} + \frac{C}{\lambda}e^{\lambda t}\cdot \sup_{0\leq s\leq t \leq T} e^{-\lambda t}\E|r_{\theta}(t,s) - r^\gamma_{\theta}(t,s)|,
\end{align*}
which further implies that, for a large enough $\lambda$,
\begin{align*}
\sup_{0\leq s\leq t \leq T} e^{-\lambda t}\E|r_{\theta}(t,s) - r^\gamma_{\theta}(t,s)| \leq C\sqrt{\gamma}. 
\end{align*}
Consequently,
\begin{align*}
d(R_\theta, R_\theta^\gamma) \leq \sup_{0\leq s\leq t \leq T} e^{-\lambda t}\Big|\E r_\theta(t,s) - \E r^\gamma_\theta(t,s)\Big| \leq \sup_{0\leq s\leq t \leq T} e^{-\lambda t}\E\Big|r_\theta(t,s) - r^\gamma_\theta(t,s)\Big| \leq C\sqrt{\gamma},
\end{align*}
as desired.
\end{proof}

\begin{lemma}\label{lem:gamma_mod_map2}
Let $X_\theta^\gamma = \cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma) = (C_\theta^\gamma, C_\theta^{\ast\gamma}, R_\theta^\gamma)$, where $(X_\theta^\gamma, X_\eta^\gamma)$ is (part of) the solution to (\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}). There exists some $C > 0$ depending on parameters of the spaces $\cS_\theta$ and $\cS_\eta$ such that $d\big(\cT_{\theta\rightarrow\eta}(X_\theta^\gamma), \cT_{\theta\rightarrow\eta}^\gamma(X_\theta^\gamma)\big) \leq C\gamma$.
\end{lemma}
\begin{proof}
Let $X_\eta = \cT_{\theta\rightarrow\eta}(X_\theta^\gamma) = (C_\eta, R_\eta)$ and $X_\eta^\gamma = \cT_{\theta\rightarrow\eta}^\gamma(X_\theta^\gamma) = (C_\eta^\gamma, R_\eta^\gamma)$.

\noindent\textbf{Part 1: bound on $d(C_\eta, C_\eta^\gamma)$} Let $\{\eta^t\}$ (resp. $\{\eta^t_\gamma\}$) be the accompany solution of $X_\eta$ (resp. $X_\eta^\gamma$), i.e., 
\begin{align*}
\eta^t &= -\frac{1}{\sigma^2}\int_0^t R_\theta^\gamma(t,s)(\eta^s + w^\ast_\gamma - \eps)\d s - w^t_\gamma, \\
\eta^t_\gamma &= -\frac{1}{\sigma^2}\int_0^{\floor{t}} R_\theta^\gamma(\floor{t},\ceil{s})(\eta^s_\gamma + w^\ast_\gamma - \eps)\d s - w^t_\gamma,
\end{align*}
where we couple the two processes with the same Gaussian process $(w^\ast_\gamma, \{w^t_\gamma\}_{t\geq 0})$ with covariance $\E[w^t_\gamma w^s_\gamma] = C_\theta^\gamma(t,s)$, $\E[w^t_\gamma w^\ast_\gamma] = C_\theta^\gamma(t,\ast)$. Then
\begin{align*}
|\eta^t - \eta^t_\gamma| \leq C\int_{\floor{t}}^t R_\theta^\gamma(t,s)\Big|\eta^s + w^\ast_\gamma - \eps\Big|\d s + C\int_0^{\floor{t}} \Big[\big|R_\theta^\gamma(t,s) - R_\theta^\gamma(\floor{t},\ceil{s})\big|\big|\eta^s + w^\ast_\gamma - \eps\big| + |R_\theta^\gamma(\floor{t},\ceil{s})||\eta^s - \eta^s_\gamma|\Big]\d s.
\end{align*}
Since both $\cT_{\theta\rightarrow\eta}$ and $\cT^\gamma_{\theta\rightarrow\eta}$ map into $\cS_\eta$ and $X_\theta^\gamma \in \cS_\theta$, we have 
\begin{align*}
\E\Big[\int_{\floor{t}}^t R_\theta^\gamma(t,s)\Big|\eta^s + w^\ast_\gamma - \eps\Big|\d s\Big]^2 \leq C\gamma^2
\end{align*}
and
\begin{align*}
\E\Big[\int_0^{\floor{t}}|R_\theta^\gamma(\floor{t},\ceil{s})||\eta^s - \eta^s_\gamma|\d s \Big]^2 \leq \frac{C}{\lambda}e^{2\lambda t} \cdot \sup_{s\in[0,T]} e^{-2\lambda s} \E(\eta^s - \eta^s_\gamma)^2.
\end{align*}
Next using Lemma \ref{lem:response_discretization_error}, we have
\begin{align*}
\E\Big[\int_0^{\floor{t}} \Big[\big|R_\theta^\gamma(t,s) - R_\theta^\gamma(\floor{t},\ceil{s})\big|\big|\eta^s + w^\ast_\gamma - \eps\big| \d s\Big]^2 \leq C\gamma.
\end{align*}
Collecting the estimates, we have for large enough $\lambda$ that
\begin{align*}
\sup_{t\in[0,T]} e^{-\lambda t} \sqrt{\E(\eta^t - \eta^t_\gamma)^2} \leq C\sqrt{\gamma}.
\end{align*}
Now choosing $\{g^t_1,g^t_2\}$ to be a Gaussian process with covariance $\E[g^t_1g^s_1] = \E[\eta^t\eta^s]$, $\E[g^t_2g^s_2] = \E[\eta^t_\gamma\eta^s_\gamma]$, and $\E[g^t_1g^s_2] = \E[\eta^t\eta^s_\gamma]$, we have
\begin{align*}
d(C_\eta, C_\eta^\gamma) \leq \sup_{t\in[0,T]}e^{-\lambda t} \sqrt{\E(g^t_1 - g^t_2)^2} = \sup_{t\in[0,T]} e^{-\lambda t} \sqrt{\E(\eta^t - \eta^t_\gamma)^2} \leq C\sqrt{\gamma}.
\end{align*}

\noindent\textbf{Part 2: bound on $d(R_\eta, R_\eta^\gamma)$} Let $r_\eta(t,s) = \frac{\partial \eta^t}{\partial w^s}$ and $r_\eta^\gamma(t,s) = \frac{\partial \eta^t_\gamma}{\partial w^s_\gamma}$ such that $R_\eta(t,s) = \frac{\delta}{\sigma^2}r_\eta(t,s)$ and $R^\gamma_\eta(t,s) = \frac{\delta}{\sigma^2}r^\gamma_\eta(t,s)$ (note that both are deterministic processes), which satisfy
\begin{align*}
r_\eta(t,s) &= \frac{1}{\sigma^2}\Big[-\int_s^t R_\theta^\gamma(t,s')r_\eta(s', s)\d s' + R_\theta^\gamma(t,s)\Big],\\
r_\eta^\gamma(t,s) &= 
\begin{cases}
\frac{1}{\sigma^2}\Big[-\int_{\ceil{s}}^{\floor{t}} R_\theta^\gamma(\floor{t}, \ceil{s'})r_\eta^\gamma(s', s)\d s' + R_\theta^{\gamma}(\floor{t},\ceil{s})\Big] & \ceil{s} \leq \floor{t},\\
\frac{1}{\sigma^2} & \ceil{s} > \floor{t},
\end{cases}
\end{align*}
using that $r_\eta^{\gamma}(t,s) = r_\eta^{\gamma}(\floor{t},\floor{s})$. First we note that for $s\leq t$ such that $\ceil{s} > \floor{t}$, there exists some $i\in \Z$ such that $s,t \in [i\gamma, (i+1)\gamma)$, which implies that $|\int_s^t R_\theta^\gamma(t,s')r_\eta(s', s)\d s'|\leq C\gamma$ and $|R_\theta^\gamma(t,s) - 1| = |R_\theta^\gamma(t,s) - R_\theta^\gamma(s,s)| \leq C\gamma$. Hence for such $s,t$, $|r_\eta(t,s) - r^\gamma_\eta(t,s)| = |r_\eta(t,s) - 1/\sigma^2| \leq C\gamma$, as desired. %\ys{(this is where $r^\gamma_\eta(t,s) = -1/\sigma^2$ is used)}. 
For the other case $\ceil{s} \leq \floor{t}$, we have
\begin{align*}
|r_\eta(t,s) - r^\gamma_\eta(t,s)| &\leq C\Big[\Big(\int_{s}^{\ceil{s}} + \int_{\floor{t}}^t\Big) R_\theta^\gamma(t,s')r_\eta(s', s)\d s' +|R_\theta^\gamma(t,s) - R_\theta^\gamma(\floor{t},\ceil{s})|\\
&\quad + \int_{\ceil{s}}^{\floor{t}} \Big(|R_\theta^\gamma(t,s') - R_\theta^\gamma(\floor{t}, \ceil{s'})||r_\eta(s',s)| + |R_\theta^\gamma(\floor{t}, \ceil{s'})||r_\eta(s', s) - r_\eta^\gamma(\floor{s'}, s)|\Big)\d s' \Big]\\
&\leq \frac{C}{\lambda} e^{\lambda t}\cdot \sup_{s \leq s' \leq t} e^{-\lambda s'}|r_\eta(s', s) - r_\eta^\gamma(s', s)| + C\gamma, 
\end{align*}
where we apply Lemma \ref{lem:response_discretization_error}. Hence for large enough $\lambda$, we have
\begin{align}\label{eq:Reta_discre_error}
d(R_\eta, R_\eta^\gamma) \leq \frac{\delta}{\sigma^2}\sup_{s\leq t\leq T} e^{-\lambda t}|r_\eta(t, s) - r_\eta^\gamma(t, s)| \leq C\gamma.
\end{align}
%\noindent\textbf{Part 3: bound on $d(R_\eta^\ast, R_\eta^{\ast\gamma})$} Let $r_\eta^\ast(t) = r_\eta(t,\ast) = \frac{\partial \eta^t}{\partial w^\ast}$ and $r_\eta^{\ast\gamma}(t) = r_\eta^{\gamma}(t,\ast) = \frac{\partial \eta^t_\gamma}{\partial w^\ast_\gamma}$ such that $R_\eta^\ast = \frac{\delta}{\sigma^2}r_\eta^\ast$ and $R^{\ast\gamma}_\eta = \frac{\delta}{\sigma^2}r^{\ast\gamma}_\eta$ (note that both are deterministic processes), which satisfies
%\begin{align*}
%r_\eta(t,\ast) = -\frac{1}{\sigma^2}\int_0^t R_\theta^\gamma(t,s)(r_\eta(s,\ast) - 1)\d s, \quad r_\eta^\gamma(t,\ast) = -\frac{1}{\sigma^2}\int_0^{\floor{t}} R_\theta^\gamma(\floor{t},\ceil{s})(r^\gamma_\eta(s,\ast) - 1)\d s,
%\end{align*}
%using $r_\eta^\gamma(t,\ast) = r_\eta^\gamma(\floor{t},\ast)$. Using again Lemma \ref{lem:response_discretization_error} and a similar argument as above, we have
%\begin{align*}
%d(R_\eta^\ast, R_\eta^{\ast\gamma}) = \frac{\delta}{\sigma^2}\sup_{t\in [0,T]} e^{-\lambda t}|r_\eta(t,\ast) - r^\gamma_\eta(t,\ast)| \leq C\gamma,
%\end{align*}
%completing the proof.
\end{proof}

\begin{lemma}\label{lem:response_discretization_error}
Let $X_\theta^\gamma = \cT_{\eta\rightarrow\theta}^\gamma(X_\eta^\gamma) = (C_\theta^\gamma, C_\theta^{\ast\gamma}, R_\theta^\gamma)$, where $(X_\theta^\gamma, X_\eta^\gamma)$ is (part of) the solution to (\ref{def:dmft_piecelinear_theta})-(\ref{def:dmft_piecelinear_Cg}) and (\ref{def:derivative_process_piecelinear_1})-(\ref{def:derivative_process_piecelinear_3}). Then for any $0\leq s \leq t \leq T$, there exists some $C > 0$ depending on the parameters of $\cS_\theta$ and $\cS_\eta$ such that $|R_\theta^\gamma(t,s) - R_\theta^\gamma(\floor{t}, \ceil{s})|\leq C\gamma$.
\end{lemma}
\begin{proof}
Denote $r_\theta(t,s) = \frac{\partial \theta^{t}_\gamma}{\partial u^s_\gamma}$ so that $R_\theta^\gamma(t,s) = \E[r_\theta(t,s)]$, which satisfies
\begin{align*}
\frac{\d}{\d t}r_\theta(t,s) = \Big(-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log (\theta^{\floor{t}}_\gamma; \alpha^{\floor{t}}_\gamma)\Big)r_\theta(\floor{t}, s) + \int_s^{\floor{t}} R_\eta^\gamma(\floor{t}, \floor{s'})r_\theta(\floor{s'}, s)\d s'.
\end{align*}
Using linearity of $t \mapsto r_\theta(t,s)$ for fixed $s$ and the fact that $X_\eta^\gamma \in \cS_\eta, X_\theta^\gamma \in \cS_\theta$, it can be readily showed that for any $0\leq s\leq t\leq T$, $|r_\theta(t,s) - r_\theta(\floor{t},s)| \leq C\gamma$ a.s.. Next using $|\partial_\theta^2 \log g(\theta; \alpha)| \leq C(S)$ uniformly over $(\theta, \alpha) \in \R \times S$ for compact set $S$, we have
\begin{align*}
&\frac{\d}{\d t}\big|r_\theta(t,s) - r_\theta(t,\ceil{s})\big|\\
&\leq \big|\frac{\d}{\d t}r_\theta(t,s) - \frac{\d}{\d t}r_\theta(t,\ceil{s})\big|\\
&\leq C\big|r_\theta(\floor{t},s) - r_\theta(\floor{t},\ceil{s})\big| + \int_{\ceil{s}}^{\floor{t}} |R_\eta^\gamma(\floor{t}, \floor{s'})||r_\theta(s', s) - r_\theta(s', \ceil{s})|\d s' + \int_{s}^{\ceil{s}}|R_\eta^\gamma(\floor{t}, \floor{s'})||r_\theta(s', \ceil{s})|\d s'\\
&\leq C\sup_{\ceil{s}\leq s' \leq t} |r_\theta(s', s) - r_\theta(s', \ceil{s})| + C\gamma.
\end{align*}
This further implies
\begin{align*}
\big|r_\theta(t,s) - r_\theta(t,\ceil{s})\big| \leq e^{Ct}\big|r_\theta(\ceil{s},s) - r_\theta(\ceil{s},\ceil{s})\big| + C\gamma.
\end{align*}
To bound $\big|r_\theta(\ceil{s},s) - r_\theta(\ceil{s},\ceil{s})\big|$, note that $r_\theta(\ceil{s},\ceil{s}) = 1$ by definition, and
\begin{align*}
r_\theta(\ceil{s}, s) = r_\theta(s, s) + (\ceil{s} - s) \cdot \Big(-\frac{\delta}{\sigma^2} + \partial_\theta^2 \log g(\theta^{\floor{s}}_\gamma;\alpha^{\floor{s}}_\gamma)\Big)r_\theta(\floor{s}, s),
\end{align*}
which satisfies $|r_\theta(\ceil{s}, s) - 1| \leq C\gamma$, as desired.
\end{proof}

\begin{lemma}\label{lem:theta_coupling}
Let $\sP(\{\theta^t\}_{t\in[0,T]})$ (resp. $\sP(\{\theta^t_\gamma\}_{t\in[0,T]})$) denote the law of the solution to (\ref{def:dmft_langevin_cont_theta}) with $X_\eta = (C_\eta, R_\eta)$ (resp. (\ref{def:dmft_piecelinear_theta}) with $X^\gamma_\eta = (C^\gamma_\eta, R^\gamma_\eta))$. Then there exists a coupling $\{\theta^t\}_{t\in[0,T]}, \{\theta^t_\gamma\}_{t\in[0,T]}$ such that
\begin{align*}
\sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E(\theta^t - \theta^t_\gamma)^2} \leq C\big(d(X_\eta, X_\eta^\gamma) + \sqrt{\gamma}\big),
\end{align*}
where $C > 0$ only depends on the parameters of the spaces $\cS_\theta$ and $\cS_\eta$.
\end{lemma}
\begin{proof}
Take $\{\theta^t\}$ to be the solution to
\begin{align*}
\theta^t =  \theta^0 + \int_0^t\Big[-\frac{\delta}{\sigma^2}(\theta^s - \theta^\ast) + \partial_\theta \log g(\theta^s;\alpha^s) + \int_0^{s} R_\eta(s, s')(\theta^{s'} - \theta^\ast)\d s' + u^s\Big]\d s + \sqrt{2}b^{t}
\end{align*}
and $\{\theta^t_\gamma\}$ to be the solution to
\begin{align*}
\theta^t_\gamma &= \theta^0 + \int_0^t\Big[-\frac{\delta}{\sigma^2}(\theta^{\floor{s}}_{\gamma} - \theta^\ast) + \partial_\theta \log g(\theta^{\floor{s}}_\gamma; \alpha^{\floor{s}}_\gamma) + \int_0^{\floor{s}} R^\gamma_\eta(s, s')(\theta_\gamma^{\floor{s'}} - \theta^\ast)\d s'  + u^s_\gamma\Big]\d s + \sqrt{2}b^{t}_\gamma,
\end{align*}
coupled with the same initialization $\theta^0$, auxiliary variable $\theta^\ast$, Brownian motion $b^t$ such that $b^t_\gamma = \frac{\ceil{t} - t}{\gamma}b^{\floor{t}} + \frac{t-\floor{t}}{\gamma}b^{\ceil{t}}$, and Gaussian processes $\{u^t\}, \{u^t_\gamma\}$ such that $\sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E(u^t - u^t_\gamma)^2} = d(C_\eta, C_\eta^\gamma)$. Then using $|\partial_\theta^2 \log g(\theta; \alpha)| \leq C(S)$ uniformly over $(\theta, \alpha) \in \R \times S$, 
\begin{align*}
\E(\theta^t - \theta^t_\gamma)^2 &\leq C\int_0^t \Big[\E(\theta^{\floor{s}}_{\gamma} - \theta^s_{\gamma})^2 + \E(\theta^s_\gamma - \theta^s)^2 + \E\Big(\int_{\floor{s}}^s R_\eta(s, s')(\theta^{s'} - \theta^\ast)\d s'\Big)^2 + \E(u^s - u^s_\gamma)^2 \\
&\quad + \E \Big(\int_0^{\floor{s}} (R_\eta(s, s')(\theta^{s'} - \theta^\ast) - R^\gamma_\eta(s, s')(\theta_\gamma^{\floor{s'}} - \theta^\ast))\d s'\Big)^2 + C\E(b^t_\gamma - b^t)^2\\
&\leq \frac{C}{\lambda}e^{2\lambda t}\cdot \Big[\sup_{t\in[0,T]} e^{-2\lambda t}\E (\theta^t - \theta^t_\gamma)^2 + \sup_{0\leq s\leq t\leq T} e^{-2\lambda t}\big(R_\eta(t,s) - R_\eta^\gamma(t,s)\big)^2\\
&\quad + \sup_{t\in[0,T]} e^{-2\lambda t}\E(u^t-u^t_\gamma)^2\Big] + C\gamma,
\end{align*}
which implies
\begin{align*}
\sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E(\theta^t - \theta^t_\gamma)^2} \leq C\Big(d(R_\eta,R_\eta^\gamma) + d(C_\eta, C_\eta^\gamma) +\sqrt{\gamma}\Big) \leq C\big(d(X_\eta, X_\eta^\gamma) + \sqrt{\gamma}\big), 
\end{align*}
as desired.
\end{proof}



\subsection{Completing the proof}

\begin{lemma}\label{lem:langevin_tight}
Assume the conditions of Theorem \ref{thm:dmft_approx}. Then almost surely as $n,d\rightarrow\infty$ with respect to the randomness of $(\btheta^0,\X,\y)$, the sequence of laws $\mu^{(n)} = \frac{1}{d}\sum_{j=1}^d \delta_{(\theta^\ast_j, (\theta^t_j)_{t\in[0,T]})}$ is uniformly tight over $\R \times C([0,T],\R)$.
\end{lemma}
\begin{proof}
Fix $\alpha \in (0,1/2)$. For any function $f\in C([0,T])$ that is $\alpha$-H\"older continuous, let $\pnorm{f}{0,\alpha} := \sup_{t,s\in[0,T]} |f(t)-f(t)|/|t-s|^\alpha$ denote the $\alpha$-H\"older norm. Let us verify the conditions of \cite[Theorem 7.3]{billingsley1968convergence}, i.e, for any $\eps > 0$, the existence of $M = M(\eps)$ such that
\begin{equation}\label{eq:tightness_io}
\begin{gathered}
\Prob(\{\mu^{(n)}\big(\{\theta^t\}_{t\in[0,T]}: |\theta^0| \geq M \big) > \eps \} \text{ happens infinitely often}) = 0,\\
\Prob(\{\mu^{(n)}\big(\{\theta^t\}_{t\in[0,T]}: \pnorm{\theta}{0,\alpha} \geq M \big) > \eps \} \text{ happens infinitely often}) = 0,
\end{gathered}
\end{equation}
where $\mu^{(n)}$ denotes the law $\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_j,\ldots, \btheta^{\tau_m}_j, \btheta^\ast_j\big)}, \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m},\theta^\ast)$, and the outer probability $\Prob$ is taken over the randomness of $(\btheta^0, \X,\y)$. To see the first claim, note that $\{\mu^{(n)}\big(\{\theta^t\}_{t\in[0,T]}: |\theta^0| \geq M \big) > \eps \}$ is the event on which $d^{-1}\sum_{j=1}^d\bm{1}\{|\btheta^0_j| \geq M\} > \eps$, so for a fixed $(n,d)$
\begin{align*}
\Prob\big(\{\mu^{(n)}\big(\{\theta^t\}_{t\in[0,T]}: |\theta^0| \geq M \big) > \eps \}\big) = \Prob\Big(\frac{1}{d}\sum_{j=1}^d \bm{1}\{|\theta^0_j| > M\} > \eps\Big). 
\end{align*}
By Assumption \ref{assump:model}, we can choose $M$ large enough such that $\Prob(|\theta^0_j| > M) \leq \eps/10$, hence under iid assumption of $(\theta^0_1,\ldots,\theta^0_d)$, the above probability is bounded by $e^{-cd}$ by the tail of binomial distribution, and the first claim of (\ref{eq:tightness_io}) follows from Borel Cantelli lemma. For the second claim, let $F(\btheta^u, \hat{\alpha}^u) = -\frac{1}{\sigma^2} \X^\top (\X \btheta^u - \y) + \sum_{j=1}^d \partial_\theta \log g(\theta^u_j,\hat{\alpha}^u) \in \R^d$, so that $\d\btheta^t = F(\btheta^t,\hat{\alpha}^t)\d t + \sqrt{2}\d \b^t$, then with $q = 1/(1-\alpha) < 2$, 
\begin{align*}
\big|\e_j^\top (\btheta^t - \btheta^s)\big| &\leq \int_s^t \big|\e_j^\top F(\btheta^u, \hat{\alpha}^u)\big|\d u + \sqrt{2}\big|\e_j^\top(\b^t - \b^s)\big|\\
&\leq |t-s|^{\alpha} \Big(\int_0^T \big|\e_j^\top F(\btheta^u, \hat{\alpha}^u)\big|^q \d u\Big)^{1/q} + \sqrt{2}\pnorm{b_j}{0,\alpha}|t-s|^{\alpha}\\
&\leq C|t-s|^{\alpha} \Big(\int_0^T \big(\e_j^\top F(\btheta^u, \hat{\alpha}^u)\big)^2 \d u\Big)^{1/2} + \sqrt{2}\pnorm{b_j}{0,\alpha}|t-s|^{\alpha}, 
\end{align*}
which implies that $\pnorm{(\btheta)_j}{0,\alpha} \leq C\Big(\int_0^T \big(\e_j^\top F(\btheta^u, \hat{\alpha}^u)\big)^2 \d u\Big)^{1/2} + \pnorm{b_j}{0,\alpha}$. Note that
\begin{align*}
\mu^{(n)}\big(\{\theta^t\}_{t\in[0,T]}: \pnorm{\theta}{0,\alpha} \geq M \big) &= d^{-1}\sum_{j=1}^d \bm{1}\{\pnorm{(\btheta)_j}{0,\alpha} \geq M\}\leq \frac{1}{dM^2}\sum_{j=1}^d \pnorm{(\btheta)_j}{0,\alpha}^2\\
&\leq \frac{C}{dM^2} \Big(\int_0^T \pnorm{F(\btheta^u, \hat{\alpha}^u)}{}^2 \d u + \sum_{j=1}^d \pnorm{b_j}{0,\alpha}^2\Big),
\end{align*}
consequently for fixed $(n,d)$, we have
\begin{align*}
\Prob(\{\mu^{(n)}\big(\{\theta^t\}_{t\in[0,T]}: \pnorm{\theta}{0,\alpha} \geq M \big) > \eps \} ) &= \Prob(d^{-1}\sum_{j=1}^d \bm{1}\{\pnorm{(\btheta)_j}{0,\alpha} \geq M\} > \eps)\\
&\leq \Prob\Big(\frac{C}{dM^2}\int_0^T \pnorm{F(\btheta^u, \hat{\alpha}^u)}{}^2 \d u > \eps/2\Big) + \Prob\Big(\frac{C}{dM^2} \sum_{j=1}^d \pnorm{b_j}{0,\alpha}^2 > \eps/2\Big).
\end{align*}
By Assumptions \ref{assump:model} and \ref{assump:prior} and standard concentration, it is easy to show that $d^{-1}\sup_{t\in[0,T]}\pnorm{\btheta^t}{}^2 \vee d^{-1} \sup_{t\in[0,T]}\pnorm{F(\btheta^t,\hat{\alpha}^t)}{}^2 \leq C$ with probability at least $1 - \exp(-cd)$, so the first probability is bounded by $1-\exp(-cd)$ for large $M$. For the second probability, it is known from \cite[Equation (17)]{benarous1994holder} that $\E \exp(\lambda\pnorm{b_j}{0,\alpha}^2) \leq C(\lambda)$ for small enough $\lambda > 0$, so 
\begin{align*}
\Prob\Big(\frac{C}{dM^2} \sum_{j=1}^d \pnorm{b_j}{0,\alpha}^2 > \eps/2\Big) \leq e^{-\frac{\lambda dM^2\eps}{C}} \E \exp(\lambda \sum_{j=1}^d \pnorm{b_j}{0,\alpha}^2\sum) \leq C^d e^{-\frac{\lambda dM^2\eps}{C}} \leq \exp(-cd), 
\end{align*}
for large enough $M$. Hence the second claim of (\ref{eq:tightness_io}) also follows from Borel Cantelli lemma, completing the proof. 
\end{proof}

We are now ready to prove Theorem \ref{thm:dmft_approx}.
\begin{proof}[Proof of Theorem \ref{thm:dmft_approx}]
By triangle inequality, we have
\begin{align*}
&W_2\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_j,\ldots, \btheta^{\tau_m}_j, \btheta^\ast_j\big)}, \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m},\theta^\ast)\Big) \leq W_2\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_j,\ldots, \btheta^{\tau_m}_j, \btheta^\ast_j\big)}, \frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_{\gamma,j},\ldots, \btheta^{\tau_m}_{\gamma,j}, \btheta^\ast_j\big)}\Big)\\
&\quad + W_2\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_{\gamma,j},\ldots, \btheta^{\tau_m}_{\gamma,j}, \btheta^\ast_j\big)}, \sP(\theta^{\tau_1}_\gamma, \ldots,\theta^{\tau_m}_\gamma,\theta^\ast)\Big) + W_2\Big(\sP(\theta^{\tau_1}_\gamma, \ldots,\theta^{\tau_m}_\gamma,\theta^\ast),\sP(\theta^{\tau_1}, \ldots,\theta^{\tau_m},\theta^\ast)\Big).
\end{align*}
Applying Lemmas \ref{lem:langevin_discretize_error}, \ref{lem:finite_dim_converge}, \ref{lem:dmft_discretization_error}, we may take first $\limsup_{n,d\rightarrow\infty}$ followed by $\gamma \rightarrow 0$ to obtain that, almost surely as $n,d\rightarrow\infty$
\begin{align*}
\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_j,\ldots, \btheta^{\tau_m}_j, \btheta^\ast_j\big)} \overset{W_2}{\to} \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m},\theta^\ast),
\end{align*}
for any finite $m$ and $\tau_1,\ldots,\tau_m\in [0,T]$. By taking the intersection over a countable number of probability-1 events, we conclude that
\begin{align*}
\Prob\Big(W_2\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big(\btheta^{\tau_1}_j,\ldots, \btheta^{\tau_m}_j, \btheta^\ast_j\big)}, \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m},\theta^\ast)\Big) \rightarrow 0, \forall m \in \Z_+, \forall \tau_1,\ldots, \tau_m \in [0,T] \cap \mathbb{Q}\Big) = 1, 
\end{align*}
where $\mathbb{Q}$ denotes the set of rational numbers. Let $\mu^{(n)}$ denote the (random) law $\frac{1}{d}\sum_{j=1}^d \delta_{((\theta^t_j)_{t\in[0,T]},\theta^\ast_j)}$. By Lemma \ref{lem:langevin_tight}, almost surely $\{\mu^{(n)}\}$ is uniformly tight over $ C([0,T],\R) \times \R$, so at the intersection of these two events, we have by \cite[Theorem 7.1]{billingsley1968convergence} that $\mu^{(n)}$ converges weakly and hence also in $W_2$ (due to finiteness of second moment) to $\sP((\theta^t)_{t\in[0,T]},\theta^\ast)$, which is uniquely determined by the finite-dimensional marginals over $\mathbb{Q}$. The claims on the $\eta$ and $\alpha$ side follow from similar arguments, so the proof is complete.

%We first prove finite-dimensional convergence. For any $m\in \Z_+$ and $\tau_1,\ldots, \tau_m \in \R_+$, and $\gamma > 0$, 
%\begin{align*}
%&\dbl\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1})_j, \ldots, (\btheta^{\tau_m})_j), (\btheta^\ast)_j\big)}, \cL(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big)\\
%&\leq \dbl\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1})_j, \ldots, (\btheta^{\tau_m})_j), (\btheta^\ast)_j\big)}, \frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1}_\gamma)_j, \ldots, (\btheta^{\tau_m}_\gamma)_j), (\btheta^\ast)_j\big)}\Big)\\
%&\quad + \dbl\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1}_\gamma)_j, \ldots, (\btheta^{\tau_m}_\gamma)_j), (\btheta^\ast)_j\big)}, \cL(\theta^{\tau_1}_\gamma,\ldots, \theta^{\tau_m}_\gamma, \theta^\ast)\Big)\\
%&\quad + \dbl\Big(\cL(\theta^{\tau_1}_\gamma,\ldots, \theta^{\tau_m}_\gamma, \theta^\ast), \cL(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big).
%\end{align*}
%First taking the limit $n,d\rightarrow\infty$, then by Lemma \ref{lem:finite_dim_converge}, we have
%\begin{align*}
%&\lim_{n,d\rightarrow\infty} \dbl\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1})_j, \ldots, (\btheta^{\tau_m})_j), (\btheta^\ast)_j\big)}, \cL(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big)\\
%&\leq \limsup_{n,d\rightarrow\infty}  \dbl\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1})_j, \ldots, (\btheta^{\tau_m})_j), (\btheta^\ast)_j\big)}, \frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1}_\gamma)_j, \ldots, (\btheta^{\tau_m}_\gamma)_j), (\btheta^\ast)_j\big)}\Big)\\
%&\quad + \dbl\Big(\cL(\theta^{\tau_1}_\gamma,\ldots, \theta^{\tau_m}_\gamma, \theta^\ast), \cL(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big) + o_P(1). 
%\end{align*}
%Now taking $\gamma \rightarrow 0$, by Lemmas \ref{lem:langevin_discretize_error} and \ref{lem:dmft_discretization_error}, we conclude that
%\begin{align*}
%\lim_{n,d\rightarrow\infty} \dbl\Big(\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1})_j, \ldots, (\btheta^{\tau_m})_j), (\btheta^\ast)_j\big)}, \cL(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big)  = o_P(1).
%\end{align*}
%It remains to show that $\dbl(\mu^{(n)}, \mu) \rightarrow_P 0$, where $\mu^{(n)} = d^{-1}\sum_{j=1}^d \delta_{\{(\btheta^t)_{j}\}_{t\in [0,T]}}$ and $\mu = \cL(\{\theta^t\}_{t\in[0,T]})$. Recall that a sequence of random variable $\{X_n\}$ satisfies $X_n \rightarrow_P 0$ if and only if for any subsequence $\{n_\ell\}_{\ell\in\Z}$, there exists a further subsequence $\{n_\ell'\}_{\ell\in \Z}$ such that $X_{n_\ell'} \rightarrow_{a.s.} 0$. Using this fact, the above conclusion shows that for any $m\in\Z_+$ and $\tau_1,\ldots, \tau_m \in [0,T] \cap \Q$, and subsequence $\{n_\ell\}$, there exists a futher subsequence $\{n_\ell'\}$ such that
%\begin{align*}
%\P\Big(\dbl(\mu^{(n_\ell')}_{\tau_1,\ldots,\tau_m}, \mu_{\tau_1,\ldots,\tau_m}) \rightarrow 0\Big) = 1,
%\end{align*}
%where $\mu^{(n_\ell')}_{\tau_1,\ldots,\tau_m} = \frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^{\tau_1})_j, \ldots, (\btheta^{\tau_m})_j), (\btheta^\ast)_j\big)}$ and $ \mu_{\tau_1,\ldots,\tau_m} = \cL(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)$. By successive refinement and a diagonal argument, there exists some further sequence $\{n_\ell''\}$ such that
%\begin{align*}
%\P\Big(\dbl(\mu^{(n_\ell'')}_{\tau_1,\ldots,\tau_m}, \mu_{\tau_1,\ldots,\tau_m}) \rightarrow 0, \forall m \in \Z, \forall \tau_1,\ldots, \tau_m \in [0,T] \cap \Q\Big) = 1.
%\end{align*}
%Since $\mu^{(n)}, \mu \in \cL([0,T],\R)$ are uniquely determined by finite-dimensional distributions on the rationals, we conclude that on the same subsequence,
%\begin{align*}
%\P\Big(\dbl(\mu^{(n_\ell'')}, \mu) \rightarrow 0\Big) = 1.
%\end{align*}
%Since for any subsequence $\{n_\ell\}$ there exists a further subsequence $\{n_\ell''\}$ such that $\dbl(\mu^{(n_\ell'')}, \mu) \rightarrow 0$ a.s., applying the above fact again yields $\dbl(\mu^{(n)}, \mu) \rightarrow_P 0$, completing the proof.
\end{proof}

\section{Proof of Theorem \ref{thm:dmftresponse}}
%The goal is to prove
%\begin{align*}
%\frac{1}{d}\Tr \bR_\theta(t,s) \rightarrow_P R_\theta(t,s), \quad \frac{1}{n}\Tr \bR_\eta(t,s) \rightarrow_P R_\eta(t,s), \quad \frac{1}{n}\Tr \bR_\eta(t,\ast) \rightarrow_P R_\eta(t,\ast).
%\end{align*}

\subsection{Step 1: Discretization of Langevin response function}
We recall the discrete, integer-indexed Langevin dynamic (\ref{eq:langevin_discrete_1})-(\ref{eq:langevin_discrete_2}) which we simplify in notation as
%\begin{align}\label{def:langevin_auxiliary}
%\tilde{\btheta}_\gamma^{t_{i+1}} = \tilde{\btheta}_\gamma^{t_i} - \gamma\bigg(\frac{1}{\sigma^2}\X^\top (\X\tilde{\btheta}^{t_i}_\gamma - \X\btheta^\ast - \beps) - \partial_\theta \log g(\tilde{\btheta}^{t_i}_\gamma;\bar{\alpha}^{t_i}_\gamma)\bigg) + \sqrt{2}(\B^{t_{i+1}} - \B^{t_i}),
%\end{align}, 
\begin{align}
\btheta^{t+1} &= \btheta^{t} - \gamma\Big[\frac{1}{\sigma^2}\X^\top(\X\btheta^{t} - \y) - \partial_\theta \log g(\btheta^{t};\bar{\alpha}^t_\gamma)\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}),\quad \bbeta^t = \X\btheta^t,\label{eq:original_theta},\\
\hat{\alpha}^{t+1} &= \hat{\alpha}^t + \gamma \cG(\hat{\alpha}^t, d^{-1}\sum_{j=1}^d \delta_{\theta^t_j}) \label{eq:original_alpha}.
\end{align}
%where we simplify the 
For any $t,s\in \Z_+$ with $s\leq t$, and $j\in[d],i\in[n]$, define two sets of perturbed dynamics
\begin{align}
\btheta^{t+1, (s,j), \eps} &:= \btheta^{t,(s,j),\eps} - \gamma\Big[\frac{1}{\sigma^2}\X^\top(\X\btheta^{t,(s,j),\eps} - \y) - \partial_\theta \log g(\btheta^{t,(s,j),\eps}, \hat{\alpha}^{t,(s,j),\eps}) - \eps \e_j \bm{1}_{t = s}\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}),\label{eq:theta_col_perturb} \\
\hat{\alpha}^{t+1, (s,j),\eps} &:= \hat{\alpha}^{t, (s,j),\eps} + \gamma \cG\Big(\hat{\alpha}^{t, (s,j),\eps}, d^{-1}\sum_{\ell=1}^d \delta_{\theta^{t, (s,j), \eps}_\ell}\Big),\label{eq:alpha_col_perturb}
\end{align}
and
\begin{align}
\btheta^{t+1, [s,i], \eps} &:= \btheta^{t,[s,i],\eps} - \gamma\Big[\frac{1}{\sigma^2}\X^\top(\X\btheta^{t,[s,i],\eps} - \y) - \partial_\theta \log g(\btheta^{t,[s,i],\eps}, \hat{\alpha}^{t,[s,i],\eps}) - \eps \X^\top  \e_i\bm{1}_{t = s}\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma})\label{eq:theta_row_perturb},\\
\hat{\alpha}^{t+1, [s,i], \eps} &:= \hat{\alpha}^{t, [s,i], \eps} + \gamma \cG\Big(\hat{\alpha}^{t, [s,i], \eps}, d^{-1}\sum_{\ell=1}^d \delta_{\theta^{t, [s,i], \eps}_\ell}\Big).\label{eq:alpha_row_perturb}
\end{align}
Same as before, let
\begin{align}\label{eq:eta_row_perturb}
\bbeta^{t,[s,i],\eps} := \X\btheta^{t, [s,i], \eps}.
\end{align}
Clearly we have $\btheta^{t, (s,j), 0} = \btheta^{t, [s,i], 0} = \btheta^t$,  $\hat{\alpha}^{t, (s,j), 0} = \hat{\alpha}^{t, [s,i], 0} = \hat{\alpha}^t$, and $\bbeta^{t,[s,i],0} = \bbeta^{t}$. For any $k,\ell\in\Z_+$ with $\ell\leq k$, let $\bR_\theta^\gamma(k,\ell) = (\bR_\theta^\gamma(k,\ell))_{i,j=1}^d \in\R^{d\times d}$ and $\bR_\eta^\gamma(k,\ell) = (\bR_\eta^\gamma(k,\ell))_{i,j=1}^n \in\R^{d\times d}$ be defined by
\begin{align*}
(\bR_\theta^\gamma(k,\ell))_{i,j} &= \frac{1}{\gamma}\partial_\eps|_{\eps = 0} \langle(\btheta^{k,(\ell,j),\eps})_i\rangle_{\x},\\
(\bR_\eta^\gamma(k,\ell))_{i,j} &= (-\frac{\delta}{\sigma^4}) \cdot \frac{1}{\gamma}\partial_\eps|_{\eps = 0} \langle (\bbeta^{k,[\ell,j],\eps})_i \rangle_{\x},
\end{align*}
where $\langle \cdot \rangle_{\x}$ denotes expectation only over the Brownian motion $\{\b^t\}$ with (\ref{eq:theta_col_perturb})-(\ref{eq:alpha_col_perturb}) and (\ref{eq:theta_row_perturb})-(\ref{eq:alpha_row_perturb}) initialized from $(\btheta^{0,(\ell,j),\eps},\hat{\alpha}^{0,(\ell,j),\eps}) = (\btheta^{0,[\ell,i],\eps},\hat{\alpha}^{0,[\ell,i],\eps})  = \x \in \R^{d\times K}$. For any $t \in \R_+$, let $[t] = \floor{t}/\gamma$ where $\floor{t}$ is given by (\ref{eq:t_floor_ceil}).


\begin{proposition}\label{prop:semigroup_discre_error}
Assume the conditions of Theorem \ref{thm:dmftresponse}. For any $T > 0$, there exists some $C > 0$ depending on $T, \sigma$ and the constants in the assumptions such that, for any $0\leq s\leq t\leq T$, 
\begin{align*}
\langle |\Tr\bR_\theta(t,s) - \Tr\bR_\theta^\gamma([t],[s])| \rangle \vee \langle |\Tr\bR_\eta(t,s) - \Tr\bR_\eta^\gamma([t],[s])| \rangle\leq C\sqrt{\gamma d}(\pnorm{\x}{} + \pnorm{\X^\top \y}{} + \sqrt{d}).
\end{align*}
\end{proposition}
\begin{proof}[Proof of Proposition \ref{prop:semigroup_discre_error}: Bound on $\Tr \bR_\theta(t,s)$]
Let $P_\gamma$ be the one step transition semigroup of the discrete dynamic (\ref{eq:original_theta})-(\ref{eq:original_alpha}), 
%\begin{align*}
%\btheta^{t+1} = \btheta^t + \gamma \Big[\log q(\btheta^t) \Big]  + \sqrt{2}(B^{(t+1)\gamma} - B^{t\gamma}),
%\end{align*} 
that is, $P_\gamma f(\x) = \langle f(\btheta^{t+1},\hat{\alpha}^{t+1})\rangle_{(\btheta^t,\hat{\alpha}^t) = \x}$ for any $f:\R^{d+K} \rightarrow \R$. Let $P_\gamma^{(j,\eps)}$ be the one step transition semigroup of the discrete dynamic
\begin{align*}
\tilde{\btheta}^{t+1} &= \tilde{\btheta}^t - \gamma\Big[\frac{1}{\sigma^2}\X^\top(\X\tilde{\btheta}^{t} - \y) - \partial_\theta \log g(\tilde{\btheta}^{t};\tilde{\alpha}^t) - \eps \e_j\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}),\\
\tilde{\alpha}^{t+1} &= \tilde{\alpha}^t + \gamma \cG\Big(\tilde{\alpha}^t, d^{-1}\sum_{\ell=1}^d \delta_{\tilde{\theta}^t_\ell}\Big),
\end{align*} 
that is, $P_\gamma^{(j,\eps)} f(\x)= \langle f(\tilde{\btheta}^{t+1}, \tilde{\alpha}^{t+1}) \rangle_{(\tilde{\btheta}^t, \tilde{\alpha}^t) = \x}$. Then we have
\begin{align*}
\langle(\btheta^{k,(\ell,j),\eps})_i\rangle = P_\gamma^{\circ \ell} P_\gamma^{(j,\eps)} P_\gamma^{\circ (k-\ell-1)} e_i(\x),
\end{align*}
where we recall $e_i(\x) = x_i$ defined in (\ref{eq:coordfuncs}) (indexing the $i$th component of $\btheta$) and we write $P_\gamma^{\circ m}$ as the $m$-fold composition of $P_\gamma$. Using the fact
\begin{align*}
\partial_\eps|_{\eps = 0} P_\gamma^{(j,\eps)} f(\x) = \gamma \cdot \langle \e_j^\top \nabla f(\btheta^{t+1}, \hat{\alpha}^{t+1})\rangle_{(\btheta^t,\hat{\alpha}^t) = \x} = \gamma P_\gamma[\partial_j f](\x),
\end{align*}
we have
\begin{align*}
\partial_\eps|_{\eps = 0} \langle(\btheta^{k,(\ell,j),\eps})_i\rangle = P_\gamma^{\circ \ell} \partial_\eps|_{\eps = 0} P_\gamma^{(j,\eps)} P_\gamma^{\circ (k-\ell-1)} e_i(\x) = \gamma P_\gamma^{\circ (\ell+1)} \partial_j P_\gamma^{\circ (k-\ell-1)} e_i(\x),
\end{align*}
which further implies that
\begin{align*}
\partial_\eps|_{\eps = 0} \Tr \bR_\theta^\gamma(k,\ell) = \sum_{j=1}^d P_\gamma^{\circ (\ell+1)} \partial_j P_\gamma^{\circ (k-\ell-1)} e_j(\x).
\end{align*}
So using the notation $[t] = \floor{t}/\gamma$, we have
\begin{align*}
\Big|\Tr \bR_\theta(t,s) - \Tr \bR^\gamma_\theta([t],[s])\Big| &= \Big|\sum_{j=1}^d  P_{s} \partial_j P_{t-s} e_j - \sum_{j=1}^d  P_\gamma^{\circ ([s]+1)} \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j\Big|\\
&\leq \underbrace{\Big|P_{s}\Big(\sum_{j=1}^d\partial_j P_{t-s} e_j - \sum_{j=1}^d \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j\Big)\Big|}_{(I)} + \underbrace{\Big|(P_s - P_\gamma^{\circ ([s]+1)})\sum_{j=1}^d \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j\Big|}_{(II)}.
\end{align*}
\noindent\textbf{Bound of $(I)$} Note that by Proposition \ref{prop:langevinsolution}-(c), $\sum_{j=1}^d\partial_j P_{t-s} e_j(\x) = \sum_{j=1}^d \langle (\V^{t-s})_{jj}\rangle_{\x}$, where $\{\x^t = (\btheta^t,\hat{\alpha}^t), \V^t\}_{t\in\R_+}$ follow the dynamic
\begin{align}\label{eq:theta_V}
\notag\d\x^t &= u(\x^t)\d t + \sqrt{2}\M \d \b^t, \quad \x^0 = \x,\\
\d \V^t &= [\nabla u(\btheta^t) \V^t]\d t, \quad \V^0 = I_{d+K},
\end{align}
with $\M, u(\cdot)$ given by (\ref{eq:jointdrift}). On the other hand, Lemma \ref{lem:discrete_bismut} yields that $\sum_{j=1}^d \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j = \sum_{j=1}^d \langle  (\tilde{\V}^{[t] - [s] - 1})_{jj} \rangle_{\x}$, where $\{\tilde{\x}^t = (\btheta^t, \hat{\alpha}^t), \tilde{\V}^t\}_{t\in\Z}$ ($(\btheta^t, \hat{\alpha}^t)$ given in (\ref{eq:original_theta})-(\ref{eq:original_alpha})) follow
\begin{align}\label{eq:theta_V_discre}
\notag\tilde{\x}^{t+1} &= \tilde{\x}^{t} + \gamma u(\tilde{\x}^t) + \sqrt{2}\M(\b^{(t+1)\gamma} - \b^{t\gamma}), \quad \tilde{\x}^0 = \x\\
\tilde{\V}^{t+1} &= \tilde{\V}^t + \gamma \nabla u(\tilde{\x}^t) \tilde{\V}^t, \quad \tilde{\V}^0 = I_{d+K}.
\end{align}
We can embed this into the continuous-time process $\{\bar{\x}^t = (\bar{\btheta}^t, \bar\alpha^t), \bar{\V}^t\}_{t\in\R_+}$ defined by
\begin{align}\label{eq:theta_V_embed}
\notag\d\bar{\x}^t &= \nabla u(\bar{\x}^{\floor{t}})\d t + \sqrt{2}\M\d \b^t, \quad \bar{\x}^0 = \x,\\
\d \bar{\V}^t &= [\nabla u(\bar{\x}^{\floor{t}}) \bar{\V}^{\floor{t}}]\d t, \quad \bar{\V}^0 = I_{d+K},
\end{align}
such that for any $t_i= i\gamma$, $(\bar{\x}^{t_i}, \bar{\V}^{t_i}) = (\tilde{\x}^i,\tilde{\V}^i)$, which further implies that $ \sum_{j=1}^d \langle  (\tilde{\V}^{[t] - [s] - 1})_{jj} \rangle_{\x} =  \sum_{j=1}^d\langle (\bar{\V}^{\gamma([t] - [s] - 1)})_{ii}\rangle_{\x} =  \sum_{j=1}^d\langle (\bar{\V}^{\floor{t} - \floor{s} - \gamma})_{ii}\rangle_{\x}$. Let us write $\V^t = [\U^t, \ast; \W^t,\ast]$ and $\bar{\V}^t = [\bar{\U}^t,\ast; \bar{\W}^t,\ast]$ in block form, where $\U^t,\bar{\U}^t \in \R^{d\times d}$ and $\W^t, \bar{\W}^t \in \R^{K\times d}$. We may now bound
\begin{align}\label{eq:semigroup_discre_1}
\notag&\Big|\sum_{j=1}^d \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j(\x) - \partial_j P_\gamma^{\circ ([t]-[s]-1)} \e_j(\x)\Big|\\
\notag&= \Big|\langle \Tr \U^{t-s} - \Tr \bar{\U}^{\floor{t}-\floor{s}-\gamma}\rangle_{\x}\Big|\\
&\leq \sqrt{d}\langle \pnorm{\U^{t-s} - \bar{\U}^{t-s}}{F}\rangle_{\x} + d\langle \pnorm{\bar{\U}^{t-s} - \bar{\U}^{\floor{t}-\floor{s}-\gamma}}{\op} \rangle_{\x}.
\end{align}
The second term satisfies $d\langle \pnorm{\bar{\U}^{t-s} - \bar{\U}^{\floor{t}-\floor{s}-\gamma}}{\op}\rangle_{\x} \leq C\gamma d$ by Lemma \ref{lem:theta_V_rough}. For the first term, we partition $\nabla u(\x^t) = [J^t_1, J^t_2; J^t_3, J^t_4]$ and $\nabla u(\bar{\x}^{\floor{t}}) = [J^{\floor{t}}_1, J^{\floor{t}}_2; J^{\floor{t}}_3, J^{\floor{t}}_4]$ with $J^t_1,J^{\floor{t}}_1\in\R^{d\times d}$ and $J^t_4, J^{\floor{t}}_4\in \R^{K\times K}$ so that 
\begin{align*}
\U^t = \U^0 + \int_0^t (J^s_1 \U^s + J^s_2 \W^s) \d s,\quad \W^t = \W^0 + \int_0^t (J^s_3 \U^s + J^s_4 \W^s) \d s,\\
\bar{\U}^t = \U^0 + \int_0^t (J^{\floor{s}}_1 \bar{\U}^{\floor{s}} + J^{\floor{s}}_2 \bar{\W}^{\floor{s}}) \d s,\quad \bar{\W}^t = \W^0 + \int_0^t (J^{\floor{s}}_3 \bar{\U}^{\floor{s}} + J^{\floor{s}}_4 \bar{\W}^{\floor{s}}) \d s.
\end{align*}
Hence
\begin{align*}
\langle\pnorm{\U^t - \bar{\U}^t}{F}\rangle_{\x} &\leq \int_0^t \Big[\langle\pnorm{J^s_1 - J^{\floor{s}}_1}{F}\pnorm{\U^s}{\op}\rangle_{\x} + \langle\pnorm{J^{\floor{s}}_1}{\op}(\pnorm{\U^s - \bar{\U}^s}{F} + \pnorm{\bar{\U}^s - \bar{\U}^{\floor{s}}}{F})\rangle_{\x}\Big] \d s\\
&\quad + \int_0^t \Big[\langle\pnorm{J^s_2 - J^{\floor{s}}_2}{F}\pnorm{\W^s}{F}\rangle_{\x} + \langle\pnorm{J^{\floor{s}}_2}{F}(\pnorm{\W^s - \bar{\W}^s}{F} + \pnorm{\bar{\W}^s - \bar{\W}^{\floor{s}}}{F})\rangle_{\x}\Big] \d s.
\end{align*}
By Lemma \ref{lem:theta_V_rough} we have $\pnorm{\U^s}{\op} \vee \sqrt{d}\pnorm{\W^s}{F} \leq C$, and it can be readily that  
\begin{equation}\label{eq:J_bound}
\begin{gathered}
\langle\pnorm{J^s_1 - J^{\floor{s}}_1}{F}\rangle_{\x} \vee \langle\pnorm{J^s_2 - J^{\floor{s}}_2}{F}\rangle_{\x} \vee\langle\pnorm{\bar{\U}^s - \bar{\U}^{\floor{s}}}{F}\rangle_{\x} \leq C\sqrt{\gamma}(\sqrt{d} + \pnorm{\x}{} + \pnorm{\X^\top \y}{}),\\
\langle\pnorm{\bar{\W}^s - \bar{\W}^{\floor{s}}}{F}\rangle_{\x} \leq C\sqrt{\gamma/d}, \quad \pnorm{J^{\floor{s}}_2}{F} \leq C\sqrt{d}, \quad \pnorm{J^{\floor{s}}_1}{\op}\leq C,
\end{gathered}
\end{equation}
we obtain that
\begin{align}\label{eq:U_bound}
\langle\pnorm{\U^t - \bar{\U}^t}{F}\rangle_{\x}\leq C\int_0^t \big(\langle\pnorm{\U^s - \bar{\U}^s}{F}\rangle_{\x} + \sqrt{d}\langle\pnorm{\W^s - \bar{\W}^s}{F}\rangle_{\x}\big) \d s + C\sqrt{\gamma}(\sqrt{d} + \pnorm{\x}{} + \pnorm{\X^\top \y}{}).
\end{align}
Next we have
\begin{align*}
\langle\pnorm{\W^t - \bar{\W}^t}{F}\rangle_{\x} &\leq \int_0^t \Big[\langle\pnorm{J^s_3 - J^{\floor{s}}_3}{F}\pnorm{\U^s}{\op}\rangle_{\x} + \langle\pnorm{J^{\floor{s}}_3}{\op}(\pnorm{\U^s - \bar{\U}^s}{F} + \pnorm{\bar{\U}^s - \bar{\U}^{\floor{s}}}{F})\rangle_{\x}\Big] \d s\\
&\quad + \int_0^t \Big[\langle\pnorm{J^s_4 - J^{\floor{s}}_4}{F}\pnorm{\W^s}{F}\rangle_{\x} + \langle\pnorm{J^{\floor{s}}_4}{F}(\pnorm{\W^s - \bar{\W}^s}{F} + \pnorm{\bar{\W}^s - \bar{\W}^{\floor{s}}}{F})\rangle_{\x}\Big] \d s.
\end{align*}
Note that by the Assumption \ref{assump:gradient}, we have $\langle\pnorm{J^s_3 - J^{\floor{s}}_3}{F}\rangle_{\x} \leq C\langle\pnorm{\btheta^s - \bar{\btheta}^{\floor{s}}}{}/d + \pnorm{\hat\alpha^s - \bar{\alpha}^{\floor{s}}}{}/\sqrt{d}\rangle_{\x} \leq C\sqrt{\gamma/d}$, and furthermore by (\ref{eq:J_bound}) and the following bounds:
\begin{align*}
\pnorm{J^{\floor{s}}_3}{F} \leq C/\sqrt{d}, \quad \langle\pnorm{J^s_4 - J^{\floor{s}}_4}{F}\rangle_{\x} \leq C\sqrt{\gamma/d}(\sqrt{d}+\pnorm{\X^\top \y}{} + \pnorm{\x}{}), \quad \pnorm{J^{\floor{s}}_4}{F} \leq C,
\end{align*}
which implies that
\begin{align}\label{eq:W_bound}
\sqrt{d}\langle\pnorm{\W^t - \bar{\W}^t}{F}\rangle_{\x} \leq C\int_0^t (\langle\pnorm{\U^s - \bar{\U}^s}{F}\rangle_{\x} + \sqrt{d}\langle\pnorm{\W^s - \bar{\W}^s}{F}\rangle_{\x})\d s + C\sqrt{\gamma}(\sqrt{d} + \pnorm{\X^\top\y}{} + \pnorm{\x}{}).
\end{align}
Combining (\ref{eq:U_bound}) and (\ref{eq:W_bound}) yields
\begin{align*}
\langle\pnorm{\U^t - \bar{\U}^t}{F} + \sqrt{d}\langle\pnorm{\W^t - \bar{\W}^t}{F}\rangle_{\x} \leq C\int_0^t (\langle\pnorm{\U^s - \bar{\U}^s}{F} + \sqrt{d}\langle\pnorm{\W^s - \bar{\W}^s}{F}\rangle_{\x})\d s + C\sqrt{\gamma}(\sqrt{d} + \pnorm{\X^\top\y}{} + \pnorm{\x}{}), 
\end{align*}
which by Lemma \ref{lem:gronwall} yields $\langle\pnorm{\U^t - \bar{\U}^t}{F}\rangle_{\x} + \sqrt{d}\langle\pnorm{\W^t - \bar{\W}^t}{F}\rangle_{\x} \leq C'\sqrt{\gamma}(\sqrt{d} + \pnorm{\X^\top\y}{} + \pnorm{\x}{})$.



%since
%\begin{align*}
%\V^t = I_d + \int_0^t \nabla^2 \log q(\btheta^s)\V^s\d s, \quad \bar{\V}^t = I_d + \int_0^t \nabla^2 \log q(\bar{\btheta}^{\floor{s}})\bar{\V}^{\floor{s}}\d s,  
%\end{align*}
%we have
%\begin{align*}
%\pnorm{\V^t - \bar{\V}^t}{F} &\leq \int_0^t \pnorm{\nabla^2\log q(\btheta^s) - \nabla^2 \log q(\bar{\btheta}^{\floor{s}})}{F}\pnorm{\V^s}{\op}\d s + \int_0^t \pnorm{\nabla^2 \log q(\bar{\btheta}^{\floor{s}})}{\op}\pnorm{\V^s - \bar{\V}^{\floor{s}}}{F}\d s\\
%&\leq C\int_0^t \pnorm{\btheta^s - \bar{\btheta}^{\floor{s}}}{}\pnorm{\V^s}{\op}\d s + \int_0^t L\pnorm{\V^s - \bar{\V}^{s}}{F} \d s + \int_0^t L\pnorm{\bar{\V}^s - \bar{\V}^{\floor{s}}}{F} \d s,
%\end{align*}
%where $L = \pnorm{\X}{\op}^2/\sigma^2 + \pnorm{f''}{\infty}$. Using the estimates in Lemma \ref{lem:theta_V_rough}, we have
%\begin{align*}
%\E_\x^\circ\pnorm{\V^t - \bar{\V}^t}{F}^2 \leq C\gamma(\pnorm{\x}{}^2 + \pnorm{\X^\top \y}{}^2 + d) + \int_0^t C\E_\x^\circ\pnorm{\V^s - \bar{\V}^{s}}{F}^2 \d s,
%\end{align*}
%so Gronwall' lemma yields $\E_\x^\circ\pnorm{\V^t - \bar{\V}^t}{F}^2 \leq C\gamma(\pnorm{\x}{}^2 + \pnorm{\X^\top \y}{}^2 + d)$. 

Hence the bound (\ref{eq:semigroup_discre_1}) reads
\begin{align}\label{eq:V_frob_norm}
\Big|\sum_{j=1}^d \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j(\x) - \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j(\x)\Big| \leq C\sqrt{\gamma d}\Big(\pnorm{\x}{} + \pnorm{\X^\top \y}{} + \sqrt{d}\Big),
\end{align}
which further implies that
\begin{align*}
(I) \leq C\gamma\sqrt{d}(\pnorm{\X^\top \y}{} + \sqrt{d} + \langle\pnorm{\btheta^s}{}\rangle_{\x}) \leq C\sqrt{\gamma d}(\pnorm{\X^\top \y}{} + \sqrt{d} + \pnorm{\x}{}),
\end{align*}
using Lemma \ref{lem:theta_V_rough} in the last step. 

\noindent\textbf{Bound of $(II)$} Let $\mathsf{f}(\x) = \sum_{j=1}^d \partial_j P_\gamma^{\circ ([t]-[s]-1)} e_j(\x)$. Then
\begin{align*}
\Big|(P_s - P_\gamma^{\circ ([s]+1)})\mathsf{f}(\x)\Big| = \Big|\langle \mathsf{f}(\x^s) \rangle_{\x}- \langle \mathsf{f}(\tilde{\x}^{[s]+1}) \rangle_{\x}\Big| = \Big| \langle \mathsf{f}(\x^s) - \mathsf{f}(\bar{\x}^{\floor{s}+\gamma})\rangle_{\x}\Big| \leq \pnorm{\mathsf{f}}{Lip}\langle \pnorm{\x^s - \bar{\x}^{\floor{s} + \gamma}}{} \rangle_{\x}, 
\end{align*}
where $\{\x^t\}_{t\in\R_+}$ and $\{\bar{\x}^t\}_{t\in\R_+}$ are given by (\ref{eq:theta_V}) and (\ref{eq:theta_V_embed}) respectively coupled with the same Brownian $\{\B^t\}_{t\in \R_+}$. By Lemma \ref{lem:theta_V_rough}, $\langle \pnorm{\x^s - \bar{\x}^{\floor{s} + \gamma}}{} \rangle_{\x}\leq \langle \pnorm{\x^s - \bar{\x}^s}{} \rangle_{\x} + \langle \pnorm{\bar{\x}^s - \bar{\x}^{\floor{s} + \gamma}}{} \rangle_{\x}\leq C\sqrt{\gamma}(\sqrt{d} + \pnorm{\X^\top \y}{} + \pnorm{\x}{})$, so it remains to bound the Lipschitz constant $\pnorm{\mathsf{f}}{Lip}$. To this end, let $\{\tilde{\x}^t_{\mathsf{y}}, \tilde{\V}^t_\mathsf{y}\}_{t\in \Z_+}$ and $\{\tilde{\x}^t_{\mathsf{y}'}, \tilde{\V}^t_{\mathsf{y}'}\}_{t\in \Z_+}$ be defined by (\ref{eq:theta_V_discre}) with initialization $\mathsf{y},\mathsf{y}'\in\R^{d+K}$ respectively. Similar as above we partition $\tilde{\V}^{t}_{\mathsf{y}} = [\tilde{\U}^{t}_{\mathsf{y}}, \ast; \tilde{\W}^{t}_{\mathsf{y}}, \ast]$ and similarly for $\tilde{\V}^{t}_{\mathsf{y}'}$, and partition $\nabla u(\tilde{\x}^t_{\mathsf{y}}) = [J^t_{1,\mathsf{y}}, J^t_{2,\mathsf{y}}; J^t_{3,\mathsf{y}}, J^t_{4,\mathsf{y}}]$, so that
\begin{align*}
\tilde{\U}^{t+1}_{\mathsf{y}} = (I + \gamma J^t_{1,\mathsf{y}}) \tilde{\U}^{t}_{\mathsf{y}} + \gamma J^t_{2,\mathsf{y}} \tilde{\W}^{t}_{\mathsf{y}},\quad  \tilde{\W}^{t+1}_{\mathsf{y}} = (I + \gamma J^t_{3,\mathsf{y}}) \tilde{\U}^{t}_{\mathsf{y}} + \gamma J^t_{4,\mathsf{y}} \tilde{\W}^{t}_{\mathsf{y}}, 
\end{align*}
and similarly for $\tilde{\U}^{t+1}_{\mathsf{y}'}, \tilde{\U}^{t+1}_{\mathsf{y}'}$. Then using $\mathsf{f}(\x) = \langle \Tr \tilde{\U}^{\tau} \rangle_{\x}$ with $\tau = [t] - [s] - 1 \in \Z_+$ as established above,
\begin{align}\label{eq:f_modulus}
|\mathsf{f}(\mathsf{y}) - \mathsf{f}(\mathsf{y}')| \leq |\langle\Tr \tilde{\U}^{\tau}_{\mathsf{y}}  - \Tr \tilde{\U}^{\tau}_{\mathsf{y}'} \rangle | \leq \sqrt{d} \langle \pnorm{\tilde{\U}^{\tau}_{\mathsf{y}} - \tilde{\U}^{\tau}_{\mathsf{y}'}}{F} \rangle.
\end{align}
To bound $\langle \pnorm{\tilde{\U}^{\tau}_{\mathsf{y}} - \tilde{\U}^{\tau}_{\mathsf{y}'}}{F} \rangle$, we apply a similar argument as in term $(I)$. Note that
\begin{align*}
\pnorm{\tilde{\U}^{t+1}_{\mathsf{y}} - \tilde{\U}^{t+1}_{\mathsf{y}'}}{F} &\leq \gamma\pnorm{J^t_{1,\mathsf{y}} - J^t_{1,\mathsf{y}'}}{F}\pnorm{\tilde{\U}^t_{\mathsf{y}}}{\op} + (1+\gamma\pnorm{J^t_{1,\mathsf{y}'}}{\op})\pnorm{\tilde{\U}^{t}_{\mathsf{y}} - \tilde{\U}^{t}_{\mathsf{y}'}}{F}\\
&\quad +  \gamma\pnorm{J^t_{2,\mathsf{y}} - J^t_{2,\mathsf{y}'}}{F}\pnorm{\tilde{\W}^t_{\mathsf{y}}}{F} + \gamma\pnorm{J^t_{2,\mathsf{y}'}}{\op}\pnorm{\tilde{\W}^{t}_{\mathsf{y}} - \tilde{\W}^{t}_{\mathsf{y}'}}{F},\\
\pnorm{\tilde{\W}^{t+1}_{\mathsf{y}} - \tilde{\W}^{t+1}_{\mathsf{y}'}}{F} &\leq \gamma\pnorm{J^t_{3,\mathsf{y}} - J^t_{3,\mathsf{y}'}}{F}\pnorm{\tilde{\U}^t_{\mathsf{y}}}{\op} + \gamma\pnorm{J^t_{3,\mathsf{y}'}}{\op}\pnorm{\tilde{\U}^{t}_{\mathsf{y}} - \tilde{\U}^{t}_{\mathsf{y}'}}{F}\\
&\quad +  \gamma\pnorm{J^t_{4,\mathsf{y}} - J^t_{4,\mathsf{y}'}}{F}\pnorm{\tilde{\W}^t_{\mathsf{y}}}{F} + (1 + \gamma\pnorm{J^t_{4,\mathsf{y}'}}{F})\pnorm{\tilde{\W}^{t}_{\mathsf{y}} - \tilde{\W}^{t}_{\mathsf{y}'}}{F}
\end{align*}
By Lemma \ref{lem:theta_V_rough}, we have $\pnorm{\tilde{\U}^t_{\mathsf{y}}}{\op} \vee \sqrt{d} \pnorm{\tilde{\W}^t_{\mathsf{y}}}{\op}\leq C$, and it can be readily verified that
\begin{align*}
\langle \pnorm{J^t_{1,\mathsf{y}} - J^t_{1,\mathsf{y}'}}{F} \rangle \vee \langle \pnorm{J^t_{2,\mathsf{y}} - J^t_{2,\mathsf{y}'}}{F}  \rangle \vee d \langle \pnorm{J^t_{3,\mathsf{y}} - J^t_{3,\mathsf{y}'}}{F}\rangle \vee \langle \pnorm{J^t_{4,\mathsf{y}} - J^t_{4,\mathsf{y}'}}{F}\rangle &\leq C\pnorm{\mathsf{y} - \mathsf{y}'}{},\\
\pnorm{J^t_{1,\mathsf{y}'}}{\op} \vee \frac{\pnorm{J^t_{2,\mathsf{y}'}}{\op}}{\sqrt{d}} \vee \sqrt{d}\pnorm{J^t_{3,\mathsf{y}'}}{\op} \vee \pnorm{J^t_{4,\mathsf{y}'}}{\op} &\leq C,
\end{align*}
hence
\begin{align*}
\langle\pnorm{\tilde{\U}^{t+1}_{\mathsf{y}} - \tilde{\U}^{t+1}_{\mathsf{y}'}}{F} \rangle &\leq (1+C\gamma)\langle \pnorm{\tilde{\U}^{t}_{\mathsf{y}} - \tilde{\U}^{t}_{\mathsf{y}'}}{F} \rangle  + C\gamma \sqrt{d}\langle\pnorm{\tilde{\W}^{t}_{\mathsf{y}} - \tilde{\W}^{t}_{\mathsf{y}'}}{F} \rangle + C\gamma \pnorm{\mathsf{y} - \mathsf{y'}}{},\\
\langle\pnorm{\tilde{\W}^{t+1}_{\mathsf{y}} - \tilde{\W}^{t+1}_{\mathsf{y}'}}{F} \rangle &\leq (1+C\gamma)\langle \pnorm{\tilde{\W}^{t}_{\mathsf{y}} - \tilde{\W}^{t}_{\mathsf{y}'}}{F} \rangle+ C\gamma\pnorm{\tilde{\U}^{t}_{\mathsf{y}} - \tilde{\U}^{t}_{\mathsf{y}'}}{F}/\sqrt{d} + C\gamma \pnorm{\mathsf{y} - \mathsf{y'}}{}/\sqrt{d},
\end{align*}
which further implies that
\begin{align*}
\langle\pnorm{\tilde{\U}^{t+1}_{\mathsf{y}} - \tilde{\U}^{t+1}_{\mathsf{y}'}}{F} + \sqrt{d} \pnorm{\tilde{\W}^{t+1}_{\mathsf{y}} - \tilde{\W}^{t+1}_{\mathsf{y}'}}{F}\rangle \leq (1+C\gamma)\langle\pnorm{\tilde{\U}^{t}_{\mathsf{y}} - \tilde{\U}^{t}_{\mathsf{y}'}}{F} + \sqrt{d} \pnorm{\tilde{\W}^{t}_{\mathsf{y}} - \tilde{\W}^{t}_{\mathsf{y}'}}{F}\rangle + C\gamma \pnorm{\mathsf{y} - \mathsf{y'}}{}.
\end{align*}
This can be solved as $\langle\pnorm{\tilde{\U}^{\tau}_{\mathsf{y}} - \tilde{\U}^{\tau}_{\mathsf{y}'}}{F}\rangle \leq C\pnorm{\mathsf{y} - \mathsf{y'}}{}$, which combined with (\ref{eq:f_modulus}) yields that $\pnorm{\mathsf{f}}{Lip} \leq C\sqrt{d}$,
%which satisfies 
%\begin{align*}
%\pnorm{\bar{\V}^{\tau}_{\x} - \bar{\V}^{\tau}_{\x'}}{F} &\leq \int_0^\tau \Big[\pnorm{(\nabla^2 \log q(\btheta^{\floor{s}}_\x) - \nabla^2 \log q(\btheta^{\floor{s}}_{\x'}))\bar{\V}^{\floor{s}}_{\x}}{F} + \pnorm{\nabla^2 \log q(\btheta^{\floor{s}}_{\x'})(\bar{\V}^{\floor{s}}_{\x} - \bar{\V}^{\floor{s}}_{\x'})}{F}\Big] \d s\\
%&\leq \int_0^\tau \pnorm{\bar{\V}^{\floor{s}}_{\x}}{\op}\pnorm{\nabla^2 \log q(\btheta^{\floor{s}}_\x) - \nabla^2 \log q(\btheta^{\floor{s}}_{\x'})}{F}\d s + C\int_0^t \pnorm{\bar{\V}^{\floor{s}}_{\x} - \bar{\V}^{\floor{s}}_{\x'}}{F} \d s\\
%&\leq C\int_0^\tau \pnorm{\btheta^{\floor{s}}_\x - \btheta^{\floor{s}}_{\x'}}{}\d s + C\int_0^t \pnorm{\bar{\V}^{\floor{s}}_{\x} - \bar{\V}^{\floor{s}}_{\x'}}{F} \d s, 
%\end{align*}
%using the bound on $\pnorm{\bar{\V}^t}{\op}$ from Lemma \ref{lem:theta_V_rough}. Since $\pnorm{\bar{\btheta}^t_\x - \bar{\btheta}^t_{\x'}}{}\leq \int_0^t \pnorm{\nabla \log q(\bar{\btheta}^{\floor{s}}_\x) - \nabla \log q(\bar{\btheta}^{\floor{s}}_{\x'})}{}\d s\leq C\int_0^t \pnorm{\bar{\btheta}^{\floor{s}}_{\x} - \bar{\btheta}^{\floor{s}}_{\x'}}{}\d s$, it holds by Gronwall's lemma that $\pnorm{\bar{\btheta}^t_\x - \bar{\btheta}^t_{\x'}}{} \leq C\pnorm{\x - \x'}{}$, which implies that
%\begin{align*}
%\pnorm{\bar{\V}^{\tau}_{\x} - \bar{\V}^{\tau}_{\x'}}{F} \leq C\pnorm{\x - \x'}{} + C\int_0^t \pnorm{\bar{\V}^{\floor{s}}_{\x} - \bar{\V}^{\floor{s}}_{\x'}}{F} \d s.
%\end{align*}
%Applying Gronwall's lemma again yields $\pnorm{\bar{\V}^{\tau}_{\x} - \bar{\V}^{\tau}_{\x'}}{F} \leq C\pnorm{\x - \x'}{}$, 
%
leading to the final bound $(II) \leq C\sqrt{\gamma d}(\sqrt{d} + \pnorm{\X^\top \y}{} + \pnorm{\x}{})$. The proof is complete by combining the bounds for $(I)$ and $(II)$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:semigroup_discre_error}: Bound on $\Tr \bR_\eta(t,s)$]
Let $P_\gamma$ be defined as above, and $P_\gamma^{[i,\eps]}$ be the one-step transition semigroup of the discrete dynamic
\begin{align*}
\tilde{\btheta}^{t+1} &= \tilde{\btheta}^t - \gamma\Big[\frac{1}{\sigma^2}\X^\top (\X\tilde{\btheta}^t - \y) - \partial_\theta \log g(\tilde{\btheta}^t;\tilde{\alpha}^t) - \eps \X^\top \e_i\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}),\\
\tilde{\alpha}^{t+1} &= \tilde{\alpha}^t + \gamma \cG(\tilde{\alpha}^t, d^{-1}\sum_{\ell=1}^d \delta_{\tilde{\theta}^t_\ell}),
\end{align*}
that is, $P_\gamma^{[i,\eps]} f(\x) = \langle f(\tilde{\btheta}^{t+1}, \tilde{\alpha}^{t+1})\rangle_{(\tilde{\btheta}^t, \tilde{\alpha}^t) = \x}$. Then for $i,j\in[n]$, we have
\begin{align*}
\langle (\bbeta^{k,[\ell,i],\eps})_j \rangle_{\x} = \langle (\X\btheta^{k,[\ell,i],\eps})_j \rangle_{\x} = P_\gamma^{\circ \ell}P^{[i,\eps]}_\gamma P_\gamma^{\circ (k-\ell-1)} x_j(\x),
\end{align*}
where we use $x_j$ to denote the map $(\btheta,\alpha) = \x \mapsto \e_j^\top \X E\x = \e_j^\top \X\btheta$ with $\e_j$ denoting the $j$th canonical basis in $\R^n$ and $E = [I_d, 0_{d\times K}] \in \R^{d\times (d+K)}$. Using the fact that
\begin{align*}
\deps P^{[i,\eps]}_\gamma f(\x) = \gamma \cdot \langle ((\X E)^\top \e_i)^\top \nabla f(\btheta^{t+1}, \hat{\alpha}^{t+1}) \rangle_{(\btheta^t, \alpha^t) = \x} = \gamma P_\gamma [\e_i^\top \X E\nabla f](\x),
\end{align*}
we have
\begin{align*}
\deps \langle (\bbeta^{k,[\ell,i],\eps})_j \rangle_{\x} = P_\gamma^{\circ \ell}\deps P^{[i,\eps]}_\gamma P_\gamma^{\circ (k-\ell-1)} (\X E)^\top \e_j(\x) = \gamma P_\gamma^{\circ (\ell+1)} \e_i^\top \X  E\nabla P_\gamma^{\circ (k-\ell-1)} [(\X E)^\top \e_j] (\x),
\end{align*}
which implies that
\begin{align*}
\deps \Tr \bR_\eta^\gamma(k,\ell) = \frac{\delta}{\sigma^4}\sum_{i=1}^n P_\gamma^{\circ (\ell+1)} \e_i^\top \X E\nabla P_\gamma^{\circ (k-\ell-1)} [(\X E)^\top \e_i] (\x) = \frac{\delta}{\sigma^4}P_\gamma^{\circ (\ell+1)} \Tr\Big[\nabla P_\gamma^{\circ (k-\ell-1)}(\x) \cdot E^\top \X^\top \X E\Big],
\end{align*}
where $\nabla P_\gamma^{\circ (k-\ell-1)}(\x) \in \R^{(d+K) \times (d+K)}$ is the Jacobian of the map $\x \mapsto P_\gamma^{\circ (k-\ell-1)}(\x)$. Hence using 
\begin{align*}
\Tr \bR_\eta(t,s) = \frac{\delta}{\sigma^4}\E_{q_s}[\Tr (\nabla P_{t-s}(\x) \cdot E^\top \X^\top \X E)] = \frac{\delta}{\sigma^4}P_s \Tr \big(\nabla P_{t-s}(\x) \cdot E^\top \X^\top \X E\big),
\end{align*}
we have
\begin{align*}
&\Big|\Tr \bR_\eta(t,s) - \Tr \bR_\eta^\gamma([t],[s])\Big|\\
&= \frac{\delta}{\sigma^4}\bigg[\underbrace{\Big|P_s \Tr\Big(\Big(\nabla P_{t-s}(\x) - \nabla P_\gamma^{\circ ([t]-[s]-1)}(\x)\Big) \cdot E^\top \X^\top \X E\Big)\Big|}_{(I)} + \underbrace{\Big|(P_s - P_\gamma^{\circ ([s]+1)})\Tr \Big(\nabla P_\gamma^{\circ ([t] - [s] - 1)}(\x) \cdot E^\top \X^\top \X E\Big)\Big|}_{(II)}\bigg].
\end{align*}
\noindent\textbf{Bound of $(I)$} Note that by Proposition \ref{prop:langevinsolution}-(c), $\Tr (\nabla P_{t-s}(\x) \cdot E^\top \X^\top \X E) = \langle \Tr (\V^{t-s} \cdot E^\top \X^\top \X E) \rangle_{\x} = \langle \Tr (\U^{t-s} \cdot \X^\top \X) \rangle_{\x} $, where $\{\x^t, \V^t\}_{t\in \R_+}$ follow the dynamic (\ref{eq:theta_V}) and we partition $\V^t = [\U^t, \ast; \W^t, \ast]$ with $\U^t \in \R^{d\times d}$. Similarly, Lemma \ref{lem:discrete_bismut} yields that $\Tr (\nabla P_\gamma^{\circ ([t]-[s]-1)}(\x)\cdot E^\top \X^\top \X E) = \langle \Tr(\tilde{\V}^{[t] - [s]-1} \cdot E^\top \X^\top \X E)\rangle_{\x} = \langle \Tr (\bar{\U}^{\floor{t} - \floor{s}-\gamma} \cdot \X^\top \X)\rangle_{\x}$, with $\{\tilde{\x}^t, \tilde{\V}^t\}_{t\in\Z_+}$ (resp. $\{\bar{\x}^t, \bar{\V}^t\}_{t\in\R_+}$) given by (\ref{eq:theta_V_discre}) (resp. (\ref{eq:theta_V_embed})), and we partition $\bar{\V}^t = [\bar{\U}^t, \ast; \bar{\W}^t, \ast]$. Hence
\begin{align*}
\Big|\Tr\Big(\Big(\nabla P_{t-s}(\x) - \nabla P_\gamma^{\circ ([t]-[s]-1)}(\x)\Big) \cdot E^\top \X^\top \X E\Big)\Big| &= \langle \Tr((\U^{t-s} - \bar{\U}^{\floor{t} - \floor{s} - \gamma}) \cdot \X^\top \X) \rangle_{\x}\\
&\leq \sqrt{d}\pnorm{\X}{\op}^2 \langle\pnorm{\U^{t-s} - \bar{\U}^{\floor{t} - \floor{s} - \gamma}}{F} \rangle_{\x}\\
&\leq \sqrt{\gamma d}\pnorm{\X}{\op}^2(\pnorm{\x}{} + \pnorm{\X^\top \y}{} + \sqrt{d}), 
\end{align*}
using the bounds that lead to (\ref{eq:V_frob_norm}). Similar to above, we arrive at $(I) \leq C\sqrt{\gamma d}(\pnorm{\x}{} + \pnorm{\X^\top \y}{} + \sqrt{d})$.

\noindent\textbf{Bound of $(II)$} Let $\mathsf{f}(\x) = \Tr \big(\nabla P_\gamma^{\circ ([t] - [s] - 1)}(\x) \cdot E^\top \X^\top \X E\big) = \Tr \big( \langle \bar{\U}^\tau \rangle_{\x} \cdot \X^\top \X\big)$, where $\tau = \floor{t} - \floor{s} - \gamma$. Then using the same arguments as above, it suffices to bound the Lipschitz constant of $\mathsf{f}$. Using the same notation and argument as in term $(I)$ above, we have
\begin{align*}
|\mathsf{f}(\mathsf{y}) - \mathsf{f}(\mathsf{y}')| \leq \Big|\langle \Tr ( (\bar{\U}_{\mathsf{y}}^\tau - \bar{\U}_{\mathsf{y}'}^\tau) \cdot \X^\top \X) \rangle\Big| \leq \sqrt{d}\pnorm{\X}{\op}^2 \langle \pnorm{\bar{\U}_{\mathsf{y}}^\tau - \bar{\U}_{\mathsf{y}'}^\tau}{F}\rangle \leq C\sqrt{d}\pnorm{\mathsf{y} - \mathsf{y}'}{},
\end{align*}
as desired.

\end{proof}

\begin{lemma}\label{lem:theta_V_rough}
Recall the dynamic $\{\x^t, \V^t\}$ in (\ref{eq:theta_V}) and $\{\bar{\x}^t, \bar{\V}^t\}$ in (\ref{eq:theta_V_embed}), and the block form $\V^t = [\U^t, \ast; \W^t,\ast]$ and $\bar{\V}^t = [\bar{\U}^t, \ast; \bar{\W}^t, \ast]$. For any given $T > 0$ and small enough $\gamma > 0$, there exists some $C > 0$ depending on $T, \pnorm{\X}{\op}$ and other problem parameters such that
\begin{align*}
\sup_{t\in[0,T]} \{\pnorm{\U^t}{\op} \vee \sqrt{d}\pnorm{\W^t}{\op} \vee \pnorm{\bar{\U}^t}{\op} \vee \sqrt{d}\pnorm{\bar{\W}^t}{\op}\} \leq C\gamma.
\end{align*}
\end{lemma}
\begin{proof}
Recall the discrete version $\tilde{\V}^t$ of $\bar{\V}^t$ given in (\ref{eq:theta_V_discre}). Let us write $\tilde{\V}^t = [\tilde{\U}^t, \ast; \tilde{\W}^t, \ast]$ in block form with $\tilde{\U}^t \in \R^{d\times d}$ and $\tilde{\W}^t \in \R^{K\times d}$. Similarly we partition $\nabla u(\tilde{\x}^t)$ as $[\tilde{J}_1^t, \tilde{J}_2^t; \tilde{J}_3^t, \tilde{J}_4^t]$ with $\tilde{J}_1^t\in\R^{d\times d}$ and $\tilde{J}^t_4 \in \R^{K\times K}$, so that 
\begin{align*}
\tilde{J}_1^t &= -\frac{1}{\sigma^2}\X^\top \X + \diag\Big[\Big(\partial_\theta^2 \log g(\theta^t_j;\hat{\alpha}^t)\Big)_{j=1}^d\Big], \quad \tilde{J}^t_2 = \Big(\partial_\theta\nabla_\alpha \log g(\theta^t_j;\hat{\alpha}^t)\Big)_{j=1}^d,\\
\tilde{J}_3^t &= \nabla_{\btheta} \cG(\hat{\alpha}^t, d^{-1}\sum_{j=1}^d \delta_{\theta^t_j}), \quad \tilde{J}^t_4 = \nabla_{\alpha} \cG(\hat{\alpha}^t, d^{-1}\sum_{j=1}^d \delta_{\theta^t_j}),
\end{align*}
and with initialization $\tilde{\U}^0 = I_d$ and $\tilde{W} = 0_{K\times d}$,
\begin{align*}
\tilde{\U}^{t+1} = (I + \gamma \tilde{J}^t_1)\tilde{\U}^t + \gamma \tilde{J}^t_2 \tilde{\W}^t, \quad \tilde{\W}^{t+1} = \gamma\tilde{J}^t_3 \tilde{\U}^t + (I+\gamma\tilde{J}^t_4)\tilde{\W}^t.
\end{align*}
By Assumptions \ref{assump:prior} and \ref{assump:gradient}, there exists some $C>0$ depending on $\pnorm{\X}{\op}, \sigma^2$ and the constants in the assumptions such that uniformly over $t\in\Z_+$, it holds that $\pnorm{\tilde{J}_1^t}{\op} \leq C, \pnorm{\tilde{J}^t_2}{F}\leq C\sqrt{d}, \pnorm{\tilde{J}^t_3}{F}\leq C/\sqrt{d}, \pnorm{\tilde{J}^t_4}{F} \leq C$, where the bound on $\tilde{J}^t_3$ follows since $\btheta \mapsto \cG(\alpha, d^{-1}\sum_{j=1}^d \delta_{\theta_j})$ is globally and uniform-in-$\alpha$ Lipschitz with constant $1/\sqrt{d}$ by Assumption \ref{assump:gradient}. We therefore have
\begin{align*}
\pnorm{\tilde{\U}^{t+1}}{\op} \leq (1+C\gamma)\pnorm{\tilde{\U}^t}{} + C\gamma \sqrt{d}\pnorm{\tilde{\W}^t}{F}, \quad \pnorm{\tilde{\W}^{t+1}}{F} \leq \frac{C\gamma}{\sqrt{d}} \pnorm{\tilde{\U}^t}{\op} + (1+C\gamma)\pnorm{\tilde{\W}^t}{F},
\end{align*}
which further implies that
\begin{align*}
\pnorm{\tilde{\U}^{t+1}}{\op} + \sqrt{d}\pnorm{\tilde{\W}^{t+1}}{\op} \leq (1+2C\gamma)\big(\pnorm{\tilde{\U}^{t}}{\op} + \sqrt{d}\pnorm{\tilde{\W}^{t}}{\op}\big).
\end{align*}
Hence for any $T \in \R_+$ assumed for simplicity to satisfy $T =N\gamma$ for some $N \in \Z_+$, we have $\pnorm{\tilde{\U}^{N}}{\op} + \sqrt{d}\pnorm{\tilde{\W}^{N}}{\op} \leq (1+2C\gamma)^{T/\gamma}(\pnorm{\tilde{\U}^{0}}{\op} + \sqrt{d}\pnorm{\tilde{\W}^{0}}{\op}) \leq C'$, as desired.  

The proof for the continuous case is similar. Write $\V^t = [\U^t, \ast; \W^t, \ast]$, $\nabla u(\x^t)$ as $[J_1^t, J_2^t; J_3^t, J_4^t]$ with $t\in \R_+$, so that
\begin{align*}
\U^t = \U^0 + \int_0^t (J^s_1 \U^s + J^s_2 \W^s)\d s, \quad \W^t = \W^0 + \int_0^t (J^s_3 \U^s + J^s_4 \W^s)\d s. 
\end{align*}
By the same bound of $J^t_1-J^t_4$ as above, we have by similar arguments that $\frac{\d}{\d t} (\pnorm{\U^t}{\op} + \sqrt{d}\pnorm{\W^t}{\op}) \leq C(\pnorm{\U^t}{\op} + \sqrt{d}\pnorm{\W^t}{\op})$, so the conclusion follows by Lemma \ref{lem:gronwall}. 
\end{proof}


%\begin{proof}
%Using a simple induction argument, it is easy to show that for any fixed $T$ and $t\leq T$, $\E_\x^\circ \pnorm{\bar{\btheta}^t}{}^2 \leq C(\pnorm{\x}{}^2 + \pnorm{\X^\top \y}{} + d)$, where $C > 0$ depends on $T, \sigma, \pnorm{\X}{\op}$. Since
%\begin{align*}
%\bar{\btheta}^t = \bar{\btheta}^{\floor{t}} + (t-\floor{t})\Big(-\frac{1}{\sigma^2}\X^\top(\X\bar{\btheta}^t - \y) - f'(\bar{\btheta}^{\floor{t}})\Big) + \sqrt{2}(\b^t - \b^{\floor{t}}),
%\end{align*}
%we have
%\begin{align*}
%\pnorm{\bar{\btheta}^t - \bar{\btheta}^{\floor{t}}}{} \leq \gamma \Big( L\pnorm{\bar{\btheta}^{\floor{t}}}{} + \frac{1}{\sigma^2}\pnorm{\X^\top \y}{}\Big) + \sqrt{2}\pnorm{\b^t - \b^{\floor{t}}}{},
%\end{align*}
%which further implies that
%\begin{align}\label{eq:theta_bar_discr}
%\E_\x^\circ \pnorm{\bar{\btheta}^t - \bar{\btheta}^{\floor{t}}}{}^2 \leq C\gamma\Big(\pnorm{\x}{}^2 + \pnorm{\X^\top \y}{}^2 + d\Big).
%\end{align}
%Using $\nabla^2 \log q(\btheta) \leq \pnorm{f''}{\infty}$ for any $\btheta$, we have
%\begin{align*}
%\pnorm{\btheta^t - \bar{\btheta}^t}{} \leq \int_0^t \pnorm{\nabla \log q(\btheta^s) - \nabla \log q(\bar{\btheta}^{\floor{s}})}{}\d s\leq C\int_0^t \pnorm{\btheta^s - \bar{\btheta}^s}{}\d s + C\int_0^t \pnorm{\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}}{}\d s,
%\end{align*}
%which by Gronwall's lemma further yields that, for any $t\leq T$, 
%\begin{align*}
%\pnorm{\btheta^t - \bar{\btheta}^t}{} \leq C\int_0^t \pnorm{\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}}{}\d s.
%\end{align*}
%Consequently, by (\ref{eq:theta_bar_discr}),
%\begin{align*}
%\E_\x^\circ \pnorm{\btheta^t - \bar{\btheta}^t}{}^2 \leq C\int_0^t \E_\x^\circ\pnorm{\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}}{}^2\d s \leq C\gamma\Big(\pnorm{\x}{}^2 + \pnorm{\X^\top \y}{}^2 + d\Big).
%\end{align*}
%On the $\V$ side, we note that
%\begin{align*}
%\pnorm{\V^t}{\op} \leq \int_0^t \pnorm{\nabla^2 \log q}{\op}\pnorm{\V^s}{\op}\d s \leq C\int_0^t \pnorm{\V^s}{\op}\d s, 
%\end{align*}
%so Gronwall's lemma yields that $\pnorm{\V^t}{\op} \leq C\pnorm{\V^0}{\op} = C$. A similar argument yields $\pnorm{\bar{\V}^t}{\op} \leq C$. We also have
%\begin{align*}
%\bar{\V}^t = \bar{\V}^{\floor{t}} + (t-\floor{t})\nabla^2 \log q(\bar{\btheta}^{\floor{t}})\bar{\V}^{\floor{t}},
%\end{align*}
%so using $\pnorm{\bar{\V}^t}{\op} \leq C$, 
%\begin{align*}
%\pnorm{\bar{\V}^t - \bar{\V}^{\floor{t}}}{F} \leq \gamma\sqrt{d} \pnorm{\nabla^2 \log q}{\op}\pnorm{\bar{\V}^{\floor{t}}}{\op} \leq C\gamma\sqrt{d}.
%\end{align*}
%\end{proof}

\begin{lemma}\label{lem:discrete_bismut}
For any fixed $\x, \v\in\R^{d+K}$, consider the following discrete dynamic
\begin{align*}
\x^{t+1} &= \x^{t} + \gamma u(\x^t) + \sqrt{2}\M(\b^{(t+1)\gamma} - \b^{t\gamma}), \quad \x^0 = \x\\
\v^{t+1} &= \v^t + \gamma [J\u](\x^t) \v^t, \quad \v^0 = \v, 
\end{align*}
where $u:\R^{d+K} \rightarrow \R^{d+K}$ is differentiable, $\M \in \R^{(d+K) \times d}$, $\{\b^t\}$ is a standard Brownian motion in $d$ dimensions, and $\gamma > 0$ is the step size. Let $P^\gamma$ denote the one-step transition semigroup of the above dynamic. Then for any differentiable $f:\R^{d+K}\rightarrow\R$, 
\begin{align*}
\v^\top \nabla [P_\gamma^{\circ k} f](\x) = \langle(\v^k)^\top\nabla f(\btheta^k)\rangle_{\x,\v}, 
\end{align*}
where $\langle \cdot \rangle_{\x,\v}$ denotes expectation over $\{\b^t\}$ under initializations $\x,\v$.
\end{lemma}
\begin{proof}
We prove by induction. The baseline case $k=0$ holds since both sides equal $\v^\top \nabla f(\x)$. Suppose the claim holds for some $k$. Since $\v^\top \nabla h(\x) = \deps h(\x + \eps \v)$, we have
\begin{align*}
\v^\top \nabla [P_\gamma^{\circ (k+1)} f](\x) =  \v^\top \nabla [P_\gamma^{\circ k}  (P_\gamma f)](\x) \overset{(*)}{=} \langle (\v^k)^\top \nabla (P_\gamma f)(\x^k)\rangle_{\x,\v},
\end{align*}
applying the induction hypothesis to $P_\gamma f$ (which is also differentiable) in $(*)$. Note that with $\mathbf{Z}\sim \N(0,\gamma)$, we have $(P_\gamma f)(\x) = \E[f(\x^{k+1})|\x^k = \x] = \E_{\mathbf{Z}} f(\x + \gamma u(\x) + \sqrt{2}\M \mathbf{Z})$, hence 
\begin{align*}
\nabla_\x (P_\gamma f)(\x) = (I + Ju(\x))^\top \E_{\langle ((I + Ju(\x^k)) \v^k)^\top  \nabla f(\x^{k+1})\rangle_{\x,\v}}  \nabla f(\x + \gamma u(\x) + \sqrt{2}\M \langle ((I + Ju(\x^k)) \v^k)^\top  \nabla f(\x^{k+1})\rangle_{\x,\v}),
\end{align*}
which implies that
\begin{align*}
\v^\top \nabla [P_\gamma^{\circ (k+1)} f](\x) &= \langle (\v^k)^\top (I + Ju(\x^k))^\top \E_{\mathbf{Z}}  \nabla f(\x^k + \gamma u(\x^k) + \sqrt{2}\M \mathbf{Z})\rangle_{\x,\v}\\
&= \langle (\v^k)^\top (I + Ju(\x^k))^\top \langle \nabla f(\x^{k+1})\rangle_{\x^k} \rangle_{\x,\v}\\
&= \langle ((I + Ju(\x^k)) \v^k)^\top  \nabla f(\x^{k+1})\rangle_{\x,\v} = \langle (\v^{k+1})^\top  \nabla f(\x^{k+1})\rangle_{\x,\v},
\end{align*}
as desired.
%
%
%the induction hypothesis yields that
%\begin{align*}
%\partial_{\eps}|_{\eps = 0} \E_{\x + \eps \v} f(\btheta^k) = \E^\circ_{\x}\Big[\iprod{\v^k}{\nabla f(\btheta^k)}\Big]
%\end{align*}
%for any fixed function $f$. For $k+1$, we have
%\begin{align*}
%f(\btheta^{k+1}) = f\Big(\btheta^k + \gamma \b(\btheta^k) + \sqrt{2\gamma}Z^{k+1}\Big) = \tilde{f}_{k+1}(\btheta^k),
%\end{align*}
%where $Z^{k+1} = (B^{(k+1)\gamma} - B^{k\gamma})/\sqrt{\gamma} \sim \N(0,1)$ and is independent of $\{\btheta^\ell, \v^\ell\}_{\ell\leq k}$, and
%\begin{align*}
%\tilde{f}_{k+1}(\btheta) = f\Big(\btheta + \gamma \b(\btheta) + \sqrt{2\gamma}Z^{k+1}\Big)
%\end{align*}
%is a random function. So using the hypothesis, we have
%\begin{align*}
%\partial_{\eps}|_{\eps = 0} \E_{\x + \eps \v} f(\btheta^{k+1}) &= \partial_{\eps}|_{\eps = 0} \E_{\x + \eps \v} \tilde{f}_{k+1}(\btheta^{k})\\
%&= \E_{Z^{k+1}}\Big[\partial_\eps|_{\eps = 0}\E_{\x+\eps\v}\Big[\tilde{f}_{k+1}(\btheta^{k})|Z^{k+1}\Big]\Big]\\
%&= \E_{Z^{k+1}} \E_{\x}\Big[\iprod{\v^k}{\nabla \tilde{f}_{k+1}(\btheta^k)}|Z^{k+1}\Big]\\
%&= \E_{Z^{k+1}} \E_{\x}\Big[\iprod{\v^k}{(I + \gamma [J\b](\btheta^k))^\top \nabla f(\btheta^{k+1})}|Z^{k+1}\Big]\\
%&= \E_{\x}\Big[\iprod{\v^{k+1}}{\nabla f(\btheta^{k+1})}\Big],
%\end{align*}
%as desired.
%We have
%\begin{align*}
%\v^\top \nabla [P_\gamma^{\circ {k+1}} f](\x) &= \partial_\eps|_{\eps = 0} [P_\gamma^{\circ {k+1}} f](\x + \eps \v)\\
%&= \partial_\eps|_{\eps = 0} \E_{\x+\eps\v}[f(\btheta^{k+1})]\\
%&= \partial_\eps|_{\eps = 0} \E_{\x+\eps\v}[f(\btheta^k + \gamma b(\btheta^t) + \sqrt{2}(B^{(t+1)\gamma} - B^{t\gamma}))]\\
%&= \partial_\eps|_{\eps = 0} \E_{\x+\eps\v}[\iprod{}{}
%\end{align*}
\end{proof}

\subsection{Step 2: Convergence of discrete Langevin response function to DMFT response function}

We first introduce some notation. For any random process $\{\rho^t\}_{t\in \Z_+}, \{\mu^t\}_{t\in\Z_+} \subset \R$, define the following system of $\{r_\theta^{(\rho,\mu)}, r_\eta\}$:
\begin{align}\label{eq:dmft_response_rho}
\notag r_\theta^{(\rho,\mu)}(t+1,s) &= \Big(1 - \frac{\gamma\delta}{\sigma^2} + \gamma \partial_\theta^2 \log g(\rho^t;\mu^t)\Big) r_\theta^{(\rho,\mu)}(t,s) + \gamma \sum_{\ell=s+1}^{t-1} \bar{R}_\eta^{\gamma}(t,\ell) r_\theta^{(\rho,\mu)}(\ell,s), \quad r_\theta^{(\rho,\mu)}(t+1,t) = \gamma,\\
r_\eta(t,s) &= \frac{1}{\sigma^2}\Big[-\sum_{\ell=s+1}^{t-1} \bar{R}^{\gamma}_\theta(t,\ell) r_\eta(\ell,s) + \bar{R}^{\gamma}_\theta(t,s)\Big],
%R_\theta^{(\rho)}(t,s) &= \E\Big[r_\theta^{(\rho)}(t,s)\Big],\quad R_\eta^{(\rho)}(t,s) = \frac{\delta}{\sigma^2}\E\Big[r_\eta^{(\rho)}(t,s)\Big].
\end{align}
where $\bar{R}_\theta^{\gamma}$ and $ \bar{R}_\eta^{\gamma}$ are the discrete response functions defined in (\ref{eq:dmft_response}). Let $\theta = \{\theta^t\}_{t\in\Z_+}$ and $\alpha= \{\alpha^t\}_{t\in\Z_+}$ be two integer-indexed processes, where $\theta^t = \bar{\theta}^{t\gamma}_\gamma$ and $\alpha^t = \bar{\alpha}^{t\gamma}_\gamma $ are given in (\ref{eq:dmft_theta_discrete1}) and (\ref{eq:dmft_alpha_discrete1}). Then by definition, 
\begin{align*}
r_\theta^{(\theta, \alpha)}(i+1,j) &\stackrel{d}{=} \overline{\frac{\partial \theta_\gamma^{t_{i+1}}}{\partial u^{t_j}_\gamma}}, \quad \bar{R}_\theta^{\gamma}(i+1,j) = \E\Big[r_\theta^{(\theta,\alpha)}(i+1,j)\Big],\\
 \quad r_\eta(i,j) &= \overline{\frac{\partial \eta_\gamma^{t_i}}{\partial w^{t_j}_\gamma}}, \quad \bar{R}_\eta^{\gamma}(i,j) = \frac{\delta}{\sigma^2} \cdot r_\eta(i,j),
 \end{align*}
 where $\{\overline{\frac{\partial \theta_\gamma^{t_{i}}}{\partial u^{t_j}_\gamma}}\}$ and $\{\overline{\frac{\partial \eta_\gamma^{t_i}}{\partial w^{t_j}_\gamma}}\}$ are given by (\ref{eq:response_1})-(\ref{eq:response_3}).

Recall the processes $\{\btheta^{t,(s,j),\eps}\}$ and $\{\btheta^{t,[s,i],\eps}\}$ defined in (\ref{eq:theta_col_perturb}) and (\ref{eq:theta_row_perturb}). The following is the main result of this section.

\begin{proposition}\label{prop:discrete_time_response}
Assume the conditions of Theorem \ref{thm:dmftresponse}. For any fixed $t > s$, it holds that %\ys{we might need to strengthen this to a.s. convergence}
 \begin{align*}
\Big\langle\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps} \Big\rangle\rightarrow_{a.s.} \bar{R}_\theta^{\gamma}(t,s), \quad  \Big\langle\frac{1}{n}\sum_{i=1}^n \partial_\eps|_{\eps = 0} \bbeta_i^{t,[s,i], \eps} \Big\rangle\rightarrow_{a.s.} \frac{\sigma^4}{\delta}\bar{R}_\eta^{\gamma}(t,s).
 \end{align*}
 \end{proposition}
\begin{proof}
By Lemma \ref{lem:perturb_key_expansion}, it holds that
\begin{align*}
\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps} = \frac{1}{d}\sum_{j=1}^d r_\theta^{(\theta_j, \hat{\alpha})}(t,s) + \frac{1}{d}\sum_{j=1}^d E_\theta^{t,(s,j)}. 
\end{align*}
where $\langle d^{-1}\sum_{j=1}^d E_\theta^{t,(s,j)} \rangle = o_{a.s.}(1)$. On the other hand, since the DMFT characterization yields that for any fixed $m\in\Z_+$, almost surely as $n,d\rightarrow\infty$
\begin{align*}
\frac{1}{d}\sum_{j=1}^d \delta_{\big((\btheta^1_j), \ldots, (\btheta^m_j)\big)} \overset{W_2}{\to} \sP(\theta^1,\ldots, \theta^m), \quad \pnorm{(\hat{\alpha}^1,\ldots,\hat{\alpha}^m) - (\alpha^1,\ldots, \alpha^m)}{} \rightarrow 0, 
\end{align*}
we conclude by Lemma \ref{lem:dmft_emp_concentrate} that
\begin{align*}
\frac{1}{d}\sum_{j=1}^d r_\theta^{(\theta_j,\hat{\alpha})}(t,s) \rightarrow_{a.s.} \E\Big[r_\theta^{(\theta, \alpha)}(t,s)\Big] = \bar{R}_\theta^{\gamma}(t,s),
\end{align*}
yielding the first claim. Similarly, 
\begin{align*}
\frac{1}{n}\sum_{i=1}^n \partial_\eps|_{\eps = 0} \bbeta_i^{t,[s,i], \eps} = \sigma^2  r_\eta(t,s) + \frac{1}{n}\sum_{i=1}^n E_\eta^{t,[s,i]} = \frac{\sigma^4}{\delta}  \bar{R}_\eta^{\gamma}(t,s) + \frac{1}{n}\sum_{i=1}^n E_\eta^{t,[s,i]}, %= (-\sigma^2) \frac{1}{d}\sum_{j=1}^d r_\eta^{(\btheta_j)}(t,s) + \frac{1}{n}\sum_{i=n}^d E_\eta^{t,[s,i]}
\end{align*}
where $\langle n^{-1}\sum_{i=1}^n E_\eta^{t,[s,i]} \rangle = o_{a.s.}(1)$, yielding the second claim.
%\begin{align*}
%\frac{1}{d}\sum_{j=1}^d r_\eta^{(\btheta_j)}(t,s) \rightarrow \E_{\rho \sim \theta_{\dmft}}\Big[r_\theta^{(\rho)}(t,s)\Big] = \frac{\sigma^2}{\delta}R^{\dmft}_\eta(t,s),
%\end{align*}
\end{proof} 


\begin{lemma}\label{lem:dmft_emp_concentrate}
Suppose that $\{\brho^t\}_{t\in \Z_+}$ is a random process in $\R^n$ such that, for some univariate random process $\rho = \{\rho^t\}_{t\in \Z_+}$ and any fixed $m\in\Z_+$, almost surely as $n,d\rightarrow\infty$, 
\begin{align*}
\frac{1}{n}\sum_{i=1}^n \delta_{\big((\brho^0)_i, \ldots, (\brho^m)_i\big)} \overset{W_2}{\to} \sP(\rho^0,\ldots, \rho^m). 
\end{align*}
Suppose that $\{\mu^t\}_{t\in \Z_+}$ (resp. $\{\bar{\mu}^t\}_{t\in \Z_+}$) is a univariate random (resp. deterministic) processes in $\R$ such that for any fixed $m\in \Z_+$, almost surely as $n,d\rightarrow\infty$, 
\begin{align*}
\pnorm{(\mu^0,\ldots,\mu^{m}) - (\bar{\mu}^0,\ldots,\bar{\mu}^{m})}{} \rightarrow 0.
\end{align*}
Then for any $t\geq s\geq 0$, with $\{\rho^t_i\}_{t\in\Z_+}$ denoting the $i$th component of $\{\brho^t_i\}_{t\in\Z_+}$,
\begin{align*}
\frac{1}{n}\sum_{i=1}^n r_{\theta}^{(\rho_i, \mu)}(t,s) \rightarrow_{a.s.} \E\big[r_\theta^{(\rho,\bar{\mu})}(t,s)\big],%, \quad \frac{1}{n}\sum_{i=1}^n r_\eta^{(\brho_i)}(t,s) \rightarrow_P \E_{\theta = (\theta^t) \sim \rho}\Big[r_\eta^{(\rho)}(t,s)\Big]. 
\end{align*}
where the expectation on the right side is taken over the random process $\{\rho^t\}_{t\in \Z_+}$.
\end{lemma}
\begin{proof}
First note that by Assumption \ref{assump:prior} and a simple induction argument it is easy to show that $\frac{1}{n}\sum_{i=1}^n r_{\theta}^{(\rho_i, \mu)}(t,s) - \frac{1}{n}\sum_{i=1}^n r_{\theta}^{(\rho_i, \bar{\mu})}(t,s)\rightarrow_{a.s.} 0$. Next we note that $r_\theta^{(\rho,\bar{\mu})}(t+1,s)$ is a function of $(\rho^1,\ldots, \rho^t)$. % and $r_\eta^{(\rho)}(t,s)$ is a function of $(\rho^1,\ldots, \rho^{t-1})$. 
So there exists some $F:\R^t \rightarrow\R$ such that
\begin{align*}
\frac{1}{n}\sum_{i=1}^n r_{\theta}^{(\rho_i, \bar{\mu})}(t+1,s) = \frac{1}{n}\sum_{i=1}^n F\big((\brho^1)_i, \ldots, (\brho^t)_i\big),%, \quad \frac{1}{n}\sum_{i=1}^n r_{\eta}^{(\brho_i)}(t,s) = \frac{1}{n}\sum_{i=1}^n G\Big((\brho^1)_i, \ldots, (\brho^{t-1})_i\Big), 
\end{align*}
and the conclusions will follow if $F$ is bounded and Lipschitz. By the bound of $\partial_\theta^2 \log g(\theta;\alpha)$ in Assumption \ref{assump:prior}, for any $0 \leq s\leq t\leq T$, clearly there exists some $C = C(T,\gamma,\delta, M)$ such that $|r_\theta^{(\rho_i, \bar{\mu})}(t,s)| \vee |R_\theta^\gamma(t,s)| \leq C$, which further implies that $F$ is bounded. Similarly, by the bound of $\partial_\theta^3 \log g(\theta;\alpha)$ in Assumption \ref{assump:prior}, it is easy to see that $\Big|\frac{\partial }{\partial a^\ell} F(a^1,\ldots, a^t)\Big| \leq C'$, so $F$ is also Lipschitz, completing the proof.
\end{proof}

As shown above, the main ingredient of Proposition \ref{prop:discrete_time_response} is the following lemma. Recall that
%We recall the discrete Langevin dynamic (\ref{eq:langevin_discrete_1}), simplified in notation as
%\begin{align}\label{eq:original}
%\btheta^{t+1} = \btheta^{t} - \gamma\Big[\frac{1}{\sigma^2}\X^\top(\X\btheta^{t} - \y) + f'(\btheta^{t})\Big] + \sqrt{2}(\B^{(t+1)\gamma} - \B^{t\gamma}).
%\end{align}
for each $j\in[d]$, we write $\theta_j = \{\theta^t_j\}_{t\in\Z_+} \subset\R$ as the $j$th coordinate of $\{\btheta^t\}_{t\in\Z_+}$ defined in (\ref{eq:original_theta}), and $\{\hat{\alpha}^t\}_{t\in\Z_+}$ is given in (\ref{eq:original_alpha}).


\begin{lemma}\label{lem:perturb_key_expansion}
Assume the conditions of Theorem \ref{thm:dmftresponse}. For each $t > s$, 
\begin{align}
\partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps} &= r_\theta^{(\theta_j,\hat{\alpha})}(t,s) + E_\theta^{t,(s,j)}, \quad j\in[d], \label{eq:induce_theta}\\
\partial_\eps|_{\eps = 0} \bbeta_i^{t,[s,i], \eps} &= \sigma^2 \cdot r_\eta(t,s) + E_\eta^{t,[s,i]}, \quad i\in[n] \label{eq:induce_eta},
\end{align}
%where we recall $\mu^t$ is the last component of $\btheta^t$, and $\theta = (\theta^t)$ is the main iterate in the DMFT equations. 
where the remainder terms satisfy
\begin{align}
\Big\langle\frac{1}{d} \sum_{j=1}^d E_\theta^{t,(s,j)} \Big\rangle \vee \Big\langle \frac{1}{n} \sum_{i=1}^n E_\eta^{t,[s,i]} \Big\rangle \rightarrow_{a.s.} 0 \text{ as } n,d\rightarrow\infty.
\end{align} 
\end{lemma}
%\begin{remark}
%It is easy to see that the sequence $\{r_\eta^{(\rho)}(t,s)\}$ in (\ref{eq:dmft_response_rho}) is deterministic and hence only depends on the law of $\rho = (\rho^t)$. By symmetry, all components of $\btheta^t$ have the same law, hence the expansion (\ref{eq:induce_eta}) holds for any $j\in[d]$ in its definition.
%\end{remark}

For the proof of Lemma \ref{lem:perturb_key_expansion}, it will be helpful to consider the following two leave-one-out versions of (\ref{eq:original_theta})-(\ref{eq:original_alpha}):
%, simplified in notation as
%\begin{align}\label{eq:original}
%\btheta^{t+1} = \btheta^{t} - \gamma\Big[\frac{1}{\sigma^2}\X^\top(\X\btheta^{t} - \y) + f'(\btheta^{t})\Big] + \sqrt{2}(\B^{(t+1)\gamma} - \B^{t\gamma}).
%\end{align}
For any $j\in[d]$, let $\X_{(j)} \in \R^{n\times d}$ denote $\X$ but with its $j$th column set to $0_n$, and define
\begin{align}\label{eq:leave_col_out}
\notag\btheta^{t+1}_{(j)} &= \btheta^{t}_{(j)} - \gamma\Big[\frac{1}{\sigma^2}\X_{(j)}^\top(\X_{(j)}\btheta^{t}_{(j)} - \y_{(j)}) - \partial_\theta \log g(\btheta^{t}_{(j)}; \hat{\alpha}^{t}_{(j)})\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma})\in \R^{d},\\
\hat{\alpha}^{t+1}_{(j)} &= \hat{\alpha}^{t}_{(j)} + \gamma \cG\Big(\hat{\alpha}^t_{(j)}, \Prob_n(\btheta^{t}_{(j)})\Big),
\end{align}
with initialization $(\btheta^{0}_{(j)}, \hat{\alpha}^0_{(j)}) = (\btheta^0, \hat{\alpha}^0)$ and $\y_{(j)} = \X_{(j)}\btheta^\ast + \beps$. Similarly, let $\X_{[i]} \in \R^{n\times d}$ denote $\X$ but with its $i$th row set to $0_d$, and define
\begin{align}\label{eq:leave_row_out}
\notag\btheta^{t+1}_{[i]} &= \btheta^{t}_{[i]} - \gamma\Big[\frac{1}{\sigma^2}\X_{[i]}^\top(\X_{[i]}\btheta^{t}_{[i]} - \y_{[i]}) - \partial_\theta \log g(\btheta^{t}_{[i]};\hat{\alpha}^t_{[i]})\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}) \in \R^{d},\\
 \hat{\alpha}^{t+1}_{[i]} &= \hat{\alpha}^{t}_{[i]} + \gamma \cG\Big(\hat{\alpha}^t_{[i]}, \Prob_n(\btheta^{t}_{[i]})\Big)
\end{align}
with initialization $(\btheta^{0}_{[i]}, \hat{\alpha}^{0}_{[i]}) = (\btheta^0, \hat{\alpha}^0)$ and $\y_{[i]} = \X_{[i]}\btheta^\ast + \beps$. The following lemma gives $\ell_2$ estimates on the difference between (\ref{eq:leave_col_out}), (\ref{eq:leave_row_out}) and the original dynamic (\ref{eq:original_theta})-(\ref{eq:original_alpha}).

\begin{lemma}\label{lem:loo_error}
Suppose that Assumptions \ref{assump:prior} and \ref{assump:gradient} hold. Fix any small enough $\gamma > 0$. For any $T_0 = \ceil{K/\gamma}$, there exists some $C > 0$ depending on $K$ and other problem parameters but not on $\gamma$ such that, almost surely as $n,d\rightarrow\infty$, it holds for any $0\leq t\leq T_0$ that 
\begin{align}
\pnorm{\btheta^{t}}{}/\sqrt{d} \vee \max_{j\in[d]} (\pnorm{\btheta^{t}_{(j)}}{}/\sqrt{d} + \pnorm{\hat{\alpha}_{(j)}}{}) \vee \max_{i\in[n]} (\pnorm{\btheta^{t}_{[i]}}{}/\sqrt{d} + \pnorm{\hat{\alpha}_{[i]}}{}) &\leq C, \label{eq:rough_l2}\\
\langle \pnorm{\btheta^{t}_{(j)} - \btheta^t}{}^2 + d\cdot\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(j)}}{}^2 \rangle \leq C(|\theta^0_j|^2 + |\theta^\ast_j|^2 + \log d), \quad \forall j\in[d],\label{eq:rough_loo_l2_col}\\
\pnorm{\btheta^{t}_{[i]} - \btheta^t}{}^2 + d\cdot\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{[i]}}{}^2 \leq C(|\eps_i|^2 + \log d), \quad \forall i \in[n]\label{eq:rough_loo_l2_row}.
\end{align}
Moreover, it holds that
\begin{align*}
&\max_{j\in[d]}\E\pnorm{\btheta^{t}_{(j)} - \btheta^t}{}^2 \vee d\cdot\max_{j\in[d]} \E\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(j)}}{}^2 \leq C, \\
&\max_{i\in[n]}\E\pnorm{\btheta^{t}_{[i]} - \btheta^t}{}^2 \vee d\cdot \max_{i\in[n]} \E\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{[i]}}{}^2 \leq C.
\end{align*}
\end{lemma}
\begin{proof}
The bound (\ref{eq:rough_l2}) follows from similar arguments as in Lemma \ref{lem:alpha_boundedness}, so we only prove (\ref{eq:rough_loo_l2_col})-(\ref{eq:rough_loo_l2_row}). The constant $C$ below does not depend on $\gamma$ but its value changes from one instance to another. 

\noindent \textbf{Bound of $\langle \pnorm{\btheta^{t}_{(j)} - \btheta^t}{}^2\rangle $} By definition, 
\begin{align*}
\btheta^t - \btheta^t_{(j)} &= \Big(I - \frac{\gamma}{\sigma^2} \X^\top \X\Big)\btheta^{t-1} - \Big(I - \frac{\gamma}{\sigma^2} \X_{(j)}^\top \X_{(j)}\Big)\btheta^{t-1}_{(j)} + \frac{\gamma}{\sigma^2}\Big(\X^\top\y - \X_{(j)}^\top \y_{(j)}\Big)\\
&\quad + \gamma \Big(\partial_\theta \log g(\btheta^{t-1};\hat{\alpha}^{t-1}) - \partial_\theta \log g(\btheta^{t-1}_{(j)};\hat\alpha^{t-1}_{(j)})\Big), 
\end{align*}
which implies that, 
\begin{align}\label{eq:leave_col_out_bound}
\notag\pnorm{\btheta^t - \btheta^t_{(j)}}{} &\leq \frac{\gamma}{\sigma^2}\pnorm{(\X_{(j)}^\top \X_{(j)} - \X^\top \X)\btheta^{t-1}_{(j)}}{} + \pnorm{(I - \frac{\gamma}{\sigma^2} \X^\top \X)(\btheta^{t-1} - \btheta^{t-1}_{(j)})}{} + \frac{\gamma}{\sigma^2}\pnorm{\X^\top\y - \X_{(j)}^\top \y_{(j)}}{}\\
\notag&\quad + \gamma\pnorm{\partial_\theta \log g(\btheta^{t-1};\hat\alpha^{t-1}) - \partial_\theta \log g(\btheta^{t-1}_{(j)};\hat\alpha^{t-1}_{(j)})}{}\\
&\leq (1+C\gamma)\pnorm{\btheta^{t-1} - \btheta^{t-1}_{(j)}}{} + C\gamma \pnorm{\hat\alpha^t - \hat\alpha^t_{(j)}}{} + \underbrace{C\gamma\big(\pnorm{(\X_{(j)}^\top \X_{(j)} - \X^\top \X)\btheta^{t-1}_{(j)}}{} +\pnorm{\X^\top\y - \X_{(j)}^\top \y_{(j)}}{}\big)}_{\rho_{t-1}}.
\end{align}
Similarly, by Assumption \ref{assump:gradient}, we have
\begin{align*}
\pnorm{\hat\alpha^t - \hat\alpha^t_{(j)}}{} \leq (1+C\gamma)\pnorm{\hat\alpha^{t-1} - \hat\alpha^{t-1}_{(j)}}{} + C\gamma\pnorm{\btheta^{t-1} - \btheta^{t-1}_{(j)}}{}/\sqrt{d}. 
\end{align*}
Combining the above two inequalities yields
\begin{align*}
\pnorm{\btheta^t - \btheta^t_{(j)}}{} + \sqrt{d}\pnorm{\hat\alpha^t - \hat\alpha^t_{(j)}}{} \leq (1+C\gamma)\big(\pnorm{\btheta^{t-1} - \btheta^{t-1}_{(j)}}{} + \sqrt{d}\pnorm{\hat\alpha^{t-1} - \hat\alpha^{t-1}_{(j)}}{}\big) + \rho_{t-1}. 
\end{align*}
Let $\Gamma = 1+C\gamma$. For $t\leq T_0$, iterating the above bound yields
\begin{align*}
\pnorm{\btheta^t - \btheta^t_{(j)}}{} + \sqrt{d}\pnorm{\hat\alpha^t - \hat\alpha^t_{(j)}}{} &\leq \Gamma^t (\pnorm{\btheta^0 - \btheta^0_{(j)}}{} + \sqrt{d}\pnorm{\hat\alpha^0 - \hat\alpha^0_{(j)}}{}) + \sum_{\ell=0}^{t-1} \Gamma^\ell \rho_{t-1-\ell} = \sum_{\ell=0}^{t-1} \Gamma^\ell \rho_{t-1-\ell},
\end{align*}
which further implies that
\begin{align*}
\langle \pnorm{\btheta^t - \btheta^t_{(j)}}{}^2 + d\pnorm{\hat\alpha^t - \hat\alpha^t_{(j)}}{}^2\rangle &\leq \langle \Big(\sum_{\ell=0}^{t-1} \Gamma^\ell \rho_{t-1-\ell}\Big)^2 \rangle \leq \sum_{\ell=0}^{t-1} \Gamma^{2\ell} \cdot \sum_{\ell=0}^{t-1} \langle \rho_{t-1-\ell}^2\rangle \leq \frac{C}{\gamma^2}\max_{0\leq \ell\leq t-1} \langle\rho_\ell^2\rangle.
\end{align*}
Let us now bound $\langle \rho_\ell^2 \rangle$.  With $\X = [\x_1,\ldots, \x_d]$, we have $\X_{(j)} = \X - \x_j \e_j^\top$ and $\X^\top \X - \X_{(j)}^\top \X_{(j)} = \X^\top \x_j \e_j^\top + \e_j \x_j^\top \X - \e_j\e_j^\top \pnorm{\x_j}{}^2$, so
\begin{align}\label{ineq:loo_1}
\notag\pnorm{(\X_{(j)}^\top \X_{(j)} - \X^\top \X)\btheta^{t-1}_{(j)}}{} &\leq \pnorm{\X^\top \x_j}{}|(\btheta^{t-1}_{(j)})_j| + |\x_j^\top \X \btheta^{t-1}_{(j)}| + \pnorm{\x_j}{}^2 |(\btheta^{t-1}_{(j)})_j|\\
&\leq C\pnorm{\X}{\op}\pnorm{\x_j}{}|(\btheta^{t-1}_{(j)})_j| + |\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)}|.
\end{align}
By Lemma \ref{lem:theta_loo_constant}, we have almost surely that $\langle |(\btheta^t_{(j)})_j| \rangle \leq C(|\theta^0_j| + 1)$ for $t\leq T_0$. Similarly, we have
\begin{align*}
\X^\top\y - \X_{(j)}^\top \y_{(j)} &= (\X^\top \X - \X_{(j)}^\top \X_{(j)})\btheta^\ast + (\X - \X_{(j)})^\top \beps\\
&= \X^\top \x_j (\btheta^\ast)_j + \e_j \x_j^\top \X\btheta^\ast - \e_j (\btheta^\ast)_j \pnorm{\x_j}{}^2 + \e_j \x_j^\top \beps,
\end{align*}
so
\begin{align}\label{ineq:loo_2}
\pnorm{\X^\top\y - \X_{(j)}^\top \y_{(j)}}{} \leq C\pnorm{\X}{\op}\pnorm{\x_j}{}|(\btheta^\ast)_j| + |\x_j^\top \X_{(j)}\btheta^\ast| + |\x_j^\top \beps|. 
\end{align}
Collecting the above two bounds yields
\begin{align*}
\langle \rho_\ell^2 \rangle \leq C\gamma^2\Big[\pnorm{\X}{\op}^2\pnorm{\x_j}{}^2(|\theta^0_j|^2 + |\theta^\ast_j|^2 + 1 ) + |\x_j^\top \X_{(j)}\btheta^\ast|^2 + \langle |\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)}|^2 \rangle + |\x_j^\top \beps|^2\Big].
\end{align*}
Since $\pnorm{\X}{\op} \leq C$ almost surely, it remains to show that $|\x_j^\top \X_{(j)}\btheta^\ast|^4 \vee |\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)}|^2  \vee |\x_j^\top \beps|^2 \leq C$ almost surely as $n,d\rightarrow\infty$. We only prove the second one, and the other two follow similarly. 
%We first note the following $\ell_2$ bound on $\btheta^t$: 
%\begin{align*}
%\pnorm{\btheta^t}{} \leq (1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + \gamma\pnorm{f''}{\infty})\pnorm{\btheta^{t-1}}{} + \frac{\gamma}{\sigma^2}\pnorm{\X^\top \y}{} + \gamma\pnorm{f'(\mathbf{0}_d)}{},
%\end{align*}
%yielding that
%\begin{align*}
%\pnorm{\btheta^t}{} \leq C(1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + \gamma\pnorm{f''}{\infty})^t\Big(\pnorm{\btheta^0}{} + \pnorm{\X^\top \y}{} + \pnorm{f'(\mathbf{0}_d)}{}\Big).
%\end{align*}
%A similar bound holds for $\pnorm{\btheta^t_{(j)}}{}$. 
By independence between $\x_j$ and $\X_{(j)},  \btheta^{t-1}_{(j)}$, we have $\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)}| \X_{(j)},\btheta^{t-1}_{(j)} \stackrel{d}{=} \N(0, \frac{1}{d}\pnorm{\X_{(j)}\btheta^{t-1}_{(j)}}{}^2)$, and the almost sure bound $\max_{j\in[d]} |\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)}|^2 \leq C\log d$ follows from (\ref{eq:rough_l2}) and a standard maximal inequality for Gaussian variables. This concludes that $\langle \rho_\ell^2\rangle \leq C\gamma^2(|\theta^0_j|^2 + |\theta^\ast_j|^2 + \log d )$ almost surely, which implies the desired bound for $\langle \pnorm{\btheta^t - \btheta^t_{(j)}}{}^2 +  d\pnorm{\hat\alpha^t - \hat\alpha^t_{(j)}}{}^2\rangle$.
%
%so $\E (\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)})^4 \leq C\E (\frac{1}{d}\pnorm{\X_{(j)}\btheta^{t-1}_{(j)}}{}^2)^2$, where
%\begin{align*}
%\frac{1}{d}\pnorm{\X_{(j)}\btheta^{t-1}_{(j)}}{}^2 \leq C\pnorm{\X}{\op}^2(1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + \gamma\pnorm{f''}{\infty})^{2t} \cdot \frac{1}{d}\Big(\pnorm{\btheta^0}{}^2 + \pnorm{\X^\top \y}{}^2 + \pnorm{f'(\mathbf{0}_d)}{}^2\Big).
%\end{align*}
%Under the condition $\E ((\btheta^0)_j)^8 \vee \E[\beps_i^8] \leq C$, we readily have $\E (\frac{1}{d}\pnorm{\X_{(j)}\btheta^{t-1}_{(j)}}{}^2)^2 \leq C$, concluding the bound for $\E\pnorm{\btheta^t - \btheta^t_{(j)}}{}^2$.
 
\noindent \textbf{Bound on $\pnorm{\btheta^{t}_{[i]} - \btheta^t}{}^2 $} Similar to above, we have
\begin{align*}
\pnorm{\btheta^t - \btheta^t_{[i]}}{} &\leq (1+C\gamma)\pnorm{\btheta^{t-1} - \btheta^{t-1}_{[i]}}{} + C\gamma\pnorm{\hat\alpha^t - \hat\alpha^t_{[i]}}{} + \underbrace{C\gamma\big(\pnorm{(\X_{[i]}^\top \X_{[i]} - \X^\top \X)\btheta^{t-1}_{[i]}}{} +\pnorm{\X^\top\y - \X_{[i]}^\top \y_{[i]}}{}\big)}_{\lambda_{t-1}},\\
\pnorm{\hat\alpha^t - \hat\alpha^t_{[i]}}{} &\leq \pnorm{\hat\alpha^{t-1} - \hat\alpha^{t-1}_{[i]}}{} + C\gamma\big(\pnorm{\hat\alpha^{t-1} - \hat\alpha^{t-1}_{[i]}}{} + \pnorm{\btheta^{t-1} - \btheta^{t-1}_{[i]}}{}/\sqrt{d}\big).
\end{align*}
which implies
\begin{align*}
\pnorm{\btheta^t - \btheta^t_{[i]}}{}^2 + d\pnorm{\hat\alpha^t - \hat\alpha^t_{[i]}}{}^2  \leq \frac{C}{\gamma^2}\max_{0\leq \ell\leq t-1}\lambda^2_\ell.
\end{align*}
Using $\X = \X_{[i]} + \e_i \bar{\x}_i^\top$, where $\bar{\x}_i\in\R^p$ denote the (transpose of) $i$th row of $\X$, we have $\X^\top \X = \X_{[i]}^\top \X_{[i]} + \bar{\x}_i\bar{\x}_i^\top$ and $\X^\top\y - \X_{[i]}^\top \y_{[i]} = \bar{\x}_i(\bar{\x}_i^\top \btheta^\ast + \beps_i)$, so
\begin{align*}
\pnorm{(\X^\top \X^\top - \X_{[i]}^\top \X_{[i]})\btheta^{t-1}_{[i]}}{} = \pnorm{\bar{\x}_i}{}|\bar{\x}_i^\top \btheta^{t-1}_{[i]}|. 
\end{align*}
Using independence between $\bar{\x}_i$ and $\btheta^{t-1}_{[i]}$, we have $\bar{\x}_i^\top \btheta^{t-1}_{[i]} | \btheta^{t-1}_{[i]} \sim \N(0, \frac{1}{d}\pnorm{\btheta^{t-1}_{[i]}}{}^2)$, which along with the bound (\ref{eq:rough_l2}) yields $\max_{i\in[n]} |\bar{\x}_i^\top \btheta^{t-1}_{[i]}| \leq C\sqrt{\log d}$ almost surely as $n,d\rightarrow\infty$. A similar argument also yields that almost surely as $n,d\rightarrow\infty$, $ \pnorm{\X^\top\y - \X_{[i]}^\top \y_{[i]}}{} \leq C(|\eps_i| + \sqrt{\log d})$ uniformly over $i\in[n]$, so the proof is complete.
%To bound $|\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)}|$, we first note the following $\ell_2$ bound on $\btheta^t$: 
%\begin{align*}
%\pnorm{\btheta^t}{} \leq (1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + \gamma\pnorm{f''}{\infty})\pnorm{\btheta^{t-1}}{} + \frac{\gamma}{\sigma^2}\pnorm{\X^\top \y}{} + \gamma\pnorm{f'(\mathbf{0}_d)}{},
%\end{align*}
%yielding that
%\begin{align*}
%\pnorm{\btheta^t}{} \leq C(1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + \gamma\pnorm{f''}{\infty})^t\Big(\pnorm{\btheta^0}{} + \pnorm{\X^\top \y}{} + \pnorm{f'(\mathbf{0}_d)}{}\Big).
%\end{align*}
%A similar bound holds for $\pnorm{\btheta^t_{(j)}}{}$. Now using independence of $\x_j$ and $\X_{(j)}, \btheta^{t-1}_{(j)}$, we have $\x_j^\top \X_{(j)}\btheta^{t-1}_{(j)}| \X_{(j)},\btheta^{t-1}_{(j)} \stackrel{d}{=} \N(0, \frac{1}{d}\pnorm{\X_{(j)}\btheta^{t-1}_{(j)}}{}^2)$, where
%\begin{align*}
%\frac{1}{d}\pnorm{\X_{(j)}\btheta^{t-1}_{(j)}}{}^2 \leq C\pnorm{\X}{\op}^2(1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + \gamma\pnorm{f''}{\infty})^{2t} \cdot \frac{1}{d}\Big(\pnorm{\btheta^0}{}^2 + \pnorm{\X^\top \y}{}^2 + \pnorm{f'(\mathbf{0}_d)}{}^2\Big).
%\end{align*}
%Consequently, under the condition $\pnorm{\btheta^0}{\infty} \leq C, |f'(0)|\leq C, \E_{\theta\sim g_\ast}[\theta^2] \leq C$, we have $\E\pnorm{\X^\top \y}{}^2 \leq Cd$, and the above analysis yields that in (\ref{ineq:loo_1}), $\E\pnorm{(\X_{(j)}^\top \X_{(j)} - \X^\top \X)\btheta^{t-1}_{(j)}}{}^2 \leq K$ for some $K > 0$ (in particular $K$ depends on $t$). Let us now bound $\E\pnorm{\X^\top\y - \X_{(j)}^\top \y_{(j)}}{}^2$. Note that
%\begin{align*}
%\X^\top\y - \X_{(j)}^\top \y_{(j)} &= (\X^\top \X - \X_{(j)}^\top \X_{(j)})\btheta^\ast + (\X - \X_{(j)})^\top \beps\\
%&= \X^\top \x_j (\btheta^\ast)_j + e_j \x_j^\top \X\btheta^\ast - e_j (\btheta^\ast)_j \pnorm{\x_j}{}^2 + e_j \x_j^\top \beps. 
%\end{align*}
%This implies
%\begin{align*}
%\E\pnorm{\X^\top\y - \X_{(j)}^\top \y_{(j)}}{}^2 \leq C\Big(\E\Big[(\pnorm{\X}{\op}^2\pnorm{\x_j}{}^2 + \pnorm{\x_j}{}^4) (\btheta^\ast_j)^2\Big] + \E(\x_j^\top \X_{(j)}\btheta^\ast)^2 + \E (\x_j^\top \beps)^2\Big) \leq K,
%\end{align*}
%under the condition that $\E_{\theta\sim g_\ast}[\theta^4] \leq C$.
\end{proof}


\begin{lemma}\label{lem:theta_loo_constant}
Fix any $\gamma > 0$. Then for $T_0 = \floor{K/\gamma}$ with $K > 0$, there exists some $C > 0$ independent of $\gamma$ such that almost surely, $\langle\sup_{0\leq t \leq T_0} \big|(\btheta^t_{(j)})_j\big|\rangle \leq C(1+|\theta^0_j|)$ for any fixed $j\in[d]$. 
\end{lemma}
\begin{proof}
Let us define the continuous-time dynamic $\{\btheta^t_{\gamma,(j)}\}_{t\in\R_+} \subset\R^d$ as 
\begin{align}\label{eq:cont_time_loo_col}
\btheta^t_{\gamma,(j)} = \btheta^0 + \int_0^t \Big[-\frac{1}{\sigma^2}\X_{(j)}^\top (\X_{(j)} \btheta_{\gamma,(j)}^{\floor{s}} - \y_{(j)}) + \partial_\theta \log g(\btheta^{\floor{s}}_{\gamma,(j)};\hat{\alpha}^{\floor{s}}_{\gamma,(j)})\Big] \d s + \sqrt{2}\b^t_\gamma, 
\end{align}
and $(\btheta^t_{\gamma,(j)})_j$ as its $j$th component, and we will show that for any $T> 0$, it holds that $\sup_{t\in[0,T]} \langle |(\btheta^t_{\gamma,(j)})_{j}| \rangle \leq C$ for some $C > 0$ depending on $T$ and other problem parameters but not on $\gamma$. Since $\btheta^k_{(j)} = \btheta^{k\gamma}_{\gamma,(j)}$, this will yield the desired conclusion. 

Consider the auxiliary process 
\begin{align*}
\btheta^t_{(j)} &= \btheta^0 + \int_0^t \Big[-\frac{1}{\sigma^2}\X_{(j)}^\top (\X_{(j)} \btheta_{\gamma,(j)}^{s} - \y_{(j)}) + \partial_\theta \log g(\btheta^{s}_{(j)};\hat{\alpha}^{s}_{(j)})\Big] \d s + \sqrt{2}\b^t,\\
\hat{\alpha}^t_{(j)} &= \hat\alpha^0 + \int_0^t \cG\big(\hat\alpha^s_{(j)}, \Prob_n(\btheta^s_{(j)})\big).
\end{align*}
Then by Assumption \ref{assump:prior} and the bound $\sup_{t\in[0,T]} \pnorm{\hat{\alpha}^t_{(j)}}{} \leq C$ that follows from similar arguments that lead to (\ref{eq:alphaconfined}), we have
\begin{align*}
|(\btheta^t_{(j)})_j| \leq |\theta^0_j| + \int_0^t \partial_\theta \log g((\btheta^s_{(j)})_j; \hat{\alpha}^s_{(j)}) \d s + \sqrt{2}|b^t_j| \leq C\int_0^t |(\btheta^s_{(j)})_j| \d s + \underbrace{C(|\theta^0_j| + 1 + \sup_{t\in[0,T]} |b^t_j|)}_{A_1(T)}.
\end{align*}
Hence by Lemma \ref{lem:gronwall}, it holds that $|(\btheta^t_{(j)})_j| \leq e^{Ct} A_1(T)$ for all $t\in[0,T]$. 

Next we bound $\sup_{t\in[0,T]} |(\btheta^t_{(j)})_j - (\btheta^t_{\gamma,(j)})_j|$. Since $(\btheta^t_{(j)})_j = \theta^0_j + \int_0^t \partial_\theta \log g((\btheta^s_{(j)})_j;\hat\alpha^s_{(j)})\d s + \sqrt{2}b^t_j$ and $(\btheta^t_{\gamma,(j)})_j = \theta^0_j + \int_0^t \partial_\theta \log g((\btheta^{\floor{s}}_{\gamma,(j)})_j;\hat\alpha^{\floor{s}}_{\gamma,(j)})\d s + \sqrt{2}b^t_{\gamma,j}$, we have by Assumption \ref{assump:prior} that
\begin{align*}
\big|(\btheta^t_{(j)})_j - (\btheta^t_{\gamma,(j)})_j\big| &\leq C\int_0^t \big|(\btheta^s_{(j)})_j - (\btheta^s_{\gamma,(j)})_j\big| + \pnorm{\hat\alpha^s_{(j)} - \hat{\alpha}^s_{\gamma,(j)}}{} \d s\\
&\quad + C\int_0^t \big|(\btheta^s_{\gamma,(j)})_j - (\btheta^{\floor{s}}_{\gamma,(j)})_j\big| + \pnorm{\hat\alpha^{\floor{s}}_{\gamma,(j)} - \hat\alpha^s_{\gamma,(j)}}{} \d s + \sqrt{2}|b^t_j - b^t_{\gamma,j}|.
\end{align*}
Using similar arguments as in (\ref{eq:theta_discrete_error}) and (\ref{eq:alpha_discrete_error}), we have
\begin{align*}
\big|(\btheta^s_{\gamma,(j)})_j - (\btheta^{\floor{s}}_{\gamma,(j)})_j\big| \leq C\gamma\sup_{u\in[0,s]} \big|(\btheta^u_{\gamma,(j)})_j - (\btheta^{\floor{u}}_{\gamma,(j)})_j\big| + C\gamma e^{CT} A_1(T) + \sqrt{2}\sup_{t\in[0,T]} |b^t_{\gamma,j} - b^{\floor{t}}_{\gamma,j}|, 
\end{align*}
and $ \pnorm{\hat\alpha^{\floor{s}}_{\gamma,(j)} - \hat\alpha^s_{\gamma,(j)}}{} \leq C\gamma$. Moreover, the conclusion of Lemma \ref{lem:langevin_discretize_error} yields that for each $T > 0$, there exists some function $h(\gamma) = h(\gamma;T) \downarrow 0$ as $\gamma\rightarrow 0$  such that $\sup_{t\in[0,T]} \pnorm{\hat\alpha^t_{(j)} - \hat\alpha^t_{\gamma,(j)}}{} \leq h(\gamma)$ so we conclude that
\begin{align*}
\sup_{u\in[0,t]} \big|(\btheta^u_{(j)})_j - (\btheta^{u}_{\gamma,(j)})_j\big| \leq C\int_0^t \sup_{u\in[0,s]}\big|(\btheta^u_{\gamma,(j)})_j - (\btheta^{u}_{\gamma,(j)})_j\big| \d s + C(h(\gamma) + \gamma e^{CT} A_1(T) + \sqrt{2}\sup_{t\in[0,T]} |b^t_{j} - b^{\floor{t}}_{j}| \vee |b^t_{j} - b^{\ceil{t}}_{j}|).
\end{align*}
Applying Lemma \ref{lem:gronwall} to the map $t\mapsto \sup_{u\in[0,t]} \big|(\btheta^u_{(j)})_j - (\btheta^{u}_{\gamma,(j)})_j\big|$ then yields that for any $t\in[0,T]$, 
\begin{align*}
\sup_{u\in[0,t]} \big|(\btheta^u_{(j)})_j - (\btheta^{u}_{\gamma,(j)})_j\big| \leq Ce^{Ct}\Big(h(\gamma) + \gamma e^{CT} A_1(T) + \sqrt{2}\sup_{t\in[0,T]} |b^t_{j} - b^{\floor{t}}_{j}| \vee |b^t_{j} - b^{\ceil{t}}_{j}|\Big).
\end{align*}
By triangle inequality, we then have
\begin{align*}
\sup_{t\in[0,T]} \big|(\btheta^t_{\gamma,(j)})_j\big| \leq Ce^{CT}\Big(1 + h(\gamma) + \gamma e^{CT} A_1(T) + \sqrt{2}\sup_{t\in[0,T]} |b^t_{j} - b^{\floor{t}}_{j}| \vee |b^t_{j} - b^{\ceil{t}}_{j}|\Big).
\end{align*}
The conclusion now follows by taking the expectation over $\{b^t_j\}$ on both sides and applying the 1-dimensional version of Lemma \ref{lem:BM_maximal}.
\end{proof}



\begin{lemma}\label{lem:response_l2_estimate}
Let $T_0 = \floor{1/\gamma}$. There exists some $(\gamma, n,d)$-independent constant $C > 0$ such that almost surely as $n,d\rightarrow\infty$, 
\begin{align*}
\max_{0\leq s \leq t\leq T_0} \max_{j\in [d]} \Big[\pnorm{\deps \btheta^{t,(s,j),\eps} }{} + \sqrt{d}\pnorm{\deps \hat\alpha^{t,(s,j),\eps}}{} \Big]\leq C\gamma,\\
\max_{0\leq s \leq t\leq T_0} \max_{i\in [n]} \Big[\pnorm{\deps \btheta^{t,[s,i],\eps} }{} + \sqrt{d}\pnorm{\deps \hat\alpha^{t,[s,i],\eps}}{} \Big]\leq C\gamma.
\end{align*}
\end{lemma}
\begin{proof}
We only prove the first claim, and the second claim follows from similar arguments. Without loss generality, we fix $j=1$, and shorthand $\btheta^{t,(s,1),\eps}, \hat\alpha^{t,(s,1),\eps}$ as $\btheta^{t,(s),\eps}, \hat\alpha^{t,(s),\eps}$. By definition of recursion we have for $t\geq s+1$
\begin{align*}
\deps \btheta^{t+1,(s),\eps} &= \Big(I - \frac{\gamma}{\sigma^2}\X^\top \X + \gamma \diag(\partial_\theta^2 \log g(\btheta^{t}; \hat\alpha^{t}))\Big) \deps \btheta^{t,(s),\eps} + \gamma \partial_\theta\nabla_\alpha \log g(\btheta^{t}; \hat\alpha^{t})\deps \hat\alpha^{t,(s),\eps},\\
\deps \hat\alpha^{t+1,(s),\eps} &= \Big(1 + \gamma \nabla_\alpha \cG(\hat\alpha^{t}, \Prob_n(\btheta^{t}))\Big) \deps \hat\alpha^{t,(s),\eps} + \gamma \nabla_{\btheta} \cG(\hat\alpha^{t}, \Prob_n(\btheta^{t}))^\top \deps \btheta^{t,(s),\eps}.
\end{align*}
By Assumptions \ref{assump:prior} and \ref{assump:gradient}, there exists some $C > 0$ depending on $\pnorm{\X}{\op},\sigma^2$ and the parameters in those assumptions such that
\begin{align*}
\pnorm{\deps \btheta^{t+1,(s),\eps}}{} &\leq (1+C\gamma)\pnorm{\deps \btheta^{t+1,(s),\eps}}{} + C\sqrt{d}\pnorm{\deps \hat\alpha^{t+1,(s),\eps}}{},\\
\pnorm{\deps \hat\alpha^{t+1,(s),\eps}}{} &\leq (1+C\gamma)\pnorm{\deps \hat\alpha^{t,(s),\eps}}{} + C\gamma \pnorm{\deps \btheta^{t,(s),\eps}}{}/\sqrt{d}, 
\end{align*}
which further implies that
\begin{align*}
\pnorm{\deps \btheta^{t+1,(s),\eps}}{} + \sqrt{d}\pnorm{\deps \hat\alpha^{t+1,(s),\eps}}{} \leq (1+C\gamma)\Big(\pnorm{\deps \btheta^{t,(s),\eps}}{} + \sqrt{d}\pnorm{\deps \hat\alpha^{t,(s),\eps}}{}\Big). 
\end{align*}
Iterating this inequality yields that for some $(\gamma, n,d)$-independent constant $C' > 0$, 
\begin{align*}
\max_{0\leq s \leq t\leq T_0} [\pnorm{\deps \btheta^{t+1,(s),\eps}}{} + \sqrt{d}\pnorm{\deps \hat\alpha^{t+1,(s),\eps}}{}] \leq C'\big(\pnorm{\deps \btheta^{s+1,(s),\eps}}{} + \sqrt{d}\pnorm{\deps \hat\alpha^{s+1,(s),\eps}}{}\big) = C'\gamma, 
\end{align*}
using $\deps \btheta^{s+1,(s),\eps} = \gamma \e_1$ and $\deps \hat\alpha^{s+1,(s),\eps} = 0$.
\end{proof}

We are now ready to prove Lemma \ref{lem:perturb_key_expansion}.

\begin{proof}[Proof of Lemma \ref{lem:perturb_key_expansion}]
We prove by induction. 
\noindent\textbf{Baseline case} When $t = 1$ and $s = 0$, direct calculation via (\ref{eq:theta_row_perturb}) shows that
\begin{align*}
\partial_\eps|_{\eps = 0} \btheta_j^{1,(0,j), \eps} = \gamma = r_\theta^{(\theta_j,\hat\alpha)}(1,0), \quad j\in[d],
\end{align*}
and similarly via (\ref{eq:theta_col_perturb}), standard concentration shows that
\begin{align*}
\partial_\eps|_{\eps = 0} \bbeta_i^{1,[0,i], \eps} = \gamma \pnorm{\X^\top \e_i}{}^2 = \gamma + E_\eta^{1,[0,i]}
\end{align*}
with $E_\eta^{1,[0,i]} \rightarrow_{a.s.} 0$, while $r_\eta(1,0) = \bar{R}_\theta^{\gamma}(1,0)/\sigma^2 = \gamma/\sigma^2$, verifying the baseline case.

 

\noindent \textbf{Induction} Suppose the hypotheses (\ref{eq:induce_theta})-(\ref{eq:induce_eta}) hold up to time $t$ and $s < t$. %Let us first derive two facts from these hypotheses.
Note that by Lemma \ref{lem:A_trace} and the same argument as in the proof of Proposition \ref{prop:discrete_time_response}, we have the induction hypothesis that: almost surely as $n,d\rightarrow\infty$, with the matrix sequence $\{A_t\}$ defined in (\ref{def:A_matrix}), 
\begin{equation}\label{eq:induction_consequence}
\begin{aligned}
\bigg\{\gamma \cdot \frac{1}{d}\Tr\Big(A_{t-1}\ldots A_{s+1}\Big),  \quad\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps} \bigg\}\rightarrow \bar{R}_\theta^{\gamma}(t,s),\\
\bigg\{\gamma \cdot \frac{1}{n}\Tr\Big(\X A_{t-1}\ldots A_{s+1} \X^\top \Big), \quad\frac{1}{n}\sum_{i=1}^n \partial_\eps|_{\eps = 0} \bbeta_i^{t,[s,i], \eps}\bigg\} \rightarrow \frac{\sigma^4}{\delta} \bar{R}_\eta^{\gamma}(t,s).
\end{aligned}
\end{equation}
%definition, 
%\begin{align*}
%\partial_\eps|_{\eps = 0} \btheta^{t,(s,j), \eps} &= \underbrace{\Big(I - \frac{\gamma}{\sigma^2}\X^\top \X - \gamma\diag(f''(\btheta^{t-1}))\Big)}_{A_{t-1}}\partial_\eps|_{\eps = 0} \btheta^{t-1,(s,j), \eps}\\
%&= A_{t-1}A_{t-2} \partial_\eps|_{\eps = 0} \btheta^{t-2,(s,j), \eps} = \ldots = A_{t-1}\ldots A_{s+1} \partial_\eps|_{\eps = 0}\btheta^{s+1,(s,j), \eps}= \gamma A_{t-1}\ldots A_{s+1} \e_j.
%\end{align*}
%This entails that
%\begin{align*}
%d^{-1}\sum_{j=1}^{d} \partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps} = \gamma \cdot \frac{1}{d}\Tr\Big(A_{t-1}\ldots A_{s+1}\Big),
%\end{align*}
%and hence we conclude by symmetry
%\begin{align}\label{eq:fact_1}
%\frac{1}{d}\E\Big[\Tr\Big(A_{t-1}\ldots A_{s+1}\Big)\Big] = \gamma^{-1} \E\Big[\partial_\eps|_{\eps = 0} \btheta_d^{t,(s,d),\eps}\Big] = \gamma^{-1} R_\theta^{(\mu)}(t,s) + o_n(1).
%\end{align}
%Similarly, 
%\begin{align}\label{eq:theta_derivative_2}
%\notag\partial_\eps|_{\eps = 0} \btheta^{t,[s,i], \eps} &= \underbrace{\Big(I - \frac{\gamma}{\sigma^2}\X^\top \X - \gamma\diag(f''(\btheta^{t-1}))\Big)}_{A_{t-1}}\partial_\eps|_{\eps = 0} \btheta^{t-1,[s,i], \eps}\\
%&= A_{t-1}A_{t-2} \partial_\eps|_{\eps = 0} \btheta^{t-2,[s,i], \eps} = \ldots = A_{t-1}\ldots A_{s+1} \deps\btheta^{s+1,[s,i], \eps} = \gamma A_{t-1}\ldots A_{s+1} \X^\top \e_i.
%\end{align}
%This implies
%\begin{align*}
%n^{-1}\sum_{i=1}^n \partial_\eps|_{\eps = 0}\bbeta_i^{t,[s,i], \eps} = \gamma \cdot \frac{1}{n}\Tr\Big(\X A_{t-1}\ldots A_{s+1} \X^\top\Big),
%\end{align*}
%and hence we conclude by symmetry
%\begin{align}\label{eq:fact_2}
%\frac{1}{n}\E\Big[\Tr\Big(\X A_{t-1}\ldots A_{s+1} \X^\top\Big)\Big] = \gamma^{-1} \E\Big[\partial_\eps|_{\eps = 0}\bbeta_n^{t,[s,n], \eps}\Big] = -\frac{\sigma^4}{\delta\gamma} R_\eta^{(\mu)}(t,s) + o_n(1)
%\end{align}

We will now establish (\ref{eq:induce_theta})-(\ref{eq:induce_eta}) for $t+1$ and $s < t+1$. 


\textbf{Claim for $\partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps}$} By symmetry we will consider the last component $\mu^{t,(s), \eps} = \btheta_d^{t,(s,d), \eps}$ and shorthand $\btheta^{t,(s,d), \eps}$ as $\btheta^{t,(s), \eps}$. First note that if $s = t$, direct calculation via (\ref{eq:theta_row_perturb}) shows that $\partial_\eps|_{\eps = 0} \mu^{t+1,(s), \eps} = \gamma = r_\theta^{(\mu,\hat\alpha)}(t+1,t)$, as desired. In what follows, we fix $s < t$. By definition, if we write $\btheta^{t,(s),\eps} = [\bar{\btheta}^{t,(s),\eps}, \mu^{t,(s),\eps}]$ with $\bar{\btheta}^{t,(s),\eps}\in\R^{d-1}$, and $\X = [\bar{\X}, \x]$ with $\bar{\X} \in \R^{n\times (d-1)}$ and $\x\in\R^n$, then
\begin{align*}
\bar{\btheta}^{t+1,(s),\eps} &= \Big(I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X}\Big)\bar{\btheta}^{t,(s),\eps} - \frac{\gamma}{\sigma^2} \bar{\X}^\top (\x \mu^{t,(s),\eps} - \y) + \gamma \partial_\theta \log g(\bar{\btheta}^{t,(s),\eps}; \hat\alpha^{t,(s),\eps}) + \sqrt{2}(\bar{\b}^{(t+1)\gamma} - \bar{\b}^{t\gamma}),\\
\mu^{t+1,(s),\eps} &= \Big(1 - \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2\Big)\mu^{t,(s),\eps} - \frac{\gamma}{\sigma^2}\x^\top (\bar{\X}\bar{\btheta}^{t,(s),\eps} - \y) + \gamma \partial_\theta \log g(\mu^{t,(s),\eps}; \hat\alpha^{t,(s),\eps}) + \sqrt{2}(b^{(t+1)\gamma} - b^{t\gamma}),\\
\hat\alpha^{t+1,(s),\eps} &= \hat\alpha^{t,(s),\eps} + \gamma \cG(\hat\alpha^{t,(s),\eps}, \Prob_n(\btheta^{t,(s),\eps}))
\end{align*}
where $\bar{\b}^t$ (resp. $b^t$) denote the first $d-1$ (resp. last) components of $\b^t$, and $\Prob_n(\btheta)$ denotes the empirical distribution of $\btheta$. Taking $\eps$ derivative of $\mu^{t+1,(s),\eps}$, we have
\begin{align}\label{eq:mu_expand_1}
\notag\partial_\eps|_{\eps = 0} \mu^{t+1,(s),\eps} &= \Big(1 -  \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2 + \gamma \partial_\theta^2 \log g(\mu^{t}; \hat\alpha^{t})\Big)\partial_\eps|_{\eps = 0} \mu^{t,(s),\eps} + \gamma\underbrace{\partial_\theta \nabla_\alpha \log g(\theta^{t};\hat\alpha^{t})^\top \deps \hat\alpha^{t,(s),\eps}}_{\rho^{t,(s)}}\\
&\quad - \frac{\gamma}{\sigma^2} \x^\top \bar{\X}\partial_\eps|_{\eps=0}\bar{\btheta}^{t,(s),\eps},
\end{align}
where we write $\btheta^t = (\bar{\btheta}^t,\mu^t)$. To evaluate $\partial_\eps|_{\eps=0}\bar{\btheta}^{t,(s),\eps}$, define $\bar{\brho}^{t,(s),\eps} := \partial_\theta \nabla_\alpha \log g(\bar{\btheta}^{t,(s),\eps};\hat\alpha^{t,(s),\eps}) \deps \hat\alpha^{t,(s),\eps} \in \R^{d-1}$, where $\partial_\theta \nabla_\alpha \log g(\bar{\btheta}^{t,(s),\eps};\hat\alpha^{t,(s),\eps}) \in \R^{(d-1)\times K}$ is given by
\begin{align*}
\Big(\partial_\theta \nabla_\alpha \log g(\bar{\btheta}^{t,(s),\eps};\hat\alpha^{t,(s),\eps})\Big)_{i,j} = \partial_\theta \partial_{\alpha_j} \log g(\theta_i^{t,(s),\eps};\hat\alpha^{t,(s),\eps}), \quad i\in[d-1], j\in[K].
\end{align*}
Then we have
\begin{align*}
\partial_\eps \bar{\btheta}^{t,(s),\eps} &= \underbrace{\Big(I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta^2 \log g(\bar{\btheta}^{t-1,(s),\eps}; \hat\alpha^{t-1,(s),\eps}))\Big)}_{\Omega^{t-1,\eps}} \partial_\eps \bar{\btheta}^{t-1,(s),\eps} - \frac{\gamma}{\sigma^2} \bar{\X}^\top \x \partial_\eps \mu^{t-1,(s),\eps} + \gamma \bar{\brho}^{t-1,(s),\eps}\\
&= \Omega^{t-1,\eps}\Big(\Omega^{t-2,\eps}\partial_\eps \bar{\btheta}^{t-2,(s),\eps} - \frac{\gamma}{\sigma^2} \bar{\X}^\top \x \partial_\eps \mu^{t-2,(s),\eps} + \gamma \bar{\brho}^{t-2,(s),\eps}\Big)  - \frac{\gamma}{\sigma^2} \bar{\X}^\top \x \cdot \partial_\eps \mu^{t-1,(s),\eps} + \gamma \bar{\brho}^{t-1,(s),\eps}\\
&=\ldots\\
&= \Omega^{t-1,\eps}\ldots \Omega^{s+1,\eps} \partial_\eps \bar{\btheta}^{s+1,(s),\eps} - \frac{\gamma}{\sigma^2} \sum_{j=s+1}^{t-2} \Omega^{t-1,\eps}\ldots \Omega^{j+1,\eps} \bar{\X}^\top \x \cdot \partial_\eps \mu^{j,(s),\eps} - \frac{\gamma}{\sigma^2}\bar{\X}^\top \x \cdot \partial_\eps \mu^{t-1,(s),\eps}\\
&\quad + \gamma \sum_{j=s+1}^{t-2} \Omega^{t-1,\eps}\ldots \Omega^{j+1,\eps} \bar{\brho}^{j,(s),\eps} + \gamma \bar{\brho}^{t-1,(s),\eps}\\
&= - \frac{\gamma}{\sigma^2} \sum_{j=s+1}^{t-2} \Omega^{t-1,\eps}\ldots \Omega^{j+1,\eps} \bar{\X}^\top \x \cdot \partial_\eps \mu^{j,(s),\eps} - \frac{\gamma}{\sigma^2}\bar{\X}^\top \x \cdot \partial_\eps \mu^{t-1,(s),\eps} + \gamma \sum_{j=s+1}^{t-2} \Omega^{t-1,\eps}\ldots \Omega^{j+1,\eps} \bar{\brho}^{j,(s),\eps} + \gamma \bar{\brho}^{t-1,(s),\eps},
\end{align*}
using the fact that $\partial_\eps \bar{\btheta}^{s+1,(s),\eps} = 0$. Plugging the above expression into (\ref{eq:mu_expand_1}), we have
\begin{align*}
\deps \mu^{t+1,(s),\eps} &= \underbrace{\Big(1 -  \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2 + \gamma \partial_\theta^2 \log g(\mu^{t}; \hat\alpha^{t})\Big) \cdot \deps \mu^{t,(s),\eps}}_{(I)}\\
&\quad +\underbrace{\Big(\frac{\gamma}{\sigma^2}\Big)^2 \sum_{j=s+1}^{t-2} \x^\top \bar{\X} \Omega^{t-1}\ldots \Omega^{j+1} \bar{\X}^\top \x \cdot \deps \mu^{j,(s),\eps}}_{(II)} + \underbrace{\Big(\frac{\gamma}{\sigma^2}\Big)^2 \pnorm{\bar{\X}^\top \x}{}^2 \cdot \deps \mu^{t-1,(s),\eps}}_{(III)}\\
&\quad - \underbrace{\frac{\gamma^2}{\sigma^2} \sum_{j=s+1}^{t-2} \x^\top \bar{\X}\Omega^{t-1}\ldots \Omega^{j+1} \bar{\brho}^{j,(s)}}_{(IV)} - \underbrace{\frac{\gamma^2}{\sigma^2} \x^\top \bar{\X} \bar{\brho}^{t-1,(s)}}_{(V)} + \underbrace{\gamma \rho^{t,(s)}}_{(VI)}, 
\end{align*}
where we shorthand $\Omega^{t,\eps = 0}$ as $\Omega^t = I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta^2 \log g(\bar{\btheta}^{t}; \alpha^t)) \in \R^{(d-1)\times (d-1)}$, $\bar{\brho}^{t,(s),\eps = 0}$ as $\bar{\brho}^{t,(s)}$, and we recall $\bar{\btheta}^{t} \in \R^{d-1}$ denote the the first $d-1$ components of $\btheta^t$. %\ys{$\Omega^t$ is the leave-one-column-out version of $A^t$}
%We may expand
%\begin{align*}
%\iprod{\bar{\X}^\top \x}{\Omega^{t-1}\ldots \Omega^{j+1} \bar{\X}^\top \x} &\approx \iprod{\bar{\X}^\top \x}{\Omega^{t-1}_{(-p)}\ldots \Omega^{j+1}_{(-p)} \bar{\X}^\top \x}\\
%&\approx \frac{1}{p} \Tr\Big(\bar{\X} \Omega^{t-1}_{(-p)}\ldots \Omega^{j+1}_{(-p)} \bar{\X}^\top\Big)\\
%&\approx -\frac{\delta\sigma^2}{\gamma} r_\eta(t,s).
%\end{align*}
To analyze these terms, let $\Omega^{j}_{(-d)} = I -\frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta^2 \log g(\bar{\btheta}^{j}_{(d)}; \hat\alpha^j_{(d)})) \in\R^{(d-1)\times (d-1)}$, with $\{\bar{\btheta}^{t}_{(d)}\}$ denoting the first $d-1$ components of $\btheta^t_{(d)}$ given by (\ref{eq:leave_col_out}).
%the leave-one-column-out version of (\ref{eq:original})
%\begin{align*}
%\bar{\btheta}^{t}_{(d)} = \bar{\btheta}^{t-1}_{(d)} - \gamma\Big[\frac{1}{\sigma^2}\bar{\X}^\top(\bar{\X}\bar{\btheta}^{t-1}_{(d)} - \y) + f'(\bar{\btheta}^{t-1}_{(d)})\Big] \in \R^{d-1}.
%\end{align*}

\noindent \textbf{Analysis of $(I)$ and $(III)$} The induction hypothesis yields $(I) = (1- \frac{\gamma\delta}{\sigma^2} + \gamma \partial_\theta^2 \log g(\mu^t; \hat\alpha^t)) r_\theta^{(\mu,\hat\alpha)}(t,s) + \mathsf{r}_I^{(d)}$, where
\begin{align*}
\mathsf{r}_I^{(d)} = \frac{\gamma}{\sigma^2}(\delta - \pnorm{\x}{}^2)(r_\theta^{(\mu,\hat\alpha)}(t,s) + E^{t,(s,d)}_\theta) +  \Big(1- \frac{\gamma\delta}{\sigma^2} + \gamma \partial_\theta^2 \log g(\mu^t;\hat\alpha^t)\Big) E^{t,(s,d)}_\theta
\end{align*}
satisfies $\langle d^{-1}\sum_{j=1}^d \mathsf{r}_I^{(j)}\rangle  \rightarrow_{a.s.} 0$. Similarly, $(III) = \delta (\frac{\gamma}{\sigma^2})^2 r_\theta^{(\mu,\hat\alpha)}(t-1,s) + \mathsf{r}_2^{(d)}$, where
\begin{align*}
\mathsf{r}_2^{(d)} = (\frac{\gamma}{\sigma^2})^2(\pnorm{\bar{\X}^\top \x}{}^2 - \delta) \cdot \Big(r_\theta^{(\mu,\hat\alpha)}(t-1,s) +  E^{t-1,(s,d)}_\theta\Big) + \delta (\frac{\gamma}{\sigma^2})^2 \cdot E^{t-1,(s,d)}_\theta
\end{align*}
satisfies $\langle d^{-1}\sum_{j=1}^d \mathsf{r}_2^{(j)} \rangle \rightarrow_{a.s.} 0$. 

\noindent\textbf{Analysis of $(II)$} We first show that for each $s+1 \leq j \leq t-2$,
\begin{align}\label{eq:loo_approximation}
\Big\langle\Big|\x^\top \bar{\X} \Omega^{t-1}\ldots \Omega^{j+1} \bar{\X}^\top \x - \x^\top \bar{\X} \Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \x\Big| \Big\rangle \leq C\sqrt{\frac{\log d}{d}}(|\theta^0_d| + |\theta^\ast_d| + \sqrt{\log d}). 
\end{align}
To see this, note that
\begin{align*}
\Big|\x^\top \bar{\X}\Omega^{t-1}\ldots \Omega^{j+1} \bar{\X}^\top \x - \x^\top \bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \x\Big| \leq \sum_{\ell = j+1}^{t-1} \underbrace{\Big|\x^\top \bar{\X}\Omega^{t-1}_{(d)} \ldots \Omega^{\ell+1}_{(d)} (\Omega^{\ell} - \Omega_{(d)}^{\ell}) \Omega^{\ell-1} \ldots \Omega^{j+1}\bar{\X}^\top \x\Big|}_{T^\ell_{(d)}},
\end{align*}
where
\begin{align*}
\Omega^{\ell} - \Omega^\ell_{(d)} &= \Big[I - \frac{\gamma}{\sigma^2}\bar{\X}^\top\bar{\X} + \gamma \diag\big(\partial_\theta^2 \log g(\bar{\btheta}^\ell; \hat\alpha^\ell)\big)\Big] - \Big[I - \frac{\gamma}{\sigma^2}\bar{\X}^\top\bar{\X} + \gamma \diag\big(\partial_\theta^2 \log g(\bar{\btheta}_{(d)}^\ell;\hat\alpha^\ell_{(d)})\big)\Big]\\
&= \gamma \diag\big(\partial_\theta^2 \log g(\bar{\btheta}^\ell;\hat\alpha^\ell) - \partial_\theta^2 \log g(\bar{\btheta}_{(d)}^\ell; \hat\alpha^\ell_{(d)})\big). 
\end{align*}
Hence by Assumption \ref{assump:prior}, 
\begin{align*}
|T^\ell_{(d)}| &= \gamma\Big|\Big(\Omega^{\ell+1}_{(d)} \ldots \Omega^{t-1}_{(d)}\bar{\X}^\top \x \circ \Omega^{\ell-1} \ldots \Omega^{j+1}\bar{\X}^\top \x\Big)^\top \big(\partial_\theta^2 \log g(\bar{\btheta}_{(d)}^\ell;\hat\alpha^\ell_{(d)}) - \partial_\theta^2 \log g(\bar{\btheta}^\ell;\hat\alpha^\ell)\big)\Big|\\
&\leq \gamma\pnorm{\Omega^{\ell+1}_{(d)} \ldots \Omega^{t-1}_{(d)}\bar{\X}^\top \x}{\infty}\pnorm{\Omega^{\ell-1} \ldots \Omega^{j+1}\bar{\X}^\top \x}{}\pnorm{\partial_\theta^2 \log g(\bar{\btheta}_{(d)}^\ell;\hat\alpha^\ell_{(d)}) - \partial_\theta^2 \log g(\bar{\btheta}^\ell;\hat\alpha^\ell)}{}\\
&\leq C\gamma\pnorm{\Omega^{\ell+1}_{(d)} \ldots \Omega^{t-1}_{(d)}\bar{\X}^\top \x}{\infty} \cdot \pnorm{\Omega^{\ell-1}}{\op} \ldots \pnorm{\Omega^{j+1}}{\op} \pnorm{\bar{\X}^\top \x}{} \cdot(\pnorm{\bar{\btheta}_{(d)}^\ell - \bar{\btheta}^\ell}{} + \pnorm{\hat\alpha^\ell_{(d)} - \hat\alpha^\ell}{}).
\end{align*}
Since $\x$ is independent of $\Omega^{\ell+1}_{(d)}, \ldots, \Omega^{t-1}_{(d)},\bar{\X}$, for each $j\in [d]$ and $\e_j\in\R^d$,  we have 
\begin{align*}
\e_j^\top \Omega^{\ell+1}_{(d)} \ldots \Omega^{t-1}_{(d)}\bar{\X}^\top \x| \Omega^{\ell+1}_{(d)}, \ldots, \Omega^{t-1}_{(d)},\bar{\X} \sim \N(0, \frac{1}{d}\pnorm{(\Omega^{\ell+1}_{(d)}\ldots, \Omega^{t-1}_{(d)}\bar{\X}^\top)^\top \e_j}{}^2)
\end{align*}
where 
\begin{align*}
\pnorm{(\Omega^{\ell+1}_{(d)}\ldots, \Omega^{t-1}_{(d)}\bar{\X}^\top)^\top \e_j}{} \leq \pnorm{\Omega^{\ell+1}_{(d)}\ldots, \Omega^{t-1}_{(d)}\bar{\X}^\top}{\op} \leq \pnorm{\Omega^{\ell+1}_{(d)}}{\op}\ldots\pnorm{\Omega^{t-1}_{(d)}}{\op}\pnorm{\bar{\X}}{\op}. 
\end{align*}
Hence using the bound $\pnorm{\Omega^{\ell}}{\op} \vee \pnorm{\Omega^{\ell}_{(d)}}{\op} \leq 1 + \frac{\gamma}{\sigma^2}\pnorm{\bar{\X}}{\op}^2 + C\gamma$ and a standard tail bound for $\pnorm{\bar{\X}}{\op}$, we have almost surely $\pnorm{\Omega^{\ell+1}_{(d)} \ldots \Omega^{t-1}_{(d)}\bar{\X}^\top \x}{\infty}^4 \leq C\sqrt{\log d/d}$.
%and each $T_\ell$ satisfies
%\begin{align*}
%%&\Big|\iprod{\bar{\X}^\top \x}{\Omega^{t-1}_{(d)} \ldots \Omega^{\ell+1}_{(d)} (\Omega^{\ell} - \Omega_{(d)}^{\ell}) \Omega^{\ell-1} \ldots \Omega^{j+1}\bar{\X}^\top \x}\Big|\\
%T_\ell &\leq \pnorm{\bar{\X}^\top \x}{}^2 \pnorm{\Omega^{t-1}_{(d)}}{\op} \ldots \pnorm{\Omega^{\ell+1}_{(d)}}{\op} \pnorm{\Omega^{\ell} - \Omega_{(d)}^{\ell}}{\op} \pnorm{\Omega^{\ell-1}}{\op} \ldots \pnorm{\Omega^{j+1}}{\op}\\
%&\leq \pnorm{\bar{\X}^\top \x}{}^2 \cdot \prod_{j+1\leq k \leq t-1: k\neq \ell} (1 + \frac{\gamma}{\sigma^2}\pnorm{\bar{\X}}{\op}^2 + \gamma\pnorm{f''}{\infty}) \cdot \gamma \pnorm{f'''}{\infty}\pnorm{\bar{\btheta}^{\ell} - \bar{\btheta}^{\ell}_{(d)}}{\infty}. 
%\end{align*}
By Lemma \ref{lem:loo_error} and a standard tail bound on $\pnorm{\bar{\X}}{\op}$, we then conclude (\ref{eq:loo_approximation}).
%\begin{align*}
%\E[T_\ell^2] \leq \gamma \pnorm{f'''}{\infty} \cdot \Big(\E \pnorm{\bar{\X}^\top \x}{}^8\Big)^{1/4} \cdot \Big[\E \Big(1 + \frac{\gamma}{\sigma^2}\pnorm{\bar{\X}}{\op}^2 + \gamma\pnorm{f''}{\infty}\Big)^{8 \cdot (t-j-2)}\Big]^{1/4} \cdot \Big[\E\pnorm{\bar{\btheta}^{\ell} - \bar{\btheta}^{\ell}_{(d)}}{\infty}^4\Big]^{1/2} \rightarrow_0, 
%\end{align*}
Now note that $\{\Omega^t_{(d)}\}$ is independent of $\x$, so in (\ref{eq:loo_approximation}), applying Hanson-Wright yields
\begin{align*}
\Prob\bigg(\Big|\x^\top \bar{\X} \Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \x - \frac{1}{d}\Tr\Big(\bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \Big)\Big| > t | \bar{\X}\bigg) \leq \exp\Big(-c\frac{d^2t^2}{\pnorm{W}{F}^2} \wedge \frac{dt}{\pnorm{W}{\op}}\Big),
\end{align*}
where $W = \bar{\X} \Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top$. Using again the tail bound on $\pnorm{\bar{\X}}{\op}$ and $\pnorm{\Omega^{t}_{(d)}}{\op} \leq (1 + \frac{\gamma}{\sigma^2}\pnorm{\bar{\X}}{\op}^2 + C\gamma)$ by Assumption \ref{assump:prior}, we therefore conclude by Borel-Cantelli lemma that
\begin{align*}
\x^\top \bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \x - \frac{1}{d}\Tr\Big(\bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \Big)\rightarrow_{a.s.} 0,
\end{align*}
%where $\E_{\x}$ denotes expectation only with respect to $\x$. 
Moreover, by the analogue of second equation of (\ref{eq:induction_consequence}) for system size $(n,d-1)$, we have
%Lemma \ref{lem:A_trace} and the same argument as in the proof of Proposition \ref{prop:discrete_time_response} both applied with system size $(n,d-1)$, we have
\begin{align*}
\frac{1}{d}\Tr\Big(\bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \Big) \rightarrow_{a.s.} \frac{\sigma^4}{\gamma}\bar{R}_\eta^{\gamma}(t,j),
\end{align*}
where we again emphasize that $\{\bbeta^{t,[j,i],\eps}\}$ is given by (\ref{eq:eta_row_perturb}) with system size $(n,d-1)$.
%\red{Suppose concentration holds}, then we further have
%\begin{align*}
%\E\bigg(\frac{1}{d}\Tr\Big(\bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \Big) - \frac{1}{d}\E\Big[\Tr\Big(\bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \Big)\Big]\bigg)^2 \rightarrow 0.
%\end{align*}
%Now by the fact (\ref{eq:fact_2}) (applied with system size $(n,p-1)$), we have
%\begin{align*}
%\frac{1}{d}\E\Big[\Tr\Big(\bar{\X}\Omega_{(d)}^{t-1}\ldots \Omega_{(d)}^{j+1} \bar{\X}^\top \Big)\Big] \rightarrow -\frac{\sigma^4}{\gamma} R^{(\mu)}_\eta(t,j).
%\end{align*}
In summary, we have shown that $(II) = \gamma\sum_{j=s+1}^{t-2} \bar{R}_\eta^{\gamma}(t,j) r_\theta^{(\mu)}(j,s) + \mathsf{r}_2^{(j)}$, with $\langle d^{-1} \sum_{j=1}^d \mathsf{r}_2^{(j)} \rangle\rightarrow_{a.s.} 0$.

\noindent\textbf{Analysis of $(IV)$-$(VI)$} We apply a similar leave-one-out argument as above. Let $\bar{\brho}^{t,(s)}_{(d)} := \partial_\theta \nabla_\alpha \log g(\bar{\btheta}^{t}_{(d)};\hat\alpha^{t}_{(d)}) \deps \hat\alpha^{t,(s),\eps}$. Then for each $s+1\leq j\leq t-2$, 
\begin{align}\label{eq:theta_loo_arg}
\notag\Big|\x^\top \bar{\X} \Omega^{t-1}\ldots \Omega^{j+1}\bar{\brho}^{j,(s)} - \x^\top \bar{\X} \Omega^{t-1}_{(d)}\ldots \Omega^{j+1}_{(d)}\bar{\brho}_{(d)}^{j,(s)}\Big| &\leq \sum_{\ell = j+1}^{t-1} \underbrace{\Big|\x^\top \bar{\X}\Omega^{t-1}_{(d)} \ldots \Omega^{\ell+1}_{(d)} (\Omega^{\ell} - \Omega_{(d)}^{\ell}) \Omega^{\ell-1} \ldots \Omega^{j+1}\bar{\brho}_{(d)}^{j,(s)}\Big|}_{u^\ell_{(d)}}\\
&\quad + \underbrace{\Big|\x^\top \bar{\X}\Omega^{t-1}_{(d)} \ldots \Omega^{j+1}_{(d)}(\bar{\brho}^{t,(s)} - \bar{\brho}^{t,(s)}_{(d)})\Big|}_{v_{(d)}}.
\end{align}
Using similar arguments as above, we have $\langle d^{-1} \sum_{j=1}^d u^\ell_{(d)} \rangle = o_{a.s.}(1)$. For the second term, we have
\begin{align*}
v_{(d)} &= \Big|\x^\top \bar{\X}\Omega^{t-1}_{(d)} \ldots \Omega^{j+1}_{(d)} \Big(\partial_\theta \nabla_\alpha \log g(\bar{\btheta}^t; \hat\alpha^t) - \partial_\theta \nabla_\alpha \log g(\bar{\btheta}^t_{(d)}; \hat\alpha^t_{(d)})\Big) \deps \alpha^{t,(s),\eps}\Big|\\
&\leq C\pnorm{\x}{}\pnorm{\bar{\X}}{\op}\pnorm{\Omega^{t-1}_{(d)} }{\op}\ldots \pnorm{\Omega^{j+1}_{(d)} }{\op}(\pnorm{\bar{\btheta}^t - \bar{\btheta}^t_{(d)}}{} + \pnorm{\hat\alpha^t - \hat\alpha^t_{(d)}}{})\pnorm{\deps \hat\alpha^{t,(s),\eps}}{},
\end{align*}
which satisfies $\langle d^{-1}\sum_{j=1}^d v_{(j)}\rangle = o_{a.s.}(1)$ by Lemmas \ref{lem:loo_error} and \ref{lem:response_l2_estimate}. On the other hand, we have
\begin{align*}
\Big|\x^\top \bar{\X} \Omega^{t-1}_{(d)}\ldots \Omega^{j+1}_{(d)}\bar{\brho}_{(d)}^{j,(s)}\Big| &= \Big|\x^\top \bar{\X} \Omega^{t-1}_{(d)}\ldots \Omega^{j+1}_{(d)} \partial_\theta\nabla_\alpha \log g(\bar{\btheta}_{(d)}^t;\hat\alpha^t_{(d)}) \cdot \deps \hat\alpha^{t,(s),\eps}\Big|\\
&\leq \pnorm{\x^\top \bar{\X} \Omega^{t-1}_{(d)}\ldots \Omega^{j+1}_{(d)} \partial_\theta\nabla_\alpha \log g(\bar{\btheta}_{(d)}^t;\hat\alpha^t_{(d)})}{}\pnorm{\deps \hat\alpha^{t,(s),\eps}}{}.  
\end{align*}
Since $\Omega^{t-1}_{(d)}, \ldots, \Omega^{j+1}_{(d)}, \partial_\theta\nabla_\alpha \log g(\bar{\btheta}_{(d)}^t;\hat\alpha^t_{(d)})$ are all independent of $\x$, the first term is almost surely bounded, hence the whole thing is $o_{a.s.}(1)$ by Lemma \ref{lem:response_l2_estimate}. This shows that each $\x^\top \bar{\X} \Omega^{t-1}\ldots \Omega^{j+1}\bar{\brho}^{j,(s)}$ is $o_{a.s.}(1)$ when averaged over the coordinates, hence both $(IV)$ and $(V)$ are $o_{a.s.}(1)$ when averaged over the coordinates. Lastly, again by Lemma \ref{lem:response_l2_estimate} we have $|\rho^{t,(s)}| \leq \pnorm{\partial_\theta\nabla_\alpha \log g(\bar{\btheta}^t;\hat\alpha^t)}{}\pnorm{\deps \hat\alpha^{t,(s),\eps}}{} = o_{a.s.}(1)$, hence $(VI) = o_{a.s.}(1)$.


Putting together the pieces, for some $E_\theta^{t+1,(s,j)}$ such that $\langle d^{-1} \sum_{j=1}^d E_\theta^{t+1,(s,j)} \rangle \rightarrow_{a.s.} 0$, we have
\begin{align*}
\partial_\eps|_{\eps = 0} \mu^{t+1,(s),\eps} &= \big(1- \frac{\gamma\delta}{\sigma^2} + \gamma \partial_\theta^2 \log g(\mu^t; \hat\alpha^t)\big) r_\theta^{(\mu,\hat\alpha)}(t,s) + \gamma\sum_{j=s+1}^{t-2} \bar{R}_\eta^{\gamma}(t,j) r_\theta^{(\mu,\hat\alpha)}(j,s)\\
&\quad +  \delta (\frac{\gamma}{\sigma^2})^2 r_\theta^{(\mu,\hat\alpha)}(t-1,s) + E_\theta^{t+1,(s,d)}\\
&= \big(1- \frac{\gamma\delta}{\sigma^2} + \gamma \partial_\theta^2 \log g(\mu^t;\hat\alpha^t)\big) r_\theta^{(\mu,\hat\alpha)}(t,s) + \gamma\sum_{j=s+1}^{t-1} \bar{R}_\eta^{\gamma}(t,j) r_\theta^{(\mu,\hat\alpha)}(j,s)  + E_\theta^{t+1,(s,d)}\\
&= r_\theta^{(\mu,\hat\alpha)}(t+1,s) + E_\theta^{t+1,(s,d)},
\end{align*}
concluding the induction. We also argue as in (\ref{eq:induction_consequence}) to obtain
\begin{align}\label{eq:fact_3}
\bigg\{\gamma \cdot \frac{1}{d}\Tr\Big(A_t\ldots A_{s+1}\Big), \quad \frac{1}{d}\sum_{j=1}^d \deps \btheta^{t+1,(s,j),\eps}_j\bigg\}=  \bar{R}_\theta^{\gamma}(t+1,s) + o_{a.s.}(1).
\end{align}
%, we have
%\begin{align*}
%\partial_\eps|_{\eps = 0} \mu^{t+1,(s),\eps} &=  \Big(1 -  \frac{\gamma\delta}{\sigma^2} - \gamma f''(\mu^t)\Big) r_{\theta}^{(\mu)}(t,s) - \gamma \sum_{j=s+1}^{t-1} R_\eta^{(\mu)}(t,j) r_\theta^{(\mu)}(j,s) + E_{\theta}^{t+1,s}\\
%&= r_{\theta}^{(\mu)}(t+1,s) + E_{\theta}^{t+1,s}, 
%\end{align*}
%where the remainder term is 
%\begin{align*}
%E_{\theta}^{t+1,s} &= \Big(1 - \frac{\gamma\delta}{\sigma^2} - \gamma f''(\mu^t)\Big) E_\theta^{t,s} + \frac{\gamma}{\sigma^2}(\delta - \pnorm{\x}{}^2) (r_\theta^{(\mu)} + E_\theta^{t,s})\\
%&\quad - \gamma \sum_{j=s+1}^{t-1} R_\eta^{(\mu)}(t,j) \cdot E_\theta^{j,s} + \Big(\frac{\gamma}{\sigma^2}\Big)^2 \sum_{j=s+1}^{t-1} \Big(\frac{\sigma^4}{\gamma}R_\eta^{(\mu)}(t,j) + \iprod{\bar{\X}^\top \x}{\Omega^{t-1}\ldots \Omega^{j+1} \bar{\X}^\top \x}\Big) \cdot (r_\theta^{(\mu)}(j,s) + E_\theta^{j,s})
%\end{align*}

\textbf{Claim for $\partial_\eps|_{\eps = 0} \bbeta_i^{t,[s,i], \eps}$} Same as above, by symmetry let us study the last component $\kappa^{t,[s],\eps} = \bbeta_n^{t,[s,n],\eps}$ and shorthand $\bbeta^{t,[s,n], \eps}$ (resp. $\btheta^{t,[s,n], \eps}$) as $\bbeta^{t,[s], \eps}$ (resp. $\btheta^{t,[s], \eps}$). If $s = t$, direct calculation via (\ref{eq:theta_col_perturb}) shows that $\partial_\eps \kappa = \gamma \pnorm{\X^\top \e_n}{}^2 = \gamma + E^{t+1,[t,n]}_\eta$ with $E^{t+1,[t,n]}_\eta \rightarrow_{a.s.} 0$, while $r_\eta(t+1,t) = \gamma/\sigma^2$, establishing the desired claim. In what follows, we fix $s < t$. By definition, if we write $\bbeta^{t,[s],\eps} = [\bar{\bbeta}^{t,[s],\eps}, \kappa^{t,[s],\eps}]$ with $\bar{\bbeta}^{t,[s],\eps}\in\R^{n-1}$ and $\kappa^{t,[s],\eps}\in\R$, $\X = [\bar{\X}; \x^\top]$ with $\bar{\X} \in \R^{(n-1)\times d}$ and $\x\in\R^d$, and $\y = [\bar{\y}; y_n]$ with $\bar{\y}\in \R^{n-1}, y_n\in\R$, then
\begin{align*}
\bar{\bbeta}^{t+1,[s], \eps} &= \bar{\bbeta}^{t,[s], \eps} + \gamma\Big[-\frac{1}{\sigma^2} \bar{\X} \big(\bar{\X}^\top (\bar{\bbeta}^{t,[s], \eps} - \bar{\y}) + \x (\kappa^{t,[s], \eps} - y_n)\big) + \bar{\X} \partial_\theta \log g(\btheta^{t,[s],\eps};\hat\alpha^{t,[s],\eps}) \Big] + \sqrt{2}\bar{\X}(\b^{(t+1)\gamma} - \b^{t\gamma}), \\
\kappa^{t+1,[s],\eps} &= \kappa^{t,[s], \eps} + \gamma\Big[-\frac{1}{\sigma^2} \x^\top \big(\bar{\X}^\top (\bar{\bbeta}^{t,[s], \eps} - \bar{\y}) + \x (\kappa^{t,[s], \eps} - y_n)\big) + \x^\top \partial_\theta \log g(\btheta^{t,[s], \eps};\hat\alpha^{t,[s], \eps}) \Big] + \sqrt{2}\x^\top (\b^{(t+1)\gamma} - \b^{t\gamma}),\\
\hat\alpha^{t+1,[s],\eps} &= \hat\alpha^{t,[s],\eps} + \gamma \cG(\hat\alpha^{t,[s],\eps} + \Prob_n(\btheta^{t,[s],\eps})). 
\end{align*}
Taking $\eps$ derivative of $\kappa^{t+1,[s],\eps}$ yields
\begin{align}\label{eq:kappa_expand}
\notag &\partial_\eps|_{\eps = 0}\kappa^{t+1,[s],\eps}\\
&\notag= \Big(1 - \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2\Big)\deps \kappa^{t,[s],\eps} - \frac{\gamma}{\sigma^2} \x^\top \bar{\X}^\top \deps \bar{\bbeta}^{t,[s], \eps} + \gamma \x^\top \diag(\partial_\theta^2 \log g(\btheta^{t}; \hat\alpha^t))\deps  \btheta^{t,[s],\eps}\\
&\notag\quad + \gamma\underbrace{\x^\top \partial_\theta\nabla_{\alpha} \log g(\btheta^t; \hat\alpha^t) \deps \hat\alpha^{t,[s],\eps}}_{\rho^{t,[s]}}\\
\notag&= \Big(1 - \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2\Big)\deps \kappa^{t,[s],\eps} + \x^\top\Big(-\frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta^2 \log g(\btheta^t;\hat\alpha^t))\Big)\deps \btheta^{t,[s],\eps} + \gamma\rho^{t,[s]}\\
&= \Big(1 - \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2\Big)\deps \kappa^{t,[s],\eps} - \x^\top \deps \btheta^{t,[s],\eps} + \x^\top \underbrace{\Big(I-\frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta^2 \log g(\btheta^t;\hat\alpha^t))\Big)}_{\Gamma^t}\deps \btheta^{t,[s],\eps}  + \gamma\rho^{t,[s]}.
\end{align}
To evaluate $\deps  \btheta^{t,[s],\eps}$, let $\brho^{t,[s]} = \partial_\theta\nabla_{\alpha} \log g(\btheta^t; \hat\alpha^t) \deps \hat\alpha^{t,[s],\eps} \in \R^d$, then
\begin{align*}
\partial_\eps|_{\eps = 0} \btheta^{t,[s], \eps} &= \Big(I - \frac{\gamma}{\sigma^2}\X^\top \X + \gamma\diag(\partial_\theta^2 \log g(\btheta^{t-1};\hat\alpha^{t-1}))\Big)\partial_\eps|_{\eps = 0} \btheta^{t-1,[s], \eps} + \gamma \brho^{t-1,[s]}\\
&= \underbrace{\Big(I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} + \gamma\diag(\partial_\theta^2 \log g(\btheta^{t-1}; \hat\alpha^{t-1}))\Big)}_{\Gamma^{t-1}}\partial_\eps|_{\eps = 0} \btheta^{t-1,[s], \eps} - \frac{\gamma}{\sigma^2}\x \deps \kappa^{t-1,[s], \eps} + \gamma \brho^{t-1,[s]}\\
&= \Gamma^{t-1} \Big(\Gamma^{t-2} \partial_\eps|_{\eps = 0} \btheta^{t-2,[s], \eps} - \frac{\gamma}{\sigma^2}\x \deps \kappa^{t-2,[s], \eps} +  \gamma \brho^{t-2,[s]}\Big)- \frac{\gamma}{\sigma^2}\x \deps \kappa^{t-1,[s], \eps} \gamma \brho^{t-1,[s]} \\
&= \ldots\\
&= \Gamma^{t-1}\ldots \Gamma^{s+1} \partial_\eps|_{\eps = 0} \btheta^{s+1,[s], \eps} - \frac{\gamma}{\sigma^2}\sum_{j=s+1}^{t-2} \Gamma^{t-1}\ldots \Gamma^{j+1} \x \cdot  \deps \kappa^{j,[s], \eps} - \frac{\gamma}{\sigma^2}\x \cdot \deps \kappa^{t-1,[s], \eps}\\
&\quad + \gamma \sum_{j=s+1}^{t-2} \Gamma^{t-1}\ldots \Gamma^{j+1} \brho^{j,[s]} + \gamma \brho^{t-1,[s]}\\
&= \gamma \Gamma^{t-1}\ldots \Gamma^{s+1}\x - \frac{\gamma}{\sigma^2}\sum_{j=s+1}^{t-2} \Gamma^{t-1}\ldots \Gamma^{j+1} \x \cdot  \deps \kappa^{j,[s], \eps} - \frac{\gamma}{\sigma^2}\x \cdot \deps \kappa^{t-1,[s], \eps}\\
&\quad + \gamma \sum_{j=s+1}^{t-2} \Gamma^{t-1}\ldots \Gamma^{j+1} \brho^{j,[s]} + \gamma \brho^{t-1,[s]},
\end{align*}
using the fact that $\partial_\eps|_{\eps = 0} \btheta^{s+1,[s], \eps} = \gamma \x$. Plugging the above expression into (\ref{eq:kappa_expand}), we have
\begin{align}\label{eq:kappa_expand_2}
\notag\partial_\eps|_{\eps = 0}\kappa^{t+1,[s],\eps} &= \Big(1 - \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2\Big)\deps \kappa^{t,[s],\eps} - \gamma \x^\top\Gamma^{t-1}\ldots \Gamma^{s+1}\x + \frac{\gamma}{\sigma^2}\sum_{j=s+1}^{t-2} \x^\top\Gamma^{t-1}\ldots \Gamma^{j+1}\x \cdot  \deps \kappa^{j,[s], \eps}\\
\notag&\quad +  \frac{\gamma}{\sigma^2} \pnorm{\x}{}^2 \cdot \deps \kappa^{t-1,[s], \eps} + \gamma \x^\top\Gamma^t\Gamma^{t-1}\ldots \Gamma^{s+1}\x - \frac{\gamma}{\sigma^2}\sum_{j=s+1}^{t-2} \x^\top\Gamma^t\Gamma^{t-1}\ldots \Gamma^{j+1}\x \cdot  \deps \kappa^{j,[s], \eps}\\
&\quad - \frac{\gamma}{\sigma^2} \x^\top\Gamma^t \x \cdot \deps \kappa^{t-1,[s], \eps} + \gamma\x^\top (\Gamma^t - I)\Big(\sum_{j=s+1}^{t-2} \Gamma^{t-1}\ldots \Gamma^{j+1}\brho^{j,[s]} + \brho^{t-1,[s]}\Big).
\end{align}
Let us analyze the terms one by one. 

\noindent\textbf{First term} Using induction hypothesis, the first term satisfies
\begin{align*}
\Big(1 - \frac{\gamma}{\sigma^2}\pnorm{\x}{}^2\Big)\deps \kappa^{t,[s],\eps} = \Big(1 - \frac{\gamma}{\sigma^2}\Big) \sigma^2 r_\eta(t,s) + \mathsf{r}_1^{[n]},
\end{align*}
with $n^{-1}\sum_{i=1}^n \mathsf{r}_1^{[i]} \rightarrow_{a.s.} 0$. 

\noindent\textbf{Second term} Let $\Gamma^t_{[n]} = I - \frac{\gamma}{\sigma^2} \bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta^2 \log g(\btheta^t_{[n]}; \hat\alpha^t_{[n]}))$ with $\btheta^t_{[n]}, \hat\alpha^t_{[n]}$ given in (\ref{eq:leave_row_out}). We claim that
\begin{align}\label{eq:claim_2}
\Big|\x^\top \Gamma^{t-1}\ldots \Gamma^{s+1}\x - \x^\top\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\x\Big| \leq C\sqrt{\frac{\log d}{d}}(|\eps_d| + \sqrt{\log d}). 
\end{align}
To see this, note that
\begin{align*}
\Big|\x^\top\Gamma^{t-1}\ldots \Gamma^{s+1}\x - \x^\top\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\x\Big| \leq \sum_{\ell=s+1}^{t-1} \Big|\underbrace{\x^\top\Gamma^{t-1}_{[n]} \ldots \Gamma^{\ell+1}_{[n]} (\Gamma^{\ell}_{[n]} - \Gamma^{\ell}) \Gamma^{\ell-1} \ldots \Gamma^{s+1}\x}_{S^\ell_{[n]}}\Big|,
\end{align*}
where $\Gamma^{\ell}_{[n]} - \Gamma^{\ell} = \gamma(\diag(\partial_\theta^2 \log g(\btheta^{\ell}_{[n]}; \hat\alpha^{\ell}_{[n]})) - \diag(\partial_\theta^2 \log g(\btheta^{\ell}; \hat\alpha^\ell)))$. Hence by Assumption \ref{assump:prior}, each $S^\ell_{[n]}$ satisfies
\begin{align*}
|S^\ell_{[n]}| &= \gamma\Big|\big(\Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1} \x \circ \Gamma^{\ell-1} \ldots \Gamma^{s+1}\x\big)^\top \big(\partial_\theta^2 \log g(\btheta^{\ell}_{[n]}; \hat\alpha^{\ell}_{[n]})) - \partial_\theta^2 \log g(\btheta^{\ell}; \hat\alpha^\ell)\big)\Big|\\
&\leq C\gamma \pnorm{\Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1} \x}{\infty}\pnorm{\Gamma^{\ell-1}}{\op}\ldots \pnorm{\Gamma^{s+1}}{\op}\pnorm{\x}{} \cdot \big(\pnorm{\btheta^{\ell} - \btheta^{\ell}_{[n]}}{} + \pnorm{\hat\alpha^{\ell} - \hat\alpha^{\ell}_{[n]}}{}\big).
%\pnorm{\x}{}^2 \pnorm{\Gamma^{t-1}_{[n]}}{\op}\ldots \pnorm{\Gamma^{\ell+1}_{[n]}}{\op} \pnorm{\Gamma^{\ell+1}_{[n]} - \Gamma^{\ell+1}}{\op} \pnorm{\Gamma^{\ell}}{\op}\ldots  \pnorm{\Gamma^{s+1}}{\op}\\
%&\leq \pnorm{\x}{}^2 \prod_{s+1\leq k\leq t-1:k\neq \ell} (1 + \pnorm{\bar{\X}}{\op}^2 + \gamma \pnorm{f''}{\infty}) \cdot \gamma \pnorm{f'''}{\infty} \pnorm{\bar{\btheta}^\ell - \bar{\btheta}^\ell_{[n]}}{\infty}. 
\end{align*}
Since $\x$ is independent of $\Gamma_{[n]}^{\ell+1},\ldots, \Gamma_{[n]}^{t+1}$, for each $j\in[d]$ and $\e_j \in \R^d$, we have
\begin{align*}
\e_j^\top \Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1} \x | \Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1} \sim \N(0, \frac{1}{d}\pnorm{(\Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1})^\top \e_j}{}^2),
\end{align*}
where
\begin{align*}
\pnorm{(\Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1})^\top \e_j}{} \leq \pnorm{\Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1}}{\op}\leq \pnorm{\Gamma_{[n]}^{\ell+1}}{\op}\ldots\pnorm{\Gamma_{[n]}^{t+1}}{\op}.
\end{align*}
Hence using the bound $\pnorm{\Gamma^\ell}{\op}\vee \pnorm{\Gamma^\ell_{[n]}}{\op} \leq 1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + C\gamma$ and a standard tail bound on $\pnorm{\X}{\op}$, we conclude that almost surely $\pnorm{\Gamma_{[n]}^{\ell+1}\ldots \Gamma_{[n]}^{t+1} \x}{\infty} \leq C\sqrt{\log d/d}$. By Lemma \ref{lem:loo_error}, we conclude (\ref{eq:claim_2}). 
%Hence by a standard tail bound on $\pnorm{\bar{\X}}{\op}$ and Lemma \ref{lem:loo_error}, we have
%\begin{align*}
%\E[T_\ell^2] \leq \gamma\pnorm{f'''}{\infty} \cdot (\E \pnorm{\x}{}^{16})^{1/4} \cdot \Big[\E \Big(1 + \pnorm{\bar{\X}}{\op}^2 + \gamma \pnorm{f''}{\infty}\Big)^{8(t-s-2)}\Big]^{1/4} \cdot \Big(\E \pnorm{\bar{\btheta}^\ell - \bar{\btheta}^\ell_{[n]}}{\infty}^4\Big)^{1/2} \rightarrow 0,
%\end{align*}
%establishing (\ref{eq:claim_2}). 
Now note that $\{\Gamma^t_{[n]}\}$ is independent of $\x$, so in (\ref{eq:claim_2}) applying Hanson-Wright yields
\begin{align*}
\Prob\Big(\Big|\x^\top\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\x - \frac{1}{d}\Tr\Big(\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\Big)\Big|>t | \bar{\X}\Big) \leq \exp\Big(-c\frac{d^2t^2}{\pnorm{\tilde{W}}{F}^2} \wedge\frac{dt}{\pnorm{\tilde{W}}{\op}} \Big),
\end{align*}
where $\tilde{W} = \Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}$. Hence using $\pnorm{\Gamma^\ell_{[n]}}{\op} \leq 1 + \frac{\gamma}{\sigma^2}\pnorm{\X}{\op}^2 + C\gamma$, we have by Borel-Cantelli lemma that
%conditioning on the event $\cA = \{\max_{\ell\leq t} \max_{i\in [n]}\pnorm{\Gamma^\ell_{[i]}}{\op}\leq C\}$ with large enough $C$ which holds with probability $1 - \exp(-cn)$, 
\begin{align*}
\x^\top\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\x - \frac{1}{d}\Tr\Big(\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\Big) \rightarrow_{a.s.} 0.
\end{align*}
Moreover, by the analogue of second equation of (\ref{eq:induction_consequence}) for system size $(n-1,d)$, we have
%\red{Assume concentration}, then
%\begin{align*}
%\E\Big[\frac{1}{d}\Tr\Big(\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\Big) - \frac{1}{d}\E\Big(\Tr\Big(\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\Big)\Big)\Big]^2 \rightarrow 0.
%\end{align*}
%By the fact (\ref{eq:fact_1}) applied with system size $(n-1,p)$, we have (recall that $\mu$ denotes the last component of $\btheta$)
\begin{align*}
\frac{1}{d}\Tr\Big(\Gamma^{t-1}_{[n]}\ldots \Gamma^{s+1}_{[n]}\Big) \rightarrow_{a.s.} \gamma^{-1} \cdot \bar{R}_\theta^{\gamma}(t,s),
\end{align*}
so in summary we have shown that, for some $\{\mathsf{r}_2^{[i]}\}_{i=1}^n$ such that $\langle n^{-1}\sum_{i=1}^n \mathsf{r}_2^{[i]} \rangle \rightarrow_{a.s.} 0$,
\begin{align*}
- \gamma \x^\top\Gamma^{t-1}\ldots \Gamma^{s+1}\x = - \bar{R}_\theta^{\gamma}(t,s) + \mathsf{r}_2^{[n]}.
\end{align*}
\noindent\textbf{Remaining terms} Similar analysis as above further shows: for some $\mathsf{r}_\ell^{[i]}$, $3\leq \ell \leq 7$ such that $\langle n^{-1}\sum_{i=1}^n \mathsf{r}_\ell^{[i]}\rangle \rightarrow_{a.s.} 0$, 
\begin{align*}
\frac{\gamma}{\sigma^2}\sum_{j=s+1}^{t-2} \x^\top\Gamma^{t-1}\ldots \Gamma^{j+1}\x \cdot  \deps \kappa^{j,[s], \eps} &= \sum_{j=s+1}^{t-2} \bar{R}_\theta^{\gamma}(t,j) r_\eta(j,s) + \mathsf{r}_3^{[n]},\\
\frac{\gamma}{\sigma^2} \pnorm{\x}{}^2 \cdot \deps \kappa^{t-1,[s], \eps} &= \gamma r_\eta(t-1,s) + \mathsf{r}_4^{[n]},\\
\gamma \x^\top\Gamma^t\Gamma^{t-1}\ldots \Gamma^{s+1}\x &\stackrel{(i)}{=} \bar{R}_\theta^{\gamma}(t+1,s) + \mathsf{r}_5^{[n]},\\
- \frac{\gamma}{\sigma^2}\sum_{j=s+1}^{t-2} \x^\top\Gamma^t\Gamma^{t-1}\ldots \Gamma^{j+1}\x \cdot  \deps \kappa^{j,[s], \eps} &\stackrel{(ii)}{=} -\sum_{j=s+1}^{t-2} \bar{R}_\theta^{\gamma}(t+1,j) r_\eta(j,s) + \mathsf{r}_6^{[n]},\\
- \frac{\gamma}{\sigma^2} \x^\top\Gamma^t \x \cdot \deps \kappa^{t-1,[s], \eps} &\stackrel{(iii)}{=} -\bar{R}_\theta^{\gamma}(t+1,t-1) r_\eta(t-1,s) + \mathsf{r}_7^{[n]},
\end{align*}
where in (i)-(iii) we have used (the size-$(n-1,d)$ analogue of) (\ref{eq:fact_3}). Lastly, we claim that the last term of (\ref{eq:kappa_expand_2}), namely $\gamma\x^\top (\Gamma^t - I)\Big(\sum_{j=s+1}^{t-2} \Gamma^{t-1}\ldots \Gamma^{j+1}\brho^{j,[s]} + \brho^{t-1,[s]}\Big)$ is $o_{a.s.}(1)$ when averaged over the coordinates. This follows from a similar leave-one-out argument applied in (\ref{eq:theta_loo_arg}), along with Lemma \ref{lem:response_l2_estimate}.




Let $E_\eta^{t+1,[s,n]} = \sum_{\ell=1}^7 \mathsf{r}_\ell^{[n]}$ so that $n^{-1} E_\eta^{t+1,[s,i]} \rightarrow_{a.s.} 0$. Plugging the above expressions into (\ref{eq:kappa_expand_2}), we have
\begin{align*}
\deps \kappa^{t+1,[s],\eps} &= \Big(1 - \frac{\gamma}{\sigma^2}\Big) \sigma^2 r_\eta(t,s) + \bar{R}_\theta^{\gamma}(t+1,s) - \sum_{j=s+1}^{t-1} \bar{R}_\theta^{\gamma}(t+1,j) r_\eta(j,s) - \bar{R}_\theta^{\gamma}(t,s)\\
&\quad + \sum_{j=s+1}^{t-1} \bar{R}_\theta^{\gamma}(t,j) r_\eta(j,s) + E_\eta^{t+1,[s,n]}\\
&= \Big[-\gamma \cdot r_\eta(t,s) + \bar{R}_\theta^{\gamma}(t+1,s) - \sum_{j=s+1}^{t-1} \bar{R}_\theta^{\gamma}(t+1,j) r_\eta(j,s)\Big] + E_\eta^{t+1,[s,n]}\\
&\quad + \underbrace{\Big[\sigma^2 r_\eta(t,s) - \bar{R}_\theta^{\gamma}(t,s)  + \sum_{j=s+1}^{t-1} \bar{R}_\theta^{\gamma}(t,j) r_\eta(j,s)\Big]}_{=0}\\
&= \bar{R}_\theta^{\gamma}(t+1,s) - \sum_{j=s+1}^{t} \bar{R}_\theta^{\gamma}(t+1,j) r_\eta(j,s) + E_\eta^{t+1,[s,n]}\\
&= \sigma^2 r_\eta(t+1,s) + E_\eta^{t+1,[s,n]}, 
\end{align*}
by definition of the system (\ref{eq:dmft_response_rho}). This concludes the induction of this step.
%To evaluate $\deps \bbeta^{t,[s], \eps}$, we have
%\begin{align*}
%\deps \bbeta^{t+1,[s], \eps} &= \underbrace{\Big(I - \frac{\gamma}{\sigma^2}\bar{\X}\bar{\X}^\top\Big)}_{\Lambda} \deps\bbeta^{t,[s], \eps} + \underbrace{\Big(-\frac{\gamma}{\sigma^2}\bar{\X}\x \deps  \kappa^{t,[s], \eps} - \gamma \bar{\X} \diag(f''(\btheta^{t})) \deps \btheta^{t,[s],\eps}\Big)}_{V_t}\\
%&= \Lambda (\Lambda \deps\bbeta^{t-1,[s], \eps} + V_{t-1}) + V_t\\
%&= \ldots = \Lambda^{t-s}  \deps\bbeta^{s+1,[s], \eps} + \sum_{j=s+1}^{t} \Lambda^{t-j} V_j = \gamma \Lambda^{t-s}  \bar{\X}\x + \sum_{j=s+1}^{t} \Lambda^{t-j} V_j.
%%& = \Lambda^{t-s}  \deps\bbeta^{s+1,[s], \eps} +  \Lambda^{t-s-1} V_{s+1} + \ldots + \Lambda V_{t-1} + V_t\\
%%&= \gamma \Lambda^{t-s}  \bar{\X}\x + \Lambda^{t-s-1} V_{s+1} + \ldots + \Lambda V_{t-1} + V_t, 
%\end{align*}
%using the fact that $\deps\bbeta^{s+1,[s], \eps} = \gamma \bar{\X}\x$. Plugging the above two expressions into (\ref{eq:kappa_expand}), we have
%\begin{align*}
%\partial_\eps|_{\eps = 0}\kappa^{t+1,[s],\eps} &= \underbrace{\Big(1 - \frac{\pnorm{\x}{}^2}{\sigma^2}\Big)\deps \kappa^{t,[s],\eps}}_{(I)} - \frac{\gamma^2}{\sigma^2} \underbrace{\iprod{\bar{\X}\x}{ \Lambda^{t-s-1}  \bar{\X}\x}}_{(II)} - \frac{\gamma}{\sigma^2} \underbrace{\iprod{\bar{\X}\x}{\sum_{j=s+1}^{t-1} \Lambda^{t-j-1} V_j}}_{(III)}\\
%&\quad - \gamma^2 \underbrace{\x^\top \diag(f''(\btheta^{t}))B_{t-1}\ldots B_{s+1} \x}_{(IV)} + \frac{\gamma^2}{\sigma^2} \underbrace{\sum_{j=s+1}^{t-1} \x^\top \diag(f''(\btheta^{t})) B_{t-1}\ldots B_{j+1} \x \cdot  \deps \kappa^{j,[s], \eps}}_{(V)}.
%\end{align*}
%Let $B^{t}_{[n]} = I -\frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} - \gamma \diag(f''(\bar{\btheta}^{j}_{[n]})) \in\R^{p\times p}$, with $\{\bar{\btheta}^{t}_{[n]}\}$ given by the leave-one-column-out version of (\ref{eq:original})
%\begin{align*}
%\bar{\btheta}^{t}_{[n]} = \bar{\btheta}^{t-1}_{[n]} - \gamma\Big[\frac{1}{\sigma^2}\bar{\X}^\top(\bar{\X}\bar{\btheta}^{t-1}_{[n]} - \y_{[n]}) + f'(\bar{\btheta}^{t-1}_{[n]})\Big] \in \R^{d}.
%\end{align*}
%Then $(V)$ satisfies
%\begin{align*}
%(V) \approx
%\end{align*}
\end{proof}

\begin{lemma}\label{lem:A_trace}
Let $\{\btheta^t,\alpha^t\}$ be given by (\ref{eq:original_theta})-(\ref{eq:original_alpha}). For each $t\in\Z_+$ define the matrix
\begin{align}\label{def:A_matrix}
A_t = I - \frac{\gamma}{\sigma^2}\X^\top \X + \gamma\diag(\partial_\theta^2 \log g(\btheta^{t}; \hat\alpha^{t})) \in \R^{d\times d}.
\end{align}
Then for any fixed $s \leq t$, almost surely as $n,d\rightarrow\infty$
\begin{align*}
\frac{1}{d}\sum_{j=1}^{d} \partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps} - \frac{\gamma}{d}\Tr\Big(A_{t-1}\ldots A_{s+1}\Big) &\rightarrow 0,\\
\frac{1}{n}\sum_{i=1}^n \partial_\eps|_{\eps = 0}\bbeta_i^{t,[s,i], \eps} - \frac{\gamma}{n}\Tr\Big(\X A_{t-1}\ldots A_{s+1} \X^\top\Big) &\rightarrow 0.
\end{align*}
\end{lemma}
\begin{proof}
By definition, with $\r^{t,(s,j)} := \partial_\theta\nabla_\alpha \log g(\btheta^t;\hat\alpha^t) \deps \hat\alpha^{t,(s,j),\eps} \in \R^d$, we have
\begin{align*}
\partial_\eps|_{\eps = 0} \btheta^{t,(s,j), \eps} &= \underbrace{\Big(I - \frac{\gamma}{\sigma^2}\X^\top \X + \gamma\diag(\partial_\theta^2 \log g(\btheta^{t-1}; \hat\alpha^{t-1}))\Big)}_{A_{t-1}}\partial_\eps|_{\eps = 0} \btheta^{t-1,(s,j), \eps} + \gamma \r^{t-1,(s,j)}\\
&= A_{t-1}(A_{t-2} \partial_\eps|_{\eps = 0} \btheta^{t-2,(s,j), \eps} + \gamma \r^{t,(s,j),\eps}) + \gamma \r^{t-1,(s,j)}\\
&= \ldots = A_{t-1}\ldots A_{s+1} \partial_\eps|_{\eps = 0}\btheta^{s+1,(s,j), \eps} + \gamma\sum_{\ell=s+1}^{t-2} A^{t-1}\ldots A^{\ell+1} \r^{\ell,(s,j)\eps} + \gamma \r^{t-1,(s,j)}\\
&= \gamma A_{t-1}\ldots A_{s+1} \e_j + \gamma\sum_{\ell=s+1}^{t-2} A^{t-1}\ldots A^{\ell+1} \r^{\ell,(s,j)\eps} + \gamma \r^{t-1,(s,j)},
\end{align*}
which implies
\begin{align*}
\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \btheta^{t,(s,j), \eps} = \frac{\gamma}{d}\Tr \big(A_{t-1}\ldots A_{s+1}\big) + \frac{\gamma}{d} \sum_{\ell=s+1}^{t-1} \sum_{j=1}^d \e_j^\top A^{t-1}\ldots A^{\ell+1} \r^{\ell,(s,j)} + \frac{\gamma}{d}  \sum_{j=1}^d \e_j^\top\r^{t-1,(s,j)}.
\end{align*}
We show the latter two terms are $o_{a.s.}(1)$. Fix $s+1\leq\ell\leq t-1$, and let $U = A^{t-1}\ldots A^{\ell+1} \partial_\theta\nabla_\alpha \log g(\btheta^t;\hat\alpha^t) \in \R^{d\times K}$, then using $\pnorm{U}{F} \leq \pnorm{A^{t-1}}{\op}\ldots\pnorm{A^{\ell+1}}{\op} \pnorm{\partial_\theta\nabla_\alpha \log g(\btheta^t;\hat\alpha^t)}{F} \leq C\sqrt{d}$ via Assumption \ref{assump:prior} and Lemma \ref{lem:response_l2_estimate}, 
\begin{align*}
\Big|\sum_{j=1}^d \e_j^\top A^{t-1}\ldots A^{\ell+1} \r^{\ell,(s,j)\eps}\Big| = \Big|\sum_{j=1}^d U_{j\cdot}^\top \deps \hat\alpha^{t,(s,j),\eps}\Big| \leq \pnorm{U}{F}\sqrt{\sum_{j=1}^d \pnorm{\deps\hat\alpha^{t,(s,j),\eps}}{}^2} \leq C\sqrt{d},
\end{align*}
which shows that $d^{-1}\sum_{j=1}^d \e_j^\top A^{t-1}\ldots A^{\ell+1} \r^{\ell,(s,j)} = o_{a.s.}(1)$. A similar argument applies to $d^{-1}\sum_{j=1}^d \e_j^\top\r^{t-1,(s,j)}$, proving the first claim.
%This entails that
%\begin{align*}
%d^{-1}\sum_{j=1}^{d} \partial_\eps|_{\eps = 0} \btheta_j^{t,(s,j), \eps} = \gamma \cdot \frac{1}{d}\Tr\Big(A_{t-1}\ldots A_{s+1}\Big),
%\end{align*}
%and hence we conclude by symmetry
%\begin{align}\label{eq:fact_1}
%\frac{1}{d}\E\Big[\Tr\Big(A_{t-1}\ldots A_{s+1}\Big)\Big] = \gamma^{-1} \E\Big[\partial_\eps|_{\eps = 0} \btheta_d^{t,(s,d),\eps}\Big] = \gamma^{-1} R_\theta^{(\mu)}(t,s) + o_n(1).
%\end{align}
For the second claim, similar arguments as above yields
\begin{align}\label{eq:theta_derivative_2}
\partial_\eps|_{\eps = 0} \btheta^{t,[s,i], \eps} &= \gamma A_{t-1}\ldots A_{s+1} \X^\top \e_i + \gamma\sum_{\ell=s+1}^{t-2} A^{t-1}\ldots A^{\ell+1} \r^{\ell,[s,i]\eps} + \gamma \r^{t-1,[s,i],\eps},
\end{align}
and hence
\begin{align*}
\frac{1}{n}\sum_{i=1}^n \partial_\eps|_{\eps = 0} \bbeta^{t,[s,i], \eps} = \frac{\gamma}{n}\Tr \big(\X A_{t-1}\ldots A_{s+1} \X^\top\big) + \frac{\gamma}{n} \sum_{\ell=s+1}^{t-1} \sum_{i=1}^n \e_i^\top \X A^{t-1}\ldots A^{\ell+1} \r^{\ell,[s,i],\eps} + \frac{\gamma}{n}  \sum_{i=1}^n \e_i^\top \X\r^{t-1,[s,i],\eps},
\end{align*}
where $\r^{t,[s,i],\eps} := \partial_\theta\nabla_\alpha \log g(\btheta^t;\hat\alpha^t) \deps \hat\alpha^{t,[s,i],\eps} \in \R^d$. Similar arguments as above show that for each $s+1\leq \ell \leq t-2$, $d^{-1}\sum_{i=1}^n \e_i^\top \X A^{t-1}\ldots A^{\ell+1} \r^{\ell,[s,i],\eps} = o_{a.s.}(1)$, and similarly for $n^{-1}\sum_{i=1}^n \e_i^\top \X\r^{t-1,[s,i],\eps}$, yielding the second claim.
%This implies
%\begin{align*}
%n^{-1}\sum_{i=1}^n \partial_\eps|_{\eps = 0}\bbeta_i^{t,[s,i], \eps} = \gamma \cdot \frac{1}{n}\Tr\Big(\X A_{t-1}\ldots A_{s+1} \X^\top\Big),
%\end{align*}
%and hence we conclude by symmetry
%\begin{align}\label{eq:fact_2}
%\frac{1}{n}\E\Big[\Tr\Big(\X A_{t-1}\ldots A_{s+1} \X^\top\Big)\Big] = \gamma^{-1} \E\Big[\partial_\eps|_{\eps = 0}\bbeta_n^{t,[s,n], \eps}\Big] = -\frac{\sigma^4}{\delta\gamma} R_\eta^{(\mu)}(t,s) + o_n(1)
%\end{align}
\end{proof}

\subsection{Step 3: Discretization of DMFT response function}

Recall $\{\bar{R}_\theta^\gamma(i,j)\}$ and $\{\bar{R}_\eta^\gamma(i,j)\}$ defined in (\ref{eq:dmft_response}).
\begin{proposition}\label{eq:response_discre_error}
Fix any $\gamma > 0$. For any $T > 0$, there exists some $C > 0$ depending on the parameters of $\cS_\theta$ and $\cS_\eta$ such that for any $s\leq t\leq T$,
\begin{align*}
|\bar{R}^\gamma_\theta([t],[s]) - \gamma R_\theta(t,s)| \vee |\bar{R}^\gamma_\eta([t],[s]) - \gamma R_\eta(t,s)| \leq C\sqrt{\gamma}.
\end{align*}
\end{proposition}
\begin{proof}
We only prove the claim for $R_\theta(t,s)$, and the claim involving $R_\eta(t,s)$ will follow similarly. By the correspondence (\ref{eq:induction_piecelinear_theta}), we have $\bar{R}^\gamma_\theta([t],[s]) = R^\gamma_\theta(\floor{t},\gamma([s]+1)) = R^\gamma_\theta(\floor{t},\ceil{s})$, and
\begin{align*}
|R_\theta(t,s) - R^\gamma_\theta(\floor{t},\ceil{s})| \leq |R_\theta(t,s) - R^\gamma_\theta(t,s)| + |R^\gamma_\theta(t,s) - R^\gamma_\theta(\floor{t},\ceil{s})|. 
\end{align*} 
Using analogous arguments to those that lead to (\ref{eq:eta_response_discre_error}), the first term is bounded by $C\sqrt{\gamma}$. The second term is bounded by $C\gamma$ by Lemma \ref{lem:response_discretization_error}, concluding the proof. 
\end{proof}


\subsection{Completing the proof}
We first prove the claim for $\bR_\theta(t,s)$. Recall that for any $\gamma > 0$, $[t] = \floor{t}/\gamma$ with $\floor{t}$ given in (\ref{eq:t_floor_ceil}). For any $\gamma > 0$, we have
\begin{align*}
\Big|\frac{1}{d}\langle \Tr \bR_\theta(t,s) \rangle - R_\theta(t,s)\Big| &\leq \Big|\frac{1}{d}\langle\Tr \bR_\theta(t,s) \rangle - \frac{1}{d} \langle\Tr \bR_\theta^\gamma([t], [s]) \rangle\Big| + \Big|\frac{1}{d}\langle\Tr \bR_\theta^\gamma([t], [s]) \rangle- \frac{1}{\gamma}\bar{R}_\theta^\gamma([t],[s])\Big|\\
&\quad + \Big|\frac{1}{\gamma}\bar{R}_\theta^\gamma([t],[s]) - R_\theta(t,s)|.
\end{align*}
By Proposition \ref{prop:discrete_time_response}, we have
\begin{align*}
\frac{1}{d}\langle \Tr \bR_\theta^\gamma([t], [s]) \rangle = \frac{1}{\gamma}\Big\langle\frac{1}{d}  \sum_{j=1}^d \deps \btheta^{[t],([s],j),\eps}_j \Big\rangle \rightarrow_{a.s.}  \frac{1}{\gamma}\bar{R}^\gamma_\theta([t],[s]).
\end{align*}
Hence almost surely as $n,d\rightarrow\infty$
\begin{align*}
\limsup_{n,d} \Big|\frac{1}{d}\langle\Tr \bR_\theta(t,s)\rangle - R_\theta(t,s)\Big| \leq \limsup_{n,d}\Big\langle\Big|\frac{1}{d}\Tr \bR_\theta(t,s) - \frac{1}{d}\Tr \bR_\theta^\gamma([t], [s])\Big|\Big\rangle + \Big|\frac{1}{\gamma}\bar{R}_\theta^\gamma([t],[s]) - R_\theta(t,s)|.
\end{align*}
The above inequality holds for any $\gamma > 0$, so the conclusion follows by taking $\gamma \rightarrow 0$ and applying Propositions \ref{prop:semigroup_discre_error} and \ref{eq:response_discre_error}. The claim for $\bR_\eta(t,s)$ by using
\begin{align*}
\Big|\frac{1}{n}\langle\Tr \bR_\eta(t,s)\rangle - R_\eta(t,s)\Big| &\leq \Big\langle\Big|\frac{1}{n}\Tr \bR_\eta(t,s) - \frac{1}{n}\Tr \bR_\eta^\gamma([t], [s])\Big|\Big\rangle + \Big|\frac{1}{n}\langle\Tr \bR_\eta^\gamma([t], [s])\rangle - \frac{1}{\gamma}\bar{R}_\eta^\gamma([t],[s])\Big|\\
&\quad + \Big|\frac{1}{\gamma}\bar{R}_\eta^\gamma([t],[s]) - R_\eta(t,s)|,
\end{align*}
where Proposition \ref{prop:discrete_time_response} yields
\begin{align*}
\frac{1}{n}\langle\Tr \bR_\eta^\gamma([t], [s])\rangle = \frac{\delta}{\sigma^4}\frac{1}{\gamma} \cdot \Big\langle\frac{1}{n}\sum_{i=1}^n \deps \bbeta^{[t],([s],i),\eps}_i \Big\rangle \rightarrow_{a.s.}  \frac{1}{\gamma}\bar{R}^\gamma_\eta([t],[s]),
\end{align*}
and the conclusion again follows by taking $\gamma \rightarrow 0$ and applying Propositions \ref{prop:semigroup_discre_error} and \ref{eq:response_discre_error}.




\section{Proof of Theorem \ref{thm:dmft_entrywise}}



\subsection{Entrywise convergence of discrete Langevin dynamic}

We introduce some further notation. For any $i\neq j\in[d]$, let $\X_{(i)}$ be $\X$ with its $i$th column set to 0, and $\X_{(i,j)}$ be $\X$ with its $i$th and $j$th column both set to $0$. Let $\y_{(i)} = \X_{(i)}\btheta^\ast + \beps$ and $\y_{(i,j)} = \X_{(i,j)}\btheta^\ast + \beps$. Analogous to the leave-one-out dynamic in (\ref{eq:leave_col_out}), consider the following leave-two-out dynamic:
\begin{align}\label{eq:leave_two_col_out}
\notag\btheta^{t+1}_{(i,j)} &= \btheta^{t}_{(i,j)} - \gamma\Big[\frac{1}{\sigma^2}\X_{(i,j)}^\top(\X_{(i,j)}\btheta^{t}_{(i,j)} - \y_{(i,j)}) - \partial_\theta \log g(\btheta^{t}_{(i,j)}; \hat{\alpha}^{t}_{(i,j)})\Big] + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma})\in \R^{d},\\
\hat{\alpha}^{t+1}_{(i,j)} &= \hat{\alpha}^{t}_{(i,j)} + \gamma \cG\Big(\hat{\alpha}^t_{(i,j)}, \Prob_n(\btheta^{t}_{(i,j)})\Big).
\end{align}
\begin{lemma}\label{|em:loo_linfty_error}
Suppose Assumptions \ref{assump:model}, \ref{assump:prior}, and \ref{assump:gradient} hold. For any $T \in \N_+$, there exists some $C > 0$ depending on $T$ (and other problem parameters) such that for any $0\leq t\leq T$, 
\begin{align}
\max_{i,j\in[d]:i\neq j} \E\big|\e_j^\top (\btheta^{t} - \btheta^{t}_{(i)}) \big|^2\leq \frac{C}{d}, \label{eq:loo_linfty}\\
\max_{i,j\in[d]: i\neq j} \E \pnorm{\hat{\alpha}^t - \hat{\alpha}_{(i)}^t - \hat{\alpha}_{(j)}^t + \hat{\alpha}^t_{(i,j)}}{}^2 \leq \frac{C}{d^2}, \label{eq:alpha_lto_l2} \\
\max_{i,j\in[d]: i\neq j}\sqrt{\sum_{k\in[d]:k\neq i,j} \Big(\e_k^\top \big(\btheta^{t} - \btheta^{t}_{(i)} - \btheta^{t}_{(j)} + \btheta^{t}_{(i,j)}\big)\Big)^2} \leq \frac{C}{\sqrt{d}} \label{eq:lto_l2}.
\end{align}
\end{lemma}
\begin{proof}
We prove by induction the in-probability versions of (\ref{eq:loo_linfty})-(\ref{eq:lto_l2}). The baseline case for $t=0$ holds by definition. Suppose the above claims hold up to some $t\geq 0$, and we will establish them for $t+1$. 

\noindent\textbf{Bound of (\ref{eq:loo_linfty})} For any fixed $i\in[d]$, we have
\begin{align*}
\btheta^{t+1} &= \btheta^t - \frac{\gamma}{\sigma^2} \X^\top (\X\btheta^t - \y) + \gamma\partial_\theta \log g(\btheta^t;\hat\alpha^t) + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}), \\
\btheta^{t+1}_{(i)} &= \btheta^t_{(i)} - \frac{\gamma}{\sigma^2} \X_{(i)}^\top (\X_{(i)}\btheta^t_{(i)} - \y_{(i)}) + \gamma\partial_\theta \log g(\btheta^t_{(i)};\hat\alpha^t_{(i)}) + \sqrt{2}(\b^{(t+1)\gamma} - \b^{t\gamma}). 
\end{align*}
Let $\bar{\X}_{(i)} \in \R^{n\times (d-1)}$ be $\X$ with its $i$th column removed. Then for any $j\in[d]$ such that $j\neq i$, we have
\begin{align*}
\e_j^\top (\btheta^{t+1} - \btheta^{t+1}_{(i)}) &= \underbrace{\e_j^\top (I - \frac{\gamma}{\sigma^2}\X^\top \X) (\btheta^t - \btheta^t_{(i)})}_{(I)} - \frac{\gamma}{\sigma^2} \underbrace{\e_j^\top (\X^\top \X - \X_{(i)}^\top \X_{(i)})\btheta^t_{(i)}}_{(II)} + \frac{\gamma}{\sigma^2} \underbrace{\e_j^\top(\X^\top \y - \X_{(i)}^\top \y_{(i)})}_{(III)}\\
&\quad + \gamma\underbrace{\big(\partial_\theta \log g(\theta^t_j;\hat\alpha^t) - \partial_\theta \log g((\btheta^t_{(i)})_j;\hat\alpha^t_{(d)})\big)}_{(IV)}.
\end{align*}
For $(I)$, we have
\begin{align*}
|(I)| &\leq |\e_j^\top (\btheta^t - \btheta^t_{(i)})| + C\gamma\Big|\x_j^\top \X (\btheta^t - \btheta^t_{(i)})\Big| \leq (1+C\gamma\pnorm{\x_j}{}^2)|\e_j^\top (\btheta^t - \btheta^t_{(i)})| + \gamma\Big|\sum_{\ell\in[d]:\ell\neq j} (\x_j^\top \x_\ell) \e_\ell^\top (\btheta^t - \btheta^t_{(i)})\Big|\\
&\leq  (1+C\gamma\pnorm{\x_j}{}^2)|\e_j^\top (\btheta^t - \btheta^t_{(i)})| + \gamma\Big|\sum_{\ell\in[d]:\ell\neq j} (\x_j^\top \x_\ell) \e_\ell^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})\Big| + \gamma\Big|\sum_{\ell\in[d]:\ell\neq j} (\x_j^\top \x_\ell) \e_\ell^\top (\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)})\Big|.
\end{align*}
Using the fact that $\pnorm{\x_j}{}^2 \leq C$ almost surely, the first term is bounded by $(1+C\gamma)|\e_j^\top (\btheta^t - \btheta^t_{(i)})|$. The second term equals $\gamma \cdot \x_j^\top \bar{\X}_{(j)} (\bar{\btheta}^t_{(j)} - \bar{\btheta}^t_{(i,j)})$, where $\bar{\X}_{(j)} \in \R^{n\times (d-1)}$ denotes $\X$ minus its $j$th column, and $\bar{\btheta}^t_{(j)}, \bar{\btheta}^t_{(i,j)} \in \R^{d-1}$ represent $\btheta^t_{(j)}, \btheta^t_{(i,j)}$ without their $j$th component. Since $\x_j$ is independent of $\bar{\X}_{(j)}, \bar{\btheta}^t_{(j)}, \bar{\btheta}^t_{(i,j)}$, we have $\x_j^\top \bar{\X}_{(j)} (\bar{\btheta}^t_{(j)} - \bar{\btheta}^t_{(i,j)}) | \bar{\X}_{(j)} \stackrel{d}{=} \N(0, d^{-1}\pnorm{\bar{\X}_{(j)} (\bar{\btheta}^t_{(j)} - \bar{\btheta}^t_{(i,j)})}{}^2)$, where by Lemma \ref{lem:loo_error}, we have the variance bound $\E\pnorm{\bar{\X}_{(j)} (\bar{\btheta}^t_{(j)} - \bar{\btheta}^t_{(i,j)})}{}^2 \leq C$. Hence we conclude that 
\begin{align*}
\sum_{\ell\in[d]:\ell\neq j} (\x_j^\top \x_\ell) \e_\ell^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)}) = O_P(1/\sqrt{d}).
\end{align*}
Let $\X_{(ij)} \in \R^{n\times (d-2)}$ be $\X$ minus its $i$th and $j$th column, and $\tilde{\btheta}^t, \tilde{\btheta}^t_{(i)}, \tilde{\btheta}^t_{(j)}, \tilde{\btheta}^t_{(i,j)}\in\R^{d-2}$ be $\btheta^t, \btheta^t_{(i)}, \btheta^t_{(j)}, \btheta^t_{(i,j)}$ minus the $i$th and $j$th component. Then the last term satisfies
\begin{align*}
\Big|\sum_{\ell\in[d]:\ell\neq j} (\x_j^\top \x_\ell) \e_\ell^\top (\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)})\Big| \leq |\x_j^\top \x_i | \Big|\e_i^\top (\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)})\Big| + \Big|\x_j^\top \bar{\X}_{(ij)}(\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)})\Big|.
\end{align*}
By Lemma \ref{lem:entrywise_bound}, we have $|\x_j^\top \x_i | \big|\e_i^\top (\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)})\big| = O_P(1/\sqrt{d})$, and by the induction hypothesis, we have
\begin{align*}
\Big|\x_j^\top \bar{\X}_{(ij)} (\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)})\Big| &\leq \pnorm{\x_j}{}\pnorm{\X}{\op} \cdot \pnorm{\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)}}{} = O_P(1/d).
\end{align*}
In summary, we have $|(I)| \leq C|\e_j^\top (\btheta^t - \btheta^t_{(i)})| + O_P(1/\sqrt{d})$. 

To bound $(II)$, we apply $\X = \X_{(i)} + \x_i\e_i^\top$ to obtain $\X^\top \X = \X_{(i)}^\top \X_{(i)}^\top + \X_{(i)}^\top \x_i\e_i^\top + \e_i \x_i^\top \X_{(i)} + \e_i\e_i^\top \pnorm{\x_i}{}^2$, so
\begin{align*}
|(II)| = \Big|\e_j^\top (\X_{(i)}^\top \x_i\e_i^\top + \e_i \x_i^\top \X_{(i)} + \e_i\e_i^\top \pnorm{\x_i}{}^2) \btheta^t_{(i)}\Big| = |\x_i^\top \x_j||\e_i^\top \btheta^t_{(i)}|, 
\end{align*}
which implies that $\E|(II)|^2 \leq C/d$ by Lemma \ref{lem:entrywise_bound} (more precisely, its analogue for the leave-one-out sequence).  For $(III)$, since $\X^\top \y - \X_{(i)}^\top \X_{(i)}^\top \x_i \btheta^\ast_i + \e_i \x_i^\top \y_{(i)} + \e_i \pnorm{\x_i}{}^2 \theta_i^\ast$, we have the same bound $\E|(III)|^2 = \E|\x_j^\top \x_i||\btheta^\ast_i|^2 \leq C/d$. Lastly, by Assumption \ref{assump:prior} we have $|(IV)| \leq C|\e_j^\top (\btheta^t - \btheta^t_{(i)})| + |\hat\alpha^t - \hat\alpha^t_{(d)}| = C|\e_j^\top (\btheta^t - \btheta^t_{(i)})| + O_P(1/\sqrt{d})$ via Lemma \ref{lem:loo_error}. Combining the above bounds yields that 
\begin{align*}
|\e_j^\top (\btheta^{t+1} - \btheta^{t+1}_{(i)})| \leq C|\e_j^\top (\btheta^{t} - \btheta^{t}_{(i)})| + O_P(1/\sqrt{d}), 
\end{align*}
which concludes the induction.


\noindent\textbf{Bound of (\ref{eq:lto_l2})} Note that for some $(\tilde{\alpha}, \tilde{\btheta})$ (resp. $(\check{\alpha}, \check{\btheta})$) on the segment connecting $(\hat\alpha^t, \btheta^t)$ and $(\hat\alpha^t_{(i)}, \btheta^t_{(i)})$ (resp. $(\hat\alpha^t_{(j)}, \btheta^t_{(j)})$ and $(\hat\alpha^t_{(i,j)}, \btheta^t_{(i,j)})$), it holds that
\begin{align*}
\hat\alpha^{t+1} - \hat\alpha^{t+1}_{(i)} &= \hat\alpha^t - \hat\alpha^t_{(i)} + \gamma \Big(\cG(\hat\alpha^t, \Prob_n(\btheta^t))  - \cG(\hat{\alpha}^t_{(i)}, \Prob_n(\btheta^t_{(i)}))\Big)\\
&= \hat\alpha^t - \hat\alpha^t_{(i)} + \gamma \nabla_\alpha \cG(\tilde{\alpha}, \Prob_n(\tilde{\btheta}))^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(i)}) + \gamma\nabla_{\btheta} \cG(\tilde{\alpha}, \Prob_n(\tilde{\btheta}))^\top (\btheta^t - \btheta^t_{(i)}), \\
\hat\alpha^{t+1}_{(j)} - \hat\alpha^{t+1}_{(i,j)} &= \hat\alpha^t_{(i)} - \hat\alpha^t_{(i,j)} + \gamma \Big(\cG(\hat\alpha^t_{(j)}, \Prob_n(\btheta^t_{(j)}))  - \cG(\hat{\alpha}^t_{(i,j)}, \Prob_n(\btheta^t_{(i,j)}))\Big)\\
&= \hat\alpha^t_{(j)} - \hat\alpha^t_{(i,j)} + \gamma \nabla_\alpha \cG(\check{\alpha}, \Prob_n(\check{\btheta}))^\top (\hat{\alpha}^t_{(j)} - \hat{\alpha}^t_{(i,j)}) + \gamma\nabla_{\btheta} \cG(\check{\alpha}, \Prob_n(\check{\btheta}))^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)}).
\end{align*}
Consequently, we have
\begin{align*}
\pnorm{\hat\alpha^{t+1} - \hat\alpha^{t+1}_{(i)} - \hat\alpha^{t+1}_{(j)} + \hat\alpha^{t+1}_{(i,j)}}{} &\leq \pnorm{\hat\alpha^{t} - \hat\alpha^{t}_{(i)} - \hat\alpha^{t}_{(j)} + \hat\alpha^{t}_{(i,j)}}{} + C \underbrace{\Big|\Big(\nabla_\alpha \cG(\tilde{\alpha}, \Prob_n(\tilde{\btheta})) - \nabla_\alpha \cG(\check{\alpha}, \Prob_n(\check{\btheta})) \Big)^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(i)})\Big|}_{(I)}\\
&\quad + C\underbrace{\pnorm{\nabla_\alpha \cG(\check{\alpha}, \Prob_n(\check{\btheta}))}{} \pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(i)} - \hat\alpha^{t}_{(j)} + \hat\alpha^{t}_{(i,j)}}{}}_{(II)}\\
&\quad + C\underbrace{\Big|\Big(\nabla_{\btheta} \cG(\tilde{\alpha}, \Prob_n(\tilde{\btheta})) - \nabla_{\btheta} \cG(\check{\alpha}, \Prob_n(\check{\btheta})) \Big)^\top (\btheta^t - \btheta^t_{(i)})\Big|}_{(III)}\\
&\quad + C\underbrace{\Big|\nabla_{\btheta} \cG(\check{\alpha}, \Prob_n(\check{\btheta}))^\top \Big(\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)}\Big) \Big|}_{(IV)}.
\end{align*}
Define the quantities
\begin{align}\label{eq:dalpha_dtheta}
\notag d(\alpha) &:= \pnorm{\hat\alpha^t - \hat\alpha^t_{(j)}}{} \vee \pnorm{\hat\alpha^t - \hat\alpha^t_{(i,j)}}{} \vee  \pnorm{\hat\alpha^t_{(i)} - \hat\alpha^t_{(j)}}{} \vee \pnorm{\hat\alpha^t_{(j)} - \hat\alpha^t_{(i,j)}}{},\\
d(\btheta) &:= \pnorm{\btheta^t - \btheta^t_{(j)}}{} \vee \pnorm{\btheta^t - \btheta^t_{(i,j)}}{} \vee  \pnorm{\btheta^t_{(i)} - \btheta^t_{(j)}}{} \vee \pnorm{\btheta^t_{(j)} - \btheta^t_{(i,j)}}{},
\end{align}
which satisfies $d(\alpha) = O_P(\sqrt{1/d})$ and $d(\btheta) = O_P(1)$ by Lemma \ref{lem:loo_error}. Then by Assumption \ref{assump:gradient}, $(I)$ satisfies
\begin{align*}
(I) \leq \pnorm{\nabla_\alpha^2 \cG}{F}d(\alpha)^2 + \pnorm{\nabla_\alpha\nabla_{\btheta} \cG}{F}d(\alpha) d(\btheta) = O_P(1/d).
\end{align*}
Term $(II) \leq C\pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(i)} - \hat\alpha^{t}_{(j)} + \hat\alpha^{t}_{(i,j)}}{}$. Term $(III)$ satisfies
\begin{align*}
(III) \leq \pnorm{\nabla_\alpha\nabla_{\btheta}\cG}{F}d(\alpha)d(\btheta) + \pnorm{\nabla_{\btheta}^2 \cG}{\op}d(\btheta)^2 = O_P(1/d).
\end{align*}
Lastly $(IV)$ satisfies
\begin{align*}
(IV) &\leq \Big|\partial_{\theta_i} \cG(\check{\alpha}, \Prob_n(\check{\btheta})) \cdot \e_i^\top  \Big(\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)}\Big)\Big|\\
&\quad + \Big|\partial_{\theta_j} \cG(\check{\alpha}, \Prob_n(\check{\btheta})) \cdot \e_j^\top  \Big(\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)}\Big)\Big|\\
&\quad + \Big|\partial_{\btheta \backslash \theta_i, \theta_j} \cG(\check{\alpha}, \Prob_n(\check{\btheta}))^\top \Big(\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)}\Big)\Big|,
\end{align*}
where we recall that $\tilde{\btheta}^t, \tilde{\btheta}^t_{(i)}, \tilde{\btheta}^t_{(j)}, \tilde{\btheta}^t_{(ij)}\in\R^{d-2}$ are $\btheta^t, \btheta^t_{(i)}, \btheta^t_{(j)}, \btheta^t_{(ij)}$ minus the $i$th and $j$th component. Again by Assumption \ref{assump:gradient}, the first two terms are $O_P(1/d)$. By the same assumption and the induction hypothesis, the last term satisfies
\begin{align*}
\Big|\partial_{\btheta \backslash \theta_i, \theta_j} \cG(\check{\alpha}, \Prob_n(\check{\btheta}))^\top \Big(\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)}\Big)\Big| \leq \pnorm{\nabla_{\btheta} \cG(\check{\alpha}, \Prob_n(\check{\btheta}))}{}\pnorm{\tilde{\btheta}^t - \tilde{\btheta}^t_{(i)} - \tilde{\btheta}^t_{(j)} + \tilde{\btheta}^t_{(i,j)}}{} = O_P(1/d).
\end{align*}
Combining the bounds of $(I)$-$(IV)$ yields the desired conclusion. 

\noindent\textbf{Bound of (\ref{eq:lto_l2})} We have
\begin{align*}
\btheta^{t+1} - \btheta^{t+1}_{(i)} &= (I - \frac{\gamma}{\sigma^2}\X^\top \X)(\btheta^t - \btheta^t_{(i)}) - \frac{\gamma}{\sigma^2} (\X^\top \X - \X_{(i)}^\top \X_{(i)})\btheta^t_{(i)}+ \frac{\gamma}{\sigma^2} (\X^\top \y - \X_{(i)}^\top \y_{(i)})\\
&\quad + \gamma \diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)}; \hat{\alpha}^t_{(i,j)})) (\btheta^t - \btheta^t_{(i)}) + \Delta^t_1,  
\end{align*}
where $\Delta^t_1 = \partial_\theta \log g(\btheta^t;\hat{\alpha}^t) - \partial_\theta \log g(\btheta^t_{(i)};\hat{\alpha}^t_{(i)}) - \diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(i,j)}))(\btheta^t - \btheta^t_{(i)})$. Similarly,
\begin{align*}
\btheta^{t+1}_{(j)} - \btheta^{t+1}_{(i,j)} &= (I - \frac{\gamma}{\sigma^2}\X_{(j)}^\top \X_{(j)})(\btheta^t_{(j)} - \btheta^t_{(i,j)}) - \frac{\gamma}{\sigma^2} (\X_{(j)}^\top \X_{(j)} - \X_{(i,j)}^\top \X_{(i,j)})\btheta^t_{(i,j)} + \frac{\gamma}{\sigma^2} (\X^\top_{(j)} \y_{(j)} - \X_{(i,j)}^\top \y_{(i,j)})\\
&\quad + \gamma \diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(i,j)})) (\btheta^t_{(j)} - \btheta^t_{(i,j)}) + \Delta^t_2, 
\end{align*}
where $\Delta^t_2 =  \partial_\theta \log g(\btheta^t_{(j)};\hat{\alpha}^t_{(j)}) - \partial_\theta \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(i,j)}) - \diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{i,j}))(\btheta^t_{(j)} - \btheta^t_{(i,j)})$. This implies that
\begin{align}\label{eq:ltw_decompose}
\notag&\btheta^{t+1} - \btheta^{t+1}_{(i)} - (\btheta^{t+1}_{(j)} - \btheta^{t+1}_{(i,j)}) = \Big(I - \frac{\gamma}{\sigma^2}\X^\top \X + \gamma \diag(\partial_\theta^2 \log g(\btheta^t))\Big)\big(\btheta^{t} - \btheta^{t}_{(i)} - (\btheta^{t}_{(j)} - \btheta^{t}_{(i,j)})\big)\\
\notag&\quad - \frac{\gamma}{\sigma^2} \underbrace{(\X^\top \X - \X_{(j)}^\top \X_{(j)})(\btheta^t_{(j)} - \btheta^t_{(i,j)})}_{(I)} - \frac{\gamma}{\sigma^2}\underbrace{\Big[(\X^\top \X - \X_{(i)}^\top \X_{(i)})\btheta^{t}_{(i)} - (\X_{(j)}^\top \X_{(j)} - \X_{(i,j)}^\top \X_{(i,j)})\btheta^t_{(i,j)}\Big]}_{(II)}\\
&\quad + \frac{\gamma}{\sigma^2}\underbrace{\Big((\X^\top \y - \X_{(i)}^\top \y_{(i)}) - (\X^\top_{(j)} \y_{(j)} - \X_{(i,j)}^\top \y_{(i,j)})\Big)}_{(III)} + \underbrace{\Delta^t_1 - \Delta^t_2}_{(IV)}.
\end{align}
To bound $(I)$, we have $\X^\top \X - \X_{(j)}^\top \X_{(j)} = \X_{(j)}^\top \x_j \e_j^\top + \e_j \x_j^\top \X_{(j)} + \e_j\e_j^\top \pnorm{\x_j}{}^2$, so
\begin{align*}
\pnorm{(I)}{} &= \Big|(\X_{(j)}^\top \x_j \e_j^\top + \e_j \x_j^\top \X_{(j)} + \e_j\e_j^\top \pnorm{\x_j}{}^2) (\btheta^t_{(j)} - \btheta^t_{(i,j)}) \Big|\\
&\leq \pnorm{\X}{\op}\pnorm{\x_j}{}|\e_j^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})| + \big|\x_j^\top \X_{(j)}(\btheta^t_{(j)} - \btheta^t_{(i,j)})\big| + \pnorm{\x_j}{}^2 \big|\e_j^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})\big|.
\end{align*}
By the induction hypothesis, the first and third term are $O_P(1/\sqrt{d})$.
%\begin{align*}
%\E\Big[\pnorm{\X}{\op}^2\pnorm{\x_j}{}^2|\e_j^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})|^2\Big] \vee \E\Big[\pnorm{\x_j}{}^4 \big|\e_j^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})\big|^2\Big] \leq C\log d/d.
%\end{align*}
For the second term, we have $\x_j^\top \X_{(j)}(\btheta^t_{(j)} - \btheta_{(i,j)})|\X_{(j)} \stackrel{d}{=} \N(0,d^{-1}\pnorm{\X_{(j)}(\btheta^t_{(j)} - \btheta^t_{(i,j)})}{}^2)$ due the independence of $\x_j$ and $\X_{(j)}, \btheta^t_{(j)}, \btheta_{(i,j)}$, and using Lemma \ref{lem:loo_error} the variance is bounded by $C/d$, so we conclude $\pnorm{(I)}{} = O_P(1/\sqrt{d})$. 

To bound $(II)$, we use $\X^\top \X - \X_{(i)}^\top \X_{(i)} = \X_{(i)}^\top \x_i \e_i^\top + \e_i \x_i^\top \X_{(i)} + \e_i\e_i^\top \pnorm{\x_i}{}^2$ and $\X_{(j)}^\top \X_{(j)} - \X_{(i,j)}^\top \X_{(i,j)} = \X_{(i,j)}^\top\x_i\e_i^\top + \e_i\x_i^\top\X_{(i,j)} + \e_i\e_i^\top \pnorm{\x_i}{}^2$, hence
\begin{align*}
(II) = \underbrace{\X_{(i)}^\top \x_i \e_i^\top \btheta^t_{(i)} - \X_{(i,j)}^\top\x_i\e_i^\top \btheta^t_{(i,j)}}_{(II_1)} + \underbrace{\e_i \x_i^\top \X_{(i)} \btheta^t_{(i)} - \e_i\x_i^\top\X_{(i,j)}\btheta^t_{(i,j)}}_{(II_2)} + \underbrace{\e_i\e_i^\top \pnorm{\x_i}{}^2 (\btheta^t_{(i)} - \btheta^t_{(i,j)})}_{(II_3)}.
\end{align*}
Using $\X_{(i,j)} = \X_{(i)} - \x_j\e_j^\top$, we have $(II_1) = \X_{(i)}^\top \x_i\e_i^\top (\btheta^t_{(i)} - \btheta^t_{(i,j)})+ \e_j \x_j^\top \x_i \e_i^\top \btheta^t_{(i,j)}$, hence by the induction hypothesis and Lemma \ref{lem:entrywise_bound}, 
\begin{align*}
\pnorm{(II_1)}{} \leq \pnorm{\X}{\op}\pnorm{\x_i}{} |\e_i^\top (\btheta^t_{(i)} - \btheta^t_{(i,j)})| + |\x_j^\top \x_i| |\e_i^\top \btheta^t_{(i,j)}| = O_P(1/\sqrt{d}).
\end{align*}
Next we have $(II_2) = \e_i \x_i^\top \X_{(i)} (\btheta^t_{(i)} - \btheta^t_{(i,j)}) + \e_i \x_i^\top \x_j \e_j^\top \btheta^t_{(i,j)}$, hence by independence of $\x_i$ with $\X_{(i)},\btheta^t_{(i)},\btheta^t_{(i,j)}$, Lemmas \ref{lem:loo_error} and \ref{lem:entrywise_bound}, we have
\begin{align*}
\pnorm{(II_2)}{} \leq  |\x_i^\top \X_{(i)} (\btheta^t_{(i)} - \btheta^t_{(i,j)})| + |\x_i^\top \x_j||\e_j^\top \btheta^t_{(i,j)}| = O_P(1/\sqrt{d}).
\end{align*}
A similar bound holds for $(II_3)$, so we conclude $\pnorm{(II)}{} = O_P(1/\sqrt{d})$.

To bound $(III)$, direct calculation shows that $(III) = \e_i \x_i^\top \x_j \theta^\ast_j + \e_j \x_i^\top \x_j \theta^\ast_i$, hence $\pnorm{(III)}{} = O_P(1/\sqrt{d})$. For $(IV)$, we write $\Delta_1 = \Lambda^1 + \Lambda^2 + \Lambda^3$, where
\begin{align*}
\Lambda^1 &= \partial_\theta \log g(\btheta^t;\hat{\alpha}^t) - \partial_\theta \log g(\btheta^t_{(i)};\hat{\alpha}^t) - \diag(\partial_\theta^2 \log g(\btheta^t_{(i)};\hat{\alpha}^t))(\btheta^t - \btheta^t_{(i)}),\\
\Lambda^2 &= \Big(\diag(\partial_\theta^2 \log g(\btheta^t_{(i)};\hat{\alpha}^t)) - \diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(i,j)}))\Big)(\btheta^t - \btheta^t_{(i)}),\\
\Lambda^3 &= \partial_\theta \log g(\btheta^t_{(i)};\hat{\alpha}^t) - \partial_\theta \log g(\btheta^t_{(i)};\hat{\alpha}^t_{(i)}),
\end{align*}
and similarly $\Delta_2 = \Gamma^1 + \Gamma^2 + \Gamma^3$, where
\begin{align*}
\Gamma^1 &= \partial_\theta \log g(\btheta^t_{(j)};\hat{\alpha}^t_{(j)}) - \partial_\theta \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(j)}) - \diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(j)}))(\btheta^t_{(j)} - \btheta^t_{(i,j)}),\\
\Gamma^2 &= \Big(\diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(j)})) - \diag(\partial_\theta^2 \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(i,j)}))\Big)(\btheta^t_{(j)} - \btheta^t_{(i,j)}),\\
\Gamma^3 &= \partial_\theta \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(j)}) - \partial_\theta \log g(\btheta^t_{(i,j)};\hat{\alpha}^t_{(i,j)}).
\end{align*}
We first claim that
\begin{align*}
\max_{k\in[d]:k\neq i,j} \Big( |\e_k^\top \Lambda^1| +  |\e_k^\top \Lambda^2| + |\e_k^\top \Gamma^1| + |\e_k^\top \Gamma^2|\Big) = O_P(1/d). 
\end{align*}
We only prove the claim for $\Lambda^1$ and $\Lambda^2$. To see the claim for $\Lambda^1$, we have by Assumption \ref{assump:prior} that
\begin{align*}
\big|\e_k^\top \Lambda^1\big| &= \Big|\partial_\theta \log g((\btheta^t)_k;\hat{\alpha}^t) - \partial_\theta \log g((\btheta^t_{(i)})_k;\hat{\alpha}^t) - \partial_\theta^2 \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t))\e_k^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})\Big|\\
&\leq C(|\e_k^\top (\btheta^t - \btheta^t_{(i,j)})| + |\e_k^\top (\btheta^t_{(i)} - \btheta^t_{(i,j)})|)\cdot |\e_k^\top (\btheta^t_{(j)} - \btheta^t_{(i,j)})|, 
\end{align*}
so the claim follows from the induction hypothesis. For $\Lambda^2$, we have by Assumption \ref{assump:prior} that
\begin{align*}
\big|\e_k^\top \Lambda^2\big| &= \Big|\partial_\theta^2 \log g((\btheta^t_{(i)})_k;\hat{\alpha}^t)) - \partial_\theta^2 \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t_{(i,j)})\Big| |\e_k^\top (\btheta^t - \btheta^t_{(i)})|\\
&\leq C\big(|\e_k^\top (\btheta^t_{(i)} - \btheta^t_{(i,j)})| + |\hat{\alpha}^t - \hat{\alpha}_{(i,j)}^t|\big)\cdot |\e_k^\top (\btheta^t - \btheta^t_{(i)})|,
\end{align*}
so the conclusion follows from the induction hypothesis and Lemma \ref{lem:loo_error}. To handle $\Lambda^3$ and $\Gamma^3$, we have
\begin{align*}
\e_k^\top (\Lambda^3 - \Gamma^3) &= \Big(\partial_\theta \log g((\btheta^t_{(i)})_k;\hat{\alpha}^t) - \partial_\theta \log g((\btheta^t_{(i)})_k;\hat{\alpha}^t_{(i)})\Big) - \Big(\partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t_{(j)}) - \partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t_{(i,j)})\Big)\\
&= \underbrace{\Big[\partial_\theta \log g((\btheta^t_{(i)})_k;\hat{\alpha}^t) - \partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t) - \partial_\theta \log g((\btheta^t_{(i)})_k;\hat{\alpha}^t_{(i)}) + \partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t_{(i)})\Big]}_{W_1}\\
&\quad + \underbrace{\Big[\partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t) - \partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t_{(i)}) - \partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t_{(j)}) + \partial_\theta \log g((\btheta^t_{(i,j)})_k;\hat{\alpha}^t_{(i,j)})\Big]}_{W_2}. 
\end{align*}
Let us bound $W_1$ and $W_2$ separately. For $W_1$, there exist $\tilde{\theta}$ and $\check{\theta}$ that lie in the segment between $(\btheta^t_{(i)})_k$ and $(\btheta^t_{(i,j)})_k$ such that
\begin{align*}
W_1 = \Big(\partial_\theta^2 \log g(\tilde{\theta}; \hat{\alpha}^t) -  \partial_\theta^2 \log g(\check{\theta}; \hat{\alpha}^t_{(i)})\Big) \cdot \e_k^\top(\btheta^t_{(i)} - \btheta^t_{(i,j)}), 
\end{align*}
hence by Assumption \ref{assump:prior} we have
\begin{align*}
|W_1| \leq C(|\e_k^\top (\btheta^t_{(i)} - \btheta^t_{(i,j)})| + |\hat{\alpha}^t - \hat{\alpha}^t_{(i)}|) \cdot |\e_k^\top(\btheta^t_{(i)} - \btheta^t_{(i,j)})|, 
\end{align*}
so $W_1 = O_P(1/d)$ by the induction hypothesis and Lemma \ref{lem:loo_error}. For $W_2$, there exist some $\tilde{\alpha}$ (resp. $\check{\alpha}$) that lies on the segment connecting $(\hat{\alpha}^t, \hat{\alpha}^t_{(i)})$ (resp. $(\hat{\alpha}^t_{(j)}, \hat{\alpha}^t_{(i,j)})$) such that
\begin{align*}
W_2 &= \partial_\theta\nabla_\alpha \log g((\btheta^t_{(i,j)})_k;\tilde{\alpha})^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(i)}) - \partial_\theta\nabla_\alpha \log g((\btheta^t_{(i,j)})_k;\check{\alpha})^\top (\hat{\alpha}^t_{(j)} - \hat{\alpha}^t_{(i,j)})\\
&= \Big(\partial_\theta\nabla_\alpha \log g((\btheta^t_{(i,j)})_k;\tilde{\alpha}) - \partial_\theta\nabla_\alpha \log g((\btheta^t_{(i,j)})_k;\check{\alpha})\Big)^\top (\hat{\alpha}^t - \hat{\alpha}^t_{(i)}) \\
&\quad + \partial_\theta\nabla_\alpha \log g((\btheta^t_{(i,j)})_k;\check{\alpha})^\top\Big(\hat{\alpha}^t - \hat{\alpha}^t_{(i)} - \hat{\alpha}^t_{(j)} + \hat{\alpha}^t_{(i,j)}\Big)\\
&\leq \pnorm{\partial_\theta \nabla_\alpha^2 \log g}{F} d(\alpha)^2 + \pnorm{\partial_\theta \nabla_\alpha \log g}{F} \pnorm{\hat{\alpha}^t - \hat{\alpha}^t_{(i)} - \hat{\alpha}^t_{(j)} + \hat{\alpha}^t_{(i,j)}}{}.
\end{align*}
Here we recall the definition of $d(\alpha)$ in (\ref{eq:dalpha_dtheta}), so by the subsequent bound on $d(\alpha)$ and the induction hypothesis, we have $W_2 = O_P(1/d)$. This concludes that $\e_k^\top (\Lambda^3 - \Gamma^3)$ and hence $\e_k^\top (IV)$ are both $O_P(1/d)$ for any $k\neq i,j$, implying $\sum_{k\in[d]:k\neq i,j} (\e_k^\top (IV))^2 = O_P(1/d)$. 

Combing back to (\ref{eq:ltw_decompose}), we conclude that
\begin{align*}
\sqrt{\sum_{k\in[d]:k\neq i,j} \Big(\e_k^\top \big(\btheta^t - \btheta^t_{(i)} - \btheta^t_{(j)} + \btheta^t_{(i,j)}\big)\Big)^2} \leq \pnorm{(I)}{} + \pnorm{(II)}{} + \pnorm{(III)}{} + \sqrt{\sum_{k\in[d]:k\neq i,j} (\e_k^\top (IV))^2} = O_P(1/\sqrt{d}),
\end{align*}
completing the induction.
\end{proof}

\begin{lemma}\label{lem:entrywise_bound}
For any fixed $T$, there exists some $C > 0$ depending on $T$ (and other problem parameters) such that $\max_{j\in[d]}\max_{0\leq t\leq T} \E |\theta^t_j|^2 \leq C$.
\end{lemma}
\begin{proof}
%Fix $T \in \Z_+$. Consider the event $\mathcal{E} = \{\max_{j\in[d]}\pnorm{\x_j}{}\leq C_0, \pnorm{\X}{\op} \leq C_0, \max_{j\in[d]} |\x_j^\top \y| \leq C_0, \max_{0\leq t \leq T }\max_{j\in[d]} \langle\pnorm{\btheta^t - \btheta^t_{(j)}}{}\rangle \leq C_0\}$. By Lemma \ref{lem:loo_error}, for large enough $C = C(T)$, the event $\cal{E}$ holds almost surely as $n,d\rightarrow\infty$. Note that for any $j\in[d]$, 
By definition, we have
\begin{align*}
\theta^{t+1}_j = \theta^t_j - \frac{\gamma}{\sigma^2} \x_j^\top \X\btheta^t + \frac{\gamma}{\sigma^2} \x_j^\top y + \gamma\partial_\theta \log g(\theta^t_j;\hat{\alpha}^t) + \sqrt{2}(b^{(t+1)\gamma}_j - b^{t\gamma}_j),
\end{align*}
so by Assumption \ref{assump:prior} and the almost sure bound $\max_{0\leq t \leq T}\pnorm{\hat\alpha^t}{} \leq C(T)$, we have
\begin{align*}
|\theta^{t+1}_j| \leq C\Big[(1+\pnorm{\x_j}{}^2 + \pnorm{\partial_\theta^2 \log g}{\infty})|\theta^t_j| + |\x_j^\top \bar{\X}_{(j)} \bar{\btheta}^t| + \pnorm{\x_j}{}^2|\theta^\ast_j| + |\x_j^\top (\bar{\X}_{(j)}\bar{\btheta}^\ast + \beps)| + 1\Big],
\end{align*}
where $\bar{\X}_{(j)}\in\R^{n\times (d-1)}$ denotes $\X$ minus its $j$th column, and $\bar{\btheta}^t, \bar{\btheta}^\ast\in\R^{d-1}$ denote $\btheta^t,\btheta^\ast$ minus their $j$th entry. It is clear that $\max_{j\in[d]}\E (\pnorm{\x_j}{}^2|\theta^\ast_j|)^2 \vee \max_{j\in[d]}\E|\x_j^\top (\bar{\X}_{(j)}\bar{\btheta}^\ast + \beps)|^2 \leq C$, while with $\bar{\btheta}^t_{(j)} \in \R^{d-1}$ denoting $\bar{\btheta}^t$ minus its $j$th entry, we have
\begin{align*}
\E|\x_j^\top \bar{\X}_{(j)} \bar{\btheta}^t|^2 \leq 2\Big(\E|\x_j^\top \bar{\X}_{(j)} \bar{\btheta}^t_{(j)}|^2 + \E|\x_j^\top \bar{\X}_{(j)} (\bar{\btheta}^t - \bar{\btheta}^t_{(j)})|^2\Big) \leq C,
\end{align*}
where we apply Lemma \ref{lem:loo_error}. The desired conclusion now follows from a simple induction.
\end{proof}

\begin{proposition}\label{prop:entrywise_discrete_approx}
Suppose Assumptions \ref{assump:model}-\ref{assump:gradient} hold. Recall the discrete DMFT system in (\ref{eq:dmft_theta_discrete1})-(\ref{eq:dmft_alpha_discrete1}). For any fixed $m\in \Z$ and $j\in[d]$, it holds as $n,d\rightarrow\infty$ that
\begin{align*}
\sP(\theta^0_j, \ldots, \theta^m_j) \overset{W_1}{\to} \sP(\bar{\theta}^{t_0}_\gamma, \ldots, \bar{\theta}^{t_m}_\gamma),
\end{align*}
where the law on both sides are taken over all the randomness.
\end{proposition}
\begin{proof}
Without loss of generality, we study the last coordinate of $\btheta^t$ denoted by $\mu^t$, and we write $\btheta^t = (\bar{\btheta}^{t}, \mu^t)$ with $\bar{\btheta}^t \in \R^{d}$. We also write $\X = [\bar{\X}, \x]$ where $\x\in\R^n$ denotes the last column of $\X$. Then it holds that
\begin{align}\label{eq:single_expansion_main}
\notag\mu^{t+1} &= (1-\frac{\gamma}{\sigma^2}\pnorm{\x}{}^2)\mu^t - \frac{\gamma}{\sigma^2}\x^\top (\bar{\X}\bar{\btheta}^t - \y) + \gamma \partial_\theta \log g(\mu^t;\hat{\alpha}^t) + \sqrt{2}(b^{(t+1)\gamma} - b^{t\gamma})\\
\notag&= (1-\frac{\gamma\delta}{\sigma^2})\mu^t - \frac{\gamma}{\sigma^2}\x^\top (\bar{\X}\bar{\btheta}^t_{(d)} - \y_{(d)}) - \frac{\gamma}{\sigma^2} \x^\top \big(\bar{\X}(\bar{\btheta}^t - \bar{\btheta}^t_{(d)}) + \y_{(d)} - \y\big) + \gamma \partial_\theta \log g(\mu^t;\hat\alpha^t) + \sqrt{2}(b^{(t+1)\gamma} - b^{t\gamma})\\
\notag&\quad - \frac{\gamma}{\sigma^2}\mu^t \cdot (\pnorm{\x}{}^2 - \delta)\\
\notag&= \mu^t - \frac{\gamma\delta}{\sigma^2} (\mu^t - \btheta^\ast_d) - \frac{\gamma}{\sigma^2}\x^\top \bar{\X}(\bar{\btheta}^t_{(d)} - \y_{(d)}) - \frac{\gamma}{\sigma^2} \x^\top \bar{\X}(\bar{\btheta}^t - \bar{\btheta}^t_{(d)}) + \gamma \partial_\theta \log g(\mu^t;\hat\alpha^t) + \sqrt{2}(b^{(t+1)\gamma} - b^{t\gamma})\\
&\quad - \frac{\gamma}{\sigma^2}(\mu^t - \theta^\ast_d)\cdot (\pnorm{\x}{}^2 - \delta).
\end{align}
Here $\btheta^t_{(d)}$ is the leave-one-out dynamic defined in (\ref{eq:leave_col_out}), and we write $\bar{\btheta}^t_{(d)}$ as its first $(d-1)$ coordinates. 

Let us now expand $\bar{\X}(\bar{\btheta}^t - \bar{\btheta}^t_{(d)})$. With $\bar{\b}^t$ denoting the first $d-1$ coordinates of $\b^t$, we have
\begin{align*}
\bar{\btheta}^{t+1} = \Big(I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X}\Big)\bar{\btheta}^t - \frac{\gamma}{\sigma^2}\bar{\X}^\top (\x \mu^t - \y) + \gamma \partial_\theta \log g(\bar{\btheta}^t;\hat{\alpha}^t) + \sqrt{2}(\bar{\b}^{(t+1)\gamma} - \bar{\b}^{t\gamma}),\\
\bar{\btheta}^{t+1}_{(d)} = \Big(I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X}\Big)\bar{\btheta}^t_{(d)} - \frac{\gamma}{\sigma^2}\bar{\X}^\top (-\y_{(d)}) + \gamma \partial_\theta \log g(\bar{\btheta}^t_{(d)};\hat{\alpha}^t_{(d)}) + \sqrt{2}(\bar{\b}^{(t+1)\gamma} - \bar{\b}^{t\gamma}),
\end{align*}
which implies that
\begin{align*}
\bar{\btheta}^{t+1}  - \bar{\btheta}^{t+1}_{(d)} &= \Big(I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X}\Big)(\bar{\btheta}^t  - \bar{\btheta}^t_{(d)}) - \frac{\gamma}{\sigma^2} \bar{\X}^\top \x(\mu^t - \theta^\ast_d) + \gamma \diag(\partial_\theta^2 \log g(\bar{\btheta}^t_{(d)};\hat\alpha^t_{(d)}))(\bar{\btheta}^t - \bar{\btheta}^t_{(d)}) + \gamma \Delta_t\\
&= \underbrace{\Big(I - \frac{\gamma}{\sigma^2}\bar{\X}^\top \bar{\X} + \gamma \diag(\partial_\theta^2 \log g(\bar{\btheta}^t_{(d)};\hat\alpha^t_{(d)}))\Big)}_{\Omega^t} (\bar{\btheta}^t  - \bar{\btheta}^t_{(d)}) - \frac{\gamma}{\sigma^2} \bar{\X}^\top \x(\mu^t - \theta^\ast_d) + \gamma \Delta_t,
\end{align*}
where $\Delta_t = \partial_\theta \log g(\bar{\btheta}^t;\hat\alpha^t) - \partial_\theta \log g(\bar{\btheta}^t_{(d)};\hat\alpha^t_{(d)}) - \diag(\partial_\theta^2 \log g(\bar{\btheta}^t_{(d)};\hat\alpha^t_{(d)})) (\bar{\btheta}^t - \bar{\btheta}^t_{(d)})$. Iterating the above identity yields that
\begin{align*}
\bar{\btheta}^{t+1}  - \bar{\btheta}^{t+1}_{(d)} = \Omega^t \ldots \Omega^0 \underbrace{(\bar{\btheta}^0 - \bar{\btheta}^0_{(d)})}_{=0} + \sum_{\ell=0}^t \Omega^t \ldots \Omega^{\ell+1} \Big(-\frac{\gamma}{\sigma^2} \bar{\X}^\top \x (\mu^\ell - \theta^\ast_d) + \gamma \Delta_\ell\Big),
\end{align*}
where we understand $\Omega^t \ldots \Omega^{\ell+1} = I_{d-1}$ for $\ell = t$. Plugging the above identity into (\ref{eq:single_expansion_main}), we have
\begin{align*}
\mu^{t+1} &= \mu^t - \frac{\gamma\delta}{\sigma^2} (\mu^t - \theta^\ast_d) + \gamma \partial_\theta \log g(\mu^t;\hat{\alpha}^t) + \Big(\frac{\gamma}{\sigma^2}\Big)^2 \sum_{\ell=0}^t \x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\bar{\X}^\top \x \cdot(\mu^\ell - \theta^\ast_d) - \frac{\gamma}{\sigma^2}\x^\top \bar{\X}(\bar{\btheta}^t_{(d)} - \y_{(d)})\\
&\quad + \sqrt{2}(b^{(t+1)\gamma} - b^{t\gamma}) - \frac{\gamma}{\sigma^2}(\mu^t - \theta^\ast_d)\cdot (\pnorm{\x}{}^2 - \delta) - \frac{\gamma^2}{\sigma^2}\sum_{\ell=0}^t \x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell.
\end{align*}
Recall from (\ref{eq:dmft_theta_discrete1}) that the $\theta$-dynamic in the discrete DMFT system takes the form (with simplified notation introduced after (\ref{eq:dmft_response_rho})):
\begin{align}\label{eq:dmft_theta_single}
\theta^{t+1} &= \theta^t - \frac{\gamma\delta}{\sigma^2} (\theta^t - \theta^\ast) + \gamma \partial_\theta \log g(\theta^t;\alpha^t) - \gamma\sum_{\ell=0}^t \bar{R}_\eta^\gamma(t,\ell)(\theta^\ell - \theta^\ast) + \gamma u^t_\gamma + \sqrt{2}(b^{(t+1)\gamma}_\gamma - b^{t\gamma}_\gamma).
\end{align}
We couple the above two processes inductively as follows:
\begin{itemize}
\item In (\ref{eq:dmft_theta_single}), we take $\theta^\ast = \theta^\ast_d$, $\theta^0 = \mu^0$, and $b^{t\gamma}_\gamma = b^{t\gamma}$.
\item Let $\tilde{u}^t = -\frac{1}{\sigma^2}\x^\top (\bar{\X}\bar{\btheta}^t_{(d)} - \y_{(d)})$. Using independence between $\x$ and $\bar{\X}, \btheta^t_{(d)}, \y_{(d)}$, we have $\E[\tilde{u}^t\tilde{u}^s|\X_{(d)}, \y_{(d)}] = \frac{\delta}{\sigma^4} n^{-1}(\bar{\X}\bar{\btheta}^t_{(d)} - \y_{(d)})^\top (\bar{\X}\bar{\btheta}^s_{(d)} - \y_{(d)})$, where by Lemma \ref{lem:loo_error} and the DMFT characterization Theorem \ref{thm:dmft_approx} the covariance converges in $L_2$ to $C_\eta^\gamma(t,s) = \frac{\delta}{\sigma^4}\E(\eta^t - w^\ast - \eps)(\eta^s - w^\ast - \eps)$. We may then construct a coupling $\{u^s_\gamma,\tilde{u}^s\}$, $0\leq s\leq t+1$ such that $\max_{0\leq s\leq t+1} \E(\tilde{u}^s - u_\gamma^s)^2 \rightarrow 0$ as $n,d\rightarrow\infty$.
\end{itemize}
Next note that by the analysis subsequent to (\ref{eq:loo_approximation}), it holds that $\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\bar{\X}^\top \x \rightarrow_{a.s.} -\frac{\sigma^4}{\gamma}\bar{R}_\eta^\gamma(t,\ell)$, hence with the above coupling, we have $\E \pnorm{(\mu^0,\ldots,\mu^{t+1}) - (\theta^0, \ldots, \theta^{t+1})}{} \rightarrow 0$ provided that
\begin{align*}
\E\Big[|\mu^t - \theta^\ast_d|\cdot |\pnorm{\x}{}^2 - \delta|\Big] \rightarrow 0,\quad \E\Big[|\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell|\Big] \rightarrow 0, \quad 0\leq \ell \leq t.
\end{align*}
The first claim holds by standard concentration. For the second claim, we decompose $\Delta_\ell = \Delta_\ell^1 + \Delta_\ell^2 + \Delta_\ell^3$, where
\begin{align*}
\Delta_\ell^1 &= \partial_\theta \log g(\bar{\btheta}^\ell;\hat{\alpha}^\ell) - \partial_\theta \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell) - \diag(\partial_\theta^2 \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell))(\bar{\btheta}^\ell - \bar{\btheta}^\ell_{(d)}),\\
\Delta_\ell^2 &= \Big(\diag(\partial_\theta^2 \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell)) - \diag(\partial_\theta^2 \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell_{(d)}))\Big)(\bar{\btheta}^\ell - \bar{\btheta}^\ell_{(d)}),\\
\Delta_\ell^3 &= \partial_\theta \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell) - \partial_\theta \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell_{(d)}).
\end{align*}
For $\Delta_\ell^1$, we have $\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell^1 \leq \pnorm{\x}{}\prod_{s=\ell+1}^t \pnorm{\Omega^s}{\op} \pnorm{\Delta_\ell^1}{}$, where
\begin{align*}
\pnorm{\Delta_\ell^1}{}^2 \leq \sum_{j:j\neq d} \pnorm{\partial_\theta^3 \log g}{\infty}^2 (\theta^\ell_j - (\btheta^\ell_{(d)})_j)^4 \leq d\pnorm{\partial_\theta^3 \log g}{\infty}^2 \pnorm{\bar{\btheta}^\ell - \bar{\btheta}_{(d)}^\ell}{\infty}^4 \leq C(\log d)^2/d, 
\end{align*}
with the last step following from Lemma \ref{|em:loo_linfty_error}. For $\Delta_\ell^2$, we similarly have
\begin{align*}
\pnorm{\Delta_\ell^2}{} \leq \pnorm{\partial_\theta^2 \nabla_\alpha \log g}{\infty}\pnorm{\hat\alpha^\ell - \hat\alpha^\ell_{(d)}}{}\pnorm{\bar{\btheta}^\ell - \bar{\btheta}^\ell_{(d)}}{} \leq C\frac{\log d}{\sqrt{d}},
\end{align*}
where we apply Lemma \ref{lem:loo_error}. For $\Delta^3_\ell$, we have
\begin{align*}
\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1} \Delta_\ell^3 &= \x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\partial_\theta\nabla_\alpha \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell_{(d)}) (\hat\alpha^\ell - \hat\alpha^\ell_{(d)})\\
&\quad + \x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\partial_\theta\nabla_\alpha^2 \log g(\bar{\btheta}^\ell_{(d)};\tilde{\alpha}^\ell) \cdot (\hat\alpha^\ell - \hat\alpha^\ell_{(d)})^{\otimes 2}, 
\end{align*}
where $\tilde{\alpha}^\ell$ lies on the segment connecting $\hat\alpha^\ell$ and $\hat\alpha^\ell_{(d)}$, and we understand $\partial_\theta\nabla_\alpha^2 \log g(\bar{\btheta}^\ell_{(d)};\tilde{\alpha}^\ell) \cdot (\hat\alpha^\ell - \hat\alpha^\ell_{(d)})^{\otimes 2}$ as the standard tensor product from $\R^{d-1}\times \R^K \times \R^K$ and $\R^K \times \R^K$ to $\R^{d-1}$. For the first term, using independence between $\x$ and $\bar\X, \{\Omega^\ell\}, \bar{\btheta}^\ell_{(d)}, \hat{\alpha}^\ell_{(d)}$, it is easy to argue that each component of $\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\partial_\theta\nabla_\alpha \log g(\bar{\btheta}^\ell_{(d)};\hat{\alpha}^\ell_{(d)}) \in \R^K$ is bounded by $\sqrt{\log d/d}$ almost surely. On the other hand, we have
\begin{align*}
\Big|\x^\top \bar{\X} \Omega^t \ldots \Omega^{\ell+1}\partial_\theta\nabla_\alpha^2 \log g(\bar{\btheta}^\ell_{(d)};\tilde{\alpha}^\ell) \cdot (\hat\alpha^\ell - \hat\alpha^\ell_{(d)})^{\otimes 2}\Big| \leq \sqrt{d}\cdot\pnorm{\x}{}\pnorm{\X}{\op}\prod_{s=\ell+1}^t \pnorm{\Omega^s}{\op}\pnorm{\partial_\theta\nabla_\alpha^2 \log g}{\op}\pnorm{\hat\alpha^\ell - \hat\alpha^\ell_{(d)}}{}^2.
\end{align*}
Hence by Lemma \ref{lem:loo_error}, its first moment converges to zero. The proof is complete.
\end{proof}

\subsection{Entrywise discretization error of Langevin dynamic}

Consider the dynamic $\{\btheta^t_\gamma, \hat{\alpha}^t_\gamma\}_{t\in \R_+}$ defined in (\ref{eq:discrete_langevin}). For any $j\in[d]$, we denote the $j$th component of $\btheta^t$ (resp. $\btheta^t_\gamma$) as $\theta^t_j$ (resp. $\theta^t_{\gamma,j}$).

\begin{proposition}\label{prop:entrywise_langevin_discretize}
Assume the conditions of Theorem \ref{thm:dmft_entrywise}. For any fixed $m\in\Z_+$, $\tau_1,\ldots,\tau_m \in \R_+$, and $j\in[d]$, it holds that as $\gamma\rightarrow 0$, 
\begin{align*}
\limsup_{n,d\rightarrow\infty} W_1\Big(\sP(\theta^{\tau_1}_{j},\ldots, \theta^{\tau_m}_{j}), \sP(\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j})\Big) \rightarrow 0.
\end{align*}
\end{proposition}
\begin{proof}
It suffices to bound $\E \pnorm{(\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j}) - (\theta^{\tau_1}_{j},\ldots, \theta^{\tau_m}_{j})}{}^2 = \sum_{\ell=1}^m \E (\theta^{\tau_\ell}_j - \theta^{\tau_\ell}_{\gamma,j})^2$.
Recall the discretized Brownian motion $\{\b^t_\gamma\}_{t\in\R_+}$ defined in (\ref{eq:hd_BM_linear}). Let $\bar{\X}\in\R^{n\times (d-1)}$ denote $\X$ minus its $j$th column, and $\bar{\btheta}^t, \bar{\btheta}^t_\gamma \in \R^{d-1}$ denote $\btheta^t, \btheta^t_\gamma$ minus the $j$th entry. By definition, we have 
\begin{align*}
\theta^t_j &= \theta^0_j + \int_0^t \Big(-\frac{1}{\sigma^2}\big(\pnorm{\x_j}{}^2 \theta^s_j + \x_j^\top \bar{\X} \bar{\btheta}^s - \x_j^\top \y\big) + \partial_\theta \log g(\theta^s_j;\hat\alpha^s)\Big)\d s + \e_j^\top \b^t,\\
\theta^t_{\gamma,j} &= \theta^0_j + \int_0^t \Big(-\frac{1}{\sigma^2}\big(\pnorm{\x_j}{}^2 \theta^{\floor{s}}_{\gamma,j} + \x_j^\top \bar{\X} \bar{\btheta}^{\floor{s}}_\gamma - \x_j^\top \y\big) + \partial_\theta \log g(\theta^{\floor{s}}_{\gamma,j};\hat\alpha^{\floor{s}}_{\gamma})\Big)\d s + \e_j^\top \b^t_\gamma,
\end{align*}
Then by Assumption \ref{assump:prior}, we have
\begin{align*}
|\theta^t_j - \theta^t_{\gamma,j}| &\leq \int_0^t \Big[(C+C\pnorm{\x_j}{}^2) |\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| + C\pnorm{\hat\alpha^s - \hat\alpha^{\floor{s}}_\gamma}{} + C|\x_j^\top \bar{\X} (\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma)|\Big] \d s + \sqrt{2}|\e_j^\top (\b^t - \b^t_\gamma)|\\
&\leq \int_0^t \Big[(C+C\pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 \leq 10\delta}) |\theta^s_j - \theta^{s}_{\gamma,j}| \d s + \int_0^t  C|\x_j^\top \bar{\X} (\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)})|\d s + \underbrace{\int_0^T C\pnorm{\hat\alpha^s - \hat\alpha^{\floor{s}}_\gamma}{} \d s}\\
&\quad + \underbrace{\int_0^T \Big[C\pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 > 10\delta} |\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| + (1+ 10C\delta) |\theta^s_{\gamma,j} - \theta^{\floor{s}}_{\gamma,j}| + C|\x_j^\top \bar{\X} (\bar{\btheta}^s_{(j)} - \bar{\btheta}^{\floor{s}}_{\gamma,(j)})|\Big] \d s + \sqrt{2}\sup_{t\in[0,T]} |b^t_j - b^t_{\gamma,j}|}_{A_1(T)}\\
&\leq \int_0^t (C + 10C\delta) |\theta^s_j - \theta^{s}_{\gamma,j}| \d s + \int_0^t C\pnorm{\X}{\op}^2 \pnorm{\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}}{} \d s + A_1(T).
\end{align*}
We may further decompose the middle term as
\begin{align*}
\pnorm{\bar{\btheta}^s - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}}{} \leq \pnorm{\bar{\btheta}^s - \bar{\btheta}^{s}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{s}_{\gamma,(j)}}{} + \pnorm{\bar{\btheta}^{s}_\gamma - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^{s}_{\gamma,(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}}{},
\end{align*}
where by Lemma \ref{lem:theta_decomp}, we have for any $t\in[0,T]$ that
\begin{align*}
\int_0^t \pnorm{\bar{\btheta}^s - \bar{\btheta}^{s}_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^{s}_{\gamma,(j)}}{} \d s \leq \exp(CT)CT\pnorm{\X}{\op}^2  \int_0^t |\theta^s_j - \theta^s_{\gamma,j}|\d s + \tilde{R}(t),
\end{align*}
for some $\tilde{R}(t)$ such that $\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]} \E \tilde{R}^2(t) \leq h(\gamma)$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$. Hence by a similar truncation argument as above applied to $\pnorm{\X}{\op}$, we conclude that for any $t\in[0,T]$, 
\begin{align*}
|\theta^t_j - \theta^t_{\gamma,j}| \leq C\int_0^t |\theta^s_j - \theta^s_{\gamma,j}|\d s + A_1(T) + A_2(T), 
\end{align*}
for some $A_2(T)$ such that $\limsup_{n,d\rightarrow\infty} \E A_2^2(T) \leq h(\gamma)$. By Lemma \ref{lem:gronwall}, this further implies
\begin{align*}
|\theta^t_j - \theta^t_{\gamma,j}| \leq \exp(Ct)(A_1(T) + A_2(T)), \quad \forall t\in[0,T]. 
\end{align*}
It remains to bound $\E A_1^2(T)$, which satisfies
\begin{align*}
\E A_1^2(T) &\leq C \E\Big(\int_0^T \pnorm{\x_j}{}^2\bm{1}_{\pnorm{\x_j}{}^2 > 10\delta} |\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| \d s\Big)^2 + C \E\Big(\int_0^T |\theta^s_{\gamma,j} - \theta^{\floor{s}}_{\gamma,j}| \d s\Big)^2 + C\E\Big(\int_0^T \pnorm{\hat\alpha^s - \hat\alpha^{\floor{s}}_\gamma}{} \d s\Big)^2\\
&\quad + C\E \Big(\int_0^T |\x_j^\top \bar{\X} (\bar{\btheta}^s_{(j)} - \bar{\btheta}^{\floor{s}}_{\gamma,(j)})| \d s\Big)^2 + C\E\sup_{t\in[0,T]} |b^t_j - b^t_{\gamma,j}|^2 := \sum_{i=1}^5 \zeta_i.
\end{align*}
By standard concentration, the term $\zeta_1$ is bounded by $C \exp(-c\sqrt{d})$.  For term $\zeta_2$, we have
\begin{align*}
|\theta^s_j - \theta^{\floor{s}}_{\gamma,j}| &\leq C\gamma\Big(\pnorm{\x_j}{}^2 |\theta^{\floor{s}}_{\gamma,j} - \theta^\ast_j| + \big|\x_j^\top \bar{\X} (\bar\btheta^{\floor{s}}_{\gamma} - \bar{\btheta}^\ast)| + |\x_j^\top\beps|\Big) + \sqrt{2} \sup_{t\in [0,T]} |b^t_j - b^{\floor{t}}_j| + |b^t_j - b^{\ceil{t}}_j|\\
&\leq C\gamma\Big(\pnorm{\x_j}{}^2 |\theta^{\floor{s}}_{\gamma,j} - \theta^\ast_j| + \big|\x_j^\top \bar{\X} (\bar\btheta^{\floor{s}}_{\gamma,(j)} - \bar{\btheta}^\ast)| + \pnorm{\x_j}{}\pnorm{\X}{\op}\pnorm{\btheta^{\floor{s}}_\gamma - \btheta^{\floor{s}}_{\gamma,(j)}}{} + |\x_j^\top\beps|\Big)\\
&\quad + \sqrt{2} \sup_{t\in [0,T]} |b^t_j - b^{\floor{t}}_j| + |b^t_j - b^{\ceil{t}}_j|,
\end{align*}
where $\{\btheta^t_{\gamma,(j)}\}_{t\in\R_+}$ is defined in (\ref{eq:cont_time_loo_col}), and $\bar{\btheta}^t_{\gamma,(j)} \in \R^{d-1}$ denotes it without the $j$th entry. By independence between $\x_j$ and $\bar{\X}, \btheta^{\floor{s}}_{\gamma,(j)}$, and the 1-dimensional version of Lemma \ref{lem:BM_maximal}, we conclude that $\zeta_2\vee \zeta_5 \leq C\gamma\log_+(1/\gamma)$. Next by the conclusion of Lemma \ref{lem:langevin_discretize_error} and bound (\ref{eq:alpha_discrete_error}), it holds that $\zeta_3 \leq h(\gamma)$ for some $h(\gamma)\downarrow 0$ as $\gamma\downarrow 0$. Lastly, $\zeta_4$ is also bounded by some $h(\gamma)$ by independence between $\x_j$ and $\bar{\X}, \bar{\btheta}^s_{(j)}, \bar{\btheta}^{\floor{s}}_{\gamma,(j)}$ and Lemma \ref{lem:langevin_discretize_error}. We therefore conclude that $\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]} \E |\theta^t_j - \theta^t_{\gamma,j}|^2 \leq h(\gamma)$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$, as desired.
%Let $\X_{(j)} \in \R^{n\times d}$ be $\X$ with its $j$th column set to zero, $\y_{(j)} = \X_{(j)}\btheta^\ast + \eps$, and $\{\btheta^t_{(j)}\}_{t\in\R_+} \subset \R^d$ be the continuous leave-one-column-out dynamic defined by
%\begin{align*}
%\btheta^t_{(j)} = \btheta^0 + \int_0^t \Big[-\frac{1}{\sigma^2}\X_{(j)}^\top (\X_{(j)} \btheta^s_{(j)} - \y_{(j)}) + \partial_\theta \log g(\btheta^s_{(j)})\Big]\d s + \sqrt{2}\b^t.
%\end{align*}
%Let $\{\btheta^t_{\gamma,(j)}\}_{t\in\R_+}$ be defined similarly, and $\bar{\btheta}^t_{(j)}, \bar{\btheta}^t_{\gamma,(j)}\in\R^{d-1}$ be $\btheta^t_{(j)}, \btheta^t_{\gamma,(j)}$ without the $j$th entry.  
\end{proof}

\begin{lemma}\label{lem:theta_decomp}
Assume the conditions of Theorem \ref{thm:dmft_entrywise}. For any fixed $T > 0$, there exists some function $h(\gamma) = h(\gamma;T) \rightarrow 0$ as $\gamma \rightarrow 0$ such that
\begin{align*}
\sup_{t\in[0,T]}\E \pnorm{\btheta^t_\gamma - \btheta^{\floor{t}}_\gamma - \btheta^t_{\gamma,(j)} + \btheta^{\floor{t}}_{\gamma,(j)}}{}^2 \leq h(\gamma), 
\end{align*}
and there exists some $R(t)$ with $\sup_{t\in[0,T]} \E R^2(t) \leq h(\gamma)$ such that almost surely, for any $t\in[0,T]$,
\begin{align*}
\pnorm{\bar{\btheta}^t - \bar{\btheta}^t_\gamma - \bar{\btheta}_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)}}{} \leq \exp(Ct)\Big[\int_0^t C\pnorm{\X}{\op}^2 |\theta^s_j - \theta^s_{\gamma,j}| \d s + R(t)\Big].
\end{align*}
\end{lemma}
\begin{proof}
We first expand $\pnorm{\btheta^{s}_\gamma - \btheta^{\floor{s}}_\gamma - \btheta^{s}_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)}}{}$. By definition, we have
\begin{align*}
\btheta^s_\gamma - \btheta^{\floor{s}}_\gamma &= (s-\floor{s})\Big[-\frac{1}{\sigma^2}\X^\top(\X\btheta^{\floor{s}}_\gamma - \y) + \partial_\theta \log g(\btheta^{\floor{s}}_\gamma; \hat\alpha^{\floor{s}}_{\gamma})\Big] + \sqrt{2}(\b^{s}_\gamma - \b^{\floor{s}}_\gamma),\\
\btheta^s_{\gamma,(j)} - \btheta^{\floor{s}}_{\gamma,(j)} &= (s-\floor{s})\Big[-\frac{1}{\sigma^2}\X_{(j)}^\top(\X_{(j)}\btheta^{\floor{s}}_{\gamma,(j)} - \y_{(j)}) + \partial_\theta \log g(\btheta^{\floor{s}}_{\gamma,(j)}; \hat\alpha^{\floor{s}}_{\gamma,(j)})\Big] + \sqrt{2}(\b^{s}_{\gamma} - \b^{\floor{s}}_{\gamma}),
\end{align*}
which implies that
\begin{align*}
\pnorm{\btheta^s_\gamma - \btheta^{\floor{s}}_\gamma - \btheta^s_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)}}{} &\leq C\gamma \Big(\pnorm{(\X^\top \X - \X_{(j)}^\top \X_{(j)})\btheta^{\floor{s}}_{\gamma,(j)}}{} + \pnorm{\X}{\op}^2\pnorm{\btheta^{\floor{s}}_{\gamma} - \btheta^{\floor{s}}_{\gamma,(j)}}{}\\
&\quad + \pnorm{\hat\alpha^{\floor{s}}_{\gamma} - \hat\alpha^{\floor{s}}_{\gamma,(j)}}{} + \pnorm{\X^\top \y - \X_{(j)}^\top \y_{(j)}}{}\Big).
\end{align*}
By bounds (\ref{ineq:loo_1}), (\ref{ineq:loo_2}), and the conclusion of Lemma \ref{lem:loo_error}, we conclude that $\E \pnorm{\btheta^s_\gamma - \btheta^{\floor{s}}_\gamma - \btheta^s_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)}}{}^2 \leq C\gamma^2$ for some $C > 0$ that does not depend on $\gamma$.

Next we have
\begin{align*}
\btheta^t - \btheta^t_\gamma &= \int_0^t -\frac{1}{\sigma^2} \X^\top \X (\btheta^s - \btheta^{\floor{s}}_\gamma) + \big[\partial_\theta \log g(\btheta^s; \hat\alpha^s) - \partial_\theta \log g(\btheta^{\floor{s}}_\gamma; \hat\alpha^{\floor{s}}_\gamma)\big]\d s + \sqrt{2}(\b^t - \b^t_\gamma),\\
\btheta_{(j)}^t - \btheta^t_{\gamma,(j)} &= \int_0^t -\frac{1}{\sigma^2} \X_{(j)}^\top \X_{(j)} (\btheta^s_{(j)} - \btheta^{\floor{s}}_{\gamma,(j)}) + \big[\partial_\theta \log g(\btheta^s_{(j)}; \hat\alpha^s_{(j)}) -  \partial_\theta \log g(\btheta^{\floor{s}}_{\gamma,(j)}; \hat\alpha^{\floor{s}}_{\gamma,(j)})\big]\d s + \sqrt{2}(\b^t - \b^t_\gamma),
\end{align*}
which implies that, with $E_{(j)} \in \R^{(d-1)\times d}$ denoting the identity matrix $I_d$ without its $j$th row, 
\begin{align*}
&\bar{\btheta}^t - \bar{\btheta}^t_\gamma - \bar{\btheta}_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)}\\
&= \int_0^t \Big[ -\frac{1}{\sigma^2}E_{(j)}\Big((\X^\top \X - \X_{(j)}^\top \X_{(j)}) (\btheta^s - \btheta^{\floor{s}}_\gamma) + \X_{(j)}^\top \X_{(j)} (\btheta^s - \btheta^s_{\gamma} - \btheta^s_{(j)} + \btheta^s_{\gamma,(j)}) + \X_{(j)}^\top \X_{(j)} (\btheta^s_{\gamma} - \btheta^{\floor{s}}_{\gamma} - \btheta^s_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)})\Big) \\
&\quad + \Big(\partial_\theta \log g(\bar{\btheta}^s; \hat\alpha^s) - \partial_\theta \log g(\bar{\btheta}^{\floor{s}}_\gamma; \hat\alpha^{\floor{s}}_\gamma) - \partial_\theta \log g(\bar{\btheta}^s_{(j)}; \hat\alpha^s_{(j)}) +  \partial_\theta \log g(\bar{\btheta}^{\floor{s}}_{\gamma,(j)}; \hat\alpha^{\floor{s}}_{\gamma,(j)})\Big)\Big] \d s.
\end{align*}
Note that
\begin{itemize}
\item Since $E_{(j)}(\X^\top \X - \X_{(j)}^\top \X_{(j)}) = E_{(j)}(\X_{(j)}^\top \x_j\e_j^\top + \e_j \x_j^\top \X_{(j)} + \e_j\e_j^\top \pnorm{\x_j}{}^2) = E_{(j)}\X_{(j)}^\top \x_j\e_j^\top$, we have
\begin{align*}
\biggpnorm{E_{(j)}(\X^\top \X - \X_{(j)}^\top \X_{(j)}) (\btheta^s - \btheta^{\floor{s}}_\gamma)}{} \leq C\pnorm{\X}{\op}^2 |\theta^s_j - \theta^s_{\gamma,j}|  + R_1(t),
\end{align*}
for some $R_1(t)$ such that $\sup_{t\in[0,T]} \E R_1^2(t) \leq h(\gamma)$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$.
\item The second term satisfies 
\begin{align*}
\pnorm{E_{(j)}\X_{(j)}^\top \X_{(j)} (\btheta^s - \btheta^s_{\gamma} - \btheta^s_{(j)} + \btheta^s_{\gamma,(j)})}{} &=\pnorm{E_{(j)}\X_{(j)}^\top \X_{(j)} (\bar{\btheta}^s - \bar{\btheta}^s_{\gamma} - \bar{\btheta}^s_{(j)} + \bar{\btheta}^s_{\gamma,(j)})}{}\\
&\leq \pnorm{\X}{\op}^2\pnorm{\bar{\btheta}^s - \bar{\btheta}^s_\gamma - \bar{\btheta}_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)}}{}.
\end{align*}
\item By the conclusion of the first part, we have $\E\pnorm{\X_{(j)}^\top \X_{(j)} (\btheta^s_{\gamma} - \btheta^{\floor{s}}_{\gamma} - \btheta^s_{\gamma,(j)} + \btheta^{\floor{s}}_{\gamma,(j)})}{}^2 \leq C\gamma^2$. 
\item For the last term, we have
\begin{align*}
\partial_\theta \log g(\bar{\btheta}^s; \hat\alpha^s) - \partial_\theta \log g(\bar{\btheta}^{\floor{s}}_\gamma; \hat\alpha^{\floor{s}}_\gamma) &= \diag(\partial_\theta^2 \log g(\tilde{\btheta};\hat\alpha^{\floor{s}}_\gamma)) (\bar{\btheta}^s - \bar{\btheta}^s_\gamma) + \Delta_1(s), \\
\partial_\theta \log g(\bar{\btheta}^s_{(j)}; \hat\alpha^s_{(j)}) - \partial_\theta \log g(\bar{\btheta}^{\floor{s}}_{\gamma,(j)}; \hat\alpha^{\floor{s}}_{\gamma,(j)}) &= \diag(\partial_\theta^2 \log g(\check{\btheta};\hat\alpha^{\floor{s}}_{\gamma,(j)})) (\bar{\btheta}^s_{(j)} - \bar{\btheta}^s_{\gamma,(j)}) + \Delta_2(s), 
\end{align*}
where $\tilde{\btheta} \in \R^{d-1}$ (resp. $\check{\btheta}$) is some point that lies on the segment connecting $\bar{\btheta}^s$ and $\bar{\btheta}^{\floor{s}}$ (resp. $\bar{\btheta}^s_{(j)}$ and $\bar{\btheta}^{\floor{s}}_{\gamma,(j)}$), and
\begin{align*}
\Delta_1(s) &= \partial_\theta \log g(\bar{\btheta}^s; \hat\alpha^s) - \partial_\theta \log g(\bar{\btheta}^s; \hat\alpha^{\floor{s}}_\gamma) + \diag(\partial_\theta^2 \log g(\tilde{\btheta};\tilde{\alpha})) (\bar{\btheta}^s_\gamma - \bar{\btheta}^{\floor{s}}_\gamma),\\
\Delta_2(s) &= \partial_\theta \log g(\bar{\btheta}^s_{(j)}; \hat\alpha^s_{(j)}) - \partial_\theta \log g(\bar{\btheta}^s_{(j)}; \hat\alpha^{\floor{s}}_{\gamma,(j)}) + \diag(\partial_\theta^2 \log g(\check{\btheta};\hat\alpha^{\floor{s}}_{\gamma,(j)})) ( \bar{\btheta}^s_{\gamma,(j)} - \bar{\btheta}^{\floor{s}}_{\gamma,(j)}).
\end{align*}
This entails that
\begin{align*}
&\partial_\theta \log g(\bar{\btheta}^s; \hat\alpha^s) - \partial_\theta \log g(\bar{\btheta}^{\floor{s}}_\gamma; \hat\alpha^{\floor{s}}_\gamma) - \partial_\theta \log g(\bar{\btheta}^s_{(j)}; \hat\alpha^s_{(j)}) + \partial_\theta \log g(\bar{\btheta}^{\floor{s}}_{\gamma,(j)}; \hat\alpha^{\floor{s}}_{\gamma,(j)})\\
&= \Big(\diag(\partial_\theta^2 \log g(\tilde{\btheta};\hat\alpha^{\floor{s}}_\gamma)) -  \diag(\partial_\theta^2 \log g(\check{\btheta};\hat\alpha^{\floor{s}}_{\gamma,(j)}))\Big)(\bar{\btheta}^s - \bar{\btheta}^s_\gamma)\\
&\quad + \diag(\partial_\theta^2 \log g(\check{\btheta};\hat\alpha^{\floor{s}}_{\gamma,(j)})) (\bar{\btheta}^s - \bar{\btheta}^s_\gamma - \bar{\btheta}^s_{(j)} + \bar{\btheta}^s_{\gamma,(j)}) + \Delta_1(s) - \Delta_2(s).
\end{align*}
Using a similar argument for (\ref{eq:loo_linfty}) below, we may show that $\sup_{t\in [0,T]} \max_{i,j\in[d]:i\neq j} \E |\e_i^\top (\btheta^t - \btheta^t_{(j)})|^2 \leq C/d$.  Applying this bound and the fact from Lemma \ref{lem:loo_error} that $\E \pnorm{\bar{\btheta}^s - \bar{\btheta}^s_\gamma}{}^2 \leq dh(\gamma)$ for $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$, we conclude that
\begin{align}\label{eq:bound_12}
\sup_{s\in[0,T]} \E\biggpnorm{\Big(\diag(\partial_\theta^2 \log g(\tilde{\btheta};\hat\alpha^{\floor{s}}_\gamma)) -  \diag(\partial_\theta^2 \log g(\check{\btheta};\hat\alpha^{\floor{s}}_{\gamma,(j)}))\Big)(\bar{\btheta}^s - \bar{\btheta}^s_\gamma)}{}^2 \leq Ch(\gamma).
\end{align}
On the other hand, we may decompose $\Delta_1(s) - \Delta_2(s)$ as
\begin{align*}
\Delta_1(s) - \Delta_2(s) &= \Big[\partial_\theta \log g(\bar{\btheta}^s; \hat\alpha^s) - \partial_\theta \log g(\bar{\btheta}^s; \hat\alpha^{\floor{s}}_\gamma)\Big] - \Big[\partial_\theta \log g(\bar{\btheta}^s_{(j)}; \hat\alpha^s_{(j)}) - \partial_\theta \log g(\bar{\btheta}^s_{(j)}; \hat\alpha^{\floor{s}}_{\gamma,(j)})\Big]\\
&\quad +  \Big(\diag(\partial_\theta^2 \log g(\tilde{\btheta};\hat\alpha^{\floor{s}}_\gamma)) -  \diag(\partial_\theta^2 \log g(\check{\btheta};\hat\alpha^{\floor{s}}_{\gamma,(j)}))\Big)(\bar{\btheta}^s_\gamma - \bar{\btheta}^{\floor{s}}_\gamma)\\
&\quad + \diag(\partial_\theta^2 \log g(\check{\btheta};\hat\alpha^{\floor{s}}_{\gamma,(j)})) (\bar{\btheta}^s_\gamma - \bar{\btheta}^{\floor{s}}_\gamma - \bar{\btheta}^s_{\gamma,(j)} + \bar{\btheta}^{\floor{s}}_{\gamma,(j)}), 
\end{align*}
where by Lemma \ref{lem:loo_error}, a similar bound to (\ref{eq:bound_12}), and the conclusion of the first part of the claim, we have $\sup_{s\in[0,T]}\E (\Delta_1(s) - \Delta_2(s))^2 \leq h(\gamma)$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$. 
\end{itemize}
In conclusion, we have shown that for any $t\in[0,T]$,
\begin{align*}
\pnorm{\bar{\btheta}^t - \bar{\btheta}^t_\gamma - \bar{\btheta}_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)}}{} \leq \int_0^t C(\pnorm{\X}{\op}^2 + 1)\pnorm{\bar{\btheta}^s - \bar{\btheta}^s_\gamma - \bar{\btheta}_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)}}{}\d s  + \int_0^t C\pnorm{\X}{\op}^2 |\theta^s_j - \theta^s_{\gamma,j}| \d s + R_2(t),
\end{align*}
for some $R_2(t)$ such that $\sup_{t\in[0,T]}\E R_2(t)^2 \leq h(\gamma)$. We may further bound for $s\in[0,t]$, 
\begin{align*}
\int_0^t C(\pnorm{\X}{\op}^2 + 1)\pnorm{\bar{\btheta}^s - \bar{\btheta}^s_\gamma - \bar{\btheta}_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)}}{}\d s &\leq C\int_0^t\pnorm{\bar{\btheta}^s - \bar{\btheta}^s_\gamma - \bar{\btheta}_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)}}{}\d s\\
&\quad + \underbrace{\int_0^t  C\pnorm{\X}{\op}^2\bm{1}_{\pnorm{\X}{\op}^2 > 10(1+\delta)}\pnorm{\bar{\btheta}^s - \bar{\btheta}^s_\gamma - \bar{\btheta}_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)}}{}\d s}_{R_3(t)}, 
\end{align*}
where by standard concentration $\limsup_{n,d} \sup_{t\in[0,T]}\E R_3^2(t) = 0$. Hence we have
\begin{align*}
\pnorm{\bar{\btheta}^t - \bar{\btheta}^t_\gamma - \bar{\btheta}_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)}}{} \leq C\int_0^t \pnorm{\bar{\btheta}^s - \bar{\btheta}^s_\gamma - \bar{\btheta}_{(j)}^s + \bar{\btheta}^s_{\gamma,(j)}}{}\d s  + \int_0^t C\pnorm{\X}{\op}^2 |\theta^s_j - \theta^s_{\gamma,j}| \d s + R_3(t)
\end{align*}
for some $R_3(t)$ such that $\limsup_{n,d\rightarrow\infty}\sup_{t\in[0,T]}\E R_3^2(t) \leq h(\gamma)$ for some $h(\gamma)\rightarrow 0$ as $\gamma\rightarrow 0$, and by Lemma \ref{lem:gronwall}, we have
\begin{align*}
\pnorm{\bar{\btheta}^t - \bar{\btheta}^t_\gamma - \bar{\btheta}_{(j)}^t + \bar{\btheta}^t_{\gamma,(j)}}{} \leq \exp(Ct)\Big[\int_0^t C\pnorm{\X}{\op}^2 |\theta^s_j - \theta^s_{\gamma,j}| \d s + R_3(t)\Big],
\end{align*}
as desired. 
\end{proof}

\subsection{Completing the proof}
Using a similar tightness argument as in the proof of Theorem \ref{thm:dmft_approx}, it suffices to show that for any fixed integer $m$, $\tau_1,\ldots,\tau_m\in\R_+$, and $j\in[d]$, it holds that $W_1(\sP(\theta^{\tau_1}_j,\ldots, \theta^{\tau_m}_j, \theta^\ast_j), \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)) \rightarrow 0$ as $n,d\rightarrow\infty$. To this end, we have for any $\gamma > 0$ that
\begin{align*}
&W_1\Big(\sP(\theta^{\tau_1}_j,\ldots, \theta^{\tau_m}_j, \theta^\ast_j), \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big) \leq  W_1\Big(\sP(\theta^{\tau_1}_j,\ldots, \theta^{\tau_m}_j, \theta^\ast_j), \sP(\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j}, \theta^\ast_j)\Big)\\
&+ W_1\Big(\sP(\theta^{\tau_1}_{\gamma,j},\ldots, \theta^{\tau_m}_{\gamma,j}, \theta^\ast_j), \sP(\bar{\theta}^{\tau_1}_{\gamma},\ldots, \bar{\theta}^{\tau_m}_{\gamma}, \theta^\ast)\Big) + W_1\Big(\sP(\bar{\theta}^{\tau_1}_{\gamma},\ldots, \bar{\theta}^{\tau_m}_{\gamma}, \theta^\ast), \sP(\theta^{\tau_1},\ldots, \theta^{\tau_m}, \theta^\ast)\Big).
\end{align*}
The desired conclusion follows by taking first $\limsup_{n,d\rightarrow\infty}$ and then $\gamma \rightarrow 0$, applying Propositions \ref{prop:entrywise_discrete_approx}, \ref{prop:entrywise_langevin_discretize}, and Lemma \ref{lem:dmft_discretization_error}.

%Recall that $\bR_{\theta}(t,s) = \big(\E[\partial_j P_{t-s} e_k(\btheta^s)]\big)_{j,k=1}^d$, where the expectation is taken with respect to the Brownian motion in $\{\btheta^t\}$. We will show that for any bounded and continuous $h(\cdot)$, 
%\begin{align*}
%\int_0^t \frac{1}{d}\Tr \bR_\theta(t,s)h(s)\d s \rightarrow \int R_\theta(t,s)h(s) \d s. 
%\end{align*}
%Define the following two perturbed processes on $[0,T]$: for each $j\in[d]$ and $\eps > 0$, 
%\begin{align*}
%\btheta^{t,(j,\eps)} &= \btheta^0 + \int_0^t \Big(-\frac{1}{\sigma^2}\X^\top (\X \btheta^{s,(j,\eps)} - \y) - f'(\btheta^{s,(j,\eps)}) + \eps \e_jh(s)\Big)\d s + \sqrt{2}\b^t,\\
%\tilde{\btheta}^{t,(j,\eps)} &= \btheta^0 + \int_0^t \Big(-\frac{1}{\sigma^2}\X^\top (\X \tilde{\btheta}^{\floor{s},(j,\eps)} - \y) - f'(\tilde{\btheta}^{\floor{s},(j,\eps)}) + \eps \e_jh(\floor{s})\Big)\d s + \sqrt{2}\b^t. 
%\end{align*}
%Let $\{\btheta^t\}$ and $\{\tilde{\btheta}^t\}$ denote the unperturbed processes with $\eps = 0$. Note that at knots, 
%\begin{align*}
%\tilde{\btheta}^{(k+1)\gamma,(j,\eps)} = \tilde{\btheta}^{k\gamma,(j,\eps)} + \gamma\Big[-\frac{1}{\sigma^2}\X^\top (\X \tilde{\btheta}^{k\gamma,(j,\eps)} - \y) - f'(\tilde{\btheta}^{k\gamma,(j,\eps)}) + \eps \e_jh(k\gamma)\Big] + \sqrt{2}(\b^{(k+1)\gamma} - \b^{k\gamma}).
%\end{align*}
%Since $\int_0^t d^{-1}\Tr \bR_\theta(t,s)\d s = \frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\btheta^{t,(j,\eps)}_j]$, we have
%\begin{align*}
%\Big|\int_0^t d^{-1}\Tr \bR_\theta(t,s)\d s - \int R_\theta(t,s)h(s) \d s\Big| \leq (I) + (II) + (III),
%\end{align*}
%where
%\begin{align}
%(I) &= \Big|\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\btheta^{t,(j,\eps)}_j] - \frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\tilde{\btheta}^{t,(j,\eps)}_j]\Big|,\\
%(II) &= \Big|\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\tilde{\btheta}^{t,(j,\eps)}_j]\Big|
%\end{align}
%\textbf{Bound of $(I)$} We start with
%\begin{align*}
%\Big|\frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\btheta^{t,(j,\eps)}_j] - \frac{1}{d}\sum_{j=1}^d \partial_\eps|_{\eps = 0} \E [\tilde{\btheta}^{t,(j,\eps)}_j]\Big| \leq \frac{1}{d}\sum_{j=1}^d\E\Big|\partial_\eps|_{\eps = 0} \btheta^{t,(j,\eps)}_j - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{t,(j,\eps)}_j\Big|,
%\end{align*}
%and let us bound the right side quantity. By definition, with
%\begin{align*}
%\W^{s} = -\frac{1}{\sigma^2}\X^\top \X - \diag\big(f''(\btheta^{s})\big), \quad \tilde{\W}^{s} = -\frac{1}{\sigma^2}\X^\top \X - \diag\big(f''(\tilde{\btheta}^{s})\big),
%\end{align*}
%we have
%\begin{align}\label{eq:theta_eps_der}
%\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)} &= \int_0^t \Big( \W^{s}\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} + \e_jh(s)\Big)\d s,\\
%\partial_\eps|_{\eps=0} \tilde{\btheta}^{t,(j,\eps)} &= \int_0^t \Big(\tilde{\W}^{\floor{s}} \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)} + \e_jh(\floor{s})\Big)\d s.
%\end{align}
%This implies
%\begin{align*}
%&\pnorm{\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)} - \partial_\eps|_{\eps=0} \tilde{\btheta}^{t,(j,\eps)}}{}\\
%&= \pnorm{\int_0^t \W^{s} \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} \d s - \int_0^t \e_j^\top \tilde{\W}^{\floor{s}} \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)} \d s + \int_0^t \e_jh(s) \d s  - \int_0^t \e_j h(\floor{s}) \d s}{}\\
%&\leq \int_0^t \pnorm{(\W^{s} - \tilde{\W}^{s}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \d s + \int_0^t \pnorm{(\tilde{\W}^{s} - \tilde{\W}^{\floor{s}}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \d s\\
%&\quad + \int_0^t \pnorm{\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)}{}\d s +  \int_0^t \pnorm{\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}\big)}{}\d s
%\end{align*}
%For the first term,
%\begin{align*}
%\pnorm{(\W^{s} - \tilde{\W}^{s}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq \pnorm{\W^{s} - \tilde{\W}^{s}}{\op}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq \pnorm{f'''}{\infty}\pnorm{\btheta^s - \tilde{\btheta}^s}{\infty}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq C\pnorm{\btheta^s - \tilde{\btheta}^s}{\infty}, 
%\end{align*}
%using Lemma \ref{lem:discrete_estimate}. For the second term, we similarly have
%\begin{align*}
%\pnorm{(\tilde{\W}^{s} - \tilde{\W}^{\floor{s}}) \partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \leq C\pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{\infty}.
%\end{align*}
%For the third term, we have
%%\begin{align*}
%%&\Big|\e_j^\top\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)\Big|\\
%%&\leq \frac{1}{\sigma^2}\Big|\e_j^\top \X^\top \X \big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)\Big| + \pnorm{f''}{\infty}\Big|\partial_\eps|_{\eps = 0} \btheta_j^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}_j^{s,(j,\eps)}\Big|\\
%%&\leq \Big(\frac{\pnorm{\x_j}{}^2}{\sigma^2} + \pnorm{f''}{\infty}\Big) \Big|\partial_\eps|_{\eps = 0} \btheta_j^{s,(j,\eps)} - \partial_\eps|_{\eps = 0}\tilde{\btheta}_j^{s,(j,\eps)}\Big| + \underbrace{\Big|\x_j^\top \sum_{k:k\neq j}\x_k \big(\partial_\eps|_{\eps = 0} \btheta_k^{s,(j,\eps)} - \partial_\eps|_{\eps = 0}\tilde{\btheta}_k^{s,(j,\eps)}\big)\Big|}_{R_j^s}.
%%\end{align*}
%\begin{align*}
%\pnorm{\tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}\big)}{} \leq \pnorm{\tilde{\W}^{\floor{s}}}{\op}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}}{} \leq L\pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)}}{},
%\end{align*}
%where $L = \frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + \pnorm{f''}{\infty}$. For the fourth term, it is bounded by $\pnorm{\tilde{\W}^{\floor{s}}}{\op}\pnorm{\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}}{}$, where, since
%\begin{align*}
%\partial_\eps|_{\eps=0} \tilde{\btheta}^s = \partial_\eps|_{\eps=0} \tilde{\btheta}^{\floor{s}} + (s - \floor{s})\Big(\tilde{\W}^{\floor{s}} \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)} + \e_jh(\floor{s})\Big),
%\end{align*}
%we have by Lemma \ref{lem:discrete_estimate} that $\pnorm{\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}}{} \leq C\gamma$. Together with the bound $\pnorm{\tilde{\W}^{\floor{s}}}{\op} \leq \frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + \pnorm{f''}{\infty}$, we have
%\begin{align*}
% \int_0^t \Big|\e_j^\top \tilde{\W}^{\floor{s}}\big(\partial_\eps|_{\eps = 0} \tilde{\btheta}^{s,(j,\eps)} - \partial_\eps|_{\eps = 0} \tilde{\btheta}^{\floor{s},(j,\eps)}\big)\Big|\d s \leq C\gamma.
%\end{align*}
%Combining the above four bounds, we have
%\begin{align*}
%\pnorm{\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)} - \partial_\eps|_{\eps=0} \tilde{\btheta}^{t,(j,\eps)}}{} &\leq L\int_0^t \sup_{u\leq s}\pnorm{\partial_\eps|_{\eps=0} \btheta^{u,(j,\eps)} - \partial_\eps|_{\eps=0} \tilde{\btheta}^{u,(j,\eps)}}{}\d s\\
%&\quad + C\int_0^t \Big(\pnorm{\btheta^s - \tilde{\btheta}^s}{\infty} + \pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{\infty}\Big)\d s + C\gamma.
%\end{align*} 
%Hence applying Lemma \ref{lem:gronwall} yields that for any $t\leq T$,
%\begin{align*}
%\Big|\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)}_j - \partial_\eps|_{\eps=0} \tilde{\btheta}_j^{t,(j,\eps)}\Big| \leq e^{C_1t} \cdot\Big[ C_2\int_0^t \Big(|\btheta^s_j - \tilde{\btheta}^s_j| + |\tilde{\btheta}^{s}_j - \tilde{\btheta}^{\floor{s}}_j| + R_j^s\Big)\d s + C\gamma\Big],
%\end{align*}
%which further implies that
%\begin{align*}
%\sum_{j=1}^d\Big|\partial_\eps|_{\eps=0} \btheta^{t,(j,\eps)}_j - \partial_\eps|_{\eps=0} \tilde{\btheta}_j^{t,(j,\eps)}\Big| \leq C\sqrt{d} \cdot \int_0^t \big(\pnorm{\btheta^s - \tilde{\btheta}^s}{} + \pnorm{\tilde{\btheta}^{s} - \tilde{\btheta}^{\floor{s}}}{} + \pnorm{\bR^s}{}\big)\d s + Cd\gamma,
%\end{align*}
%where $\bR^s = (R^s_1,\ldots, R^s_d)$.
%
%
%\begin{lemma}
%Control $\pnorm{\btheta^s - \tilde{\btheta}^s}{}$ and $\pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{}$
%\end{lemma}
%\begin{proof}
%Since
%\begin{align*}
%\pnorm{\btheta^t}{} \leq \pnorm{\btheta^0}{} + \int_0^t \Big(\frac{1}{\sigma^2}\pnorm{\X^\top}{\op}^2 + \pnorm{f''}{\infty}\Big)\pnorm{\btheta^s}{}\d s + t\sqrt{d}|f'(0)| + \sqrt{2}\pnorm{\b^t}{},
%\end{align*}
%we have by Lemma \ref{lem:gronwall} that
%\begin{align*}
%\pnorm{\btheta^t}{} \leq e^{Lt}\Big[\pnorm{\btheta^0}{} + t\sqrt{d}|f'(0)| + \sqrt{2}\pnorm{\b^t}{}\Big],
%\end{align*}
%which implies that $\E\pnorm{\btheta^t}{}^2 \leq C(\pnorm{\btheta^0}{}^2 + d)$. A similar bound holds for $\E\pnorm{\tilde{\btheta}^t}{}^2$. Note that
%\begin{align*}
%\tilde{\btheta}^s = \tilde{\btheta}^{\floor{s}} + (s-\floor{s})\Big(-\frac{1}{\sigma^2}\X^\top (\X \tilde{\btheta}^{\floor{s}} - \y) - f'(\tilde{\btheta}^{\floor{s}}) \Big) + \sqrt{2}(\b^s - \b^{\floor{s}}),
%\end{align*}
%hence
%\begin{align*}
%\E\pnorm{\tilde{\btheta}^s - \tilde{\btheta}^{\floor{s}}}{}^2 \leq C\gamma^2\Big(\pnorm{\X}{\op}^4 \E\pnorm{\tilde{\btheta}^{\floor{s}}}{}^2 + \pnorm{\X^\top \y}{}^2\Big) + C\gamma d \leq C\gamma(\pnorm{\btheta^0}{}^2 + \pnorm{\X^\top \y}{}^2 + d). 
%\end{align*}
%\end{proof}
%
%
%
%\begin{lemma}\label{lem:discrete_estimate}
%Fix any $T > 0$. Then there exist some $C > 0$ depending on $T, \pnorm{h}{\infty}$, such that for any $t \leq T$,
%\begin{align*}
%\sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} \leq Ce^{Lt}
%\end{align*}
%\end{lemma}
%\begin{proof}
%Note that $\pnorm{\W^{s,(j)}}{\op} \leq L := \frac{1}{\sigma^2}\pnorm{\X}{\op}^2 + \pnorm{f''}{\infty}$. For any fixed $T > 0$ and $t\leq T$, we have
%\begin{align*}
%\sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} &\leq \int_0^t L \pnorm{\partial_\eps|_{\eps = 0} \btheta^{s,(j,\eps)}}{} \d s + \int_0^t |h(s)|\d s\\
%&\leq L\int_0^t \sup_{u\leq s}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} \d s + C,
%\end{align*}
%where $C$ depends on $t$ and $\pnorm{h}{\infty}$. Applying Lemma \ref{lem:gronwall} to $t\mapsto \sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{}$, we obtain
%\begin{align*}
%\sup_{u \leq t}\pnorm{\partial_\eps|_{\eps = 0} \btheta^{u,(j,\eps)}}{} \leq Ce^{Lt}.
%\end{align*}
%\end{proof}






==> existence.tex <==
\section{Proof of Proposition \ref{prop:dmftsolexists}}
The proof is divided into three steps:
\begin{enumerate}
\item We define auxiliary functions $\Phi_{C_\theta}, \Phi_{R_\theta}, \Phi_{C_\eta}, \Phi_{R_\eta}, \Phi_{R_\eta^\ast}$ via a set of deterministic equations, which will serve as upper bounds to $C_\theta, R_\theta, C_\eta, R_\eta, R_\eta^\ast$ in the DMFT system.
\item We define a space $\cS_\eta$ for the triplet $X_\eta = (C_\eta, R_\eta, R_\eta^\ast)$ such that for each given $X_\eta$, the $\theta$ equation (\ref{def:dmft_langevin_cont_theta}) and response (\ref{def:response_theta}) admit a unique solution. Similarly, we define $\cS_\theta$ for the triplet $X_\theta = (C_\theta, C_\theta^\ast, R_\theta)$ such that for each given $X_\theta$, the $\eta$ equation (\ref{def:dmft_langevin_cont_eta}) and responses (\ref{def:response_g})-(\ref{def:derivative_langevin_ostar}) admit a unique solution. 
\item We construct a map $\cT$ from $\cS_\eta$ to $\cS_\eta$, which we show to be contractive under some metric. Hence by Banach fixed point theorem, it admits a unique fixed point which recovers the DMFT solution. 
\end{enumerate}

\subsection{Auxiliary functions}

Consider the following deterministic system of equations of $(\Phi_{R_\theta}, \Phi_{C_\theta}, \Phi_{R_\eta}, \Phi_{R_\eta^\ast}, \Phi_{C_\eta})$:
\begin{equation}\label{eq:auxiliary_eq}
\begin{aligned}
\frac{\d}{\d t}\Phi_{R_\theta}(t) &= (\frac{\delta}{\sigma^2} + L)\Phi_{R_\theta}(t) + \int_0^t \Phi_{R_\eta}(t-s)\Phi_{R_{\theta}}(s)\d s,\\
\frac{\d }{\d t}\Phi_{C_\theta}(t) &= 2K_{C_\theta}\cdot\Big(\Phi_{C_\theta}(t) + \int_0^t (t-s+1)^2\Phi_{R_\eta}^2(t-s)\Phi_{C_\theta}(s)\d s + \Phi_{R^\ast_\eta}^2(t) + \Phi_{C_\eta}(t) + 1\Big)., \\
\Phi_{R_\eta}(t) &= \frac{1}{\sigma^2}\Big(\int_0^t \Phi_{R_\theta}(t-s)\Phi_{R_\eta}(s)\d s + \frac{\delta}{\sigma^2}\Phi_{R_\theta}(t)\Big),\\
\Phi_{R_\eta^\ast}(t) &= \frac{1}{\sigma^2}\int_0^t \Phi_{R_\theta}(t-s)(\Phi_{R_\eta^\ast}(s) + \frac{\delta}{\sigma^2})\d s,\\
\Phi_{C_\eta}(t) &= \frac{2\delta}{\sigma^4}\Big[\frac{1}{\sigma^4}\int_0^t t \cdot \Phi^2_{R_\theta}(t-s) \Phi_{C_\eta}(s)\d s + 2\Phi_{C_\theta}(t) + 2 \E[(\theta^\ast)^2] + \sigma^2\Big],
\end{aligned}
\end{equation}
with initialization $\Phi_{R_\theta}(0)$ and $\Phi_{C_\theta}(0)$ satisfying
\begin{align}\label{eq:auxiliary_init}
\Phi_{R_\theta}(0) \geq 1, \quad \Phi_{C_\theta}(0) \geq \E[(\theta^0)^2].
\end{align}

\begin{lemma}
The system (\ref{eq:auxiliary_eq}) with initialization (\ref{eq:auxiliary_init}) admits a unique solution.
\end{lemma}
\begin{proof}
For any $\{\alpha_i\}_{i=1}^{11} \in \R_+$, we establish the uniqueness of
\begin{equation}
\begin{aligned}
\frac{\d}{\d t}f_1(t) &= \alpha_1f_1(t) + \int_0^t f_2(t-s)f_1(s)\d s,\\
f_2(t) &= \alpha_2\int_0^t f_1(t-s)f_2(s)\d s + \alpha_3f_1(t),\\
f_3(t) &= \alpha_4\int_0^t f_1(t-s)(f_3(s) + \alpha_5)\d s,\\
\frac{\d }{\d t} f_4(t) &= \alpha_6\Big(f_4(t) + \int_0^t (t-s+1)^2 \cdot f_2^2(t-s)f_4(s)\d s + f_3^2(t) + f_5(t) + 1\Big),\\
f_5(t) &= \alpha_7\int_0^t (t-s+1)^2\cdot f_1^2(t-s) f_5(s)\d s + \alpha_{8}f_4(t) + \alpha_{9},
\end{aligned}
\end{equation}
with initialization $f_1(0) = \beta_1, f_2(0) = \beta_2$. The correspondence with (\ref{eq:auxiliary_eq}) is $f_1(t) = \Phi_{R_\theta}(t), f_2(t) = \Phi_{R_\eta}(t), f_3(t) = \Phi_{R_\eta^\ast}(t), f_4(t) = \Phi_{C_\theta}(t), f_5(t) = \Phi_{C_\eta}(t)$.

\noindent{\textbf{Solution of $f_1(t)$ and $f_2(t)$}} For any $f:\R_+\rightarrow \R$ and $\lambda > 0$, let $\pnorm{f}{\lambda} \equiv \pnorm{f}{1,\lambda} \equiv \int_0^\infty e^{-\lambda t}|f(t)| \d t$. For any $\eps_1, \eps_2 > 0$ such that 
\begin{align}\label{eq:eps_condition_1}
\alpha_3\eps_1 < \eps_2, \quad \eps_2 < \frac{\alpha_3}{\alpha_2}, \quad \eps_1 < \frac{1}{2\alpha_4}, 
\end{align}
define the space
\begin{align*}
\cS_{12} \equiv \{(f_1,f_2): \pnorm{f_1}{\lambda} \leq \eps_1, \pnorm{f_2}{\lambda} \leq \eps_2, f_1(0) = \beta_1\},
\end{align*}
equipped with the metric
\begin{align*}
d((f_1,f_2), (\tilde{f}_1,\tilde{f}_2)) = 4\alpha_3\pnorm{f_1 - \tilde{f}_1}{\lambda} + \pnorm{f_2 - \tilde{f}_2}{\lambda}. 
\end{align*}
It is clear that $(\cS_{12}, d)$ is complete. Define the map $(\bar{f}_1,\bar{f}_2) = \cT_{12}((f_1,f_2))$ as
\begin{align*}
\bar{f}_1(t) &= \beta_1 + \alpha_1\int_0^t f_1(s) \d s + \int_0^t \Big(\int_0^s f_2(s-s')f_1(s')\d s'\Big)\d s,\\
\bar{f}_2(t) &= \alpha_2\int_0^t f_1(t-s)f_2(s)\d s + \alpha_3f_1(t).
\end{align*}
We will show that, for large enough $\lambda$, $\cT_{12}$ maps $\cS_{12}$ to itself and is contractive. To see the former claim, direct calculation yields that
\begin{align*}
\pnorm{\bar{f}_1}{\lambda} = \frac{\beta_1}{\lambda} + \alpha_1\cdot\frac{\pnorm{f_1}{\lambda}}{\lambda} + \frac{\pnorm{f_1}{\lambda} \cdot \pnorm{f_2}{\lambda}}{\lambda} \leq \frac{\beta_1 + \eps_1(\alpha_1 + \eps_2)}{\lambda} \leq \eps_1,
\end{align*}
for large enough $\lambda$ (depending on $\alpha_1,\beta_1,\eps_1,\eps_2$). Similarly,
\begin{align*}
\pnorm{\bar{f}_2}{\lambda} = \alpha_2 \cdot \frac{\pnorm{f_1}{\lambda}\pnorm{f_2}{\lambda}}{\lambda} + \alpha_3\pnorm{f_1}{\lambda} \leq \frac{\alpha_2\eps_1\eps_2}{\lambda} + \alpha_3\eps_1 \leq \eps_2
\end{align*}
for large enough $\lambda$ (depending on $\alpha_2,\alpha_3,\eps_1,\eps_2$), using the condition $\alpha_3\eps_1 < \eps_2$ in the last step. For contractivity, direct calculation shows that, with $(\bar{f}_1,\bar{f}_2) = \cT_{12}((f_1,f_2))$ and $(\bar{g}_1,\bar{g}_2) = \cT_{12}((g_1,g_2))$,
\begin{align*}
\pnorm{\bar{f}_1 - \bar{g}_1}{\lambda} \leq \frac{\alpha_1 + \eps_2}{\lambda}\pnorm{f_1-g_1}{\lambda} + \frac{\eps_1}{\lambda}\pnorm{f_2-g_2}{\lambda}, \quad \pnorm{\bar{f}_2 - \bar{g}_2}{\lambda} \leq (\alpha_2\eps_2 + \alpha_3)\pnorm{f_1-g_1}{\lambda} + \alpha_2\eps_1\pnorm{f_2-g_2}{\lambda}.
\end{align*}
Hence for any $K_1, K_2 > 0$, 
\begin{align*}
K_1\pnorm{\bar{f}_1 - \bar{g}_1}{\lambda} + K_2\pnorm{\bar{f}_2 - \bar{g}_2}{\lambda} \leq K_1\pnorm{f_1 - g_1}{\lambda}\Big(\frac{\alpha_1 + \eps_2}{\lambda} + \frac{K_2}{K_1}(\alpha_2\eps_2 + \alpha_3)\Big) + K_2\pnorm{f_2-g_2}{\lambda} \cdot \Big(\frac{K_1}{K_2}\frac{\eps_1}{\lambda} + \alpha_2\eps_1\Big).
\end{align*}
Plugging in $K_2 =1$ and $K_1 = 4\alpha_3$ and using the condition $\eps_2 < \alpha_3/\alpha_2$, we have $d((\bar{f}_1,\bar{f}_2), (\bar{g}_1,\bar{g}_2)) \leq d((f_1,f_2), (g_1,g_2))/2$, showing the contractivity of $\cT_{12}$. Hence by Banach fixed point theorem, there exists a solution $(f_1(t),f_2(t))$ belonging to $\cS_{12}$.
\medskip

\noindent{\textbf{Solution of $f_3(t)$}} For any $\eps_3$ such that
\begin{align}\label{eq:eps_condition_2}
\eps_3 \geq 2\alpha_4\alpha_5 \eps_1, 
\end{align}
let
\begin{align*}
\cS_3 \equiv \{f_3:\pnorm{f_3}{\lambda} \leq \eps_3\}. 
\end{align*}
Define the map
\begin{align*}
\bar{f}_3(t) \equiv \cT_3[f_3](t) \equiv \alpha_4\int_0^t f_1(t-s)(f_3(s) + \alpha_5)\d s.
\end{align*}
We have
\begin{align*}
\pnorm{\bar{f}_3}{\lambda} \leq \alpha_4\pnorm{f_1}{\lambda}\pnorm{f_3}{\lambda} + \alpha_4\alpha_5\pnorm{f_1}{\lambda} \leq \alpha_4\eps_1\eps_3 + \alpha_4\alpha_5\eps_1 \leq \eps_3,
\end{align*}
using the conditions (\ref{eq:eps_condition_1}) and (\ref{eq:eps_condition_2}) in the last step. Moreover, for $f_3,g_3\in \cS_3$ and $\bar{f}_3 = \cT_3(f_3)$, $\bar{g}_3 = \cT_3(g_3)$,
\begin{align*}
\pnorm{\bar{f}_3 - \bar{g}_3}{\lambda} \leq \alpha_4 \pnorm{f_1}{\lambda}\pnorm{f_3 - g_3}{\lambda} \leq \alpha_4\eps_1\pnorm{f_3 - g_3}{\lambda} \leq \frac{1}{2}\pnorm{f_3 - g_3}{\lambda}. 
\end{align*}
Hence $\cT_3$ maps $\cS_3$ into itself and is contractive, and by the Banach fixed point theorem, there exists a solution for $f_3(t)$ in $\cS_3$.

\noindent{\textbf{Solution of $f_4(t)$ and $f_5(t)$}} We study the solution of $f_4(t)$ and $f_5(t)$ given $f_i(t)$, $i=1,2,3$ as established above. For any $f:\R_+ \rightarrow\R$ and $\lambda > 0$, let $\pnorm{f}{\infty, \lambda} \equiv \sup_{t\in[0,\infty)} e^{-\lambda t}|f(t)|$. For $\eps_4,\eps_5 > 0$ such that
\begin{align}\label{eq:eps_condition_3}
\eps_4 > \beta', \quad \eps_5 > \max\{\alpha_8\eps_4, \alpha_9\},
\end{align}
define the space
\begin{align*}
\cS_{45} = \{(f_4, f_5): \pnorm{f_4}{\infty, \lambda} \leq \eps_4, \pnorm{f_5}{\infty, \lambda} \leq \eps_5, f_4(0) = \beta' > 0\},
\end{align*}
equipped with the metric
\begin{align*}
d((f_4,f_5), (\tilde{f}_4,\tilde{f}_5)) = 4\alpha_8\pnorm{f_4 - \tilde{f}_4}{\infty,\lambda} + \pnorm{f_5 - \tilde{f}_5}{\infty,\lambda}. 
\end{align*}
Define the map $(\bar{f}_4, \bar{f}_5) = \cT_{45}(f_4, f_5)$, where
\begin{align*}
\frac{\d }{\d t} \bar{f}_4(t) &= \alpha_6\Big(f_4(t) + \int_0^t (t-s+1)^2 \cdot f_2^2(t-s)f_4(s)\d s + f_3^2(t) + f_5(t) + 1\Big),\\
\bar{f}_5(t) &= \alpha_7\int_0^t (t-s+1)^2\cdot f_1^2(t-s) f_5(s)\d s + \alpha_{8}f_4(t) + \alpha_{9},
\end{align*}
with initialization $\bar{f}_4(0) = \beta'$. We will show that $\cT_{45}$ maps $\cS_{45}$ into itself and is a contraction. For the first claim, note that
\begin{align*}
\bar{f}_4(t) = \beta' + \alpha_6\int_0^t f_4(s)\d s + \alpha_6\int_0^t \d s'\Big(\int_0^s (s-s'+1)^2 \cdot f_2^2(s-s')f_4(s')\d s'\Big) + \alpha_6 \int_0^t f_3^2(s)\d s + \alpha_6\int_0^t f_5(s)\d s + \alpha_6 \cdot t.
\end{align*}
We have $\sup_{t\in \R_+} \beta' e^{-\lambda t} = \beta', \sup_{t\in R_+} te^{-\lambda t} = 1/(e\lambda)$,
\begin{align*}
\int_0^t f_4(s)\d s \leq \frac{e^{\lambda t}}{\lambda}\pnorm{f_4}{\infty, \lambda}, \quad \int_0^t f_3^2(s)\d  \leq \frac{e^{\lambda t}}{\lambda}\pnorm{f_3}{\infty, \lambda/2}^2,\quad \int_0^t f_5(s)\d s \leq \frac{e^{\lambda t}}{\lambda}\pnorm{f_5}{\infty,\lambda}, 
\end{align*}
and
\begin{align*}
\int_0^t \d s'\Big(\int_0^s (s-s'+1)^2 \cdot f_2^2(s-s')f_4(s')\d s'\Big) &= \int_0^t \d s' f_4(s') \int_{s'}^t (s-s'+1)^2 f_2^2(s-s')\d s\\
&= \int_0^t \d s' f_4(s') \int_{0}^{t-s'} (s+1)^2 f_2^2(s)\d s\\
&\leq \int_0^t \d s' f_4(s') \Big(\int_{0}^{t-s'} (s+1)^2 f_2^2(s) e^{-\lambda s/2}\d s\Big) \cdot e^{\lambda(t-s')/2}\\
&\leq \underbrace{\int_0^\infty (s+1)^2 f_2^2(s) e^{-\lambda s/2}\d s}_{F_2(\lambda)} \cdot \int_0^t f_4(s)e^{\lambda(t-s)/2}\d s\\
&\leq F_2(\lambda) \cdot \pnorm{f_4}{\infty,\lambda} e^{\lambda t/2} \int_0^t e^{\lambda s/2}\d s \leq F_2(\lambda)\cdot \frac{2e^{\lambda t}}{\lambda} \cdot \pnorm{f_4}{\infty,\lambda}. 
\end{align*}
Here $F_2(\lambda) < \infty$ for large enough $\lambda$ since $f_2 \in \cS_{12}$. This implies 
\begin{align*}
\pnorm{\bar{f}_4}{\infty,\lambda} \leq \beta' + \frac{\alpha_6}{e\lambda} + \frac{\alpha_6(1+2F_2(\lambda))}{\lambda}\pnorm{f_4}{\infty,\lambda} + \frac{\alpha_6\pnorm{f_3}{\infty, \lambda/2}^2}{\lambda} + \frac{\alpha_6\pnorm{f_5}{\infty,\lambda}}{\lambda},
\end{align*}
hence under the condition (\ref{eq:eps_condition_3}), $\pnorm{\bar{f}_4}{\infty,\lambda} \leq \eps_4$ for large enough $\lambda$. Using a similar argument, we have
\begin{align*}
\pnorm{\bar{f}_5}{\infty, \lambda} \leq \alpha_7\cdot F_1(\lambda)\pnorm{f_5}{\infty,\lambda} + \alpha_8\pnorm{f_4}{\infty,\lambda} + \alpha_9,
\end{align*}
where $F_1(\lambda) = \int_0^\infty (s+1)^2f_1^2(s)e^{-\lambda s}\d s$ (again $F_1(\lambda) < \infty$ for large enough $\lambda$ since $f_1\in \cS_{12}$). Hence under the condition (\ref{eq:eps_condition_3}), we have $\pnorm{\bar{f}_5}{\infty, \lambda} \leq \eps_5$ for large enough $\lambda$. This concludes that $\cT_{45}$ maps $\cS_{45}$ into itself. To see it is a contraction, let $(\bar{f}_4,\bar{f}_5) = \cT_{45}((f_4,f_5))$ and $(\bar{g}_4,\bar{g}_5) = \cT_{45}((g_4,g_5))$, then
\begin{align*}
\bar{f}_4(t) - \bar{g}_4(t) &\quad= \alpha_6\int_0^t (f_4(s) - g_4(s))\d s + \alpha_6\int_0^t \d s'\Big(\int_0^s (s-s'+1)^2 \cdot f_2^2(s-s') (f_4(s') - g_4(s'))\d s'\Big)\\
&\quad  + \alpha_6\int_0^t (f_5(s) - g_5(s))\d s, 
\end{align*}
so using the same argument as above yields
\begin{align*}
\pnorm{\bar{f}_4 - \bar{g}_4}{} \leq \frac{\alpha_6(1+2F_2(\lambda))}{\lambda}\pnorm{f_4-g_4}{\infty,\lambda} + \frac{\alpha_6}{\lambda}\pnorm{f_5-g_5}{\infty.\lambda}. 
\end{align*}
Similarly,
\begin{align*}
\bar{f}_5(t) - \bar{g}_5(t) &= \alpha_7\int_0^t (t-s+1)^2\cdot f_1^2(t-s) (f_5(s) - g_5(s))\d s + \alpha_{8}(f_4(t) - g_4(t)),
\end{align*}
and hence
\begin{align*}
\pnorm{\bar{f}_5 - \bar{g}_5}{} \leq \frac{\alpha_7 F_1(\lambda)}{\lambda}\pnorm{f_5 - g_5}{\infty,\lambda} + \alpha_8\pnorm{f_4 - g_4}{\infty,\lambda}.
\end{align*}
So for any $K_1, K_2 > 0$, we have
\begin{align*}
K_1\pnorm{\bar{f}_4 - \bar{g}_4}{\infty,\lambda} + K_2\pnorm{\bar{f}_5 - \bar{g}_5}{\lambda} \leq K_1\pnorm{f_4 -g_4}{\infty,\lambda}\cdot\Big(\frac{\alpha_6(1+2F_2(\lambda))}{\lambda} + \frac{K_2\alpha_8}{K_1}\Big) + K_2\pnorm{f_5 - g_5}{\infty,\lambda}\cdot\Big(\frac{\alpha_7F_1(\lambda)}{\lambda} + \frac{\alpha_6K_1}{\lambda K_2}\Big).
\end{align*}
Plug in $K_2 = 1$, $K_1 = 1/(4\alpha_8)$ and choose $\lambda$ large enough, we see $d((\bar{f}_4,\bar{f}_5), (\bar{g}_4, \bar{g}_5)) \leq d((f_4,f_5), (g_4, g_5))/2$, hence $\cT_{45}$ is contractive, and by Banach fixed point theorem, it admits a fixed point solution $f_4(t), f_5(t)$. 
\end{proof}

\subsection{Spaces $\cS_\eta$ and $\cS_\theta$}\label{subsec:space_S_eta_theta}
Recall the auxiliary functions $(\Phi_{R_\theta}, \Phi_{C_\theta}, \Phi_{R_\eta}, \Phi_{R_\eta^\ast}, \Phi_{C_\eta})$ defined in (\ref{eq:auxiliary_eq}). Let $\mathcal{S}_\eta \equiv \mathcal{S}_\eta(T,\Phi_{R_\eta})$ be the set of $X_\eta = (R_\eta(t,s), R_\eta(t,\ast), C_\eta(t,s))$ such that
\begin{itemize}
\item $C_\eta(t,s)$ is a psd covariance kernel (hence satisfies $C_\eta(t,s) = C_\eta(s,t)$) satisfying
\begin{align}\label{eq:Ceta_cond_1}
0 \leq C_\eta(t,t) \leq \Phi_{C_\eta}(t)
\end{align}
and
\begin{align}\label{eq:Ceta_cond_2}
\big|C_\eta(t,t) - 2C_\eta(t,s) + C_\eta(s,s)\big| \leq M_{C_\eta} \cdot |t-s|
\end{align}
for some $M_{C_\eta} > 0$.
\item $R_\eta(t,s)$ is measurable with $R_\eta(t,s) = 0$ for $t < s$. For $0 \leq s \leq t \leq T$, it holds that
\begin{align}\label{eq:Reta_cond_1}
|R_\eta(t,s)| \leq \Phi_{R_\eta}(t-s). 
\end{align} 
\item $R_\eta(t,\ast)$ is continuous for $t\in[0,T]$ and satisfies $|R_\eta(t,\ast)| \leq \Phi_{R_\eta^\ast}(t)$.
\end{itemize}
Similarly, let $\mathcal{S}_\theta \equiv \mathcal{S}_\theta(T,\Phi_{R_\theta})$ be the set of $X_\theta = (R_\theta(t,s), C_\theta(t,\ast), C_\theta(t,\ast))$ such that
\begin{itemize}
\item $C_\theta(t,s)$ is a psd covariance kernel (hence satisfies $C_\theta(t,s) = C_\theta(s,t)$) satisfying
\begin{align}\label{eq:Ctheta_cond_1}
0 \leq C_\theta(t,t) &\leq \Phi_{C_\theta}(t)
\end{align}
and
\begin{align}\label{eq:Ctheta_cond_2}
\big|C_\theta(t,t) - 2C_\theta(t,s) + C_\theta(s,s)\big| &\leq M_{C_\theta} \cdot |t-s|, \quad t,s\in [0,T], 
\end{align}
for some $M_{C_\theta} > 0$.
\item $R_\theta(t,s)$ is measurable with $R_\theta(t,s) = 0$ for $t < s$. For $0 \leq s \leq t \leq T$, it holds that
\begin{align}\label{eq:Rtheta_cond}
|R_\theta(t,s)| \leq \Phi_{R_\theta}(t-s),
\end{align}
and for $0\leq r \leq s \leq t \leq T$, it holds that
\begin{align}\label{eq:Rtheta_cont}
|R_\theta(t,r) - R_\theta(s,r)| \leq M_{R_\theta}\cdot |t - s|
\end{align}
for some $M_{R_\theta} > 0$.
\end{itemize}

%\begin{align*}
%\mathcal{S}_\eta &\equiv \mathcal{S}_\eta(T,\Phi_{R_\eta}) \equiv \{X_\eta = (R_\eta(t,s), R_\eta(t,\ast), C_\eta(t,s)): |R_\eta(t,s)| \leq \Phi_{R_\eta}(t-s)\},\\
%\mathcal{S}_\theta &\equiv \mathcal{S}_\theta(T,\Phi_{R_\theta}) \equiv \{X_\theta = (R_\theta(t,s), C_\theta(t,s), C_\theta(t,\ast)): |R_\theta(t,s)| \leq \Phi_{R_\theta}(t-s)\}.
%\end{align*}




%For any $T > 0$ and $\lambda > 0$, let
%\begin{align*}
%E_1 \equiv C([0,T], \R),
%\end{align*}
%the space of continuous real-valued functions on $[0,T]$ equipped with the metric
%\begin{align}\label{eq:metric_1}
%d(g_1,g_2) \equiv d(g_1,g_2;\lambda, T) \equiv \sup_{t\in[0,T]} e^{-\lambda t}|g_1(t) - g_2(t)|.
%\end{align}

\begin{lemma}\label{lem:sub_theta_solution}
Suppose Assumption \ref{assump:lipschitz} holds. Fix any $T > 0$, initialization $\theta^0$ of (\ref{eq:theta_1}) and $\frac{\partial \theta^s}{\partial u^s} = 1$ of (\ref{eq:theta_2}), and realization of $\theta^\ast$. Then for any $X_\eta = (\{R_\eta(t,s)\}, \{R_\eta(t,\ast)\}, \{C_\eta(t,s)\}) \in \mathcal{S}_\eta$ and $\{\alpha^t\} \in C([0,T],\R)$ such that $\sup_{t\in[0,T]} |\alpha^t| \leq M_\alpha$, there exists a pathwise unique  (with respect to the randomness of $\{u^t\}$ and $\{B^t\}$) solution of the following system:
\begin{align}
\d\theta^t &= \Big[{-}\frac{\delta}{\sigma^2}(\theta^t-\theta^*) + \partial_\theta \log g(\theta^t;\alpha^t)(\theta^t)
-\int_0^{t} R_\eta(t, s)\theta^{s}\d s-R_\eta(t,*)\theta^\ast
+ u^t\Big]\d t + \sqrt{2}\,\d B^t,\label{eq:theta_1}\\
\frac{\d}{\d t}\alpha^t &= \cF(\alpha^t, \cL(\theta^t)), \label{eq:alpha_1}\\
\frac{\d }{\d t}\frac{\partial\theta^t}{\partial u^s} &= -\bigg(
\frac{\delta}{\sigma^2} - \partial^2_\theta \log g(\theta^t;\alpha^t)\bigg)\frac{\partial \theta^{t}}{\partial u^s} -\int_s^{t} R_\eta(t,s')\frac{\partial \theta^{s'}}{\partial u^s}\d s',\label{eq:theta_2}
\end{align}
where $(\{u^t\},\{B^t\})$ are distributed as in (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}). 
\end{lemma}
\begin{proof}
First note that
\begin{align*}
\E[(u^t-u^s)^2] = C_\eta(t,t) - 2 C_\eta(t,s) + C_\eta(s,s) \leq M_{C_\eta} \cdot |t-s|, 
\end{align*}
hence by Kolmogorov's continuity theorem (cf. \cite[Theorem 2.9]{legall2016brownian}), it holds that $t\mapsto u^t$ is continuous with probability one (note that for Gaussian processes, modulus of the type $\E[(u^t-u^s)^2] \lesssim |t-s|^\alpha$ for any $\alpha > 0$ suffices for continuity). On the other hand, the Brownian motion $\{b^t\}$ has continuous sample paths with probability 1, so in the following we will prove existence and uniqueness of solution in the intersection of these two events.  

To show the existence and uniqueness of solution to the system (\ref{eq:theta_1})-(\ref{eq:alpha_1}), we first show that for (\ref{eq:theta_1}) and (\ref{eq:alpha_1}) individually. More specifically, we first show for any given $X_\eta$ and $\alpha = \{\alpha^t\}$ such that $\sup_{t\in[0,T]} \pnorm{\alpha^t}{} \leq M_\alpha$ for some $M_\alpha > 0$,  (\ref{eq:theta_1}) admits a unique solution. To see this, for any $\theta = \{\theta^t\}_{t\in[0,T]} \in C([0,T], \R)$, define the map from $C([0,T],\R)$ to itself:
\begin{align*}
(\Gamma \theta)^t = \theta^0 + \int_0^t \Big[-\frac{\delta}{\sigma^2}(\theta^s - \theta^\ast) + \partial_\theta \log g(\theta^s;\alpha^s)\Big]\d s - \int_0^t \Big(\int_0^s R_\eta(s,s')\theta^{s'}\d s'\Big)\d s - \int_0^t \Big(R_\eta(s,\ast)\theta^\ast - u^s\Big)\d s + \sqrt{2}B^t. 
\end{align*}
Note that $\Gamma$ is well-defined since both $\{R_\eta(t,\ast)\}$ and $\{u^t\}$ are continuous and hence integrable over $[0,T]$. 
%Since $\{u_t\} \in L^1([0,T])$ and $\{B^t\}$ is continuous with probability one, $\Gamma$ maps $C([0,T],\R)$ into itself on such event. 
We will now establish that $\Gamma$ is a contractive mapping under the metric
\begin{align*}
d(g_1,g_2) \equiv d(g_1,g_2;\lambda, T) \equiv \sup_{t\in[0,T]} e^{-\lambda t}|g_1(t) - g_2(t)|
\end{align*}
for some large enough $\lambda$. To see this, note that for $\theta = \{\theta^t\}$ and $\tilde{\theta} = \{\tilde{\theta}^t\} \in C([0,T],\R)$ such that $\theta^0 = \tilde{\theta}^0$,
\begin{align*}
d(\Gamma \theta, \Gamma\tilde{\theta}) &= \sup_{t\in[0,T]} e^{-\lambda t}|(\Gamma \theta)^t - (\Gamma \tilde{\theta})^t|\\
&\stackrel{(i)}{\leq}  \sup_{t\in[0,T]} e^{-\lambda t} \Big[(\frac{\delta}{\sigma^2} + L)\int_0^t |\theta^s - \tilde{\theta}^s| \d s + \Big|\int_0^t \Big(\int_s^t R_\eta(s',s)\d s'\Big)(\theta^s - \tilde{\theta}^s)\d s\Big| \Big]\\
&\leq \sup_{t\in[0,T]} e^{-\lambda t} \Big[(\frac{\delta}{\sigma^2} + L)(\int_0^t e^{\lambda s}\d s) \sup_{u\in [0,T]}e^{-\lambda u}|\theta^u - \tilde{\theta}^u| + \int_0^t \Big(\int_s^t \Phi_{R_\eta}(s' - s)\d s'\Big) e^{\lambda s}\d s \cdot \sup_{u\in[0,T]}e^{-\lambda u}|\theta^u - \tilde{\theta}^u| \Big]\\
&\stackrel{(ii)}{\leq} \frac{\delta/\sigma^2 + L}{\lambda} d(\theta,\tilde{\theta}) + \frac{1}{\mu(\lambda - \mu)}d(\theta, \tilde{\theta}), 
\end{align*}\\
where we apply Assumption \ref{assump:lipschitz}-(c) in (i) with $L = C(M_\alpha)$, and the condition $\Phi_{R_\eta}(t)\leq e^{\mu t}$ for $t\geq 0$ in (ii). This entails that $d(\Gamma \theta, \Gamma\tilde{\theta}) \leq d(\theta, \tilde{\theta})/2$ for large enough $\lambda$ (depending on $L,\delta,\sigma,\mu$), establishing the contractivity of $\Gamma$. Hence by Banach fixed point theorem, $\Gamma$ admits a fixed point which is the unique solution of (\ref{eq:theta_1}). 
%Moreover, this solution satisfies
%\begin{align*}
%\E(\theta^t)^2 &\leq C\Big[1 + \E(\theta^0)^2 + \int_0^t \E(\theta^s)^2 \d s + \int_0^t \E(\partial_\theta \log g(\theta^s;\alpha^s))^2\d s + \int_0^t \E (\theta^s)^2 \cdot \Big(\int_s^t R_\eta(s',s)\d s'\Big)^2\d s\\
%&\quad + \Big(\int_0^t R_\eta(s,\ast)\d s\Big)^2 \cdot \E(\theta^\ast)^2 + \int_0^t \E(u^s)^2 \d s\Big]. 
%\end{align*}
%We first apply $\int_0^t \E(\theta^s)^2 \d s \leq \frac{e^{2\lambda t}}{2\lambda} \sup_{t\in[0,T]} e^{-2\lambda t} \E(\theta^t)^2$. Next using assumption (\ref{eq:mix_deriv_lip}),
%\begin{align*}
%\int_0^t \E(\partial_\theta \log g(\theta^s;\alpha^s))^2\d s &\leq 2 \int_0^t \E(\partial_\theta \log g(\theta^s;0))^2\d s + 2 \int_0^t \E(\partial_\theta \log g(\theta^s;\alpha^s) - \partial_\theta \log g(\theta^s;0))^2\d s\\
%&\leq C\Big[1 + \int_0^t \E(\theta^s)^2\d s + \int_0^t \E(\theta^s)^2 \cdot \pnorm{\alpha^s}{}^2 \d s\Big]
%\end{align*}
Similarly, 
%Next we establish the existence and uniqueness of solution to (\ref{eq:alpha_1}) given any continuous random process $\theta = \{\theta^t\}$. 
define the map
\begin{align*}
(\Gamma \alpha)^t = \alpha^0 + \int_0^t \cF(\alpha^s, \cL(\theta^s))\d s. 
\end{align*}
For any $\alpha = \{\alpha^t\} \in C([0,T], \R^K)$, let $\pnorm{\alpha}{} = \sup_{t\in [0,T]} e^{-\lambda t} \pnorm{\alpha^t}{}$ for some $\lambda > 0$ to be specified later.  By Assumption \ref{assump:lipschitz}-(a), for any $\{\alpha^t\} \in C([0,T],\R^K)$ and $t\in [0,T]$, 
\begin{align*}
\pnorm{(\Gamma \alpha)^t}{} &\leq \pnorm{\alpha^0}{} + \int_0^t C(\pnorm{\alpha^s}{} + 1)\d s\\
&\leq (\pnorm{\alpha^0}{} + CT) + \int_0^t Ce^{\lambda s} \sup_{u\in[0,T]} e^{-\lambda u} \pnorm{\alpha^u}{}\d s\\
&\leq (\pnorm{\alpha^0}{} + CT) + \frac{C}{\lambda} e^{\lambda t} \pnorm{\alpha}{},
\end{align*}
yielding that $\pnorm{\Gamma\alpha}{} = \sup_{t\in [0,T]} e^{-\lambda t} \pnorm{(\Gamma \alpha)^t}{} \leq (\pnorm{\alpha^0}{} + CT) + \frac{1}{2} \pnorm{\alpha}{}$ for $\lambda \geq 2C$. This entails that $\Gamma$ maps the Banach space $C^\circ([0,T], \R^K) := C([0,T], \R^K) \cap \{\alpha: \pnorm{\alpha}{} \leq 2(\pnorm{\alpha^0}{} + CT)\}$ into itself. Moreover, for any $\alpha = \{\alpha^t\}$ and $\tilde{\alpha} = \{\tilde{\alpha}^t\}$ in the above space with $\alpha^0 = \tilde{\alpha}^0$, Assumption \ref{assump:lipschitz}-(b) yields
\begin{align*}
\big|(\Gamma\alpha)^t - (\Gamma \tilde{\alpha})^t \big| &\leq \int_0^t \Big|\cF(\alpha^s, \cL(\theta^s)) - \cF(\tilde{\alpha}^s, \cL(\theta^s))\Big| \d s\\
&\leq C \int_0^t e^{\lambda s}\d s \cdot \sup_{t\in [0,T]} e^{-\lambda t}\pnorm{\alpha^t - \tilde{\alpha}^t}{}\\
&\leq \frac{Ce^{\lambda t}}{\lambda} \sup_{t\in [0,T]} e^{-\lambda t}\pnorm{\alpha^t - \tilde{\alpha}^t}{}. 
\end{align*}
Hence under the metric $d(\alpha, \tilde{\alpha}) = \sup_{t\in[0,T]} e^{-\lambda t}\pnorm{\alpha^t - \tilde{\alpha}^t}{}$, we have $d(\Gamma \alpha, \Gamma \tilde{\alpha}) \leq 0.1 d(\alpha, \tilde{\alpha})$ for large enough $\lambda$. This implies $\Gamma$ is a contraction and admits a fixed point in $C^\circ([0,T],\R^K)$, which is the unique solution of (\ref{eq:alpha_1}) in this space. This is also the unique solution in $C([0,T],\R^K)$ because a similar consideration as above using Assumption \ref{assump:lipschitz}-(a) shows that any solution of (\ref{eq:alpha_1}) must satisfy 
\begin{align}\label{eq:alpha_bound}
\pnorm{\alpha}{} \leq 2(\pnorm{\alpha^0}{} + CT).
\end{align}
%Moreover, this solution satisfies 
%\begin{align*}
%\frac{\d}{\d t}\pnorm{\alpha^t}{} \leq \pnorm{\frac{\d}{\d t}\alpha^t}{} \leq \pnorm{\cL(\alpha^t, \delta_0)}{} + W_2(\cL(\theta^t), \delta_0) \leq \pnorm{\cL(0, \delta_0)}{} + C\pnorm{\alpha_t}{} + \sqrt{\E (\theta^t)^2} , 
%\end{align*}
%where $C_0 = \sup_{P\in \cP_2(\R)} \pnorm{\cF(0_K, P)}{}$ \ys{need this to be finite}. This implies $\pnorm{\alpha^t}{} \leq \frac{C_0}{C}(e^{Ct}-1) + \pnorm{\alpha^0}{}e^{Ct}$, hence 
%\begin{align}\label{eq:alpha_bound}
%\sup_{t\in[0,T]} \pnorm{\alpha^t}{}\leq M_\alpha, \quad M_\alpha = \frac{C_0}{C}(e^{CT}-1) + \pnorm{\alpha^0}{}e^{CT}.
%\end{align}

Next we establish the joint solution to (\ref{eq:theta_1})-(\ref{eq:alpha_1}). Let $\cL_T$ denote the laws on $C([0,T],\R)$. Define the map $\Gamma: \cL_T \times C^\circ([0,T], \R^K)$ as follows: $\Gamma(q_\theta, \alpha) = (\bar{q}_\theta, \bar{\alpha})$, where $\bar{q}_\theta$ is the law of the solution to (\ref{eq:theta_1}) with input $\alpha = \{\alpha^t\}$, and $\bar{\alpha}$ is the solution to (\ref{eq:alpha_1}) with input $q_\theta = \{q_\theta^t\}$. For $q_1, q_2 \in \cL_T$, let
\begin{align*}
d(q_{\theta,1}, q_{\theta,2}) = \inf_{\theta_1 \sim q_{\theta,1}, \theta_2 \sim q_{\theta,2}} \sup_{t\in[0,T]} e^{-\lambda t} \sqrt{\E (\theta_1^t - \theta_2^t)^2},
\end{align*}
and we equip $\cL_T \times C^\circ([0,T], \R^K)$ with the distance $d((q_{\theta,1}, \alpha_1), (q_{\theta,2}, \alpha_2)) = d(q_{\theta,1}, q_{\theta,2}) + d(\alpha_1, \alpha_2)$ with $d(\alpha_1,\alpha_2) = \sup_{t\in[0,T]} e^{-\lambda t} \pnorm{\alpha^t_1 - \alpha^t_2}{}$. For $(q_{\theta,i},\alpha_i)$ and $(\bar{q}_{\theta,i},\bar{\alpha}_i) = \Gamma(q_{\theta,i},\alpha_i)$, $i=1,2$, let us compute $d((\bar{q}_{\theta,1}, \bar{\alpha}_1), (\bar{q}_{\theta,2}, \bar{\alpha}_2))$. Let $\bar{\theta}_1$ and $\bar{\theta}_2$ be the solution of (\ref{eq:theta_1}) with input $\alpha_1$ and $\alpha_2$ and the same Gaussian process $\{u^t\}$ and $\{B^t\}$, i.e.,
\begin{align*}
\bar{\theta}^t_i = \theta^0 + \int_0^t \Big[-\frac{\delta}{\sigma^2}(\bar{\theta}_i^s - \theta^\ast) + \partial_\theta \log g(\bar{\theta}_i^s;\alpha_i^s)\Big]\d s - \int_0^t \Big(\int_0^s R_\eta(s,s')\bar{\theta}_i^{s'}\d s'\Big)\d s - \int_0^t \Big(R_\eta(s,\ast)\theta^\ast - u^s\Big)\d s + \sqrt{2}B^t.
\end{align*}
Then the law of $\bar{\theta}_1$ (resp. $\bar{\theta}_2$) is $\bar{q}_{\theta,1}$ (resp. $\bar{q}_{\theta,2}$), and
\begin{align*}
\E(\bar{\theta}^t_1 - \bar{\theta}^t_2)^2 &= \E\Big[-\frac{\delta}{\sigma^2} \int_0^t (\bar{\theta}_1^s - \bar{\theta}^s_2)\d s + \int_0^t \big(\partial_\theta \log g(\bar{\theta}_1^s;\alpha_1^s) - \partial_\theta \log g(\bar{\theta}_2^s;\alpha_2^s))\d s - \int_0^t(\bar{\theta}^s_1 - \bar{\theta}^s_2)\Big(\int_s^t R_\eta(s',s)\d s'\Big) \d s \Big]^2\\
&\leq 3t \cdot \Big[\Big(\frac{\delta}{\sigma^2}\Big)^2\underbrace{\int_0^t \E(\bar{\theta}_1^s - \bar{\theta}^s_2)^2\d s}_{(I)} + \underbrace{\int_0^t \E\big(\partial_\theta \log g(\bar{\theta}_1^s;\alpha_1^s) - \partial_\theta \log g(\bar{\theta}_2^s;\alpha_2^s))^2\d s}_{(II)}\\
&\quad + \underbrace{\int_0^t \E(\bar{\theta}^s_1 - \bar{\theta}^s_2)^2 \cdot \Big(\int_s^t R_\eta(s',s)\d s'\Big)^2 \d s}_{(III)}\Big]
\end{align*}
Term $(I)$ is bounded by $\frac{e^{2\lambda t}}{2\lambda} \sup_{t\in[0,T]} e^{-2\lambda t} \E(\bar{\theta}^t_1 - \bar{\theta}^t_2)^2$. Next using Assumption \ref{assump:lipschitz}-(c) and the fact that $\alpha_1,\alpha_2 \in C^\circ([0,T],\R^K)$,
\begin{align*}
(II) &\leq 2\int_0^t \E\big(\partial_\theta \log g(\bar{\theta}_1^s;\alpha_1^s) - \partial_\theta \log g(\bar{\theta}_2^s;\alpha_1^s))^2\d s + 2\int_0^t \E\big(\partial_\theta \log g(\bar{\theta}_2^s;\alpha_1^s) - \partial_\theta \log g(\bar{\theta}_2^s;\alpha_2^s))^2\d s\\
&\leq C\int_0^t \E(\bar{\theta}_1^s - \bar{\theta}_2^s)^2 \d s + C\int_0^t \pnorm{\alpha^s_1 - \alpha_2^s}{}^2 \d s \leq \frac{Ce^{2\lambda t}}{2\lambda} \sup_{t\in [0,T]} e^{-2\lambda t}\E(\bar{\theta}_1^t - \bar{\theta}_2^t)^2 + \frac{Ce^{2\lambda t}}{2\lambda}d^2(\alpha^1,\alpha^2). 
\end{align*}
Term $(III)$ is also bounded by $\frac{e^{2\lambda t}}{2\lambda} \sup_{t\in[0,T]} e^{-2\lambda t} \E(\bar{\theta}^t_1 - \bar{\theta}^t_2)^2$, so we conclude that for large $\lambda$, 
\begin{align*}
d^2(\bar{q}_{\theta,1}, \bar{q}_{\theta,2}) \leq \sup_{t\in [0,T]} e^{-2\lambda t}\E(\bar{\theta}^t_1 - \bar{\theta}^t_2)^2 \leq (0.1)^2 d^2(\alpha^1,\alpha^2),
\end{align*}
implying $d(\bar{q}_{\theta,1}, \bar{q}_{\theta,2}) \leq 0.1 \cdot d(\alpha^1,\alpha^2)$. On the other hand, using $\bar{\alpha}_i^t = \alpha^0 + \int_0^t \cF(\bar{\alpha}_i^s, q^s_{\theta,i})$, $i=1,2$, we have
\begin{align}\label{eq:alpha_modulus}
\notag\pnorm{\bar{\alpha}_1^t - \bar{\alpha}_2^t}{} &\leq \int_0^t \pnorm{\cF(\bar{\alpha}_1^s, q_{\theta,1}^s) - \cF(\bar{\alpha}_2^s, q^s_{\theta,2})}{} \d s\\
\notag&\leq \int_0^t \pnorm{\cF(\bar{\alpha}_1^s, q_{\theta,1}^s) - \cF(\bar{\alpha}_2^s, q^s_{\theta,1})}{} \d s + \int_0^t \pnorm{\cF(\bar{\alpha}_2^s, q_{\theta,1}^s) - \cF(\bar{\alpha}_2^s, q^s_{\theta,2})}{} \d s\\
&\leq C\int_0^t \pnorm{\bar{\alpha}_1^s - \bar{\alpha}_2^s}{}\d s + C\int_0^t W_2(q_{\theta,1}^s, q_{\theta,2}^s)\d s.
\end{align}
Let $\theta_1$ and $\theta_2$ be a coupling of $q_{\theta,1}$ and $q_{\theta,2}$ such that $\sup_{t\in[0,T]} e^{-\lambda t} \sqrt{\E (\theta_1^t - \theta_2^t)^2} = d(q_{\theta,1},q_{\theta,2})$. Then
\begin{align*}
W_2(q_{\theta,1}^s, q_{\theta,2}^s) \leq \sqrt{\E(\theta_1^s - \theta_2^s)^2} \leq e^{\lambda s} \cdot \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E(\theta_1^t - \theta_2^t)^2} = e^{\lambda s} \cdot d(q_{\theta,1},q_{\theta,2}).
\end{align*}
This implies
\begin{align*}
\pnorm{\bar{\alpha}_1^t - \bar{\alpha}_2^t}{} &\leq C\int_0^t \pnorm{\bar{\alpha}_1^s - \bar{\alpha}_2^s}{}\d s + C \int_0^t e^{\lambda s} \d s \cdot d(q_{\theta,1},q_{\theta,2})\\
&\leq \frac{Ce^{\lambda t}}{\lambda} d(\bar{\alpha}_1, \bar{\alpha}_2) + \frac{Ce^{\lambda t}}{\lambda} d(q_{\theta,1},q_{\theta,2}), 
\end{align*}
which further implies that, for large enough $\lambda$, 
\begin{align*}
d(\bar{\alpha}_1,\bar{\alpha}_2) \leq 0.1 \cdot d(q_{\theta,1},q_{\theta,2}).
\end{align*}
We therefore conclude that $d((\bar{q}_{\theta,1}, \bar{\alpha}_1), (\bar{q}_{\theta,2}, \bar{\alpha}_2)) \leq 0.1 \cdot d((q_{\theta,1}, \alpha_1), (q_{\theta,2}, \alpha_2))$, which implies that $\Gamma$ is a contraction that maps $\cL_T \times C^\circ([0,T], \R^K)$ into itself. By the Banach fixed point theorem, it admits a unique fixed point which is the unique solution to (\ref{eq:theta_1})-(\ref{eq:alpha_1}).



%Now let $\Omega = C([0,T], \R) \times \{\alpha \in C([0,T],\R^K): \sup_{t\in[0,T]} \pnorm{\alpha^t}{} \leq M_\alpha\}$, and for each $X_\eta \in \cS_\eta$ and $\bar{\theta} = (\theta, \alpha) \in \Omega$, define the map $\bar{\Gamma}: \Omega \rightarrow \Omega$ as follows: $(\Gamma \bar{\theta})[\theta]$, the $\theta$ component of $\Gamma \bar{\theta}$, is the solution to (\ref{eq:theta_1}), and $(\Gamma \bar{\theta})[\alpha]$, the $\alpha$ component of $\Gamma \bar{\theta}$, is the solution to (\ref{eq:alpha_1}) when the input random process is $(\Gamma \bar{\theta})[\theta]$ (randomness comes from $\{u^t\}$ and $\{b^t\}$). Then if we equip $\Omega$ with the following metric: for $\bar{\btheta}_i = (\theta_i, \alpha_i)$ for $i=1,2$,
%\begin{align*}
%d(\bar{\theta}_1, \bar{\theta}_2) = \sup_{t\in[0,T]} e^{-\lambda t} |\theta^t_1 - \theta^t_2| + \sup_{t\in[0,T]} e^{-\lambda t} \pnorm{\alpha^t_1 - \alpha^t_2}{}, 
%\end{align*}
%then the above calculation shows that, for a large enough $\lambda$, $d(\bar{\Gamma}\bar{\theta}_1, \bar{\Gamma}\bar{\theta}_2) \leq \eps \cdot d(\bar{\theta}_1,\bar{\theta}_2)$ for any $\eps > 0$. This shows $\bar{\Gamma}$ is a contraction and thus has a unique fixed point in $\Omega$, which is the solution to the system (\ref{eq:theta_1}) and (\ref{eq:alpha_1}).




Given the existence and uniqueness of the $\theta$ solution, it suffices to establish the existence and uniqueness of solution of (\ref{eq:theta_2}) for a fixed realization of $\theta = \{\theta^t\}_{t\in[0,T]}$. Moreover, since the equation (\ref{eq:theta_2}) is separable in the time index $s$, it suffices to show existence and uniqueness for a fixed $s$. To this end, consider the space $C([s,T], \R)$ equipped with the norm $d(r_1,r_2;\lambda, T) \equiv \sup_{t\in[s,T]} e^{-\lambda t}|r_1^t - r_2^t|$. For any sequence $r = \{r^t\}_{t\in[s,T]}$, define the map
\begin{align*}
(\Gamma r)^t = 1 - \int_s^t \Big(\frac{\delta}{\sigma^2} - \partial_\theta^2 \log g(\theta^s;\alpha^s)\Big)r^{s'}\d s' - \int_s^t \Big(\int_s^{s'} R_\eta(s,s'')r^{s''}\d s''\Big)\d s,\quad t\in[s,T].
\end{align*} 
It is clear that $\Gamma r$ is continuous so $\Gamma$ maps $C([s,T], \R)$ into itself. Moreover, for any $r,\tilde{r} \in C([s,T], \R)$,
\begin{align*}
d(\Gamma r, \Gamma \tilde{r}) &= \sup_{t\in[s,T]} e^{-\lambda t} |(\Gamma r)^t - (\Gamma \tilde{r})^t|\\
&\leq \sup_{t\in[s,T]} e^{-\lambda t}\Big[(\frac{\delta}{\sigma^2} + L)\int_s^t |r^{s'} - \tilde{r}^{s'}|\d s' + \int_s^t \Big|\int_{s'}^t R_\eta(s'', s')\d s''\Big| |r^{s'} - \tilde{r}^{s'}| \d s'\Big]\\
&\leq \frac{\delta/\sigma^2 + L}{\lambda} d(r,\tilde{r}) + \frac{1}{\mu(\lambda - \mu)}d(r, \tilde{r}), 
\end{align*}
using the same argument as above. Hence $\Gamma$ is contractive and its unique fixed point, which satisfies the boundary condition $r^s = 1$, is the unique solution of (\ref{eq:theta_2}) with initialization $\frac{\partial \theta^s}{\partial u^s} = 1$ for the fixed $s\in[0,T]$.
\end{proof}

\begin{lemma}\label{lem:sub_eta_solution}
Suppose Assumption \ref{assump:lipschitz} holds. Then for any fixed $T > 0$ and $X_\theta = (\{R_\theta(t,s)\}, \{C_\theta(t,s)\}, \{C_\theta(t,\ast)\}) \in \mathcal{S}_\theta$, there exists with probability 1 (with respect to the randomness of $\{w^t\}$) a unique solution of the following system:
\begin{align}
\eta^t &= -\frac{1}{\sigma^2}\int_0^{t} R_\theta(t,s)\big(\eta^s - w^\ast -
\eps\big)\d s + w^t,\label{eq:eta_1}\\
\frac{\partial \eta^t}{\partial w^s} &= -\frac{1}{\sigma^2}\Big[\int_{s}^{t} R_\theta(t,s')\frac{\partial \eta^{s'}}{\partial w^s}\d s' + R_\theta(t,s)\Big]\label{eq:eta_2}\\
\frac{\partial \eta^t}{\partial w^\ast} &= -\frac{1}{\sigma^2}\int_{0}^{t}R_\theta(t,s')\Big(\frac{\partial \eta^{s'}}{\partial w^\ast}-1\Big)\d s',\label{eq:eta_3}
\end{align}
where $(\{w^t\},w^\ast,e)$ are distributed as in (\ref{def:dmft_langevin_cont_theta})-(\ref{def:dmft_langevin_alpha}). 
\end{lemma}
\begin{proof}
The proof is similar to that of Lemma \ref{lem:sub_theta_solution} so we only present the argument for (\ref{eq:eta_1}). Note that
\begin{align*}
\E[(w^t-w^s)^2] = C_\theta(t,t) - 2 C_\theta(t,s) + C_\theta(s,s) \leq M_{C_\theta} \cdot |t-s|, 
\end{align*}
hence by Kolmogorov's continuity theorem (cf. \cite[Theorem 2.9]{legall2016brownian}), it holds that $t\mapsto u^t$ is continuous with probability one. In the following we will prove existence and uniqueness of solution in this event.  

For any $\eta = \{\eta^t\}_{t\in[0,T]} \in C([0,T], \R)$, define the map
\begin{align*}
(\Gamma \eta)^t = -\frac{1}{\sigma^2}\int_0^{t} R_\theta(t,s)\big(\eta^s - w^\ast - \eps\big)\d s + w^t. 
\end{align*}
Note that $\Gamma$ is well-defined and maps $C([0,T],\R)$ into itself since $|R_\theta(t,s)| \leq \Phi_{R_\theta}(t-s)\leq \Phi_{R_\theta}(T)$ by assumption and $w^t$ is continuous. 
%Since $\{u_t\} \in L^1([0,T])$ and $\{B^t\}$ is continuous with probability one, $\Gamma$ maps $C([0,T],\R)$ into itself on such event. 
We will now establish that $\Gamma$ is a contractive mapping under the metric
\begin{align*}
d(g_1,g_2) \equiv d(g_1,g_2;\lambda, T) \equiv \sup_{t\in[0,T]} e^{-\lambda t}|g_1(t) - g_2(t)|
\end{align*}
for some large enough $\lambda$. To see this, note that for $\eta = \{\eta^t\}$ and $\tilde{\eta} = \{\tilde{\eta}^t\} \in C([0,T],\R)$,
\begin{align*}
|(\Gamma \eta)^t - (\Gamma\tilde{\eta})^t| \leq \frac{1}{\sigma^2}\int_0^t |R_{\theta}(t,s)||\eta^s - \tilde{\eta}^s|\d s \leq \frac{\Phi_{R_\theta}(T)}{\sigma^2} \cdot \sup_{t\in[0,T]} e^{-\lambda t}|\eta^t - \tilde{\eta}^t| \cdot \int_0^t e^{\lambda s}\d s \leq \frac{\Phi_{R_\theta}(T)}{\sigma^2} \cdot \frac{e^{\lambda t}}{\lambda}d(\eta,\tilde{\eta}).
\end{align*}
 This entails that $d(\Gamma \eta, \Gamma\tilde{\eta}) \leq d(\eta, \tilde{\eta})/2$ for large enough $\lambda$, establishing the contractivity of $\Gamma$. Hence by Banach fixed point theorem, $\Gamma$ admits a fixed point which is the unique solution of (\ref{eq:eta_1}).
\end{proof}

%\begin{lemma}\label{lem:sub_alpha_solution}
%Suppose Assumption \ref{assump:lipschitz} holds. For any fixed $T > 0$, initialization $\alpha^0$, and random process $\{\theta^t\}$, there exists a unique deterministic process $\{\alpha^t\}$ in $\cA$ with continuous sample path such that
%\begin{align}\label{eq:alpha_equation}
%\frac{\d}{\d t} \alpha^t = \cF(\alpha^t, \cL(\theta^t)).
%\end{align}
%\ys{boundary issue for $\cA$? can we choose $\cA$ to be entire $\R^K$?}
%\end{lemma}
%\begin{proof}
%The argument is same as above. Consider the map
%\begin{align*}
%(\Gamma \alpha)^t = \alpha^0 + \int_0^t \cF(\alpha^s, \cL(\theta^s)) \d s,
%\end{align*}
%which maps $C([0,T], \R^K)$ into itself. Then for $\alpha = \{\alpha^t\}$ and $\tilde{\alpha} = \{\tilde{\alpha}^t\}$ in $C([0,T],\R^K)$ with $\alpha^0 = \tilde{\alpha}^0$, using the metric $d(g_1,g_2) = \sup_{t\in[0,T]} e^{-\lambda t}|g_1(t) - g_2(t)|$, 
%\begin{align*}
%\pnorm{(\Gamma \alpha)^t - (\Gamma \tilde{\alpha})^t}{} \leq \int_0^t \pnorm{\cF(\alpha^s, \cL(\theta^s)) - \cF(\tilde{\alpha}^s, \cL(\theta^s))}{} \d s \leq \int_0^t C\pnorm{\alpha^s - \tilde{\alpha}^s}{}\d s \leq \frac{Ce^{\lambda t}}{\lambda} \cdot d(\alpha, \tilde{\alpha}), 
%\end{align*}
%so $\Gamma$ is a contraction for large enough $\lambda$, and its unique fixed point in $C([0,T], \R^K)$ is the unique solution to (\ref{eq:alpha_equation}).
%\end{proof}



\subsection{Contractive mapping}




For any $X_\eta = (R_\eta, R_\eta^\ast, C_\eta) \in \cS_\eta$, define a map $\cT_{\eta\rightarrow \theta}: X_\eta \rightarrow X_\theta = (R_\theta, C_\theta, C_\theta^\ast)$ as follows. Let $\theta = \{\theta^t\}_{t\in[0,T]}$, $\alpha = \{\alpha^t\}_{t\in[0,T]}$, and $\{\frac{\partial \theta^t}{\partial u^s}\}_{0\leq s \leq t\leq T}$ be the unique solution to (\ref{eq:theta_1})-(\ref{eq:theta_2}) guaranteed by Lemma \ref{lem:sub_theta_solution}, and then
\begin{align*}
R_\theta(t,s) \equiv \E\Big[\frac{\partial \theta^t}{\partial u^s}\Big], \quad C_\theta(t,s) \equiv \E[\theta^t\theta^s], \quad C^\ast_\theta(t) \equiv \E[\theta^t\theta^\ast].
\end{align*}
Similarly, for any $X_\theta = (R_\theta, C_\theta, C_\theta^\ast) \in \cS_\theta$, define a map $\cT_{\theta\rightarrow\eta}: X_\theta \rightarrow X_\eta = (R_\eta, R_\eta^\ast, C_\eta)$ as follows. Let $\eta = \{\eta^t\}_{t\in[0,T]}$, $\{\frac{\partial \eta^t}{\partial \omega^s}\}_{0\leq s < t \leq T}$, and $\{\frac{\partial \eta^t}{\partial \omega^\ast}\}_{t\in[0,T]}$ be the unique solution of (\ref{eq:eta_1})-(\ref{eq:eta_3}) guaranteed by Lemma \ref{lem:sub_eta_solution}, and then
\begin{align*}
R_\eta(t,s) \equiv \frac{\delta}{\sigma^2}\E\Big[\frac{\partial \eta^t}{\partial \omega^s}\Big], \quad R_\eta(t,\ast) \equiv \frac{\delta}{\sigma^2}\E\Big[\frac{\partial \eta^t}{\partial \omega^\ast}\Big], \quad C_\eta(t,s) \equiv \frac{\delta}{\sigma^4}\E[(\eta^t - \omega^\ast - \eps)(\eta^s - \omega^\ast - \eps)].
\end{align*}
Finally, define the composite map
\begin{align}\label{eq:composite_map}
\cT_{\eta\rightarrow\eta} \equiv \cT_{\theta\rightarrow\eta} \circ \cT_{\eta\rightarrow\theta}. 
\end{align}
The rest of this subsection is divided into two parts:
\begin{itemize}
\item (\textbf{Part 1}) We show in Lemma \ref{lem:Trange_theta_2_eta} (resp. Lemma \ref{lem:Trange_eta_2_theta}) that $\cT_{\theta \rightarrow \eta}$ maps $\cS_\theta$ into $\cS_\eta$ (resp. $\cT_{\eta \rightarrow \theta}$ maps $\cS_\eta$ into $\cS_\theta$). 
\item (\textbf{Part 2}) We equip $\cS_\eta$ and $\cS_\theta$ with certain metric and derive the modulus of continuity of the maps $\cT_{\eta \rightarrow \theta}$ and $\cT_{\theta \rightarrow \eta}$ in Lemmas  \ref{lem:modulus_eta_2_theta} and \ref{lem:modulus_theta_2_eta}, thereby concluding in Lemma \ref{lem:T_contract} that $\cT_{\eta\rightarrow\eta}$ in (\ref{eq:composite_map}) is a contraction under the above metric.
\end{itemize}
%For any two $X_i = (C_\eta^i, R_\eta^i, R_\eta^{\ast i})$, $i=1,2$, let $Y_i = T_{\eta\rightarrow\theta}(X_i) = (R_\theta^i, C_\theta^i, C_\theta^{\ast i})$. Then
%\begin{align*}
%d(\cT_{\eta\rightarrow\eta}(X^1), \cT_{\eta\rightarrow\eta}(X^2)) &= d(\cT_{\theta\rightarrow\eta}(Y^1), cT_{\theta\rightarrow\eta}(Y^2))\\
%&\leq d(\cT_{\theta\rightarrow\eta}(R_\theta^1, C_\theta^1, C_\theta^{\ast 1}), \cT_{\theta\rightarrow\eta}(R_\theta^1, C_\theta^1, C_\theta^{\ast 2})) + d(\cT_{\theta\rightarrow\eta}(R_\theta^1, C_\theta^1, C_\theta^{\ast 2}), cT_{\theta\rightarrow\eta}(R_\theta^1, C_\theta^2, C_\theta^{\ast 2})) + d(\cT_{\theta\rightarrow\eta}(R_\theta^i, C_\theta^i, C_\theta^{\ast i}), cT_{\theta\rightarrow\eta}(R_\theta^i, C_\theta^i, C_\theta^{\ast i}))
%\end{align*}

\begin{lemma}\label{lem:Trange_theta_2_eta}
$\cT_{\theta \rightarrow \eta}$ maps $\cS_\theta$ into $\cS_\eta$.
\end{lemma}
\begin{proof}
(\textbf{Condition for $C_\eta$}) Note that $C_\eta(t,s) = \frac{\delta}{\sigma^4}\E[\xi^t\xi^s]$ is a covariance kernel, where the process $\{\xi^t\}$ is defined as $\xi^t = \eta^t - w^\ast - \eps$ and satisfies
\begin{align*}
\xi^t = -\frac{1}{\sigma^2}\int_0^t R_\theta(t,s)\xi^s \d s + w^t - w^\ast - \eps. 
\end{align*}
This entails
\begin{align*}
\E[(\xi^t)^2] &\leq 2\E\Big[\frac{1}{\sigma^4}\Big(\int_0^t R_\theta(t,s)\xi^s\d s\Big)^2 + (w^t - w^\ast - \eps)^2\Big]\\
&\leq 2\Big[\frac{1}{\sigma^4}\int_0^t (t-s+1)^2 \cdot R_\theta(t,s)^2 \E[(\xi^s)^2]\d s \cdot \int_0^t (t-s+1)^{-2}\d s + 2 C_\theta(t,t) + 2 \E[(\theta^\ast)^2] + \sigma^2\Big]\\
&\leq 2\Big[\frac{1}{\sigma^4}\int_0^t (t-s+1)^2 \cdot \Phi^2_{R_\theta}(t-s) \E[(\xi^s)^2]\d s + 2 \Phi_{C_\theta}(t) + 2 \E[(\theta^\ast)^2] + \sigma^2\Big].
\end{align*}
Recall the equation for $\Phi_{C_\eta}(\cdot)$ in (\ref{eq:auxiliary_eq}):
\begin{align*}
\Phi_{C_\eta}(t) = \frac{2\delta}{\sigma^4}\Big[\frac{1}{\delta}\int_0^t (t-s+1)^2 \cdot \Phi^2_{R_\theta}(t-s) \Phi_{C_\eta}(s)\d s + 2\Phi_{C_\theta}(t) + 2 \E[(\theta^\ast)^2] + \sigma^2\Big],
\end{align*}
we therefore conclude that $C_\eta(t,t) \leq \Phi_{C_\eta}(t)$. On the other hand, for $t\geq s$, it holds that
\begin{align*}
0 &\leq C_\eta(t,t) - 2 C_\eta(t,s) + C_\eta(s,s)\\
&= \frac{\delta}{\sigma^4}\E[(\xi^t - \xi^s)^2]\\
&= \frac{\delta}{\sigma^4}\E\Big[\Big(-\frac{1}{\sigma^2}\int_0^t R_\theta(t,r)\xi^r\d r + \frac{1}{\sigma^2}\int_0^s R_\theta(s,r)\xi^r\d r + w^t - w^s\Big)^2\Big]\\
&\leq 3\cdot\Big[\frac{\delta}{\sigma^8} \E \Big(\int_0^s \big(R_\theta(t,r) - R_\theta(s,r)\big) \xi^r \d r\Big)^2 + \frac{\delta}{\sigma^8} \E\Big(\int_s^t R_\theta(t,r)\xi^r\d r\Big)^2 + \E(w^t - w^s)^2\Big].
\end{align*}
Using condition (\ref{eq:Rtheta_cont}) and $C_\eta(t,t)\leq \Phi_{C_\eta}(t)$ established above, it holds that $\E \Big(\int_0^s \big(R_\theta(t,r) - R_\theta(s,r)\big) \xi^r \d r\Big)^2 \leq K_1|t-s|$ for some $K_1 > 0$ depending on $M_{R_\theta}, T, \Phi_{C_\eta}(T)$. The second term $\E\Big(\int_s^t R_\theta(t,r)\xi^r\d r\Big)^2 \leq K_2|t-s|$ for some $K_2 > 0$ depending on $\Phi_{R_\theta}(T), T, \Phi_{C_\eta}(T)$, and the third term $\E(w^t - w^s)^2 = C_\theta(t,t) - 2C_\theta(t,s) + C_\theta(s,s) \leq M_{C_\theta}\cdot |t-s|$, so we have verified (\ref{eq:Ceta_cond_2}) for some $M_{C_\eta}$ depending on $\delta, \sigma, M_{C_\theta}, \Phi_{R_\theta}(T), T, \Phi_{C_\eta}(T)$.

\noindent (\textbf{Condition for $R_\eta$}) By definition, it holds that
\begin{align*}
R_\eta(t,s) = -\frac{1}{\sigma^2}\Big[\int_s^t R_\theta(t,s')R_\eta(s',s)\d s' + \frac{\delta}{\sigma^2}R_\theta(t,s)\Big], 
\end{align*}
hence
\begin{align*}
|R_\eta(t,s)| &\leq \frac{1}{\sigma^2}\Big(\int_s^t |R_\theta(t,s')||R_\eta(s',s)|\d s' + \frac{\delta}{\sigma^2}|R_\theta(t,s)|\Big)\\
&\leq \frac{1}{\sigma^2}\Big(\int_s^t \Phi_{R_\theta}(t-s')|R_\eta(s',s)|\d s' + \frac{\delta}{\sigma^2}\Phi_{R_\theta}(t-s)\Big).
\end{align*}
Recall the equation for $\Phi_{R_\eta}$ in (\ref{eq:auxiliary_eq}):
\begin{align*}
\Phi_{R_\eta}(t) = \frac{1}{\sigma^2}\Big(\int_0^t \Phi_{R_\theta}(t-s)\Phi_{R_\eta}(s)\d s + \frac{\delta}{\sigma^2}\Phi_{R_\theta}(t)\Big),
\end{align*}
which satisfies $\Phi_{R_\eta}(0) = (\delta/\sigma^4)\Phi_{R_\theta}(0) \geq \delta/\sigma^4 = \delta/\sigma^4|R_\theta(s,s)| = |R_\eta(s,s)|$, hence we conclude that $|R_\eta(t,s)|\leq \Phi_{R_\eta}(t-s)$, verifying (\ref{eq:Reta_cond_1}).

\noindent (\textbf{Condition for $R_\eta^\ast$}) By definition, it holds that
\begin{align*}
R_\eta(t,\ast) = -\frac{1}{\sigma^2}\int_{0}^{t}R_\theta(t,s)\Big(R_\eta(s,\ast)-\frac{\delta}{\sigma^2}\Big)\d s,
\end{align*}
hence
\begin{align*}
|R_\eta(t,\ast)| \leq \frac{1}{\sigma^2}\int_0^t |R_\theta(t,s)|\Big(|R_\eta(s,\ast)| + \frac{\delta}{\sigma^2}\Big)\d s \leq \frac{1}{\sigma^2}\int_0^t \Phi_{R_\theta}(t-s)\Big(|R_\eta(s,\ast)| + \frac{\delta}{\sigma^2}\Big)\d s.
\end{align*}
Recall the equation for $\Phi_{R_\eta^\ast}$ in (\ref{eq:auxiliary_eq}):
\begin{align*}
\Phi_{R_\eta^\ast}(t) = \frac{1}{\sigma^2}\int_0^t \Phi_{R_\theta}(t-s)\Big(\Phi_{R_\eta^\ast}(s) + \frac{\delta}{\sigma^2}\Big)\d s,
\end{align*}
which satisfies $\Phi_{R_\eta^\ast}(0) = R_\eta(0,\ast) = 0$, hence we conclude that $|R_\eta(t,\ast)| \leq \Phi_{R_\eta^\ast}(t)$.
\end{proof}




\begin{lemma}\label{lem:Trange_eta_2_theta}
$\cT_{\eta\rightarrow \theta}$ maps $\cS_\eta$ into $\cS_\theta$.
\end{lemma}
\begin{proof}
(\textbf{Condition for $C_\theta$}) Note that $C_\theta$ is a covariance kernel by definition so it suffices to verify claims (\ref{eq:Ctheta_cond_1}) and (\ref{eq:Ctheta_cond_2}). For (\ref{eq:Ctheta_cond_1}), let
\begin{align*}
b(t,\theta) \equiv b(t, \{\theta^s\}_{s\in[0,t]}; \theta^\ast,\{u^s\}_{s\in[0,t]}) \equiv {-}\frac{\delta}{\sigma^2}(\theta^t-\theta^*) + \partial_\theta \log g(\theta^t;\alpha^t) -\int_0^{t} R_\eta(t, s)\theta^{s}\d s -R_\eta(t,*)\theta^\ast + u^t. 
\end{align*}
Apply Ito's formula to the map $x \mapsto x^2$ yields
\begin{align*}
\frac{\d \E [(\theta^t)^2]}{\d t} = 2\Big(\E[\theta^t \cdot b(t,\theta)] + 1\Big) \leq \E[(\theta^t)^2] +\E[b^2(t,\theta)] + 2.
\end{align*}
%Hence with
%\begin{align*}
%\frac{\d\sqrt{\E[(\theta^t)^2]}}{\d t} = \frac{1}{2\sqrt{\E[(\theta^t)^2]}}\frac{\d \E (\theta^t)^2}{\d t}, 
%\end{align*}
%it holds that
%\begin{align*}
%\Big|\frac{\d\sqrt{\E[(\theta^t)^2]}}{\d t}\Big| \leq \sqrt{\E[b^2(t,\theta)]} + \frac{1}{\sqrt{\E[(\theta^t)^2]}}.
%\end{align*}
It remains to bound $\E[b^2(t,\theta)]$ as follows:
\begin{align*}
\E[b^2(t,\theta)] %&\leq K_{C_\theta}\Big(\E[(\theta^t - \theta^\ast)^2] + \E[(f'(\theta^\ast)^2] + t\cdot \int_0^t R^2_\eta(t,s)\E[(\theta^s)^2] + R_{\eta}^2(t,\ast) \E[(\theta^\ast)^2] + \E[(u^t)^2]\Big)\\
&\leq K_{C_\theta}\Big(\E[(\theta^t)^2] + \int_0^t (t-s+1)^{-2} \d s\cdot \int_0^t (t-s+1)^2\Phi_{R_\eta}^2(t-s)\Phi_{C_\theta}(s)\d s + \Phi_{R^\ast_\eta}^2(t) + \Phi_{C_\eta}(t) + 1\Big)\\
&\leq K_{C_\theta}\Big(\E[(\theta^t)^2] + \int_0^t (t-s+1)^2\Phi_{R_\eta}^2(t-s)\Phi_{C_\theta}(s)\d s + \Phi_{R^\ast_\eta}^2(t) + \Phi_{C_\eta}(t) + 1\Big)
\end{align*}
where with $M_\alpha = 2(\pnorm{\alpha^0}{} + CT)$ and $\pnorm{\alpha}{} = \sup_{t\in [0,T]} e^{-\lambda t}\pnorm{\alpha^t}{}$,
\begin{align*}
K_{C_\theta} = 30\Big((\frac{\delta}{\sigma^2} + L)^2 + \sup_{\pnorm{\alpha}{}\leq M_\alpha} |\partial_\theta \log g(0;\alpha)|^2 + \E[(\theta^\ast)^2] + 1\Big),
\end{align*}
and we have used (i) $|R_\eta(t,s)| \leq \Phi_{R_\eta}(t-s)$; (ii) $|R_{\eta}(t,\ast)| \leq \Phi_{R_\eta^\ast}(t)$; (iii) $\E[(u^t)^2] = C_\eta(t,t) \leq \Phi_{C_\eta}(t)$; (iv) $\sup_{t\in[0,T]} \pnorm{\alpha^t}{}\leq M_\alpha$. This concludes that
\begin{align*}
\Big|\frac{\d\E[(\theta^t)^2]}{\d t}\Big| \leq 2K_{C_\theta}\cdot\Big(\E[(\theta^t)^2] + \int_0^t (t-s+1)^2\Phi_{R_\eta}^2(t-s)\Phi_{C_\theta}(s)\d s + \Phi_{R^\ast_\eta}^2(t) + \Phi_{C_\eta}(t) + 1\Big).
\end{align*}
Recall the equation for $\Phi_{C_\theta}$ from (\ref{eq:auxiliary_eq}):
\begin{align*}
\frac{\d }{\d t}\Phi_{C_\theta}(t) = 2K_{C_\theta}\cdot\Big(\Phi_{C_\theta}(t) + \int_0^t (t-s+1)^2\Phi_{R_\eta}^2(t-s)\Phi_{C_\theta}(s)\d s + \Phi_{R^\ast_\eta}^2(t) + \Phi_{C_\eta}(t) + 1\Big).
\end{align*}
Since the initial condition satisfies $\Phi_{C_\theta}(0) \geq C_\theta(0,0) = \E[(\theta^0)^2]$, we conclude that $C_\theta(t,t) \leq \Phi_{C_\theta}(t)$.

Next we prove (\ref{eq:Ctheta_cond_2}). For $t\geq s$, since
\begin{align*}
\theta^t - \theta^s = \int_s^t \Big(-\frac{\delta}{\sigma^2}(\theta^r - \theta^\ast) + \partial_\theta \log g(\theta^r;\alpha^r)\Big)\d r - \int_s^t \Big(\int_0^r R_\eta(r,r')\theta^{r'}\d r'\Big)\d r - \int_s^t R_\eta(r,\ast)\theta^\ast + \int_s^t u^r\d r + \sqrt{2}(b^t - b^s), 
\end{align*}
it holds that
\begin{align*}
&C_\theta(t,t) - 2C_\theta(t,s) + C_\theta(s,s)\\
&= \E[(\theta^t - \theta^s)^2]\\
&\leq 20|t-s|\cdot \Big(\int_s^t \Big[(\frac{\delta}{\sigma^2})^2\E[(\theta^r - \theta^\ast)^2] + L^2 \E[(\theta^r)^2] + (\frac{\delta}{\sigma^2})^2 \sup_{\pnorm{\alpha}{}\leq M_\alpha} |\partial_\theta \log g(0;\alpha)|^2\\
&\quad + r \cdot \int_0^r R_\eta(r,r')^2 \E[(\theta^{r'})^2]\d r'+ R_\eta(r,\ast)^2 \E[(\theta^\ast)^2]\Big]\d r + 1\Big)\\
&\leq K|t-s|\Big(\Phi_{C_\theta}(T) + \Phi_{R_\eta}^2(T) + \Phi_{R_\eta^\ast}^2(T) + 1\Big),
\end{align*}
where $K > 0$ is some constant that depends on $T, \delta,\sigma, L$, and we have used the fact that $\Phi_{C_\theta}(\cdot), \Phi_{R_\eta}(\cdot), \Phi_{R_\eta^\ast}(\cdot)$ are nondecreasing. This verifies (\ref{eq:Ctheta_cond_2}). 

\noindent(\textbf{Condition for $R_\theta$}) Let $\bar{R}_\theta(t,s) \equiv \E|\frac{\partial \theta^t}{\partial u^s}|$ so that $|R_\theta(t,s)|\leq \bar{R}_\theta(t,s)$ by definition. Note that
\begin{align}\label{eq:theta_response_dt}
\notag\frac{\d}{\d t}\Big|\frac{\partial \theta^t}{\partial u^s}\Big| \leq \Big|\frac{\d}{\d t}\frac{\partial \theta^t}{\partial u^s}\Big| &\leq \big(|\partial_\theta^2 \log g(\theta^t;\alpha^t)| + \frac{\delta}{\sigma^2}\big)\Big|\frac{\partial \theta^t}{\partial u^s}\Big| + \int_s^t |R_\eta(t,s')|\Big|\frac{\partial \theta^{s'}}{\partial u^s}\Big|\d s\\
&\leq (\frac{\delta}{\sigma^2} + L)\Big|\frac{\partial \theta^t}{\partial u^s}\Big| + \int_s^t \Phi_{R_\eta}(t-s')\Big|\frac{\partial \theta^{s'}}{\partial u^s}\Big|\d s',
\end{align}
where apply Assumption \ref{assump:lipschitz} and the fact that $\pnorm{\alpha}{} \leq M_\alpha$ established in (\ref{eq:alpha_bound}). Taking expectation on both sides yields
\begin{align*}
\frac{\d}{\d t}\bar{R}_\theta(t,s) %&= \E\frac{\d}{\d t}\Big|\frac{\partial \theta^t}{\partial u^s}\Big| \leq \E\Big|\frac{\d}{\d t}\frac{\partial \theta^t}{\partial u^s}\Big| \leq \E\Big[\big(|f''(\theta^t)| + \frac{\delta}{\sigma^2}\big)\Big|\frac{\partial \theta^t}{\partial u^s}\Big| + \int_s^t |R_\eta(t,s')|\Big|\frac{\partial \theta^{s'}}{\partial u^s}\Big|\d s\Big]\\
\leq (\frac{\delta}{\sigma^2} + L)\bar{R}_\theta(t,s) + \int_s^t \Phi_{R_\eta}(t-s')\bar{R}_{\theta}(s',s)\d s'.
\end{align*}
Recall the equation for $\Phi_{R_\theta}$ in (\ref{eq:auxiliary_eq}):
\begin{align*}
\frac{\d}{\d t}\Phi_{R_\theta}(t) = (\frac{\delta}{\sigma^2} + L)\Phi_{R_\theta}(t) + \int_0^t \Phi_{R_\eta}(t-s)\Phi_{R_\theta}(s)\d s. 
\end{align*}
Hence with initialization $\Phi_{R_\theta}(0) \geq \bar{R}_\theta(0,0) = 1$, we conclude that $|R_\theta(t,s)|\leq \bar{R}_\theta(t,s) \leq \Phi_{R_\theta}(t-s)$. On the other hand, for any fixed $r\leq s\leq t$, we have
\begin{align*}
R_\theta(t,r) - R_\theta(s,r) = -\int_s^t \E\Big[\Big(\frac{\delta}{\sigma^2} - \partial_\theta^2 \log g(\theta^{s'};\alpha^{s'})\Big)\frac{\partial \theta^{s'}}{\partial u^r}\Big]\d s' - \int_s^t\Big(\int_r^{s'} R_\eta(s',s'')R_\theta(s'',r)\d s''\Big)\d s',
\end{align*}
hence using the above bound for $\bar{R}_\theta(t,s)$, we have
\begin{align*}
|R_\theta(t,r) - R_\theta(s,r)| \leq K'|t-s|\Big(\Phi_{R_\theta}(T) + \Phi_{R_\eta}(T)\Phi_{R_\theta}(T) + 1\Big), 
\end{align*}
where $K' > 0$ is some constant that depends on $T, \delta,\sigma, L$.
\end{proof}





Next we equip the space $\cS_\eta$ and $\cS_\theta$ with metrics. For two response functions $R_\eta = \{R_\eta(t,s)\}_{0\leq s\leq t\leq T}$ and $\tilde{R}_\eta = \{\tilde{R}_\eta(t,s)\}_{0\leq s\leq t\leq T}$, let
\begin{align}\label{eq:response_metric}
d(R_\eta, \tilde{R}_{\eta}) \equiv d(R_\eta, \tilde{R}_{\eta}; \lambda, T) \equiv \sup_{0\leq s \leq t \leq T} e^{-\lambda t} \big|R_\eta(t,s) - \tilde{R}_\eta(t,s)\big|, 
\end{align}
and the distance between $R_\theta$ and $\tilde{R}_\theta$ be defined similarly. Analogously, for two response functions $R^\ast_\eta = \{R_\eta(t,\ast)\}_{t\in [0,T]}$ and $\tilde{R}^\ast_\eta = \{\tilde{R}_\eta(t,\ast)\}_{t\in [0,T]}$, let
\begin{align*}
d(R^\ast_\eta, \tilde{R}^\ast_{\eta}) \equiv d(R^\ast_\eta, \tilde{R}^\ast_{\eta}; \lambda, T) \equiv \sup_{t \in [0,T]} e^{-\lambda t} \big|R_\eta^\ast(t,\ast) - \tilde{R}^\ast_\eta(t,\ast)\big|. 
\end{align*}
For two correlation functions $(C_\theta, C_\theta^\ast) = \{C_\theta(t,s), C_\theta(t,\ast)\}_{t,s\in[0,T]}$ and $(\tilde{C}_\theta,\tilde{C}_\theta^\ast) = \{\tilde{C}_\theta(t,s), \tilde{C}(t,\ast)\}_{t,s\in[0,T]}$, let
\begin{align*}
d\big((C_\theta, C_\theta^\ast), (\tilde{C}_\theta,\tilde{C}_\theta^\ast)\big) &\equiv d((C_\theta, C_\theta^\ast), (\tilde{C}_\theta,\tilde{C}_\theta^\ast); \lambda, T)\\
&\equiv \inf_{\{w^t,w^\ast\}\sim (C_\theta,C_\theta^\ast), \{\tilde{w}^t, \tilde{w}^\ast\} \sim (\tilde{C}_\theta, \tilde{C}_\theta^\ast)} \sup_{t\in [0,T]} e^{-\lambda t} \sqrt{\E (w^t - \tilde{w}^t)^2}, 
\end{align*}
where the infimum is taken over coupling of Gaussian processes $(\{w^t,w^\ast\}, \{\tilde{w}^t,\tilde{w}^\ast\})$ such that $\{w^t,w^\ast\}$ (resp. $\{\tilde{w}^t\}$) has covariance $C_\theta, C_\theta^\ast$ (resp. $\tilde{C}_\theta$), i.e., $\E[w^tw^s] = C_\theta(t,s)$ and $\E[w^tw^\ast] = C_\theta(t,\ast)$. Let the distance between $C_\eta$ and $\tilde{C}_\eta$ be defined similarly. 

%Analogously, for two correlation functions $C^\ast_\theta = \{C_\theta(t,\ast)\}_{t\in[0,T]}$ and $\tilde{C}_\theta^\ast = \{\tilde{C}_\theta(t,\ast)\}_{t\in[0,T]}$, let
%\begin{align*}
%d(C^\ast_\theta, \tilde{C}^\ast_{\theta}) \equiv d(C^\ast_\theta, \tilde{C}^\ast_{\theta}; \lambda, T) \equiv \sup_{t \in [0,T]} e^{-\lambda t} \big|C_\theta(t,\ast) - \tilde{C}_\theta(t,\ast)\big|. 
%\end{align*}
Lastly, for $X_\eta = (R_\eta, R_\eta^\ast, C_\eta)$ and $\tilde{X}_\eta = (\tilde{R}_\eta, \tilde{R}_\eta^\ast, \tilde{C}_\eta)$ in $\mathcal{S}_\eta$, let
\begin{align}\label{eq:dist_Seta}
d(X_\eta, \tilde{X}_\eta) \equiv d(X_\eta, \tilde{X}_\eta;\lambda, T) \equiv d(R_\eta, \tilde{R}_\eta) + d(R^\ast_\eta, \tilde{R}^\ast_\eta) + d(C_\eta, \tilde{C}_\eta).
\end{align}
Similarly, for $X_\theta = (R_\theta, C_\theta, C^\ast_\theta)$ and $\tilde{X}_\theta = (\tilde{R}_\theta, \tilde{C}_\theta, \tilde{C}^\ast_\theta)$ in $\mathcal{S}_\theta$, let
\begin{align}\label{eq:dist_Stheta}
d(X_\theta, \tilde{X}_\theta) \equiv d(X_\theta, \tilde{X}_\theta;\lambda, T) \equiv d(R_\theta, \tilde{R}_\theta) + d(C_\theta, \tilde{C}_\theta) + d(C^\ast_\theta, \tilde{C}^\ast_\theta).
\end{align}



\begin{lemma}[Modulus of $\cT_{\eta\rightarrow\theta}$]\label{lem:modulus_eta_2_theta}
Let $X^i = (C_\eta^i, R_\eta^i, R_\eta^{\ast i}) \in \cS_\eta$ and $Y^i = \cT_{\eta\rightarrow\theta}(X^i) = (R_\theta^i, C_\theta^i, C_\theta^{\ast i}) \in \cS_\theta$ for $i=1,2$. Then for any given $\eps > 0$,
\begin{align*}
d(Y^1, Y^2; \lambda, T) \leq \eps \cdot d(X^1,X^2;\lambda, T),
\end{align*}
for large enough $\lambda$ (depending on $\delta, \sigma, L, T, \Phi_{C_\eta}(T), \Phi_{R_\eta}(T), \eps$).
\end{lemma}
\begin{proof}
By definition, it suffices to bound $d((C_\theta^1, C_\theta^{\ast 1}), (C_\theta^2, C_\theta^{\ast 2});\lambda,T)$ and $d(R_\theta^1, R_\theta^2;\lambda, T)$.

\noindent \textbf{Part 1: Bound of $d((C_\theta^1, C_\theta^{\ast 1}), (C_\theta^2, C_\theta^{\ast 2});\lambda,T)$} For simplicity, in the following we only bound the distance between the $C_\theta$ component, i.e., 
\begin{align*}
d(C_\theta^1,C_\theta^2;\lambda, T) = \inf_{\{w_1^t\}\sim C^1_\theta, \{w_2^t\} \sim C^2_\theta} \sup_{t\in [0,T]} e^{-\lambda t} \sqrt{\E (w_1^t - w_2^t)^2}, 
\end{align*}
where the infimum is taken over coupling of Gaussian processes $(\{w_1^t\}, \{w_2^t\})$ such that $\{w_1^t\}$ (resp. $\{w_2^t\}$) has covariance $C^1_\theta$ (resp. $C^2_\theta$); additional arguments for the $C_\theta^\ast$ component will follow analogously.

Writing $C_\theta^i = C_\theta(C_\eta^i, R^i_\eta, R_\eta^{\ast i})$ to make the dependence explicit, we have
\begin{align*}
d(C_\theta^1, C_\theta^2) &\leq d\Big(C_\theta(C_\eta^1, R^1_\eta, R_\eta^{\ast 1}), C_\theta(C_\eta^2, R^1_\eta, R_\eta^{\ast 1})\Big) + d\Big(C_\theta(C_\eta^2, R^1_\eta, R_\eta^{\ast 1}), C_\theta(C_\eta^2, R^2_\eta, R_\eta^{\ast 1})\Big)\\
&\quad + d\Big(C_\theta(C_\eta^2, R^2_\eta, R_\eta^{\ast 1}), C_\theta(C_\eta^2, R^2_\eta, R_\eta^{\ast 2})\Big) \equiv (I) + (II) + (III).
\end{align*}
\textbf{Bound of $(I)$} Let $\{u_1^t\}_{t\in[0,T]}$ and $\{u_2^t\}_{t\in[0,T]}$ be a optimal coupling in the definition of $d(C^1_\eta, C^2_\eta)$, i.e., 
\begin{align}\label{eq:opt_u_couple}
\sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(u_1^t - u_2^t)^2]} = d(C_\eta^1, C_\eta^2).
\end{align}
Let $\{\theta_1^t\}$ and $\{\theta_2^t\}$ be the solutions to (\ref{eq:theta_1}) driven by $\{u_1^t\}$ and $\{u_2^t\}$ respectively, a common Brownian motion $\{b^t\}$, initialization $\theta^0$, and $\theta^\ast$, i.e., 
\begin{align}\label{eq:theta_modulus_def}
\theta_i^t = \theta^0 + \int_0^t \Big(-\frac{\delta}{\sigma^2}(\theta^s_i - \theta^\ast) + \partial_\theta \log g(\theta^s_i;\alpha^s_i)\Big)\d s - \int_0^t \Big(\int_0^s R^1_\eta(s,s')\theta^{s'}\d s'\Big)\d s - \int_0^t \Big(R^1_\eta(s,\ast)\theta^\ast - u^s_i\Big)\d s + \sqrt{2}b^t.
\end{align}
By definition, we have $\E[\theta_1^t\theta_1^s] = \E[\theta_2^t\theta_2^s] = C_\theta(t,s)$. Moreover, 
\begin{align*}
\theta_1^t - \theta_2^t = \int_0^t \Big(-\frac{\delta}{\sigma^2}(\theta^s_1 - \theta^s_2) + (\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2))\Big)\d s - \int_0^t (\theta^s_1 - \theta^s_2)\Big(\int_s^t R^1_\eta(s',s)\d s'\Big)\d s + \int_0^t (u^s_1 - u^s_2) \d s.
\end{align*}
Hence
\begin{align*}
\E[(\theta^t_1 - \theta^t_2)^2] &\leq 4\Big[\E \Big(\int_0^t \frac{\delta}{\sigma^2}|\theta^s_1 - \theta^s_2|\d s\Big)^2 + \E \Big(\int_0^t |\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2)|\d s\Big)^2\\
&\quad + \E \Big(\int_0^t |\theta^s_1 - \theta^s_2|\Big(\int_s^t R^1_\eta(s',s)\d s'\Big)\d s\Big)^2 + \E \Big(\int_0^t |u^s_1 - u^s_2| \d s\Big)^2\Big]\\
&\leq 4\Big[t \cdot \int_0^t (\frac{\delta}{\sigma^2})^2\E[(\theta^s_1 - \theta^s_2)^2]\d s + \int_0^t t \cdot \E\Big(\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2)\Big)^2\d s\\
&\quad + t\cdot \int_0^t \E(\theta^s_1 - \theta^s_2)^2\Big(\int_s^t R^1_\eta(s',s)\d s'\Big)^2\d s + t\cdot \int_0^t \E[(u^s_1 - u^s_2)^2] \d s\Big] \equiv 4 \cdot \sum_{i=1}^4 (I_i). 
\end{align*}
Term $(I_1)$ satisfies
\begin{align*}
\int_0^t t\cdot (\frac{\delta}{\sigma^2})^2\E[(\theta^s_1 - \theta^s_2)^2]\d s &= t\cdot (\frac{\delta}{\sigma^2})^2 \int_0^t e^{2\lambda s}e^{-2\lambda s}\E[(\theta^s_1 - \theta^s_2)^2]\d s\\
&\leq t\cdot (\frac{\delta}{\sigma^2})^2\cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2] \int_0^t e^{2\lambda s}\d s\\
&= \frac{K_1}{\lambda}e^{2\lambda t} \cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2],
\end{align*}
where $K_1 > 0$ depends on $\delta,\sigma, L, T$. To bound $(I_2)$, we have $(I_2) \leq 2 (I_{2,1}) + 2 (I_{2,2})$, where
\begin{align*}
(I_{2,1}) &= \E \Big(\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_1)\Big)^2,\\
(I_{2,2}) &= \E \Big(\partial_\theta \log g(\theta^s_2;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2)\Big)^2. 
\end{align*}
Using $\pnorm{\alpha}{} \leq M_\alpha$ given in (\ref{eq:alpha_bound}), Assumption \ref{assump:lipschitz} yields that for some $L > 0$, 
\begin{align*}
\E \Big(\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_1)\Big)^2 \leq L \E(\theta^s_1 - \theta^s_2)^2. 
\end{align*}
On the other hand, a similar calculation as in (\ref{eq:alpha_modulus}) yields
\begin{align*}
\Big|\partial_\theta \log g(\theta^s_2;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2)\Big| \leq C\pnorm{\alpha^s_1 - \alpha^s_2}{} \leq C\int_0^s \sqrt{\E(\theta^{s'}_1 - \theta^{s'}_2)^2} \d s',
\end{align*}
which satisfies
\begin{align*}
\int_0^t \E\Big[\partial_\theta \log g(\theta^s_2;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2)\Big]^2 \d s \leq C\int_0^t \E(\theta^{s}_1 - \theta^{s}_2)^2 \d s \leq \frac{Ce^{2\lambda t}}{\lambda}\sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2],
\end{align*}
which concludes that $(I_2) \leq \frac{K_2}{\lambda}e^{2\lambda t} \cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2]$. For term $(I_3)$, using the condition $|R^1_\eta(t,s)| \leq \Phi_{R_\eta}(t-s) \leq \Phi_{R_\eta}(T)$, we have
\begin{align*}
\int_0^t t\cdot \E[(\theta^s_1 - \theta^s_2)^2]\Big(\int_s^t R^1_\eta(s',s)\d s'\Big)^2\d s \leq \frac{K_3}{\lambda}e^{2\lambda t} \cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2].
\end{align*}
Lastly for $(I_4)$, using (\ref{eq:opt_u_couple}), we have
\begin{align*}
\int_0^t t \cdot \E[(u^s_1 - u^s_2)^2] \d s \leq \frac{K_4}{\lambda}e^{2\lambda t} \cdot d^2(C_\eta^1, C_\eta^2).
\end{align*}
Hence for any given $\eps$, by choosing a large enough $\lambda$ (depending on $K_1-K_4, \eps$), we have
\begin{align*}
\sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2] \leq 0.1^2\eps^2 \cdot d^2(C_\eta^1, C_\eta^2) \leq 0.1^2\eps^2 \cdot d^2(X^1,X^2). 
\end{align*}
Lastly, by choosing $\{g^t_1,g^t_2\}$ to be a Gaussian process with matching covariance structure as $\{\theta^t_1, \theta^t_2\}$ (i.e., $\E[g^t_1g^s_2] = \E[\theta_1^t\theta^s_2]$), we have
\begin{align*}
(I) \leq \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(g^t_1 - g^t_2)^2]} = \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(\theta^t_1 - \theta^t_2)^2]} \leq 0.1\eps \cdot d(X^1,X^2).
\end{align*}

\textbf{Bound of $(II)$} Similar to (\ref{eq:theta_modulus_def}) above, for $i=1,2$, let
\begin{align*}
\theta_i^t = \theta^0 + \int_0^t \Big(-\frac{\delta}{\sigma^2}(\theta^s_i - \theta^\ast) + \partial_\theta \log g(\theta^s_i;\alpha^s_i)\Big)\d s - \int_0^t \Big(\int_0^s R^i_\eta(s,s')\theta^{s'}\d s'\Big)\d s - \int_0^t \Big(R^1_\eta(s,\ast)\theta^\ast - u^s\Big)\d s + \sqrt{2}B^t, 
\end{align*}
coupled with the same initialization $\theta^0$, $\theta^\ast$, Gaussian process $\{u^t\}$ and Brownian motion $\{B^t\}$. Then
\begin{align*}
\theta_1^t - \theta_2^t &= \int_0^t \Big(-\frac{\delta}{\sigma^2}(\theta^s_1 - \theta^s_2) + (\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2))\Big)\d s\\
&\quad - \Big[\int_0^t \theta^s_1 \Big(\int_s^t R^1_\eta(s',s)\d s'\Big)\d s - \int_0^t \theta^s_2 \Big(\int_s^t R^2_\eta(s',s)\d s'\Big)\d s\Big].
\end{align*}
Hence
\begin{align*}
\E[(\theta_1^t - \theta_2^t)^2] &\leq 4\cdot\Big[\E \Big(\int_0^t \frac{\delta}{\sigma^2}|\theta^s_1 - \theta^s_2|\d s\Big)^2 + \E \Big(\int_0^t (\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2))\d s\Big)^2\\
&\quad + \E \Big(\int_0^t |\theta^s_1 - \theta^s_2|\Big(\int_s^t R^1_\eta(s',s)\d s'\Big)\d s\Big)^2  + \E \Big(\int_0^t \Big|\int_s^t (R_\eta^1(s',s) - R_\eta^2(s',s))\d s'\Big| |\theta_2^s| \d s\Big)^2\Big]\\
&\leq 4\cdot\Big[\int_0^t t\cdot \frac{\delta}{\sigma^2}\E[(\theta^s_1 - \theta^s_2)]^2\d s + \int_0^t t \cdot \E\Big(\partial_\theta \log g(\theta^s_1;\alpha^s_1) - \partial_\theta \log g(\theta^s_2;\alpha^s_2)\Big)^2\d s \\
&\quad + \int_0^t t\cdot \E[(\theta^s_1 - \theta^s_2)^2] \Big(\int_s^t R^1_\eta(s',s)\d s'\Big)^2\d s\\
&\quad + \int_0^t t\cdot \Big(\int_s^t (t-s)\cdot \big(R_\eta^1(s',s) - R_\eta^2(s',s)\big)^2\d s'\Big) \E[(\theta_2^s)^2] \d s\Big].
\end{align*}
Using the same argument as above, the first three terms are bounded by $\frac{K_1}{\lambda}e^{2\lambda t}\sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2]$. For the third term, using the definition of the metric (\ref{eq:response_metric}) and the condition that $\E[(\theta^2_s)^2] = C_\theta(s,s) \leq \Phi_{C_\theta}(T)$ via Lemma \ref{lem:Trange_eta_2_theta}, we have
\begin{align*}
\int_0^t t\cdot \Big(\int_s^t (t-s)\cdot \big(R_\eta^1(s',s) - R_\eta^2(s',s)\big)^2\d s'\Big) \E[(\theta_2^s)^2] \d s \leq \frac{K_2}{\lambda}e^{2\lambda t} \cdot d^2(R_\eta^1,R_\eta^2),
\end{align*}
where $K_2>0$ depends on $T, \Phi_{C_\theta}(T)$. Hence again by choosing $\lambda$ large enough, we have
\begin{align*}
(II) \leq  \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(\theta^t_1 - \theta^t_2)^2]} \leq 0.1\eps \cdot d(R_\eta^1,R_\eta^2) \leq 0.1\eps \cdot d(X^1,X^2).
\end{align*}

\textbf{Bound of $(III)$} The proof is essentially the same as the one for $(II)$ by considering 
\begin{align*}
\theta_i^t = \theta^0 + \int_0^t \Big(-\frac{\delta}{\sigma^2}(\theta^s_i - \theta^\ast) + \partial_\theta \log g(\theta^s_i;\alpha^s_i)\Big)\d s - \int_0^t \Big(\int_0^s R^2_\eta(s,s')\theta^{s'}\d s'\Big)\d s - \int_0^t \Big(R^i_\eta(s,\ast)\theta^\ast - u^s\Big)\d s + \sqrt{2}B^t
\end{align*}
for $i=1,2$. Following the same argument as above yields
\begin{align*}
(III) \leq  \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(\theta^t_1 - \theta^t_2)^2]} \leq 0.1\eps \cdot d(R_\eta^{\ast 1},R_\eta^{\ast 2}) \leq 0.1\eps \cdot d(X^1,X^2).
\end{align*}
Combining the bounds for $(I)-(III)$ yields that, for large enough $\lambda$, 
\begin{align*}
d(C_\theta^1, C_\theta^2;\lambda, T) \leq 0.3\eps \cdot d(X^1,X^2).
\end{align*}

\textbf{Part 2: Bound of $d(R_\theta^1, R_\theta^2;\lambda, T)$} First by definition, for $i=1,2$, we have
\begin{align*}
\frac{\partial \theta_i^t}{\partial u^s} = 1 - \int_s^t \Big( \frac{\delta}{\sigma^2} - \partial_\theta^2 \log g(\theta_i^{s'};\alpha^{s'}_i)\Big)\frac{\partial \theta_i^{s'}}{\partial u^s}\d s' - \int_s^t \Big(\int_{s}^{s'} R^i_\eta(s',s'')\frac{\partial \theta_i^{s''}}{\partial u^s}\d s''\Big)\d s',
\end{align*}
where $\{\theta_i^t\}$  is the (unique) solution to (\ref{eq:theta_1}) with parameters $X^i = (C_\eta^i, R_\eta^i, R_\eta^{\ast i})$. This implies
\begin{align*}
\frac{\partial \theta_1^t}{\partial u^s} - \frac{\partial \theta_2^t}{\partial u^s} &= \int_s^t \Big(\partial_\theta^2 \log g(\theta_1^{s'})\cdot \frac{\partial \theta_1^{s'}}{\partial u^s} - \partial_\theta^2 \log g(\theta_2^{s'})\cdot \frac{\partial \theta_2^{s'}}{\partial u^s}\Big)\d s' - \frac{\delta}{\sigma^2}\int_s^t \Big(\frac{\partial \theta_1^{s'}}{\partial u^s} - \frac{\partial \theta_2^{s'}}{\partial u^s}\Big)\d s'\\
&\quad - \int_s^t \Big[\int_{s}^{s'} \Big(R^1_\eta(s',s'')\frac{\partial \theta_1^{s''}}{\partial u^s} - R^2_\eta(s',s'')\frac{\partial \theta_2^{s''}}{\partial u^s}\Big)\d s''\Big]\d s', 
\end{align*}
which further implies that $\E\Big|\frac{\partial \theta_1^t}{\partial u^s} - \frac{\partial \theta_2^t}{\partial u^s}\Big|\leq 5\sum_{j=1}^5 \zeta_j$, where
\begin{align*}
\zeta_1 &= \int_s^t \E\Big[\Big|\partial_\theta^2 \log g(\theta_1^{s'};\alpha^{s'}_1) - \partial_\theta^2 \log g(\theta_2^{s'};\alpha^{s'}_2)\Big|\Big|\frac{\partial \theta_1^{s'}}{\partial u^s}\Big|\Big]\d s',\\
\zeta_2 &= \int_s^t \E\Big[|\partial_\theta^2 \log g(\theta_2^{s'};\alpha^{s'}_2)|\Big|\frac{\partial \theta_1^{s'}}{\partial u^s} - \frac{\partial \theta_2^{s'}}{\partial u^s}\Big|\Big]\d s',\\
\zeta_3 &= \frac{\delta}{\sigma^2}\int_s^t \E\Big[\Big|\frac{\partial \theta_1^{s'}}{\partial u^s} - \frac{\partial \theta_2^{s'}}{\partial u^s}\Big|\Big]\d s',\\
\zeta_4 &= \int_s^t \int_s^{s'} \E\Big[\Big|R^1_\eta(s',s'') - R^2_\eta(s',s'')\Big|\Big|\frac{\partial \theta_1^{s''}}{\partial u^s}\Big|\Big]\d s''\d s',\\
\zeta_5 &= \int_s^t \int_s^{s'} \E\Big[|R^2_\eta(s',s'')|\Big|\frac{\partial \theta_1^{s''}}{\partial u^s} - \frac{\partial \theta_2^{s''}}{\partial u^s}\Big|\Big]\d s''\d s'.
\end{align*}
\noindent \textbf{Bound of $\zeta_1$} Using Assumption \ref{assump:lipschitz}-(c), (\ref{eq:alpha_bound}), and a similar calculation as in (\ref{eq:alpha_modulus}), we have
\begin{align*}
\Big|\partial_\theta^2 \log g(\theta_1^{s'};\alpha^{s'}_1) - \partial_\theta^2 \log g(\theta_2^{s'};\alpha^{s'}_2)\Big| &\leq \Big|\partial_\theta^2 \log g(\theta_1^{s'};\alpha^{s'}_1) - \partial_\theta^2 \log g(\theta_2^{s'};\alpha^{s'}_1)\Big| + \Big|\partial_\theta^2 \log g(\theta_2^{s'};\alpha^{s'}_1) - \partial_\theta^2 \log g(\theta_2^{s'};\alpha^{s'}_2)\Big|\\
&\leq C(|\theta_1^{s'} - \theta_2^{s'}| + \pnorm{\alpha^{s'}_1 - \alpha^{s'}_2}{})\\
&\leq C(|\theta_1^{s'} - \theta_2^{s'}| + \int_0^{s''} \sqrt{\E(\theta^{s''}_1 - \theta^{s''}_2)^2} \d s''),
\end{align*}
hence
\begin{align*}
\zeta_1 \leq L \sqrt{\int_s^t \E\Big[\big(\theta_1^{s'} - \theta_2^{s'}\big)^2\Big]\d s'} \cdot \sqrt{\int_s^t \E\Big[\Big(\frac{\partial \theta_1^{s'}}{\partial u^s}\Big)^2\Big]\d s'}. 
\end{align*}
By the proof of Part 1, we have $\sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(\theta^t_1 - \theta^t_2)^2]} \leq 0.1\eps \cdot d(X^1,X^2)$, so
\begin{align*}
\int_s^t \E\Big[\big(\theta_1^{s'} - \theta_2^{s'}\big)^2\Big]\d s' \leq \sup_{t\in[0,T]} e^{-2\lambda t}\E[(\theta^t_1 - \theta^t_2)^2] \cdot \int_s^t e^{2\lambda s'}\d s' \leq (0.1\eps)^2 \cdot d^2(X^1,X^2) \cdot \frac{e^{2\lambda t}}{\lambda}.
\end{align*}
On the other hand, (\ref{eq:theta_response_dt}) implies that $\Big|\frac{\partial \theta_1^{s'}}{\partial u^s}\Big|\leq \Phi_{R_\theta}(t-s)$ a.e., hence we conclude
\begin{align*}
\zeta_1 \leq \frac{K_1}{\sqrt{\lambda}}e^{\lambda t} \cdot 0.1\eps \cdot d(X^1, X^2) \leq e^{\lambda t} \cdot 0.01\eps \cdot d(X^1, X^2) 
\end{align*}
for large enough $\lambda$, where $K_1 > 0$ depends on $\Phi_{R_\theta}(T), L, T$.

\noindent \textbf{Bound of $\zeta_2$ and $\zeta_3$} Using $|\partial_\theta^2 \log g(\theta_2^{s'};\alpha^{s'}_2)| \leq L$ via Assumption \ref{assump:lipschitz}-(c) and (\ref{eq:alpha_bound}), we have for large enough $\lambda$
\begin{align*}
\zeta_2 \leq L \int_s^t e^{\lambda s'} e^{-\lambda s'}\E\Big[\Big|\frac{\partial \theta_1^{s'}}{\partial u^s} - \frac{\partial \theta_2^{s'}}{\partial u^s}\Big|\Big]\d s' &\leq  \frac{L}{\lambda}e^{\lambda t}\cdot \sup_{0\leq s\leq t\leq T}e^{-\lambda t}\E\Big[\Big|\frac{\partial \theta_1^{t}}{\partial u^s} - \frac{\partial \theta_2^{t}}{\partial u^s}\Big|\Big]\\
&\leq \frac{e^{\lambda t}}{4} \cdot \sup_{0\leq s\leq t\leq T}e^{-\lambda t}\E\Big[\Big|\frac{\partial \theta_1^{t}}{\partial u^s} - \frac{\partial \theta_2^{t}}{\partial u^s}\Big|\Big].
\end{align*}
The same bound holds for $\zeta_3$.

\noindent \textbf{Bound of $\zeta_4$} Using the definition of the metric (\ref{eq:response_metric}) and the bound $\Big|\frac{\partial \theta_1^{s'}}{\partial u^s}\Big|\leq \Phi_{R_\theta}(t-s)$ a.e., we have
\begin{align*}
\zeta_4 \leq \frac{K_2}{\lambda}e^{\lambda t} \cdot d(R_\eta^1, R_\eta^2) \leq e^{\lambda t} \cdot 0.01\eps \cdot d(X^1, X^2) 
\end{align*}
for large enough $\lambda$, where $K_2 > 0$ depends on $\Phi_{R_\theta}(T)$ and $T$.

\noindent \textbf{Bound of $\zeta_5$} Using the condition $|R^2_\eta(t,s)| \leq \Phi_{R_\eta}(t-s)$, we have
\begin{align*}
\zeta_5 \leq \frac{K_3}{\lambda}e^{\lambda t} \cdot \sup_{0\leq s\leq t\leq T}e^{-\lambda t}\E\Big[\Big|\frac{\partial \theta_1^{t}}{\partial u^s} - \frac{\partial \theta_2^{t}}{\partial u^s}\Big|\Big] \leq \frac{e^{\lambda t}}{4} \cdot \sup_{0\leq s\leq t\leq T}e^{-\lambda t}\E\Big[\Big|\frac{\partial \theta_1^{t}}{\partial u^s} - \frac{\partial \theta_2^{t}}{\partial u^s}\Big|\Big]
\end{align*}
for large enough $\lambda$, where $K_3 > 0$ depends on $\Phi_{\eta}(T)$ and $T$.

Combining the bounds for $\zeta_1 - \zeta_5$, we have
\begin{align*}
d(R^1_\theta, R_\theta^2;\lambda, T) \leq \sup_{0\leq s\leq t\leq T} e^{-\lambda t} \E\Big|\frac{\partial \theta_1^t}{\partial u^s} - \frac{\partial \theta_2^t}{\partial u^s}\Big| \leq 0.3 \eps \cdot d(X^1,X^2),
\end{align*}
and the claim of the lemma follows from combining part 1 and 2.
\end{proof}


\begin{lemma}[Modulus of $\cT_{\theta\rightarrow\eta}$]\label{lem:modulus_theta_2_eta}
Let $Y^i = (R_\theta^i, C_\theta^i, C_\theta^{\ast i}) \in \cS_\theta$ and $X^i = \cT_{\theta\rightarrow\eta}(Y^i) = (C_\eta^i, R_\eta^i, R_\eta^{\ast i})$ for $i=1,2$. Then for some $C > 0$ depending on $\delta, \sigma, \Phi_{R_\eta}(T)$, it holds 
\begin{align*}
d(Y^1, Y^2; \lambda, T) \leq C\cdot d(X^1,X^2;\lambda, T)
\end{align*}
for large enough $\lambda$ (depending on $\delta, \sigma, L, T, \Phi_{C_\theta}(T), \Phi_{R_\theta}(T)$).
\end{lemma}
\begin{proof}
The proof is similar to that of Lemma \ref{lem:modulus_eta_2_theta} so we will omit some repetitive details. By definition, it suffices to bound $d(C_\eta^1, C_\eta^2;\lambda, T)$, $d(R_\eta^1, R_\eta^2;\lambda, T)$, and $d(R_\eta^{\ast 1}, R_\eta^{\ast 2};\lambda, T)$. 

\noindent \textbf{Part 1: Bound of $d(C_\eta^1, C_\eta^2;\lambda, T)$} Writing $C_\eta^i = C_\eta(C_\theta^i, C_\theta^{\ast i}, R^i_\theta)$ to make the dependence explicit, we have
\begin{align*}
d(C_\eta^1, C_\eta^2) &\leq d(C_\eta(C_\theta^1, C_\theta^{\ast 1}, R^1_\theta),C_\eta(C_\theta^1, C_\theta^{\ast 1}, R^2_\theta)) + d(C_\eta(C_\theta^1, C_\theta^{\ast 1}, R^2_\theta),C_\eta(C_\theta^2, C_\theta^{\ast 2}, R^2_\theta))\\
&\equiv (I) + (II).
\end{align*}
\noindent \textbf{Bound of $(I)$} For $i=1,2$, let
\begin{align*}
\eta^t_i &= -\frac{1}{\sigma^2}\int_0^{t} R^i_\theta(t,s)\big(\eta_i^s - w^\ast - e\big)\d s + w^t
\end{align*}
be the (unique) solution to (\ref{eq:eta_1}) coupled with the same $(\{w^t\}, w^\ast)$. Then $\xi_i^t \equiv \eta_i^t - w^\ast - e$ satisfies
\begin{align*}
\xi^t_i = -\frac{1}{\sigma^2}\int_0^{t} R^i_\theta(t,s)\xi_i^s \d s + w^t - w^\ast - e,
\end{align*}
and $C_\eta[C_\theta^i, C_\theta^{\ast i}, R^i_\theta](t,s) = \frac{\delta}{\sigma^4}\E[\xi^t_i\xi^s_i]$ for $i=1,2$. This entails
\begin{align*}
\E[(\xi^t_1 - \xi^t_2)^2] &\leq \frac{2}{\sigma^4} \cdot \Big[\E\Big(\int_0^t (R^1_\theta(t,s) - R^2_\theta(t,s))\xi_1^s \d s\Big)^2 +  \E\Big(\int_0^t R^2_\theta(t,s)(\xi_1^s - \xi^s_2)\d s\Big)^2\Big]\\
&\leq \frac{2}{\sigma^4} \cdot \Big[\int_0^t t\cdot (R^1_\theta(t,s) - R^2_\theta(t,s))^2 \E[(\xi_1^s)^2] \d s +  \int_0^t t\cdot (R^2_\theta(t,s))^2 \E[(\xi_1^s - \xi^s_2)^2]\d s\Big].
\end{align*}
By the definition of the metric (\ref{eq:response_metric}) and the bound $C_\eta(t,t) \leq \Phi_{C_\eta}(T)$, for any $\eps > 0$, the first term satisfies
\begin{align*}
\frac{1}{\sigma^4}\cdot \int_0^t t\cdot (R^1_\theta(t,s) - R^2_\theta(t,s))^2 \E[(\xi_1^s)^2] \d s \leq \frac{K_1}{\lambda}e^{2\lambda t} \cdot d^2(R^1_\theta, R^2_\theta) \leq e^{2\lambda t} \cdot (0.1\eps)^2 \cdot \frac{\sigma^4}{\delta}d^2(Y^1,Y^2)
\end{align*}
for large enough $\lambda$, where $K_1$ depends on $\sigma, \delta, \Phi_{C_\eta}(T), T, \eps$. Using the condition $|R^2_\theta(t,s)| \leq \Phi_{R_\theta}(t-s)\leq \Phi_{R_\theta}(T)$, the second term satisfies
\begin{align*}
\frac{1}{\sigma^4} \cdot \int_0^t t\cdot (R^2_\theta(t,s))^2 \E[(\xi_1^s - \xi^s_2)^2]\d s \leq \frac{K_2}{\lambda}e^{2\lambda t} \cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E[(\xi^t_1 - \xi^t_2)^2] \leq \frac{1}{10}e^{2\lambda t} \cdot \sup_{t\in[0,T]} e^{-2\lambda t}\E[(\xi^t_1 - \xi^t_2)^2]
\end{align*}
for large enough $\lambda$. We therefore conclude
\begin{align*}
\sup_{t\in[0,T]} e^{-2\lambda t}\E[(\xi^t_1 - \xi^t_2)^2] \leq (0.2\eps)^2 \frac{\sigma^4}{\delta}\cdot d^2(Y^1,Y^2).
\end{align*}
Let $\{g^t_1,g^t_2\}$ be a Gaussian process with covariance $\E[g^t_1g^s_2] = \frac{\delta}{\sigma^4} \E[\xi^t_1\xi^s_2]$, then $\{g^t_i\}$ has covariance $C_\eta^i$ for $i=1,2$, and hence
\begin{align*}
(I) \leq \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(g^t_1 - g^t_2)^2]} = \frac{\sqrt{\delta}}{\sigma^2} \cdot \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(\xi^t_1 - \xi^t_2)^2]} \leq (0.2\eps) \cdot d(Y^1,Y^2).
\end{align*}

\noindent \textbf{Bound of $(II)$} Let $(\{w^t_1\},w^\ast_1)$ and $(\{w^t_2\},w^\ast_2)$ be an optimal coupling in the definition of $d\big((C^1_\theta, C^{\ast 1}_\theta), (C^2_\theta, C^{\ast 2}_\theta)\big)$, i.e., 
\begin{align*}
\sqrt{\E[(w^\ast_1 - w^\ast_2)^2]} + \sup_{t\in [0,T]} e^{-\lambda t}\sqrt{\E[(w^t_1 - w^t_2)^2]} = d\Big((C^1_\theta, C^{\ast 1}_\theta), (C^2_\theta, C^{\ast 2}_\theta)\Big).
\end{align*}
For $i=1,2$, let
\begin{align*}
\eta^t_i &= -\frac{1}{\sigma^2}\int_0^{t} R^2_\theta(t,s)\big(\eta_i^s - w^\ast_i - e\big)\d s + w^t_i, 
\end{align*}
be the (unique) solution to (\ref{eq:eta_1}) coupled driven by $(\{w^t_1\},w^\ast_1)$ and $(\{w^t_2\},w^\ast_2)$, and with $\xi^t_i = \eta^t_i - w^\ast_i - e$, 
\begin{align*}
\xi^t_i = -\frac{1}{\sigma^2}\int_0^{t} R^2_\theta(t,s)\xi_i^s \d s + w^t_i - w^\ast_i - e.
\end{align*}
Then a similar argument as above shows that, for large enough $\lambda$, 
\begin{align*}
\sup_{t\in[0,T]} e^{-2\lambda t}\E[(\xi^t_1 - \xi^t_2)^2] \leq 4\frac{\sigma^4}{\delta}\cdot d^2((C^1_\theta, C^{\ast 1}_\theta), (C^2_\theta, C^{\ast 2}_\theta)) \leq 4\frac{\sigma^4}{\delta}\cdot d^2(Y^1,Y^2),
\end{align*}
hence
\begin{align*}
(II) \leq \frac{\sqrt{\delta}}{\sigma^2} \cdot \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(\xi^t_1 - \xi^t_2)^2]} \leq 2 \cdot d(Y^1,Y^2).
\end{align*}
By choosing $\eps$ small enough, combining the bounds for $(I)$ and $(II)$ yields $d(C_\eta^1, C_\eta^2) \leq 2.01 d(Y^1,Y^2)$.
\medskip

\noindent \textbf{Part 2: Bound of $d(R_\eta^1, R_\eta^2;\lambda, T)$ and $d(R_\eta^{\ast 1}, R_\eta^{\ast 2};\lambda, T)$} By definition, we have for $i=1,2$,
\begin{align*}
R_\eta^i(t,s) = -\frac{1}{\sigma^2}\int_s^t R_\theta^i(t,s')R_\eta^i(s',s)\d s' - \frac{\delta}{\sigma^4}R_\theta^i(t,s),
\end{align*}
hence
\begin{align*}
|R^1_\eta(t,s) - R^2_\eta(t,s)| &\leq \frac{1}{\sigma^2}\int_s^t |R_\theta^1(t,s') - R_\theta^2(t,s')||R_\eta^1(s',s)|\d s' + \frac{1}{\sigma^2}\int_s^t |R_\theta^2(t,s')||R_\eta^1(s',s) - R_\eta^2(s',s)|\d s'\\
&\quad + \frac{\delta}{\sigma^4}|R^1_\theta(t,s) - R^2_\theta(t,s)|.
\end{align*}
Using $|R_\eta^1(s',s)| \leq \Phi_{R_\eta}(s'-s)\leq \Phi_{R_\eta}(T)$, the first term is bounded by $\frac{\Phi_{R_\eta}(T)}{\sigma^2}\frac{e^{\lambda t}}{\lambda}d(R_\theta^1, R_\theta^2)$. Similarly, using $|R_\theta^2(t,s')| \leq \Phi_{R_\theta}(t-s) \leq \Phi_{R_\theta}(T)$, the second term satisfies
\begin{align*}
\frac{1}{\sigma^2}\int_s^t |R_\theta^2(t,s')||R_\eta^1(s',s) - R_\eta^2(s',s)|\d s' \leq \frac{\Phi_{R_\theta}(T)}{\sigma^2}\frac{e^{\lambda t}}{\lambda}d(R_\eta^1, R_\eta^2) \leq \frac{1}{2}e^{\lambda t}d(R_\eta^1, R_\eta^2),
\end{align*}
for large enough $\lambda$. The third term is bounded by $\frac{\delta}{\sigma^4}e^{\lambda t} d(R_\theta^1,R_\theta^2)$. Combining the three terms yields 
\begin{align*}
d(R^1_\eta, R^2_\eta) \leq C\cdot d(R^1_\theta, R^2_\theta) \leq C\cdot d(Y^1,Y^2)
\end{align*}
for some $C>0$ depending on $\Phi_{R_\eta}(T), \delta, \sigma$. Analogous arguments for $d(R_\eta^{\ast 1}, R_\eta^{\ast 2};\lambda, T)$ yields
\begin{align*}
d(R^{\ast 1}_\eta, R^{\ast 2}_\eta) \leq 0.01 \cdot d(R^1_\theta, R^2_\theta) \leq 0.01 \cdot d(Y^1, Y^2)
\end{align*}
for large enough $\lambda$. Combining parts 1 and 2 yields the claim of the lemma. 
\end{proof}

\begin{lemma}[Contractivity of $\cT$]\label{lem:T_contract}
For $i=1,2$, let $X_\eta^i = (C_\eta^i, R_\eta^i, R_\eta^{\ast i}) \in \cS_\eta$. Then for large enough $\lambda$ (depending on $\delta, \sigma, L, T, \Phi_{C_\theta}(T), \Phi_{R_\theta}(T)$), it holds that
\begin{align*}
d(\cT(X_\eta^1), \cT(X_\eta^2);\lambda, T) \leq \frac{1}{2} d(X^1_\eta, X^2_\eta;\lambda,T).
\end{align*}
\end{lemma}
\begin{proof}
Let $X^i_\theta \equiv \cT_{\eta\rightarrow\theta}(X^i_\eta)$ for $i=1,2$. By Lemmas \ref{lem:Trange_eta_2_theta} and \ref{lem:Trange_theta_2_eta}, $X^i_\theta \in \cS_\theta$, and $\cT(X_\eta^i) = \cT_{\theta\rightarrow\eta}(X^i_\theta) \in \cS_\eta$. Hence by Lemmas \ref{lem:modulus_eta_2_theta} and \ref{lem:modulus_theta_2_eta},
\begin{align*}
d(\cT(X_\eta^1), \cT(X_\eta^2);\lambda, T) \leq \eps \cdot d(X_\theta^1), X_\theta^2);\lambda, T) \leq C\eps \cdot d(X_\eta^1, X_\eta^2), 
\end{align*}
and the conclusion follows by choosing $\eps = 1/(2C)$.
\end{proof}

\subsection{Completion of proof}
\begin{proof}[Proof of Proposition \ref{prop:dmftsolexists}]
Let
\begin{align*}
\bar{\cS}_\eta \equiv \{X_\eta = (R_\eta, R_\eta^\ast, C_\eta): R_\eta \in L^\infty([0,T]^2,\R), R_\eta^\ast \in L^\infty([0,T],\R), C_\eta \in L^\infty([0,T]^2, \R)\}
\end{align*}
be the space of bounded functions equipped with the $L^\infty$ metric $d_\infty$, i.e., 
\begin{align*}
d_\infty(X^1_\eta, X^2_\eta) &\equiv d_\infty(R^1_\eta, R^2_\eta) + d_\infty(R^{\ast 1}_\eta, R^{\ast 2}_\eta) + d_\infty(C^1_\eta, C^2_\eta)\\
&\equiv \sup_{s,t\in[0,T]} |R^1_\eta(t,s) - R^2_\eta(t,s)| + \sup_{t\in[0,T]} |R^{1}_\eta(t,\ast) - R^{2}_\eta(t,\ast)| + \sup_{t,s\in[0,T]} |C^1_\eta(t,s) - C^2_\eta(t,s)|.
\end{align*}
It is clear that $(\bar{\cS}_\eta, d_\infty)$ is a Banach space and $\cS_\eta$ is a closed subset of $\cS_\eta$. Let $X^{(0)}_\eta$ be an arbitrary element of $\cS_\eta$, and $X^{(n)}_\eta \equiv \cT_{\eta \rightarrow \eta}(X^{(n-1)}_\eta)$ be defined recursively. By the contractive property established in Lemma \ref{lem:T_contract}, $\{X^{(n)}_\eta\}_{n\in \Z_+}$ is a Cauchy sequence under the metric $d$. We claim that it is also a Cauchy sequence under the metric $d_\infty$. It clearly holds for the $R_\eta$ and $R_\eta^\ast$ components since $d(R^1_\eta, R^2_\eta;\lambda, T)$ (resp. $d(R^{\ast 1}_\eta, R^{\ast 2}_\eta;\lambda, T)$) is equivalent to $d_\infty(R^1_\eta, R^2_\eta)$ (resp. $d_\infty(R^{\ast 1}_\eta, R^{\ast 2}_\eta)$) up to some constants depending on $T$ (which is finite). On the other hand, for any $C^1_\eta, C^2_\eta \in \cS_\eta$ which are covariance kernels, let $\{g^t_1\}$ (resp. $\{g^t_2\}$) be a Gaussian process with covariance structure $C^1_\eta$ (resp. $C^2_\eta$), then
\begin{align*}
|C^1_\eta(t,s) - C^2_\eta(t,s)| &= \big|\E[g^t_1g^s_1] - \E[g^t_2g^s_2]\big|\\
&\leq \big|\E[g^t_1(g^s_1 - g^s_2)] + \E[g^s_2(g^t_1 - g^t_2)]\big|\\
&\leq \sqrt{\E[(g^t_1)^2]}e^{\lambda T}\cdot \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(g^t_1 - g^t_2)^2]} + \sqrt{\E[(g^s_2)^2]}e^{\lambda T}\cdot \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(g^t_1 - g^t_2)^2]}\\
&\leq 2\Phi_{C_\eta}(T)e^{\lambda T} \cdot \sup_{t\in[0,T]} e^{-\lambda t}\sqrt{\E[(g^t_1 - g^t_2)^2]} + d(C^1_\eta,C^2_\eta;\lambda, T).
\end{align*}
Taking the infimum over all couplings of $\{g^t_1\}$ and $\{g^t_2\}$ yields $d_\infty(C^1_\eta, C^2_\eta) \leq 2\Phi_{C_\eta}(T)e^{\lambda T} \cdot d(C^1_\eta, C^2_\eta;\lambda, T)$, which concludes that $\{X^{(n)}_\eta\}_{n\in \Z_+}$ is also a Cauchy sequence under the metric $d_\infty$. Hence by completeness, there exists some limiting point $X^\ast_\eta$ in $\cS_\eta$ (since it is closed), which is also the fixed point of the map $\cT_{\eta\rightarrow\eta}$. Let $X^\ast_\theta = \cT_{\eta\rightarrow\theta}(X^\ast_\eta) \in \cS_\theta$, and then Lemmas \ref{lem:sub_theta_solution} and \ref{lem:sub_eta_solution} guarantee the existence of a solution to the DMFT system. This solution is also unique because if there are two solutions $\{\theta^t_i, \eta^t_i, R_\theta^i, C_\theta^{i}, C_\theta^{\ast i}, R_{\eta}^i, R_\eta^{\ast i}, C_\eta^i\}$ for $i=1,2$, then $(R_{\eta}^i, R_\eta^{\ast i}, C_\eta^i) \in \cS_\eta$ by Lemma \ref{lem:Trange_theta_2_eta}, and by definition they are also fixed points of the map $\cT_{\eta\rightarrow\eta}$, hence uniqueness results from uniqueness of fixed points of $\cT_{\eta\rightarrow\eta}$.
\end{proof}




==> replica.tex <==
\section{Replica-symmetric predictions for the posterior overlaps}\label{appendix:replica}

Suppose that $n/d = \delta$, $X_{ij} \sim_{i.i.d.} \N(0, \frac{1}{d})$, the true prior of $\btheta^\ast$ is $g^\ast$, and the nominal prior is $g$ in the following posterior distribution:
\begin{align*}
P_g(\btheta|\X,\y) = \frac{(2\pi\sigma^2)^{-n/2}e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2}}\prod_{j=1}^d g(\theta_j)}{Z_n},
\end{align*}
where with $\Xi_n = \int e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2}}g(\btheta) \d\btheta$, 
\begin{align*}
Z_n = Z_n(\X,\y) = \int (2\pi\sigma^2)^{-\frac{n}{2}}e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2}}\prod_{j=1}^d g(\theta_j) \d\btheta = (2\pi\sigma^2)^{-\frac{n}{2}}\Xi_n.
\end{align*}
The goal is to compute the limiting free energy
\begin{align*}
\lim_{d\rightarrow \infty} \frac{1}{d}\E_{g^\ast} \log Z_n = -\frac{\delta}{2}\log(2\pi\sigma^2) + \lim_{d\rightarrow \infty} \frac{1}{d}\E_{g^\ast} \log \Xi_n,
\end{align*}
where the expectation is taken over the model $\y = \X\btheta^\ast + \beps$ with $\btheta^\ast \sim_{iid} g^\ast$. The replica trick applies the formula
\begin{align}\label{ineq:replica_3}
\lim_{d\rightarrow\infty} \frac{1}{d}\E_{g^\ast} \log \Xi_n = \lim_{k\downarrow 0}\partial_k\big[\lim_{d\rightarrow\infty} \frac{1}{d}\log\E_{g^\ast} \Xi_n^k\big], 
\end{align}
where we treat $k$ as an integer. We have 
\begin{align*}
\E_{g^\ast} \Xi_n^k &= \E_{g^\ast} \int g(\btheta^1)\ldots g(\btheta^k) e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k \pnorm{\y - \X\btheta^a}{}^2} \d\btheta^1\ldots\d\btheta^k\\
&= \E_{\X}\int g^\ast(\btheta^0) (2\pi\sigma^2)^{-\frac{n}{2}}e^{-\frac{\pnorm{\y - \X\btheta^0}{}^2}{2\sigma^2}}e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k \pnorm{\y - \X\btheta^a}{}^2} \d\btheta^0\d\btheta^1\ldots\d\btheta^k\d \y\\
&= \E_{\X}\int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k) \prod_{i=1}^n \Big[\int(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y_i - \x_i^\top\btheta^0)^2}{2\sigma^2}}e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k (y_i - \x_i^\top\btheta^a)^2}\d y_i\Big]\d\btheta^0\d\btheta^1\ldots\d\btheta^k\\
&= \int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k) \Big[\int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - \x^\top\btheta^0)^2}{2\sigma^2}}e^{-\frac{1}{2\sigma^2}\sum_{a=1}^k (y - \x^\top\btheta^a)^2}}\d y\Big]^n\d\btheta^0\d\btheta^1\ldots\d\btheta^k,
\end{align*}
where $\x \sim \N(0, d^{-1}I_d)$, and we use overline to denote the average with respect to $\x$. Let
\begin{align*}
v^0 \equiv \x^\top \btheta^0, v^a \equiv \x^\top \btheta^a, \quad a\in[k],
\end{align*}
we have $(v^0,v^1,\ldots,v^k) \sim \N(0, Q)$ conditioning on $(\btheta^0,\btheta^k)$, where $Q_{ab} = d^{-1}\iprod{\btheta^a}{\btheta^b}$. Hence we have
\begin{align}\label{ineq:replica_1}
\notag\E_{g^\ast}\Xi_n^k &= \int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k) \Big[\int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - v^0)^2}{2\sigma^2} - \sum_{a=1}^k \frac{(y - v^a)^2}{2\sigma^2}}}\d y\Big]^n\d\btheta^0\d\btheta^1\ldots\d\btheta^k\\
&= \int_{[-M,M]^{\frac{(k+1)(k+2)}{2}}} e^{n\mathcal{G}(Q)} \mu_k(Q) \prod_{0\leq a\leq b \leq k}\d Q_{ab}, 
\end{align}
where
\begin{align*}
\mathcal{G}(Q) = \log \int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - v^0)^2}{2\sigma^2} - \sum_{a=1}^k \frac{(y - v^a)^2}{2\sigma^2}}}\d y,
\end{align*}
and
\begin{align*}
\mu_k(Q) = \int g^\ast(\btheta^0)g(\btheta^1)\ldots g(\btheta^k)\prod_{0\leq a\leq b \leq k} \delta(\iprod{\btheta^a}{\btheta^b} - dQ_{ab})\d\btheta^0\ldots\d\btheta^k
\end{align*}
is the probability weight of the shell
\begin{align*}
\mathcal{S}(Q) = \{(\btheta^0,\ldots,\btheta^k): d^{-1}\iprod{\btheta^a}{\btheta^b} = Q_{a,b}, 0\leq a\leq b\leq k\}.
\end{align*}
Suppose $-d^{-1}\log \mu_k(Q) \rightarrow_{d\rightarrow\infty} \mathcal{I}(Q)$ for some rate function $\mathcal{I}(Q)$, then applying the Laplace method to (\ref{ineq:replica_1}) yields
\begin{align}\label{ineq:replica_2}
\lim_{d\rightarrow\infty} \frac{1}{d}\log\E_{g^\ast} \Xi_n^k = \sup_{Q} \big[\delta \mathcal{G}(Q) - \mathcal{I}(Q)\big]. 
\end{align}
By the replica-symmetric ansatz, the optimal $Q$ takes the form
\begin{align*}
Q = 
\begin{bmatrix}
r & m & m & m & \ldots & m\\
m & p & q & q & \ldots & q\\
m & q & p & q & \ldots & q\\
\ldots\\
m & q & q & q & \ldots & p
\end{bmatrix}.
\end{align*}
Let us now evaluate $\mathcal{G}(Q)$ and $\mathcal{I}(Q)$ under this ansatz. Denote
\begin{align*}
v^0 = u\sqrt{r-\frac{m^2}{q}} - t\frac{m}{\sqrt{q}}, \quad v^a = z^a\sqrt{p-q} - t\sqrt{q},
\end{align*}
where $u,t,\{z^a\}_{a=1}^k$ are standard normal variables. Then
\begin{align*}
e^{\mathcal{G}(Q)} &= \int \overline{(2\pi\sigma^2)^{-\frac{1}{2}}e^{-\frac{(y - v^0)^2}{2\sigma^2} - \sum_{a=1}^k \frac{(y - v^a)^2}{2\sigma^2}}}\d y\\
&= (2\pi\sigma^2)^{-1/2}\E_{u,t,z^a}\int e^{-\frac{r-m^2/q}{2\sigma^2}\big[u - (r-m^2/q)^{-1/2}(y + tm/\sqrt{q})\big]^2} e^{-\frac{p-q}{2\sigma^2}\sum_{a=1}^k\big[z^a - (p-q)^{-1/2}(y + t\sqrt{q})\big]^2} \d y\\
&= (2\pi\sigma^2)^{-1/2}\big[1+\sigma^{-2}(r-m^2/q)\big]^{-1/2}\big[1+\sigma^{-2}(p-q)\big]^{-k/2}\E_t \int e^{-\frac{1}{2(\sigma^2 + r-m^2/q)}\big[y + \frac{tm}{\sqrt{q}}\big]^2}e^{-\frac{k}{2(\sigma^2 + p-q)}\big[y + t\sqrt{q}\big]^2}\d y\\
&\equiv (2\pi\sigma^2)^{-1/2}\big[1+\sigma^{-2}(r-m^2/q)\big]^{-1/2}\big[1+\sigma^{-2}(p-q)\big]^{-k/2}\E_t \int e^{-\frac{\mathsf{A_1}}{2}y^2 - \frac{\mathsf{A}_2}{2}t^2 - \mathsf{B}t}\\
&= (2\pi\sigma^2)^{-1/2}\big[1+\sigma^{-2}(r-m^2/q)\big]^{-1/2}\big[1+\sigma^{-2}(p-q)\big]^{-k/2}\E_t \int e^{-\frac{\mathsf{A_1}}{2}y^2} e^{-\frac{\mathsf{A}_2}{2}(t + \frac{\mathsf{B}}{\mathsf{A}_2})^2} e^{\frac{\mathsf{B}^2}{2\mathsf{A}_2}}\d y,
\end{align*}
where with $\mathsf{U} = 1 + \sigma^{-2}(r-m^2/q)$ and $\mathsf{V} = 1 + \sigma^{-2}(p-q)$, 
\begin{align*}
\mathsf{A}_1 &= \frac{\sigma^{-2}}{\mathsf{U}} + \frac{k\sigma^{-2}}{\mathsf{V}},\\
\mathsf{A}_2 &= \frac{\sigma^{-2}}{\mathsf{U}}\frac{m^2}{q} + \frac{k\sigma^{-2}}{\mathsf{V}}q,\\
\mathsf{B} &= \frac{\sigma^{-2}}{\mathsf{U}}\frac{ym}{\sqrt{q}} + \frac{k\sigma^{-2}}{\mathsf{V}}y\sqrt{q}. 
\end{align*}
Consequently,
\begin{align*}
e^{\mathcal{G}(Q)} &= (2\pi\sigma^2)^{-1/2}V^{-\frac{k-1}{2}}\big[(1+\sigma^{-2}r)\mathsf{V} + kq\sigma^{-2}\mathsf{U}\big]^{-1/2} \int e^{-\frac{\mathsf{A}_1}{2}y^2 + \frac{\mathsf{B}^2}{2(\mathsf{A}_2 + 1)}}\d y\\
&= (2\pi\sigma^2)^{-1/2}V^{-\frac{k-1}{2}}\big[(1+\sigma^{-2}r)\mathsf{V} + kq\sigma^{-2}\mathsf{U}\big]^{-1/2} \int e^{-\frac{y^2}{2}\frac{\sigma^{-2}\mathsf{V} + k\sigma^{-2}\big[1+\sigma^{-2}(r-2m+q)\big]}{(1+r\sigma^{-2})\mathsf{V} + kq\sigma^{-2}\mathsf{U}}}\d y\\
&= \mathsf{V}^{-\frac{k-1}{2}}\big[\mathsf{V} + k(1+\sigma^{-2}(r-2m+q))\big]^{-1/2}.
\end{align*}
Next we evaluate the rate function $\mathcal{I}(Q)$. Since $d^{-1}\iprod{\btheta^a}{\btheta^b}$ is a set of sample means of $d$ i.i.d. variables with law $\mu = \mathcal{L}(\{\theta^a_1\theta^b_1\}_{0\leq a, b\leq k})$ on $\R^{(k+1)^2}$, Cramer's theorem yields that
\begin{align}\label{eq:rate_func}
\mathcal{I}(Q) = \sup_{\{\tilde{Q}_{ab}\}_{0\leq a, b\leq k}} \big[\iprod{\tilde{Q}}{Q} - M(\tilde{Q})\big],
\end{align}
where $M = M_\mu$ is the cumulant generating function of law $\mu$ evaluated as
\begin{align*}
M(\tilde{Q}) = \log \E_{\{Q_{ab}\}_{0\leq a, b\leq k} \sim \mu} e^{\iprod{\tilde{Q}}{Q}} = \log \int g^{\ast}(\theta^0)g(\theta^1)\ldots g(\theta^k) e^{\sum_{0\leq a,b\leq k} \tilde{Q}_{ab}\theta^a\theta^b} \d\theta^0\ldots \d\theta^k.
\end{align*}
Again by the RS ansatz, the optimal $\tilde{Q}$ in (\ref{eq:rate_func}) takes the form
\begin{align*}
\tilde{Q} = 
\begin{bmatrix}
c & d & d & d & \ldots & d\\
d & g & f & f & \ldots & f\\
d & f & g & f & \ldots & f\\
\ldots\\
d & f & f & f & \ldots & g
\end{bmatrix}.
\end{align*}
Hence with $\btheta = (\theta^0,\ldots, \theta^k) \in \R^{k+1}$,
\begin{align*}
M(\tilde{Q}) = M(c,d,f,g) &= \E e^{\iprod{\tilde{Q}}{\btheta\btheta^\top}}\\
&=\E \exp\Big[c(\theta^0)^2 + 2d\theta^0 \cdot \sum_{a=1}^k \theta^a + g \sum_{a=1}^k (\theta^a)^2 + f\sum_{1\leq a\neq b\leq k} \theta^a\theta^b\Big]\\
&=\E \exp\Big[\Big(\frac{d}{\sqrt{f}}\theta^0 + \sqrt{f}\sum_{a=1}^k \theta^a\Big)^2 + (c - \frac{d^2}{f})(\theta^0)^2 + (g-f)(\sum_{a=1}^k \theta^a)^2\Big]\\
&= \E_{\btheta}\E_{z\sim \N(0, \frac{f}{2d^2})}\exp\Big[\frac{2d}{\sqrt{f}}z\Big(\frac{d}{\sqrt{f}}\theta^0 + \sqrt{f}\sum_{a=1}^k \theta^a\Big)+ (c - \frac{d^2}{f})(\theta^0)^2 + (g-f)(\sum_{a=1}^k \theta^a)^2\Big]\\
&= \E_z \E_{\theta^0 \sim g^\ast}\Big(e^{\frac{2d^2}{f}z\theta^0 + (c-\frac{d^2}{f})(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2dz\theta + (g-f)\theta^2}\Big)\Big]^k,
\end{align*}
and therefore
\begin{align*}
\mathcal{I}(Q) = \sup_{c,d,f,g} \bigg\{rc + kpg + 2kmd + k(k-1)qf - \log\Big(\E_z \E_{\theta^0 \sim g^\ast}\bigg[e^{\frac{2d^2}{f}z\theta^0 + (c-\frac{d^2}{f})(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2dz\theta + (g-f)\theta^2}\Big)\Big]^k\bigg]\bigg\}.
\end{align*}
Combining (\ref{ineq:replica_3}), (\ref{ineq:replica_2}), and (\ref{eq:rate_func}), the RS ansatz yields that
\begin{align}\label{eq:replica_4}
\lim_{d\rightarrow\infty} \frac{1}{d}\E_{g^\ast}\log \Xi_n = \sup_{r,m,p,q}\inf_{c,d,f,g} \partial_k|_{k\downarrow 0}\big[f^{RS}(c,d,f,g, r,m,p,q;k)\big],
\end{align}
where
\begin{align*}
f^{RS} &= -\frac{(k-1)\delta}{2}\log[1+\sigma^{-2}(p-q)] - \frac{\delta}{2}\log\big[1+\sigma^{-2}(p-q)+k(1+\sigma^{-2}(r-2m+q))\big]\\
&\quad - (rc + kpg + 2kmd + k(k-1)qf) + \log\Big(\E_z \E_{\theta^0 \sim g^\ast}\bigg[e^{\frac{2d^2}{f}z\theta^0 + (c-\frac{d^2}{f})(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2dz\theta + (g-f)\theta^2}\Big)\Big]^k\bigg]\bigg\}.
\end{align*}
We first represent the optimal $(c,d,f,g)$ in $(r,m,p,q)$ for $k\downarrow 0$. To this end, we have
\begin{align}\label{eq:critical_1}
\notag\partial_r f^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow c = 0,\\
\notag\partial_m f^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow d = \frac{\delta\sigma^{-2}}{2\big[1+\sigma^{-2}(p-q)\big]},\\
\notag\partial_q\partial_k f^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow f = \frac{\delta\sigma^{-2}\big[1+\sigma^{-2}(r-2m+q)\big]}{2\big[1+\sigma^{-2}(p-q)\big]^2},\\
\partial_p\partial_kf^{RS}|_{k\downarrow 0} = 0 &\Longrightarrow g = f - d. 
\end{align}
Plugging these into $M(\cdot)$, we have
\begin{align}\label{eq:mgf_critical}
\notag M(c,d,f,g) &= \E_{z\sim \N(0,\frac{f}{2d^2})} \E_{\theta^0 \sim g^\ast}\Big(e^{\frac{2d^2}{f}z\theta^0 -\frac{d^2}{f}(\theta^0)^2}\Big) \Big[\E_{\theta\sim g}\Big(e^{2d z\theta -d\theta^2}\Big)\Big]^k\\
&= \sqrt{\frac{\eta}{2\pi}} \int \E_{g^\ast} e^{-\frac{\eta}{2}(z-\theta^0)^2} \Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]^k \d z,
\end{align}
where we define $(\eta,\xi)$ as
\begin{align}\label{def:eta_xi}
\eta = \frac{2d^2}{f},\quad 2d = \xi.
\end{align}
Let us now represent $(r,m,p,q)$ in $(\xi, \eta)$. From (\ref{eq:rate_func}), the critical $(Q,\tilde{Q})$, denoted by $(Q^\ast,\tilde{Q}^\ast)$ (parametrized under the RS ansatz by $p,q,r,m,c,d,f,g$), satisfies
\begin{align*}
Q^\ast = \frac{\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\btheta\btheta^\top\big]}{\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\big]} = \frac{\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\btheta\btheta^\top\big]}{M(\tilde{Q}^\ast)} \stackrel{k\downarrow 0}{\longrightarrow}\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\btheta\btheta^\top\big],
\end{align*}
where the last step follows since $M(\tilde{Q}^\ast) \rightarrow 1$ as $k\downarrow 0$ from (\ref{eq:mgf_critical}). As an example, let us compute $Q^\ast_{01} = m$, where
\begin{align*}
\E\big[e^{\iprod{\tilde{Q}^\ast}{\btheta\btheta^\top}}\theta^0\theta^1\big] &= \sqrt{\frac{\eta}{2\pi}}\int \E_{\theta^0\sim g^\ast}\Big[\theta^0 e^{-\frac{\eta}{2}(z - \theta^0)^2}\Big] \cdot \frac{\E_{\theta \sim g^\ast}\Big[\theta e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]}{\E_{\theta \sim g^\ast}\Big[e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]} \cdot \Big\{\E_{\theta \sim g^\ast}\Big[e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]\Big\}^k \d z\\
&\stackrel{k\downarrow 0}{\longrightarrow}\sqrt{\frac{\eta}{2\pi}}\int \E_{\theta^0\sim g^\ast}\Big[\theta^0 e^{-\frac{\eta}{2}(z - \theta^0)^2}\Big] \cdot \frac{\E_{\theta \sim g^\ast}\Big[\theta e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]}{\E_{\theta \sim g^\ast}\Big[e^{\xi\theta z - \frac{\xi}{2}\theta^2}\Big]} \d z\\
&= \E_{(g^\ast;\eta^{-1})} \big[\theta\av{\theta}_{(g;\xi^{-1})}\big].
\end{align*}
Here we introduce the scalar channel indexed by prior $g$ and noise level $\sigma^2$: 
\begin{align}\label{eq:scalar_channel}
Y = \theta + \eps, \quad \theta \sim g, \eps \sim \N(0,\sigma^2), 
\end{align}
and use $\E_{(g;\sigma^2)}$ to denote the expectation under this channel, and
\begin{align*}
\av{f(\theta)}_{(g;\sigma^2)} = \E[f(\theta)| Y = y] = \frac{\int f(\theta) e^{-\frac{(y-\theta)^2}{2\sigma^2}}g(\d\theta)}{\int  e^{-\frac{(y-\theta)^2}{2\sigma^2}}g(\d\theta)}
\end{align*}
to denote the posterior average. A similar calculation yields that
\begin{align}\label{eq:replica_parameter}
r &= Q^\ast_{00} = \E_{(g_\ast;\eta^{-1})}\big[\theta^2\big],\\
p &= Q^\ast_{11} = \E_{(g_\ast;\eta^{-1})}\big[\av{\theta^2}_{(g;\xi^{-1})}\big],\\
q &= Q^\ast_{12} = \E_{(g_\ast;\eta^{-1})}\big[\av{\theta}^2_{(g;\xi^{-1})}\big],
\end{align}
from which we obtain
\begin{align}\label{eq:consistent_1}
\notag r-2m+q &= \E_{(g_\ast;\eta^{-1})}\big[(\theta - \av{\theta}_{g;\xi^{-1}})^2\big],\\
p - q &= \E_{(g_\ast;\eta^{-1})}\big[\av{\theta^2}_{g;\xi^{-1}} - \av{\theta}^2_{g;\xi^{-1}}\big].
\end{align}
On the other hand, (\ref{eq:critical_1}) yields
\begin{align}\label{eq:consistent_2}
r-2m+q = \delta\eta^{-1} - \sigma^2, \quad p - q = \delta\xi^{-1} - \sigma^2.
\end{align}
Combining (\ref{eq:consistent_1}) and (\ref{eq:consistent_2}) yields the self-consistent equation for the critical $(\eta_\star, \xi_\star)$:
\begin{align}\label{eq:replica_consistent}
\notag\delta \eta^{-1} &= \sigma^2 + \E_{(g_\ast;\eta^{-1})}\big[(\theta - \av{\theta}_{g;\xi^{-1}})^2\big],\\
\delta \xi^{-1} &= \sigma^2 + \E_{(g_\ast;\eta^{-1})}\big[\av{\theta^2}_{g;\xi^{-1}} - \av{\theta}^2_{g;\xi^{-1}}\big].
\end{align}
Lastly, note that (recall (\ref{eq:mgf_critical}))
\begin{align*}
\partial_k|_{k\downarrow 0} \log M(\tilde{Q}^\ast) &= \partial_k|_{k\downarrow 0} \log \Big[\sqrt{\frac{\eta}{2\pi}} \int \E_{g^\ast} e^{-\frac{\eta}{2}(z-\theta^0)^2} \Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]^k \d z\Big]\\
&= \partial_k|_{k\downarrow 0} \log \E_{z\sim(g^\ast;\eta^{-1})}\big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\big]^k\\
&= \partial_k|_{k\downarrow 0} \E_{z\sim(g^\ast;\eta^{-1})}\Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]^k\\
&\stackrel{(*)}{=} \E_{z\sim(g^\ast;\eta^{-1})} \log\Big[\E_{\theta\sim g} e^{\frac{\xi}{2}z^2 
- \frac{\xi}{2}(\theta-z)^2}\Big]\\
&= \frac{\xi}{2}(\E_{g^\ast}[\theta^2] + \eta^{-1}) + \frac{1}{2}\log(2\pi\xi^{-1}) + \E_{z\sim(g^\ast;\eta^{-1})}\log p_{(g;\xi^{-1})}(z),
\end{align*}
where we use $p_{(g;\xi)}(\cdot)$ to denote the density of $Y$ in the scalar channel (\ref{eq:scalar_channel}). Then by plugging the critical $(r,m,p,q,c,d,f,g)$ into (\ref{eq:replica_4}), we have
\begin{align*}
\lim_{d} d^{-1}\E_{g^\ast} \log \Xi_n &= -\frac{\delta}{2}\log\big[1+\sigma^{-2}(p-q)\big] - \frac{\delta}{2}\frac{1+\sigma^{-2}(r-2m+q)}{1+\sigma^{-2}(p-q)} - (pg + 2md-qf) + \partial_k|_{k\downarrow 0} \log M(\tilde{Q}^\ast)\\
&= -\frac{\delta}{2}\log\Big(\frac{\delta}{\sigma^2\xi}\Big) - \frac{\delta\xi}{2\eta} - \xi\sigma^2 + \frac{\xi^2}{2\eta}\sigma^2 + \frac{\delta}{2} + \frac{\xi}{2\eta} + \frac{1}{2}\log(2\pi\xi^{-1}) + \E_{z\sim(g^\ast;\eta^{-1})}\log p_{(g;\xi^{-1})}(z),
\end{align*}
where $(\xi,\eta)$ are given by (\ref{eq:replica_consistent}).

\begin{remark}[Correctly specified case]
In this case, the RS ansatz posits that $d = f$ so $\eta = \xi$, and hence the above RS formula implies that
\begin{align*}
\lim_d d^{-1}I(\y; \btheta) &= \lim_d -d^{-1}\E_{\btheta^\ast \stackrel{i.i.d.}{\sim} g} \log \int e^{-\frac{\pnorm{\X(\btheta - \btheta^\ast)}{}^2}{2\sigma^2} + \frac{\beps^\top \X(\btheta - \btheta^\ast)}{\sigma^2}} \prod_{j=1}^p g(\theta_j)\d\btheta\\
&= -\lim_d d^{-1}\E_{g^\ast} \log \Xi_n - \frac{\delta}{2}\\
&= \frac{\delta}{2}\log\Big(\frac{\delta}{\sigma^2\xi}\Big) - \frac{\delta}{2} + \frac{\xi\sigma^2}{2} - \frac{1}{2}\log(2\pi\xi^{-1}) - \frac{1}{2} + H(Y;g,\xi^{-1}), 
\end{align*}
where $H(Y;g,\xi^{-1})$ denotes the differential entropy of the law of $Y$ in the channel (\ref{eq:scalar_channel}) with prior $g$ and noise variance $\xi^{-1}$, and $\xi$ solves the equation
\begin{align*}
\delta \xi^{-1} &= \sigma^2 + \E_{(g;\xi^{-1})}\big[\av{\theta^2}_{g;\xi^{-1}} - \av{\theta}^2_{g;\xi^{-1}}\big].
\end{align*}
This is previously proved in, e.g., Theorem 3.2 of \cite{barbier2020mutual} (with the change of variable $E = \delta\xi^{-1} - \sigma^2$ therein), as
\begin{align*}
\lim_d d^{-1}I(\y; \btheta) = \inf i^{RS}(\xi^{-1}),
\end{align*}
where
\begin{align*}
i^{RS}(\xi^{-1}) = \frac{1}{2}\Big(\delta\log(\frac{\delta}{\sigma^2\xi}) - \delta + \frac{\sigma^2}{\xi^{-1}}\Big) + i_{(g;\xi^{-1})}(Y;\theta)
\end{align*}
with $i_{(g;\xi^{-1})}(Y;\theta)$ denotes the mutual information of the scalar channel (\ref{eq:scalar_channel}).
\end{remark}

\begin{remark}[Gaussian prior with mismatched variance]
Suppose $g^\ast = \N(0,\tau^2_\ast)$ and $g = \N(0,\tau^2)$, then 
\begin{align*}
&\lim_d d^{-1}\E_{g^\ast} \log \int e^{-\frac{\pnorm{\y - \X\btheta}{}^2}{2\sigma^2} - \frac{\pnorm{\btheta}{}^2}{2\tau^2}}\d\btheta\\
&= \frac{1}{2}\log(2\pi\tau^2) + \lim_d d^{-1}\E_{g^\ast} \log \Xi_n\\
&= -\frac{\delta}{2}\log\Big(\frac{\delta}{\sigma^2\xi}\Big) - \frac{\delta\xi}{2\eta} - \xi\sigma^2 + \frac{\xi^2}{2\eta}\sigma^2 + \frac{\delta}{2} + \frac{\xi}{2\eta} + \frac{1}{2}\log(\xi^{-1}) -\frac{1}{2}\log\big(\tau^2+\xi^{-1}) - \frac{\tau^2_\ast + \eta^{-1}}{2(\tau^2+\xi^{-1})} + \frac{1}{2}\log(2\pi\tau^2), 
\end{align*}
where we use $p_{g;\xi^{-1}}(y) = (2\pi (\tau^2 + \xi^{-1}))^{-1/2} e^{-\frac{y^2}{2(\tau^2 + \xi^{-1})}}$, and hence $\E_{y\sim (g^\ast;\eta^{-1})} \log p_{g;\xi^{-1}}(y) = -\frac{1}{2}\log\big[2\pi(\tau^2+\xi^{-1})\big] - \frac{\tau^2_\ast + \eta^{-1}}{2(\tau^2+\xi^{-1})}$. Next note that $\av{\theta}_{(g;\xi^{-1})} = \frac{\tau^2}{\tau^2 + \xi^{-1}}y$ and $\av{\theta^2}_{(g;\xi^{-1})} = \Big(\frac{\tau^2}{\tau^2 + \xi^{-1}}y\Big)^2 + \frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}$, so the consistent equation for $\xi$ reads
\begin{align}\label{eq:consistent_xi}
\delta \xi^{-1} = \sigma^2 + \frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}. 
\end{align}
Then the above RS formula can be further simplified as
\begin{align*}
&=\frac{\delta}{2}\log\Big(\frac{\sigma^2\xi}{\delta}\Big) + \frac{1}{2}\log\Big(\frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}\Big) + \frac{1}{2}\log(2\pi) - \frac{\tau_\ast^2}{2(\tau^2+\xi^{-1})} + \frac{\delta}{2} -\sigma^2\xi - \frac{1}{2\eta(\tau^2+\xi^{-1})}\big[\underbrace{(1+\tau^2\xi)(\delta-\sigma^2\xi-1) + 1}_{=0}\big]\\
&= \frac{\delta}{2}\log\Big(\frac{\sigma^2\xi}{\delta}\Big) + \frac{1}{2}\log\Big(\frac{\tau^2\xi^{-1}}{\tau^2 + \xi^{-1}}\Big) + \frac{1}{2}\log(2\pi) - \frac{\tau_\ast^2}{2(\tau^2+\xi^{-1})} + \frac{\delta}{2} -\sigma^2\xi,
\end{align*}
where $\xi$ is given by (\ref{eq:consistent_xi}). This is previously proved rigorously in Theorem 3.4 of \cite{barbier2021performance}, with change of variable $c = \rho - q = \delta\xi^{-1} - \sigma^2$ therein. The same reference also shows that the limiting MSE is
\begin{align*}
\mse(g;g^\ast) \equiv \lim_{d\rightarrow\infty} d^{-1}\E_{g^\ast} \pnorm{\av{\btheta}_g - \btheta^\ast}{}^2 = \frac{\sigma^2\tau^4 + \delta\xi^{-2}\tau_\ast^2}{\delta(\xi^{-1} + \tau^2)^2 - \tau^4}.
\end{align*}
In the replica notation, this corresponds to $q + \tau_\ast^2- 2m$, given by (\ref{eq:replica_parameter}).
\end{remark}




==> response.tex <==
\section{Response function of adaptive dynamics (Proof of Proposition \ref{prop:responseexists})}\label{sec:response}

In this section, we establish regularity properties of the
adaptive Langevin equations (\ref{eq:langevin_sde}--\ref{eq:gflow}) and their
associated Markov semigroup. We then prove
Proposition \ref{prop:responseexists} and give an explicit form for the response
function.

The evolution of $\x^t:=(\btheta^t,\widehat\alpha^t)$ by
(\ref{eq:langevin_sde}--\ref{eq:gflow}) may be written as a joint
Markovian diffusion on $\R^{d+K}$,
\begin{equation}\label{eq:joint_sde}
\d\x^t=u(\x^t)\d t+\sqrt{2}\,\M\,\d\b^t
\end{equation}
where $\x=(\btheta,\widehat\alpha)$,
\begin{equation}\label{eq:jointdrift}
\begin{aligned}
u(\x)&=\bigg(\frac{1}{\sigma^2} \X^\top (\y-\X\btheta)
+\Big(\partial_\theta \log g(\theta_j;\widehat\alpha)\Big)_{j=1}^d,\,
\cG\Big(\widehat\alpha,\frac{1}{d}\sum_{j=1}^d \delta_{\theta_j}\Big)\bigg)
\in \R^{d+K},\\
\M&=\begin{pmatrix} \I_d \\ 0_{d \times K} \end{pmatrix}
\in \R^{(d+K) \times d}.
\end{aligned}
\end{equation}
We remark that the coefficient matrix $\M\M^\top$ is singular when $K \geq 1$,
so this joint diffusion is not uniformly elliptic; we will verify existence of
the response function $R_{AB}$ for the function classes
(\ref{eq:testclass}--\ref{eq:driftclass}) via an adaptation of the method of
\cite{chen2020mathematical} for elliptic diffusions.

We recall our notation
\[\langle f(\x^t) \rangle=\E[f(\x^t) \mid \X,\y,\x^0]\]
for the expectation over only the Brownian motion $\{\b^t\}_{t \geq 0}$,
i.e.\ conditional on the data $(\X,\y)$ and initial condition
$\x^0=(\btheta^0,\widehat\alpha^0)$. This depends implicitly on the choice of
initial condition, and we will write
\begin{equation}\label{eq:semigroup}
P_tf(\x)=\langle f(\x^t) \rangle_{\x^0=\x}=\E[f(\x^t) \mid \X,\y,\x^0=\x]
\end{equation}
to make explicit the dependence on the initial condition when needed. Here
$\{P_t\}_{t \geq 0}$ is the Markov semigroup associated to
(\ref{eq:joint_sde}), which we verify below is well-defined on the function
class $\cA$. We denote its corresponding infinitesimal generator $\L$ by
\begin{equation}\label{eq:generator}
\L f(\x)=u(\x)^\top \nabla f(\x)+\Tr \M\M^\top \nabla^2 f(\x).
\end{equation}
Throughout this section $(\X,\y,n,d)$ are fixed, and all constants may depend
additionally on $(\X,\y,n,d)$.

\begin{proposition}\label{prop:langevinsolution}
Suppose Assumptions \ref{assump:prior} and \ref{assump:gradient} hold,
let $u_i:\R^{d+K} \to \R$ be the $i^\text{th}$ coordinate of $u$ in
(\ref{eq:joint_sde}), and let $\partial_j u_i$ and $\partial_j\partial_k u_i$
denote its first-order and second-order partial derivatives.
\begin{enumerate}[(a)]
\item For any $\x=(\btheta,\widehat\alpha) \in \R^{d+K}$ the diffusion (\ref{eq:joint_sde})
has a pathwise unique strong solution $\{\x^t\}_{t \geq 0}
=\{(\btheta^t,\widehat\alpha^t)\}_{t \geq 0}$ with initial condition $\x^0=\x$.

For any $r,T>0$ there exists
$C_{r,T}>0$ such that for all $t \in [0,T]$ and initial conditions with
$\|\widehat\alpha\|_2 \leq r$,
\begin{equation}\label{eq:alphaconfined}
\|\widehat\alpha^t\|_2 \leq C_{r,T}.
\end{equation}
\item For every $i=1,\ldots,d+K$ and $t \geq 0$, the coordinate
$x_i^t \equiv x_i^t(\x)$ of $\x^t$
is a $C^2$ function of the initial condition $\x$.
Its gradient $\v_i^t=\nabla x_i^t(\x) \in \R^{d+K}$ and Hessian
$\H_i^t=\nabla^2 x_i^t(\x) \in \R^{(d+K) \times (d+K)}$
are solutions to the first and second variation processes
\begin{equation}\label{eq:firstsecondvar}
\begin{cases}
\d \v_i^t=\sum_{j=1}^{d+K} \partial_j u_i(\x^t) \cdot \v_j^t\,\d t\\
\d \H_i^t=\big(\sum_{j,k=1}^{d+K} \partial_j\partial_k u_i(\x^t) \cdot
\v_j^t\v_k^{t\top}+\sum_{j=1}^{d+K} \partial_j u_i(\x^t) \cdot \H_j^t\big)\d t
\end{cases}
\quad \text{ for } i=1,\ldots,d+K,
\end{equation}
with initialization $\v_i^0=\e_i$ (the $i^\text{th}$ standard basis vector
in $\R^{d+K}$) and $\H_i^0=0$.

For any $r,T>0$, there exists $C_{r,T}>0$
such that for all $t \in [0,T]$ and
initial conditions with $\|\widehat\alpha\|_2 \leq r$,
\[\|\v_i^t\|_2,\|\H_i^t\|_\op \leq C_{r,T} \qquad
\text{ for } i=1,\ldots,d+K.\]
\item For any $f \in \cA$, the map $(t,\x) \mapsto P_t f(\x)$ belongs to
$C^{1,2}([0,\infty) \times \R^{d+K})$, and furthermore
$P_t f \in \cA$. For any $t \geq 0$ and $\x \in \R^{d+K}$,
letting $\{\x^t\}_{t \geq 0}$ and $\{(\v_i^t,\H_i^t)_{i=1}^{d+K}\}_{t \geq 0}$
be as defined in parts (a) and (b), we have
\begin{equation}\label{eq:Ptspaceder}
\begin{aligned}
\nabla P_t f(\x) &=\bigg \langle \sum_{j=1}^{d+K} \partial_j
f(\x^t)\v_j^t\bigg\rangle\\
\nabla^2 P_t f(\x)
&=\bigg\langle \sum_{j,k=1}^{d+K} \partial_j\partial_k f(\x^t)
\v_j^t\v_k^{t\top}+\sum_{j=1}^{d+K} \partial_j f(\x^t)\H_j^t \bigg\rangle
\end{aligned}
\end{equation}
and
\begin{equation}\label{eq:forwardbackward}
\partial_t P_t f(\x)=P_t \L f(\x)=\L P_t f(\x).
\end{equation}
\end{enumerate}
\end{proposition}
\begin{proof}
Note that under Assumptions \ref{assump:prior} and \ref{assump:gradient},
each component of
$u:\R^{d+K} \to \R^{d+K}$ belongs to $\cB$, i.e.\ each function
$\partial_j u_i$ and $\partial_j\partial_k u_i$
is bounded and H\"older-continuous globally over $\btheta \in \R^d$
and locally over $\alpha \in \R^K$.
Fix any $r,T>0$ and consider any initial condition
$\x=(\btheta,\widehat\alpha) \in \R^{d+K}$ with $\|\widehat\alpha\|_2 \leq r$.
For some $R>r$ to be determined,
let $\iota_R:\R^K \to \R^K$ be a smooth function with bounded first and second
derivatives, such that $\iota_R(\alpha)=\alpha$ for
$\|\alpha\|_2<R$ and $\|\iota_R(\alpha)\|_2 \leq R+1$ for all $\alpha \in \R^K$.
Consider the diffusion
\begin{equation}\label{eq:truncated_sde}
\d\x_R^t=u_R(\x_R^t)\d t+\sqrt{2}\,\M\,\d\b^t,
\qquad u_R(\btheta,\widehat\alpha):=u(\btheta,\iota_R(\widehat\alpha))
\end{equation}
with the same initial condition $\x_R^0=\x$. Then the first and second
derivatives of $u_R$ are globally
bounded and H\"older-continuous on all of $\R^{d+K}$.
In particular, $u_R$ is Lipschitz, so there exists a unique strong
solution $\{\x_R^t\}_{t \geq 0}:=\{(\btheta_R^t,\widehat\alpha_R^t)\}_{t \geq
0}$ of (\ref{eq:truncated_sde}) (c.f.\ \cite[Theorem
II.1.2]{kunita1984stochastic}). Under the linear growth
condition of Assumption \ref{assump:gradient}(a), integrating the component
\[\d\widehat\alpha_R^t=\cG\bigg(\iota_R(\widehat\alpha_R^t),\;\frac{1}{d}\sum_{j=1}^d
\delta_{\theta_{R,j}^t}\bigg)\]
of (\ref{eq:truncated_sde})
gives $\|\widehat\alpha_R^t\|_2 \leq e^{Ct}(1+\|\widehat\alpha_R^0\|_2)$.
Thus, choosing $R=e^{CT}(1+r)$,
we have $u_R(\x_R^t)=u(\x_R^t)$ for all $t \leq T$,
implying $\{\x_R^t\}_{t \in [0,T]}$
is also the unique solution of
(\ref{eq:joint_sde}) for times $t \leq T$. Since $r,T>0$ are arbitrary,
there then exists a unique strong solution $\{\x^t\}_{t \geq 0}$ to
(\ref{eq:joint_sde}) with any initial condition $\x^0=\x$,
which coincides with $\{\x_R^t\}_{t \in [0,T]}$ for any
$T>0$, $r \geq \|\widehat\alpha\|_2$, and $R=e^{CT}(1+r)$. This shows also
$\|\widehat \alpha^t\|_2=\|\widehat \alpha_R^t\|_2 \leq e^{CT}(1+r)$ for all $t
\in [0,T]$, establishing part (a).

For (b--c), we may assume (by replacing $u$ with $u_R$ for $R=e^{CT}(1+r)$ and
sufficiently large $r,T>0$) that each $\partial_j u_i$ and $\partial_j\partial_k
u_i$ is globally bounded and H\"older-continuous on $\R^{d+K}$. Then
\cite[Theorem II.3.1]{kunita1984stochastic} shows that
$\x^t$ is $C^1$ in the initial condition $\x$, with
derivative $\V^t:=\der_\x \x^t \in \R^{(d+K) \times (d+K)}$
solving the first-variation equation
\[\d\V^t=[\der u(\x^t)]\V^t\d t,\qquad \V^0=\I.\]
Noting that $\v_i^t=\nabla x_i^t(\x)$
is (the transpose of) the $i^\text{th}$ row of $\V^t$, this gives the first
equation of (\ref{eq:firstsecondvar}) with initialization $\v_i^0=\e_i$.
Now letting $C \equiv C_{r,T}>0$
be an upper bound for $\sup_{\x \in \R^{d+K}} \|\der u(\x)\|_{\op}$, note that
integrating the above implies $\|\v_i^t\|_2 \leq \|\V^t\|_\op \leq e^{CT}$
for all $t \leq T$. Consider the joint diffusion
\begin{align*}
\d(\x^t,\V^t)=P(\x^t,\V^t) \d t
+\sqrt{2}(\M\,\d\b^t,0), \qquad P(\x,\V)=\Big(u(\x),[\der u(\x)]\V\Big).
\end{align*}
By boundedness and H\"older-continuity of
$\partial_j u_i$ and $\partial_j\partial_k u_i$, we see that 
$P(\x,\V)$ has bounded and H\"older-continuous derivative $\d P(\x,\V)$ 
restricted to $\|\V\|_\op \leq e^{CT}$. Thus
\cite[Theorem II.3.1]{kunita1984stochastic} applied again
shows that $(\x^t,\V^t)$ is $C^1$ in the initial condition $(\x,\V)$. 
Denoting its derivative $\U^t:=\der_{(\x,\V)}(\x^t,\V^t)$ and identifying
$\U^t$ and $\d P(\x,\V)$ as
square matrices of dimension $d+K+(d+K)^2$ under the vectorization of $\V$,
\cite[Theorem II.3.1]{kunita1984stochastic} implies that
$\U^t$ solves the second-variation equation
\begin{equation}\label{eq:Uevolution}
\d\U^t=[\der P(\x^t,\V^t)]\U^t\d t, \qquad \U^0=\I.
\end{equation}
Noting that $\H_i^t=\nabla^2 x_i^t(\x)$
is the block of $\U^t$ corresponding to $\d_\x \v_i^t$,
and that the block corresponding to $\d_\x \x^t$ is $\V^t$,
one may check that the restriction of (\ref{eq:Uevolution})
to the $\d_\x \v_i^t$ block gives the second equation of
(\ref{eq:firstsecondvar}) with initialization $\H_i^0=0$.
Now letting $C' \equiv C_{r,T}'>0$ be an upper bound
for $\sup_{\x,\V:\|\V\|_\op \leq e^{CT}} \|\der P(\x,\V)\|_\op$
and integrating the above, we get $\|\H_i^t\|_\op
\leq \|\U^t\|_\op \leq e^{C'T}$ for all $t \leq T$. This shows part (b).

For part (c), consider any $f \in \cA$.
Fix any $r,T>0$, and consider $t \in [0,T]$
and an initial condition $\x=(\btheta,\widehat\alpha)$
with $\|\widehat\alpha\|_2 \leq r$. Applying (b) and the chain rule,
\begin{equation}\label{eq:fderivs}
\begin{aligned}
\nabla_\x f(\x^t(\x))&=\sum_{j=1}^{d+K} \partial_j f(\x^t)\v_i^t\\
\nabla_\x^2 f(\x^t(\x))&=\sum_{j,k=1}^{d+K} \partial_j\partial_k f(\x^t)
\v_j^t\v_k^{t\top}+\sum_{j=1}^{d+K} \partial_j f(\x^t)\H_j^t.
\end{aligned}
\end{equation}
By the boundedness of $\alpha^t,\v_i^t,\H_i^t$ shown in (a--b) and the condition
$f \in \cA$,
the right sides of (\ref{eq:fderivs}) are bounded and continuous in $(t,\x)$
over $t \in [0,T]$ and $\|\widehat\alpha\|_2 \leq r$. Then dominated convergence
implies $\nabla P_t f(\x)=\nabla_\x \langle f(\x^t) \rangle_{\x^0=\x}
=\langle \nabla_\x f(\x^t(\x)) \rangle$
and $\nabla^2 P_t f(\x)=\nabla_\x^2 \langle f(\x^t) \rangle_{\x^0=\x}
=\langle \nabla_\x^2 f(\x^t(\x)) \rangle$,
where these are also bounded and continuous in $(t,\x)$ over $t \in [0,T]$ and
$\|\widehat\alpha\|_2 \leq r$. This shows all statements for
$\nabla P_t f,\nabla^2 P_tf$ in (c), including the local boundedness of $\nabla
P_t f, \nabla^2 P_tf$ defining the condition $P_t f \in \cA$ since $r>0$
here is arbitrary. For the derivative in $t$, by It\^o's formula
\[f(\x^t)=f(\x)+\int_0^t \L f(\x^s)\d s+\int_0^t \nabla f(\x^s)^\top
\sqrt{2}\,\M\,\d\b^s\]
where $\L$ is the generator defined in (\ref{eq:generator}).
Since $\nabla f(\x^s)$ is bounded over $s \in [0,t]$ and $\x^s$ is adapted to
the filtration of $\{\b^s\}$, the last term is a
martingale, so taking expectations gives
\[P_t f(\x)=\langle f(\x^t) \rangle=f(\x)+\int_0^t \langle \L f(\x^s) \rangle\d s.\]
Hence, differentiating in $t$,
\begin{equation}\label{eq:generatorprop1}
\partial_t P_tf(\x)=\langle \L f(\x^t) \rangle=P_t\L f(\x).
\end{equation}
Applying this at $t=0$ gives $\L f(\x)=\partial_t P_t f(\x)|_{t=0}$. Then
applying this with $P_t f \in \cA$ in place of $f$,
\[\L P_t f(\x)=\partial_s P_{t+s}f(\x)|_{s=0}=\partial_s \langle P_sf(\x^t)
\rangle|_{s=0}
\overset{(*)}{=} \langle \L f(\x^t) \rangle=P_t \L f(\x).\]
Here, to justify $(*)$, we note that $\partial_s P_s f(\x^t)=P_s \L f(\x^t)$
by (\ref{eq:generatorprop1}). By Jensen's inequality,
$\langle (P_s \L f(\x^t))^2 \rangle
\leq \langle \L f(\x^{t+s})^2 \rangle
=\langle (u(\x^{t+s})^\top \nabla f(\x^{t+s})+\Tr \M\M^\top \nabla^2
f(\x^{t+s}))^2 \rangle \leq C(1+\langle \|\x^{t+s}\|_2^2 \rangle)$, the last
inequality holding for some $C>0$ by
boundedness of $\nabla f(\x^{t+s}),\nabla^2 f(\x^{t+s})$
and the Lipschitz growth of $u$. 
\cite[Theorem II.2.1]{kunita1984stochastic} implies that $\x^t$ is uniformly
bounded in $L^2$ over $t \in [0,T]$, so $\langle (P_s \L f(\x^t))^2 \rangle$
is uniformly bounded and hence $\partial_s P_s f(\x^t)=P_s \L f(\x^t)$ is
uniformly integrable in a neighborhood of $s=0$.
Then dominated convergence implies both $(*)$ and
continuity of this derivative $\langle \L f(\x^t) \rangle$ in $(t,\x)$. This
shows all statements of (c).
\end{proof}

Now fix a function $h:[0,\infty) \to \R$ and $\eps>0$, and consider
the perturbed dynamics of Proposition \ref{prop:responseexists},
\begin{equation}\label{eq:perturbed_sde}
\d \x^t=u^\eps(t,\x^t)\d t+\sqrt{2}\,\M\,\d\b^t
\end{equation}
where
\[u^\eps(t,\x)=
\bigg(\frac{1}{\sigma^2} \X^\top (\y-\X\btheta)
+\Big(\partial_\theta \log g(\theta_j;\widehat\alpha)\Big)_{j=1}^d
+\eps h(t)\nabla_{\btheta} B(\btheta,\widehat\alpha),\;
\cG\Big(\widehat\alpha,\frac{1}{d}\sum_{j=1}^d \delta_{\theta_j}\Big)\bigg).\]
For $t \geq s \geq 0$,
denote its (time inhomogeneous) Markov semigroup operators and infinitesimal
generator by
\[P_{s,t}^\eps f(\x)=\langle f(\x^t) \rangle_{\x^s=\x}
=\E[f(\x^t) \mid \X,\y,\x^s=\x],
\qquad \L_t^\eps f(\x)=u^\eps(t,\x)^\top \nabla f(\x)+
\Tr \M\M^\top \nabla^2 f(\x).\]
The following statements are analogous to those of Proposition
\ref{prop:langevinsolution} for this perturbed process.

\begin{proposition}\label{prop:perturbedsolution}
Suppose Assumptions \ref{assump:prior} and \ref{assump:gradient} hold,
$h:[0,\infty) \to \R$ is
continuous and bounded, and $\partial_{\theta_j} B:\R^{d+K} \to \R$ belongs to
$\cB$ for each $j=1,\ldots,d$.
\begin{enumerate}[(a)]
\item For any $\x=(\btheta,\widehat\alpha) \in \R^{d+K}$ and $s \geq 0$,
(\ref{eq:perturbed_sde}) has a pathwise unique strong solution
$\{\x^{t,\eps}\}_{t \geq s}=\{(\btheta^{t,\eps},\widehat
\alpha^{t,\eps})\}_{t \geq s}$
over $t \in [s,\infty)$ with initial condition $\x^{s,\eps}=\x$.

For any $r>0$ and $T>0$, there exists $C_{r,T}>0$ such that for any
$\eps \in [0,1]$, $s \geq 0$, and initial condition with $\|\widehat\alpha\|_2
\leq r$, and $t \in [s,s+T]$,
\[\|\widehat \alpha^{t,\eps}\|_2 \leq C_{r,T}.\]
\item For any $f \in \cA$,
the map $(s,t,\x) \mapsto P_{s,t}^\eps f$ belongs to
$C^{1,2}(\{s,t:0 \leq s \leq t\} \times \R^{d+K})$,
and furthermore $P_{s,t}^\eps f \in \cA$. We have
\begin{equation}\label{eq:backwardequation}
\partial_t P_{s,t}^\eps f(\x)=P_{s,t}^\eps \L_t^\eps f(\x),
\qquad \partial_s P_{s,t}^\eps f(\x)={-}\L_s^\eps P_{s,t}^\eps f(\x).
\end{equation}
\end{enumerate}
\end{proposition}
\begin{proof}
We omit the superscript $\eps$ and write $\x^t \equiv \x^{t,\eps}$.
The same arguments as in Proposition \ref{prop:langevinsolution} show
(a), where for any fixed $r,T>0$ and initial condition with
$\|\widehat\alpha\|_2 \leq r$, the solution $\{\x^t\}_{t \in [s,s+T]}$
coincides with that in a system where $u^\eps$ is globally Lipschitz and
H\"older-continuous, uniformly over $\eps \in [0,1]$.

For (b), the same arguments as in Proposition \ref{prop:langevinsolution} also
show that each component $x_i^t \equiv x_i^t(s,\x)$ of this solution
is $C^2$ in $\x$, with gradient $\v_i^t=\nabla_\x x_i^t(s,\x)$
and Hessian $\H_i^t=\nabla_\x^2 x_i^t(s,\x)$ solving
\[\begin{cases}
\d \v_i^t=\sum_{j=1}^{d+K} \partial_j u_i^\eps(t,\x^t) \cdot \v_j^t\,\d t\\
\d \H_i^t=\big(\sum_{j,k=1}^{d+K} \partial_j\partial_k u_i^\eps(t,\x^t) \cdot
\v_j^t{\v_k^t}^\top+\sum_{j=1}^{d+K} \partial_j u_i^\eps(t,\x^t) \cdot
\H_j^t\big)\d t
\end{cases}\]
with initializations $\v_i^s=\e_i$ and $\H_i^s=0$.
These solutions satisfy $\|\v_i^t\|_2,\|\H_i^t\|_\op \leq C_{r,T}$ for any
$t \in [s,s+T]$ and initial condition $\x=(\btheta,\widehat\alpha)$
with $\|\widehat\alpha\|_2 \leq r$. Furthermore, writing
$\x^t(s,\x)$, $\v_i^t(s,\x)$, and $\H_i^t(s,\x)$ to make explicit their
dependence on the initial condition $\x^s=\x$,
\cite[Theorem II.2.2]{kunita1984stochastic} implies that
$\{\x^t(s,\x),(\v_i^t(s,\x))_{i=1}^{d+K},(\H_i^t(s,\x))_{i=1}^{d+K}\}_{t \geq s}$
is jointly H\"older continuous in $(s,t,\x)$. Then for any $f \in \cA$,
a dominated convergence argument
as in Proposition \ref{prop:langevinsolution}
shows that $\nabla P_{s,t}^\eps f(\x)$ and $\nabla^2 P_{s,t}^\eps f(\x)$
exist and may be computed by differentiating in $\x$ under the integral, that
these derivatives are continuous in $(s,t,\x)$, and that they are bounded
over initial conditions $\x^s=\x$ with $\|\widehat\alpha\|_2 \leq r$, implying
$P_{s,t}^\eps f \in \cA$.

The same argument as in
Proposition \ref{prop:langevinsolution} using It\^o's formula shows
\[\partial_t P_{s,t}^\eps f(\x)=P_{s,t}^\eps \L_t^\eps f(\x)
=\langle\L_t^\eps f(\x^t) \rangle_{\x^s=\x}.\]
This is also continuous in $(s,t,\x)$
by dominated convergence because $\L_t^\eps f(\x)$ is 
continuous in $(t,\x)$, $\x^t \equiv \x^t(s,\x)$ is continuous in $(s,\x)$, and
$|\L_t^\eps f(\x^t(s,\x))|=|u^\eps(t,\x^t(s,\x))^\top
\nabla f(\x^t(s,\x))+\Tr \M\M^\top \nabla^2 f(\x^t(s,\x))|
\leq C(1+\|\x^t(s,\x)\|_2)$ which is uniformly bounded in $L^2$ over
$s,t \leq T$ by \cite[Theorem II.2.1]{kunita1984stochastic},
hence uniformly integrable.

Finally, for the derivative in $s$, we have by It\^o's formula for any $h>0$,
\[P_{s-h,s}^\eps f(\x)=\langle f(\x^s) \rangle_{\x^{s-h}=\x}
=f(\x)+\int_{s-h}^s \langle \L_u^\eps f(\x^u) \rangle_{\x^{s-h}=\x} \,\d u.\]
By the above uniform integrability of $|\L_t^\eps f(\x^t(s,\x))|$ and the
dominated convergence theorem,
we have $\lim_{h \downarrow 0,\,\,u \uparrow s}
\langle \L_u^\eps f(\x^u) \rangle_{\x^{s-h}=\x}=\L_s^\eps(\x)$.
So taking the limit $h \to 0$ above and rearranging shows
\begin{equation}\label{eq:lowerderiv}
\L_s^\eps f(\x)=\lim_{h \downarrow 0} \frac{P_{s-h,s}^\eps f(\x)-f(\x)}{h}.
\end{equation}
Then for any $s \leq t$, applying this to $P_{s,t}^\eps f \in \cA$
in place of $f$ gives
\[\lim_{h \downarrow 0} \frac{P_{s,t}^\eps f(\x)-P_{s-h,t}^\eps f(\x)}{h}
=\lim_{h \downarrow 0}
\frac{P_{s,t}^\eps f(\x)-P_{s-h,s}^\eps(P_{s,t}^\eps f)(\x)}{h}
={-}\L_s^\eps P_{s,t}^\eps f(\x),\]
i.e.\ $P_{s,t}^\eps f(\x)$ is left-differentiable in $s$. Here
${-}\L_s^\eps P_{s,t}^\eps f(\x)
={-}u^\eps(s,\x)^\top \nabla P_{s,t}^\eps f(\x)
-\Tr \M\M^\top \nabla^2 P_{s,t}^\eps f(\x)$ is continuous in $(s,t,\x)$
by the continuity of $\nabla P_{s,t}^\eps f$ and
$\nabla^2 P_{s,t}^\eps f$ shown above. Then
$P_{s,t}^\eps f(\x)$ is differentiable in $s$ with derivative $\partial_s P_{s,t}^\eps f(\x)={-}\L_s^\eps P_{s,t}^\eps
f(\x)$. This shows all statements of part (b).
\end{proof}

We now prove Proposition \ref{prop:responseexists} and show that the
response function $R_{AB}$ is given explicitly by
\begin{equation}\label{eq:explicitresponse}
R_{AB}(t,s)=P_s\Big(\nabla_{\btheta} B^\top \nabla_{\btheta}
P_{t-s}A\Big)(\btheta^0,\widehat\alpha^0).
\end{equation}
Here, $\{P_t\}_{t \geq 0}$ is the Markov semigroup (\ref{eq:semigroup})
for the unperturbed diffusion $\{(\btheta^t,\alpha^t)\}_{t \geq 0}$.
For $f:\R^{d+K} \to \R$, $\nabla_{\btheta} f:\R^{d+K} \to \R^d$ denotes
its gradient with respect to the $\btheta$ variable only.

The argument for Proposition \ref{prop:responseexists}
is similar to \cite[Theorem 3.9]{chen2020mathematical}, using the
Kolmogorov backward equation (\ref{eq:backwardequation}) and the regularity
properties of $P_t$ and $P_{s,t}^\eps$ established in Propositions
\ref{prop:langevinsolution} and \ref{prop:perturbedsolution}, which replace the
uniform-ellipticity Schauder estimates of \cite{chen2020mathematical}.

\begin{proof}[Proof of Proposition \ref{prop:responseexists}]
Fix any $A \in \cA$, continuous bounded $h:[0,\infty) \to \R$,
and $0 \leq s \leq t$. Let $\{\x^t\}_{t \geq 0}$ and
$\{\x^{t,\eps}\}_{t \geq 0}$ be the solutions to the
unperturbed and perturbed diffusions. For $u \in [s,t]$, define
$f^\eps(u,\x)=P_{u,t}^\eps A(\x)$. Then by It\^o's formula (applied to
the unperturbed process $\{\x^t\}_{t \geq 0}$),
\[f^\eps(t,\x^t)=f^\eps(s,\x^s)+\int_s^t (\partial_u+\L)f^\eps(u,\x^u)
\d u+\int_s^t \nabla_\x f^\eps(u,\x^u)^\top \sqrt{2}\,\M\d\b^u.\]
By the bound for $\|\widehat\alpha^u\|_2$ in Proposition
\ref{prop:langevinsolution}(a) and the condition $P_{u,t}^\eps A \in \cA$ in
Proposition \ref{prop:perturbedsolution}(b), we have that $\nabla_\x
f^\eps(u,\x^u)$ is uniformly bounded for $u \in [s,t]$, so the last term is a
martingale. Then, taking expectations under the initial condition $\x^s=\x$
and applying (\ref{eq:backwardequation}),
\begin{align*}
\langle A(\x^t) \rangle_{\x^s=\x}=\langle f^\eps(t,\x^t) \rangle_{\x^s=\x}
&=f^\eps(s,\x)+\int_s^t \langle (\partial_u+\L)f^\eps(u,\x^u) \rangle_{\x^s=\x}
\d u\\
&=P_{s,t}^\eps A(\x)+\int_s^t \langle ({-}\L_u^\eps+\L)P_{u,t}^\eps A(\x^u)
\rangle_{\x^s=\x}\d u\\
&=P_{s,t}^\eps A(\x)-\int_s^t \eps h(u)\langle(\nabla_{\btheta} B^\top
\nabla_{\btheta} P_{u,t}^\eps A)(\x^u)\rangle_{\x^s=\x}\d u\\
&=P_{s,t}^\eps A(\x)-\eps \int_s^t h(u)P_{u-s}(\nabla_{\btheta} B^\top
\nabla_{\btheta} P_{u,t}^\eps A)(\x) \d u.
\end{align*}
Applying this also with $\eps=0$ and $P_{s,t}^0=P_{t-s}$ and
taking the difference, we obtain the identity
\begin{equation}\label{eq:perturbationidentity}
P_{s,t}^\eps A(\x)-P_{t-s} A(\x)
=\eps \int_s^t h(u)P_{u-s}(\nabla_{\btheta} B^\top \nabla_{\btheta} P_{u,t}^\eps
A)(\x) \d u.
\end{equation}

From the definition of $P_t f(\x)$ and
form of $\nabla P_t f(\x)$ in (\ref{eq:Ptspaceder}), we have
\begin{align}
P_{u-s}(\nabla_{\btheta} B^\top \nabla_{\btheta} P_{u,t}^\eps A)(\x)
&=\langle (\nabla_{\btheta} B^\top \nabla_{\btheta} P_{u,t}^\eps A)(\x^{u-s})
\rangle,\label{eq:UI1}\\
\nabla P_{u-s}(\nabla_{\btheta} B^\top \nabla_{\btheta} P_{u,t}^\eps A)(\x)
&=\Bigg\langle \sum_{i=1}^{d+K} \partial_i[\nabla_{\btheta} B^\top \nabla_{\btheta}
P_{u,t}^\eps A](\x^{u-s})\v_i^{u-s}\Bigg\rangle,\label{eq:UI2}
\end{align}
where the expectations $\langle \cdot \rangle$ on the right side are taken under
the initial condition $\x^0=\x$.
For $\x=(\btheta,\widehat\alpha)$ with $\|\widehat\alpha\|_2 \leq r$,
$u \in [s,t]$, and $\eps \in [0,1]$, we have that
$\|\alpha^{u-s}\|_2$ is bounded by Proposition \ref{prop:langevinsolution}(a),
$\nabla_{\btheta} B \in \cB$ by assumption, and
$P_{u,t}^\eps A \in \cA$ by Proposition \ref{prop:perturbedsolution}(b),
which together imply that
\[|(\nabla_{\btheta} B^\top \nabla_{\btheta} P_{u,t}^\eps A)(\x^{u-s})|,\,
|\partial_i[\nabla_{\btheta} B^\top \nabla_{\btheta} P_{u,t}^\eps
A](\x^{u-s})| \leq C(1+\|\x^{u-s}\|_2)\]
for some $C>0$. Then these quantities are bounded in $L^2$ and hence
uniformly integrable by \cite[Theorem II.2.1]{kunita1984stochastic}.
Furthermore $\|\v_i^{u-s}\|_2$ is bounded by
Proposition \ref{prop:langevinsolution}(b), so the integrands of
both (\ref{eq:UI1}--\ref{eq:UI2}) are uniformly integrable
over $\|\widehat\alpha\|_2 \leq r$, $u \in [s,t]$, and $\eps \in [0,1]$.
Applying dominated convergence, we may
differentiate (\ref{eq:perturbationidentity}) under the integral in $\btheta$,
\[\nabla_{\btheta} P_{s,t}^\eps A(\x)-\nabla_{\btheta} P_{t-s} A(\x)
=\eps \int_s^t h(u)\nabla_{\btheta} P_{u-s}(\nabla_{\btheta} B^\top \nabla_{\btheta} P_{u,t}^\eps A)(\x) \d u,\]
and take the limit $\eps \to 0$ to get
$\nabla_{\btheta} P_{s,t}^\eps A(\x) \to \nabla_{\btheta} P_{t-s} A(\x)$. Applying this with $s=u$
to the right side of (\ref{eq:perturbationidentity}), and
taking the limit $\eps \to 0$ in (\ref{eq:perturbationidentity}) using uniform
integrability of (\ref{eq:UI1}), we arrive at
\[\lim_{\eps \to 0} \frac{P_{s,t}^\eps A(\x)-P_{t-s} A(\x)}{\eps}
=\int_s^t h(u)P_{u-s}(\nabla_{\btheta} B^\top \nabla_{\btheta} P_{t-u}A)(\x) \d u.\]
For $s=0$, this means
\[\lim_{\eps \to 0} \frac{1}{\eps}\Big(\langle A(\x^{t,\eps}) \rangle-\langle
A(\x^t) \rangle\Big)
=\int_0^t h(u)P_u(\nabla_{\btheta} B^\top \nabla_{\btheta} P_{t-u}A)(\x) \d u,\]
verifying that (\ref{eq:responsedef})
holds with response function $R_{AB}$ given by (\ref{eq:explicitresponse}).

For uniqueness, observe that if $\tilde R_{AB}$ is different from $R_{AB}$
(on a positive measure subset of $(s,t)$), then there exists a continuous
bounded function $h:[0,\infty) \to \R$ such that $\int_0^t R_{AB}(t,s)h(s)\d s
\neq \int_0^t \tilde R_{AB}(t,s)h(s)\d s$, contradicting that both
$R_{AB},\tilde R_{AB}$ satisfy (\ref{eq:responsedef}).
Thus this response function $R_{AB}$ is unique.
\end{proof}






